EnvOS: Auditing Computer-Use Agents When the World Moves On : Phenomenon-Based Task Construction, Certification, and Evidence-Based Evaluation

Computer-use agents built on large language models (LLMs) work in software that can change while they act: an appointment moves, a policy is revised, a record is updated. Testing agents under such changes is harder than it looks. When an agent fails, the cause may be the agent, but it may also be a change that did not fire as intended, an update the agent never received, or a grader that scored the episode wrongly. We introduce EnvOS, a framework for building and certifying environments that change mid-task. Before any agent runs, EnvOS checks that each change fires correctly, that the task remains solvable, and that the grader separates correct from incorrect behavior; after each run, separate code re-checks the verdict from archived evidence. We apply it to stale information, where a value the agent has already seen changes before the agent acts on it. In clinic booking, Claude Opus 5 succeeds on 0/16 tasks when nothing extra is shown, 2/16 when reminded to re-check the source, and 15/16 when the updated value is shown; the gain over the reminder holds after correcting for all tests (p = 0.00293). In insurance-claim approval, Opus 5 re-checks on its own and succeeds on 10/10, whereas Claude Sonnet 5 rises from 1/10 to 9/10 when the current policy is shown again, a gain significant in its pre-registered test but not after correcting for all tests. Whether an agent caught a change thus varied with the model and the interface. We also stress-test the grading itself: on corrupted episodes designed blind from the rules, the EnvOS pipeline accepted none of 26 as clean, and on an externally generated set it caught 25 of 39, against 4 for simple log checks. Because every EnvOS environment is generated from a seed and graded by an audited automatic verifier, the same environments are natural candidates for training agents with reinforcement learning from verifiable rewards.

==> claims.tex <==
% GENERATED BY claims.py -- DO NOT EDIT BY HAND.
% Every manuscript number is a macro derived from a hashed frozen artifact under audit/.
% Regenerate: python claims.py ; verify: python claims.py --verify

\newcommand{\ACCertChecks}{223\xspace}  % ac.cert_checks: sum over certificates over check
\newcommand{\ACCertFailed}{0\xspace}  % ac.cert_failed: count failed over check
\newcommand{\ACCertN}{6\xspace}  % ac.cert_n: count over certificate
\newcommand{\ACClean}{2/2\xspace}  % ac.ACClean: pass count over rollout
\newcommand{\ACCliCalls}{138\xspace}  % ac.cli: count over policy call
\newcommand{\ACCounted}{5\xspace}  % ac.counted: count counted over rollout
\newcommand{\ACLfour}{1/1\xspace}  % ac.ACLfour: pass count over rollout
\newcommand{\ACLthree}{1/1\xspace}  % ac.ACLthree: pass count over rollout
\newcommand{\ACLthreePlus}{1/1\xspace}  % ac.ACLthreePlus: pass count over rollout
\newcommand{\ACModelFailures}{0\xspace}  % ac.model_failures: count over counted rollout
\newcommand{\ACRollouts}{6\xspace}  % ac.rollouts: count over rollout
\newcommand{\ACVoided}{1\xspace}  % ac.voided: count voided over rollout
\newcommand{\ACWallMinutes}{30.4\xspace}  % ac.wall_min: sum of wall clock (min) over rollout
\newcommand{\ASeventeenDate}{2026-09-23\xspace}  % r22.a17_date: ADDENDUM 17's date over -
\newcommand{\AbsApplications}{Its finalized implementation is evaluated prospectively in two workflows, clinic booking and insurance-claim approval.\xspace}  % abs.applications: APP.two over -
\newcommand{\AbsApplicationsState}{We evaluate the finalized protocol prospectively in two workflows, insurance-claim approval and clinic booking.\xspace}  % r28.abs_app: r28: the abstract's applications over -
\newcommand{\AbsAuditClause}{Independent audits re-derive every validity verdict of the historical blocks (\VindAgree of \VindAttempts agree under the rules as implemented) and the booked clinic of every historical booking, but verify no historical success in full; on the prospective blocks, with clinic calendar compatibility resting on stated design conditions, every outcome term is resolved and agreeing with the evaluator on \ProspEndpointFull of \ProspCounted counted rollouts.\xspace}  % abs.audit: audit clause over -
\newcommand{\AbsBCClause}{In clinic booking, counterbalanced no-panel, cue-and-link and current-value conditions on \BlockBCInstancesWords fresh instances (Claude Opus~5) showed at the registered block-local level that displaying the current location increased success relative to the cue-and-link panel, with no rejection of cue versus no panel, and every block-local rejection survives the paper-wide Holm analysis.\xspace}  % abs.bc: abstract/introduction/conclusion clause for Block BC over -
\newcommand{\AbsBCHolmS}{Over all \HolmPaperMWords{} claim-bearing tests, LIVE--CUE's Holm $p=\BlockBCLiveCueHolmPaper$.\xspace}  % r37f.abs_bc_holm: r37 final reviews: the abstract's BC paper-wide arithmetic over -
\newcommand{\AbsBCR}{In clinic booking, Claude Opus~5 succeeded on \BlockBCFRXOffAPassFrac{} instances with no panel, \BlockBCFRXCueAPassFrac{} with a cue-and-link panel and \BlockBCFRXLiveAPassFrac{} when the same panel displayed the current location (LIVE--CUE: \BlockBCLiveCueRescue{} rescues, \BlockBCLiveCueHarm{} harms and \BlockBCLiveCueTie{} ties, block-local Holm $p=\BlockBCLiveCueHolmLocal$; CUE--OFF: block-local Holm $p=\BlockBCCueOffHolmLocal$). At the registered block-local level, displaying the current location increased success relative to this cue-and-link panel. The CUE--OFF contrast did not reject; this does not establish absence of a cue effect. Contradiction, salience, and reduced verification effort remain possible explanations.\xspace}  % r31.abs_bc: r31: the abstract's clinic result over -
\newcommand{\AbsBCSentence}{ \AbsBCClause\xspace}  % r28.abs_bc: r28: BC's one abstract sentence, only once it has an admissible result over -
\newcommand{\AbsChalMissS}{ It still counted \ExtPipeFATotal{} of \ExtCorTotal{} as clean.\xspace}  % r37f.abs_chal_miss: r37 final reviews: the abstract: the external challenge's misses over -
\newcommand{\AbsChalR}{In a run-once \ChallengeN-case archive challenge, the independent outcome scorer met \ChallengeScorerMet/\ChallengeN{} frozen expectations and validity re-derivation \ChallengeVindMet/\ChallengeN, exposing both coverage and blind spots.\xspace}  % r31.abs_chal: r31: the abstract's challenge sentence over -
\newcommand{\AbsChalThree}{Evaluator audits exposed their own limits: on a sealed challenge, validity re-derivation met \ChallengeVindMet/\ChallengeN{} expectations; on a second, specified without implementation or outcome access, the pipeline counted none of \BlindCorrupt{} corruptions as clean but gave no verdict on \BlindPipeErr; on a third, which an external agent designed and generated, it caught more corruptions than raw-log baselines in both workflows.\xspace}  % r34.ext.abs: r34 external challenge: the abstract's challenge sentence (three challenges) over -
\newcommand{\AbsChalTwo}{Evaluator audits exposed their own limits: on a sealed \ChallengeN-case challenge, validity re-derivation met \ChallengeVindMet/\ChallengeN{} frozen expectations; on a second challenge specified without access to the implementation or model outcomes, the combined pipeline counted none of \BlindCorrupt{} corruptions as clean but gave no verdict on \BlindPipeErr, and the outcome scorer alone counted \BlindScorerFA{} as clean.\xspace}  % r32.abs_chal: r32: the abstract's challenge sentence over -
\newcommand{\AbsChallengeClause}{A sealed, run-once archive challenge of \ChallengeN{} cases bounds each auditing layer: the independent outcome scorer met all \ChallengeN{} frozen expectations, the validity re-derivation \ChallengeVindMet{} and the evaluator's archived verdicts \ChallengeEvalMet, and the misses are reported, not repaired.\xspace}  % chal.r27.abs: r27 challenge text (scorer 28/28, validity 24/28, evaluator 10/28) over -
\newcommand{\AbsClmBSReading}{the panel increased full-task success at the registered local level, but no block-local rejection survives the paper-wide Holm analysis\xspace}  % abs.clmbs: CLM-BS's registered reading as sealed FRAG templates, with the paper-wide qualifier over -
\newcommand{\AbsClmClause}{In insurance-claim approval, where the approved amount is derived, without the panel Claude Opus~5 succeeded on \BlockClmBOffPass of \BlockClmBClmOffAN instances under silent supersession; the registered rescue-opportunity threshold was not met.\xspace}  % abs.clm: clause for Block CLM-B over -
\newcommand{\AbsClmCompressed}{In insurance-claim approval, Claude Opus~5 re-read the changed policy record and succeeded on all \BlockClmBClmOffAN{} silent-change instances without re-exposure, whereas Claude Sonnet~5 succeeded on \BlockClmBSClmOffAPassFrac{} without and \BlockClmBSClmOnAPassFrac{} with review-step re-exposure (\BlockClmBSOnOffRescue{} rescues, \BlockClmBSOnOffHarm{} harms, \BlockClmBSOnOffTie{} ties; exact paired $p=\BlockClmBSOnOffP$). The instruction explicitly defines correctness by the policy value at approval, so we scope this contrast to the tested task and interface.\xspace}  % r28.abs_clm: r28: the abstract's claims result (GPT-6 r20 compression) over -
\newcommand{\AbsClmR}{In insurance-claim approval, Claude Opus~5 re-read the changed policy record and succeeded on \BlockClmBClmOffAPassFrac{} silent-change instances without review-step re-exposure, whereas Claude Sonnet~5 succeeded on \BlockClmBSClmOffAPassFrac{} without and \BlockClmBSClmOnAPassFrac{} with re-exposure (\BlockClmBSOnOffRescue{} rescues, \BlockClmBSOnOffHarm{} harms, \BlockClmBSOnOffTie{} ties; exact paired $p=\BlockClmBSOnOffP$).\xspace}  % r31.abs_clm: r31: the abstract's claims result (counts only) over -
\newcommand{\AbsClmS}{In insurance-claim approval, Claude Opus~5 succeeded on \BlockClmBClmOffAPassFrac{} silent-change instances without review-step re-exposure, Claude Sonnet~5 on \BlockClmBSClmOffAPassFrac{} without and \BlockClmBSClmOnAPassFrac{} with it (\BlockClmBSOnOffRescue{} rescues, \BlockClmBSOnOffHarm{} harms, \BlockClmBSOnOffTie{} ties; registered block-local $p=\BlockClmBSOnOffP$; retrospective \HolmPaperMWords-test Holm $p=\HolmPaperClmBS$).\xspace}  % r37f.abs_clm: r37 final reviews: the abstract's claims result over -
\newcommand{\AbsWorkflowsR}{We evaluate the finalized protocol prospectively in two workflows under one controlled semantic-browser interface.\xspace}  % r31.abs_wf: r31: the abstract's applications over -
\newcommand{\ActionBudget}{48\xspace}  % spec.max_steps: declared budget over action
\newcommand{\AdmissionAnineteenStatus}{pass\xspace}  % r21.admission: ADDENDUM 19 admission (decisive sentinel) over -
\newcommand{\Alpha}{0.05\xspace}  % spec.alpha: significance level over -
\newcommand{\AtwoChangedDismissedLog}{8\xspace}  % A2.S-L2.dismissed_log: count with the notice's token on a browser request in the raw access log over counted rollout
\newcommand{\AtwoChangedFail}{1\xspace}  % A2.S-L2.fail: count over counted rollout
\newcommand{\AtwoChangedFirst}{6\xspace}  % A2.changed_first: count over pair
\newcommand{\AtwoChangedN}{8\xspace}  % A2.S-L2.n: count over counted rollout
\newcommand{\AtwoChangedPass}{7\xspace}  % A2.S-L2.pass: count over counted rollout
\newcommand{\AtwoChangedReread}{7\xspace}  % A2.changed_reread: count over counted changed rollout
\newcommand{\AtwoChangedWilsonHi}{0.98\xspace}  % A2.S-L2.wilson_hi: Wilson 95% upper over counted rollout
\newcommand{\AtwoChangedWilsonLo}{0.53\xspace}  % A2.S-L2.wilson_lo: Wilson 95% lower over counted rollout
\newcommand{\AtwoCleanFail}{0\xspace}  % A2.S-L0.fail: count over counted rollout
\newcommand{\AtwoCleanN}{2\xspace}  % A2.S-L0.n: count over counted rollout
\newcommand{\AtwoCleanPass}{2\xspace}  % A2.S-L0.pass: count over counted rollout
\newcommand{\AtwoCleanSeeds}{2\xspace}  % spec.clean_seeds: count of clean-control seeds over seed
\newcommand{\AtwoCleanWilsonHi}{1.00\xspace}  % A2.S-L0.wilson_hi: Wilson 95% upper over counted rollout
\newcommand{\AtwoCleanWilsonLo}{0.34\xspace}  % A2.S-L0.wilson_lo: Wilson 95% lower over counted rollout
\newcommand{\AtwoCliCalls}{484\xspace}  % A2.cli_calls: sum over policy call
\newcommand{\AtwoControlDismissedLog}{8\xspace}  % A2.S-C.dismissed_log: count with the notice's token on a browser request in the raw access log over counted rollout
\newcommand{\AtwoControlFail}{0\xspace}  % A2.S-C.fail: count over counted rollout
\newcommand{\AtwoControlN}{8\xspace}  % A2.S-C.n: count over counted rollout
\newcommand{\AtwoControlPass}{8\xspace}  % A2.S-C.pass: count over counted rollout
\newcommand{\AtwoControlReread}{3\xspace}  % A2.control_reread: count over counted control rollout
\newcommand{\AtwoControlWilsonHi}{1.00\xspace}  % A2.S-C.wilson_hi: Wilson 95% upper over counted rollout
\newcommand{\AtwoControlWilsonLo}{0.68\xspace}  % A2.S-C.wilson_lo: Wilson 95% lower over counted rollout
\newcommand{\AtwoCounted}{18\xspace}  % A2.counted: count over rollout
\newcommand{\AtwoEffect}{0.125\xspace}  % A2.effect: discordant-pair proportion over pair
\newcommand{\AtwoEffectHi}{0.47\xspace}  % A2.effect_hi: Wilson 95% upper over pair
\newcommand{\AtwoEffectLo}{0.02\xspace}  % A2.effect_lo: Wilson 95% lower over pair
\newcommand{\AtwoEpisodes}{19\xspace}  % A2.episodes: count over rollout
\newcommand{\AtwoFailReread}{0\xspace}  % A2.fail_reread: count over failed changed rollout
\newcommand{\AtwoGateBatterySha}{\texttt{721d666d}\xspace}  % pre.a2_gate_battery_sha: digest ADDENDUM 3 records for Block A2's mutation battery over -
\newcommand{\AtwoGateFilesSurviving}{0\xspace}  % pre.a2_gate_files_surviving: of the two digest-recorded gate files, how many survive among 14 battery/leak files under audit/ over file
\newcommand{\AtwoGateLeakSha}{\texttt{60cb0ce4}\xspace}  % pre.a2_gate_leak_sha: digest ADDENDUM 3 records for Block A2's leak audit over -
\newcommand{\AtwoHeFail}{9\xspace}  % A2.He_fail: observed H_e over failed changed rollout
\newcommand{\AtwoHeMax}{24\xspace}  % A2.He_max: max observed H_e: actions strictly between notice (C3) and the /new/1->/new/2 submission over counted changed rollout
\newcommand{\AtwoHeMin}{9\xspace}  % A2.He_min: min observed H_e: actions strictly between notice (C3) and the /new/1->/new/2 submission over counted changed rollout
\newcommand{\AtwoHeSecondMax}{12\xspace}  % A2.He_second_max: second-largest observed H_e over counted changed rollout
\newcommand{\AtwoImageDeliveryMin}{0.96\xspace}  % A2.image_delivery_min: min over counted rollout
\newcommand{\AtwoInfraErrors}{0\xspace}  % A2.infra_errors: sum over rollout
\newcommand{\AtwoInstructionDistinct}{7\xspace}  % A2.instruction_distinct: distinct sha256 across the block's instructions over instruction text
\newcommand{\AtwoInstructionIdenticalInstances}{8\xspace}  % A2.instruction_identical: count of seeds whose every archived rollout (all arms, counted and replaced) carries one instruction sha256 over instance
\newcommand{\AtwoInstructionInstances}{8\xspace}  % A2.instruction_instances: count of seeds with archived rollouts over instance
\newcommand{\AtwoManifestSha}{\texttt{b66756ff}\xspace}  % A2.manifest_sha: sha256 prefix over -
\newcommand{\AtwoMemoPct}{97\xspace}  % A2.memo_pct: share with a memo over policy call
\newcommand{\AtwoMemoSteps}{469\xspace}  % A2.memo_steps: count with a memo over policy call
\newcommand{\AtwoModelId}{\texttt{claude-opus-5}\xspace}  % A2.model: resolved model id (all rows) over rollout
\newcommand{\AtwoModulePackaged}{1\xspace}  % supp.a2_module_packaged: 1 if Block A2's task module (by digest) ships in code_snapshots/ over -
\newcommand{\AtwoModuleSha}{\code{17f6c7cd72f2}\xspace}  % coh.a2_module: Block A2's task-module digest (no copy survives) over -
\newcommand{\AtwoModuleWhere}{Block~A2's task module (\AtwoModuleSha), absent from the working tree, was recovered from a backup and verified by its digest, and ships in the supplement\xspace}  % supp.a2_module_text: where Block A2's task module survives over -
\newcommand{\AtwoNNeg}{0\xspace}  % A2.n_neg: count over pair
\newcommand{\AtwoNPos}{1\xspace}  % A2.n_pos: count over pair
\newcommand{\AtwoNTied}{7\xspace}  % A2.n_tied: count over pair
\newcommand{\AtwoNoticeDelivered}{8\xspace}  % A2.notice_delivered: count with a delivered notice frame (C3.step) over counted changed rollout
\newcommand{\AtwoP}{1.00\xspace}  % A2.p: exact two-sided sign test over pair
\newcommand{\AtwoPairs}{8\xspace}  % A2.pairs: count over pair
\newcommand{\AtwoPrecommitSha}{\texttt{e056cf19}\xspace}  % A2.precommit_sha: sha256 prefix of the pre-registration at block time over -
\newcommand{\AtwoReadTargetViolations}{0\xspace}  % A2.read_target_violations: sum over counted rollout
\newcommand{\AtwoReadTargetViolationsAll}{1\xspace}  % A2.read_target_violations_all: sum incl. the replaced episode over rollout
\newcommand{\AtwoReadViolationEpisodes}{1\xspace}  % A2.read_violation_episodes: count of episodes voided as harness_error by a read addressed to a file other than the frame over rollout
\newcommand{\AtwoRederivedSignatures}{5\xspace}  % A2.rederived_signatures: count whose signature the DEFECT #8 archive re-derivation changed over rollout
\newcommand{\AtwoReplaced}{1\xspace}  % A2.replaced: count over rollout
\newcommand{\AtwoSSuccessN}{4\xspace}  % A2S.success_n: count over successful changed rollout
\newcommand{\AtwoSSuccessReread}{3\xspace}  % A2S.success_reread: count re-reading /sessions at or after the firing request and before the clinic select over successful changed rollout
\newcommand{\AtwoSeedList}{8--15\xspace}  % spec.a2_seed_list: exact seed list (paired instances) over seed
\newcommand{\AtwoStaleFlagged}{1\xspace}  % A2.stale_flagged: count over counted changed rollout
\newcommand{\AtwoStaleUnflagged}{0\xspace}  % A2.stale_unflagged: count over counted changed rollout
\newcommand{\AtwoStepsMax}{39\xspace}  % A2.steps_max: max over counted rollout
\newcommand{\AtwoStepsMin}{22\xspace}  % A2.steps_min: min over counted rollout
\newcommand{\AtwoSuccessN}{7\xspace}  % A2.success_n: count over successful changed rollout
\newcommand{\AtwoSuccessReread}{7\xspace}  % A2.success_reread: count over successful changed rollout
\newcommand{\AtwoVOneExposed}{8\xspace}  % A2.v1_exposed: count with v1_exposed over counted changed rollout
\newcommand{\AtwoWallHours}{1.48\xspace}  % A2.wall_hours: sum of wall clock over rollout
\newcommand{\AuditFlaggedByDistractor}{4\xspace}  % audit.silent_flagged_distractor: count over counted rollout
\newcommand{\AuditReplayMatches}{78\xspace}  % audit.replay: count over counted rollout
\newcommand{\AuditRows}{78\xspace}  % audit.rows: count over counted rollout
\newcommand{\AuditSilentFlagged}{4\xspace}  % audit.silent_flagged: count over counted rollout
\newcommand{\AuditSilentReports}{22\xspace}  % audit.silent_reports: count over counted rollout
\newcommand{\AuditSilentStale}{23\xspace}  % audit.silent_stale: count over counted rollout
\newcommand{\AuditSilentStatesMove}{0\xspace}  % audit.silent_states_move: count over counted rollout
\newcommand{\AuditsEstablishedR}{On the prospective claims blocks, independent implementations resolve every outcome term of all \ClmCountedTotal{} counted rollouts and re-derive every validity verdict without disagreement, and a post-hoc raw-record reconstruction reaches the same labels on all \SweepN{} episodes: agreement on the reported records, not an unbiased estimate of defect-detection performance.\xspace}  % r31.audits: r31: Section 6's closing paragraph over -
\newcommand{\BBudgetCounted}{23\xspace}  % pre.b_counted: Block B counted budget (ADDENDUM 5) over rollout
\newcommand{\BCMainText}{Historical Block~B's value panel (Appendix~\ref{sec:historical}) did two things at the review step: it cued a re-check of this session, and it delivered the value. Block~BC asks exactly one question, cue or value: each of \BlockBCInstances fresh instances (seeds \BlockBCSeedList) is assigned OFF-A, CUE-A and LIVE-A in a \BlockBCOrderWord{} counterbalanced order, beside \BlockBCControls LIVE-I controls. OFF--CUE asks whether prompting re-verification helps; CUE--LIVE whether directly showing the current value adds further benefit. The confirmatory family is LIVE--CUE (primary) and CUE--OFF (key secondary, tested unconditionally), Holm-adjusted within the block; the estimand is the effect at the fixed \ActionBudget-action budget, so it includes the navigation effort the value saves. Claude Sonnet~5 runs the same instances as Block~BCS; the design's enlargement before any BC rollout is disclosed in Appendix~\ref{app:disclosures}.\par\paragraph{Result.} \BlockBCReadingBody\par\paragraph{Sonnet (BCS).} \BlockBCSShortForm{} Rows for one instance under different models are not pooled, and cross-model differences are descriptive.\xspace}  % r29.bc.main: Section 5.2 by BC's state (blind reviews r29: no pending filler in the main flow) over -
\newcommand{\BCMainTextR}{Historical Block~B's value panel (Appendix~\ref{sec:historical}) did two things at the review step: it cued a re-check of this session, and it delivered the value. Block~BC separates the two: each of \BlockBCInstances fresh instances is assigned OFF-A, CUE-A and LIVE-A in a \BlockBCOrderWord{} counterbalanced order, beside \BlockBCControls LIVE-I controls. CUE--OFF asks whether adding the cue-and-link panel changes success (key secondary, tested unconditionally), and LIVE--CUE (primary) whether displaying the current value in it does, Holm-adjusted within the block; the estimand is the total effect at the fixed \ActionBudget-action budget, so it includes the navigation effort the value saves. The design's enlargement before any BC rollout is disclosed in Appendix~\ref{app:disclosures}.\par\paragraph{Result.} Claude Opus~5 succeeded on \BlockBCFRXOffAPassFrac{} OFF-A, \BlockBCFRXCueAPassFrac{} CUE-A and \BlockBCFRXLiveAPassFrac{} LIVE-A instances. LIVE--CUE yielded \BlockBCLiveCueRescue{} rescues, \BlockBCLiveCueHarm{} harms and \BlockBCLiveCueTie{} ties (net \BlockBCLiveCueNetCI, exact $p=\BlockBCLiveCueP$; block-local Holm $p=\BlockBCLiveCueHolmLocal$). CUE--OFF yielded \BlockBCCueOffRescue{} rescues, \BlockBCCueOffHarm{} harms and \BlockBCCueOffTie{} ties (net \BlockBCCueOffNetCI, exact $p=\BlockBCCueOffP$; block-local Holm $p=\BlockBCCueOffHolmLocal$). Only \BlockBCFRXCueALinkFollowed{} of \BlockBCFRXCueAN{} CUE-A runs followed the panel's link (descriptive). At the registered block-local level, displaying the current location increased success relative to this cue-and-link panel. The CUE--OFF contrast did not reject; this does not establish absence of a cue effect. Contradiction, salience, and reduced verification effort remain possible explanations. The LIVE-I controls passed \BlockBCFRXLiveIPassFrac; nothing is attributed to the panel from unmatched controls. The independent scorer reconstructs appointment availability from archived rows; calendar compatibility is not re-derived but rests on stated design conditions (the generator and state preservation), whose checks are reported separately. Under that condition, every outcome term is resolved and agreeing with the evaluator on \BlockBCEndpointFull of \BlockBCCounted counted rollouts (Table~\ref{tab:coverage}). Independent validity re-derivation agrees with the archive on \BlockBCVindAgree{} attempts. The LIVE--CUE rejection survives the paper-wide Holm analysis over \HolmPaperM claim-bearing tests (adjusted $p=\BlockBCLiveCueHolmPaper$).\xspace}  % r31.bc_main: r31: Section 5.2 over -
\newcommand{\BCMainTextS}{Historical Block~B's value panel (Appendix~\ref{sec:historical}) did two things at the review step: it cued a re-check of the session and delivered the value. The clinic block with Opus~5 (BC) separates the two. Each of \BlockBCInstances fresh instances runs with no panel (OFF-A), the cue-and-link panel (CUE-A) and the value panel (LIVE-A) in a \BlockBCOrderWord{} counterbalanced order, beside \BlockBCControls LIVE-I controls. The primary contrast, LIVE--CUE, asks whether showing the value changes success; the key secondary, CUE--OFF, tests the cue-and-link panel against no panel (unconditionally). Both are Holm-adjusted within the block. The estimand is the total effect at the fixed \ActionBudget-action budget, including the navigation the value saves. The design was enlarged before any BC rollout (Appendix~\ref{app:disclosures}).\par\paragraph{Result.} Claude Opus~5 succeeded on \BlockBCFRXOffAPassFrac{} OFF-A, \BlockBCFRXCueAPassFrac{} CUE-A and \BlockBCFRXLiveAPassFrac{} LIVE-A instances. LIVE--CUE yielded \BlockBCLiveCueRescue{} rescues, \BlockBCLiveCueHarm{} harms and \BlockBCLiveCueTie{} ties (net \BlockBCLiveCueNetCI, exact $p=\BlockBCLiveCueP$; block-local Holm $p=\BlockBCLiveCueHolmLocal$). CUE--OFF yielded \BlockBCCueOffRescue{} rescues, \BlockBCCueOffHarm{} harms and \BlockBCCueOffTie{} ties (net \BlockBCCueOffNetCI, exact $p=\BlockBCCueOffP$; block-local Holm $p=\BlockBCCueOffHolmLocal$). Only \BlockBCFRXCueALinkFollowed{} of \BlockBCFRXCueAN{} CUE-A runs followed the panel's link (descriptive). At the registered block-local level, displaying the current location increased success relative to this cue-and-link panel. The CUE--OFF contrast did not reject; this does not establish absence of a cue effect. Contradiction, salience, and reduced verification effort remain possible explanations. The LIVE-I controls passed \BlockBCFRXLiveIPassFrac; nothing is attributed to the panel from unmatched controls. The independent scorer reconstructs appointment availability from archived rows; calendar compatibility is not re-derived but rests on stated design conditions (the generator and state preservation), whose checks are reported separately. Under that condition, every outcome term is resolved and agreeing with the evaluator on \BlockBCEndpointFull of \BlockBCCounted counted rollouts (Table~\ref{tab:coverage}). Independent validity re-derivation agrees with the archive on \BlockBCVindAgree{} attempts. The LIVE--CUE rejection survives the paper-wide Holm analysis over \HolmPaperM claim-bearing tests (adjusted $p=\BlockBCLiveCueHolmPaper$).\xspace}  % r37f.bc_main: r37 final reviews: Section 5.2 over -
\newcommand{\BCRCNeed}{13\xspace}  % r22.bc_rc_need: minimum favourable discordances for R-C over discordant pair
\newcommand{\BCRCReachText}{An instance favours at most one adjacent contrast (CUE-A must pass to favour CUE--OFF and fail to favour LIVE--CUE), so the reading that both reject under the block-local Holm analysis (R-C) needs at least 7 favourable discordances on one and 6 on the other, 13 in all, with none adverse: with 16 triples it is reachable only if at least 13 of them are favourable.\xspace}  % r22.bc_rc: R-C's reachability at the spec's size over -
\newcommand{\BCRCReachWord}{reachable only with at least 13 favourable triples\xspace}  % r22.bc_rc_word: R-C, in a phrase over -
\newcommand{\BCRuleCheck}{registered rule = mirror\xspace}  % r30.bc_rule_check: r30: BC's readings from the registered rule equal the mirror's on the real inputs over -
\newcommand{\BCRuleSourceSha}{\texttt{493abaaeeb4b}\xspace}  % r21.bc_rule_src: sha256 prefix of audit/block_report.py as snapshotted (the rule the BC-family selector mirrors) over -
\newcommand{\BCSAttempts}{24\xspace}  % r34.bcs_attempts: attempts in BCS's search log over attempt
\newcommand{\BCSCellsCounted}{21\xspace}  % r34.bcs_cells_counted: registered cells with a counted row over cell
\newcommand{\BCSCellsRegistered}{51\xspace}  % r34.bcs_cells: registered BCS cells (arm x instance), spec over cell
\newcommand{\BCSExecSentence}{ \emph{Execution record (no interpretation).} Block~BCS counted \BCSCellsCounted{} of its \BCSCellsRegistered{} registered cells in \BCSAttempts{} attempts (\BCSNotCounted{} not counted) before its registered launch cutoff, 12:00~UTC on 25~September. No attempt was logged between 19:30~UTC on 24~September and 04:34~UTC on 25~September: an edit to the paper generator had changed the source digest of the sealed reading rule, so the block's launch gate refused to resume it. The rule was restored byte-identically and the block resumed from its frozen search log, re-running no counted row (\code{REPAIR\_\allowbreak{}r33/\allowbreak{}BCS\_\allowbreak{}HALT\_\allowbreak{}DEVIATION.md}). The registered terminal rule had made the runner's failure terminal, so the resumption is a disclosed deviation (Appendix~\ref{app:disclosures}).\xspace}  % r34.bcs_exec: r34: BCS's execution record (counts, cutoff, halt window and cause), appended to its appendix paragraph over -
\newcommand{\BCSHaltPointer}{\paragraph{Block BCS: halt and resumption (a disclosed deviation).} An operator error in a paper file, not a rollout outcome, halted Block~BCS for about nine hours: an edit changed the source digest of the sealed reading rule, and the block's launch gate refused to resume it. Under the registered terminal rule the runner's failure was terminal; instead the rule was restored byte-identically and the block resumed from its frozen search log, re-running no counted row, with its cells, order and cutoff unchanged. The operator had seen the verdicts of its first four attempts; the resumption depended on none of them. The block ended incomplete at its registered experiment cutoff, so both of its paper-wide slots enter as $p=1$ placeholders (Appendix~\ref{app:bc}).\xspace}  % r34.bcs_halt_ptr: r34: the disclosures appendix's pointer to BCS's halt and resumption over -
\newcommand{\BCSNotCounted}{3\xspace}  % r34.bcs_not_counted: attempts not counted (validity first) over attempt
\newcommand{\BCSRuleCheck}{unfinished: registered reporter withholds every reading; mirror selects INCOMPLETE\xspace}  % r34.bcs_rule_check: r34: BCS's readings from the registered reporter equal the mirror's on the real inputs over -
\newcommand{\BGCDispositionDetail}{The terminal disposition recorded before the experiment cutoff lists the unmet launch preconditions: its release manifest, its admission link and its inline-delivery dry run.\xspace}  % r31.bgc_detail: r31: BGC's unmet preconditions over -
\newcommand{\BGCDispositionPinned}{pinned\xspace}  % r31.bgc_pin: r31: BGC's terminal disposition, pinned over -
\newcommand{\BMinEffect}{4\xspace}  % pre.b_mme: minimum meaningful effect (ADDENDUM 5) over pair
\newcommand{\BPairs}{10\xspace}  % pre.b_pairs: Block B pairs (ADDENDUM 5) over pair
\newcommand{\BPairsMinusOne}{9\xspace}  % pre.b_pairs_minus_one: Block B pairs less the one pair against that the exact test tolerates (ADDENDUM 5) over pair
\newcommand{\BPairsWords}{ten\xspace}  % pre.b_pairs_words: Block B's pairs, in words over pair
\newcommand{\BRescueExemptPreOutcome}{none\xspace}  % r22.b_exempt_pre: pre-outcome rules (S0-S6, ADDENDA 1-9) that decide Block B's rescue by the primary test alone over rule
\newcommand{\BRescueGate}{5\xspace}  % pre.b_gate: rescue-opportunity gate (ADDENDUM 5) over pair
\newcommand{\BSAmendAddenda}{11 and 12\xspace}  % coh.bs_amend_addenda: addenda applied at the amendment over -
\newcommand{\BSInvalidUnderRule}{8\xspace}  % rules.bs.invalid_under_rule: invalid BS attempts had the screenshot rule been enforced over rollout
\newcommand{\BSManifestNow}{\code{ead3fa67655a}\xspace}  % coh.bs_manifest: manifest after the amendment over -
\newcommand{\BSPreAmendCounted}{1\xspace}  % coh.bs_pre_counted: of which counted over counted rollout
\newcommand{\BSPreAmendManifest}{\code{9aa433099a46}\xspace}  % coh.bs_pre_manifest: pre-amendment manifest digest over -
\newcommand{\BSPreAmendRows}{4\xspace}  % coh.bs_pre: Block BS rows run under the pre-amendment manifest over rollout
\newcommand{\BSPreAmendSurvives}{0\xspace}  % coh.bs_pre_survives: manifest files with the pre-amendment digest that survive over file
\newcommand{\BSReserveLeft}{3\xspace}  % rules.bs.reserve_left: reserve left for the new voids over rollout
\newcommand{\BSReserveTotal}{6\xspace}  % rules.bs.reserve_total: BS block reserve over rollout
\newcommand{\BSReserveUsed}{3\xspace}  % rules.bs.reserve_used: BS reserve already used over rollout
\newcommand{\BSeedList}{20--29\xspace}  % pre.b_seed_list: exact seed list over seed
\newcommand{\BlindAdmClaims}{27\xspace}  % r31.blind.claims.adm: r31 blind challenge: claims cases admitted over case
\newcommand{\BlindAdmClinic}{9\xspace}  % r31.blind.clinic.adm: r31 blind challenge: clinic cases admitted over case
\newcommand{\BlindAdmitted}{36\xspace}  % r31.blind.adm: r31 blind challenge: cases admitted and run over case
\newcommand{\BlindAmbiguous}{1\xspace}  % r31.blind.amb: r31 blind challenge: specifications GPT-6 itself marked ambiguous over case specification
\newcommand{\BlindAppendixText}{\emph{This is neither the sealed challenge (Table~\ref{tab:challenge}) nor the post-hoc author-built checks of Appendix~\ref{app:posthoc}, and it changes neither result.} \emph{Design.} GPT-6 (ChatGPT, a new temporary chat with memory off) received a brief of verbatim excerpts of the registered rules (the claims pre-registration and the clinic addenda that govern Block~BC) and an archive schema (file list, what each log records, one type skeleton per file); the brief held no code, no paper text, no earlier case, class or finding, and no model outcome, and three redactions removed a historical defect label, a defect narrative and changelog identifiers. It returned \BlindSpecs{} case specifications (\BlindSpecsPerWorkflow{} per workflow: \BlindSpecClaimsCorrupt{} corruptions and \BlindSpecClaimsControls{} controls each), each with its expected verdict, its rule basis and any accepted alternative; they were parsed without edits, and GPT-6 marked \BlindAmbiguous{} as ambiguous. \emph{Implementation and seal.} The authors fixed the base-selection, exclusion and scoring rules while the answer was still being generated, then implemented each specification on a copy of a counted prospective archive (claims: Blocks CLM-B and CLM-BS; clinic: Block~BC), editing every copy of a fact and recomputing recorded digests. The answer, specifications, cases, expectations and all implementation, run and comparison code were sealed at \BlindSealUTC. A second GPT-6 temporary chat compared every implementation with its specification and judged \BlindAdmitted{} of the \BlindImplemented{} implemented ones faithful; its decision was recorded at \BlindFidelityUTC. The authors checked every admitted expectation against the rule text and disputed none. The run began at \BlindRunUTC, used no model and no world, and the tool and case files did not change during it. \emph{Exclusions (pre-declared rules).} Of the specifications, \BlindNoBase{} had no base archive meeting their stated requirement: \BlindNoBaseClinic{} clinic ones (\BlindNoBaseOffSucc{} need a successful OFF-A episode, and Block~BC has none) and \BlindNoBaseClaims{} claims one; the brief, being blind, did not say which outcomes each level contains, and the fidelity reviewer judged \BlindUnfaithful{} (\BlindUnfaithfulIDs) unfaithful; none of these ran. Admitted: \BlindAdmClaims{} claims cases (\BlindCorruptClaims{} corruptions, \BlindUncountedClaims{} of them expected uncounted, and \BlindControlsClaims{} controls) and \BlindAdmClinic{} clinic cases (\BlindCorruptClinic{} corruptions, all expected uncounted, and \BlindControlsClinic{} controls). \emph{Tools.} \emph{claims}: combined pipeline (classifier, void gate), evaluator with classifier, claims validity re-derivation (C8), independent scorer, simple raw-log baseline (r28), repaired raw-log checker (r29); \emph{clinic}: combined pipeline (driver row, void gate), evaluator with classifier (refresh), BC validity re-derivation, independent scorer, simple raw-log clinic baseline (r29). The clinic evaluator path re-applies what the harness computes from archived evidence, with the world readouts as archived. Two disclosed deviations: the runner crashed in its own bookkeeping on the case with a deleted trajectory before any claims tool ran, and after a one-line fix (both runner digests recorded) the claims part ran once; and the brief described the agent-attributed access log as the same list as the trajectory's, so three cases were implemented on the trajectory's copy with the slice re-derived, which the fidelity reviewer was told and confirmed.\par\paragraph{Results and every miss.} Table~\ref{tab:blind-tools} gives each tool; Table~\ref{tab:blind-cases} every case. The combined pipeline accepted all \BlindControls{} controls, counted no corruption as clean and rejected or flagged \BlindPipeCaught{} of the \BlindCorrupt{} corruptions. It missed three: on KC01, KC08 (missing trajectory, missing required artifact) the classifier alone returned the expected \code{harness\_error}, but the evaluator raised a file-not-found error, so the pipeline reached no verdict; on KC13 (missing required ON review panel) it rejected the case as \code{invalid\_intervention} rather than \code{observation\_not\_delivered}, because the evaluator's panel-geometry validity term precedes the delivery row. The claims validity re-derivation counted \BlindClaimsCEightFa{} corruptions as clean (KC06, KC07, KC09, KC11, KC12, KC13, KC14, KC15, KC20); each falls under a countedness row it does not re-derive by design, since it re-derives intervention validity only. The independent scorer counted \BlindClaimsScorerFa{} claims corruptions as clean (KC02, KC03, KC04, KC05, KC06, KC11, KC14, KC15, KC20): it does not read the stop reason, recorded infrastructure errors, read-target violations, per-call model identity, harness text across steps, access-log episode stamps or the arm payload. In the clinic, Block~BC's validity re-derivation and the scorer both counted LC07 (supplied-frame failure on silent arm) as clean: the validity script re-derives frame supply from the frame file, which the case left in place, and the scorer's input check gates only rows the driver counted; the operational driver voided the case as expected, and in a block that disagreement triggers the void gate. The simple raw-log baselines counted \BlindClaimsBaselineFa{} of the \BlindUncountedClaims{} claims corruptions expected uncounted as clean (the repaired checker the same cases) and \BlindClinicBaselineFa{} of the \BlindUncountedClinic{} clinic ones; none reads stop reasons, infrastructure errors, read targets, prompts, episode stamps or arm payloads. The clinic baseline accepted every control but never reports the booked-slot term I1 as passing, so it meets no exact expectation.\par\paragraph{Limits.} Coverage is uneven: the clinic side has \BlindCorruptClinic{} corruptions, all expected uncounted, and no outcome-invariant corruption, because every such specification needed a base outcome Block~BC does not contain; \BlindClaimsLZero{} of the \BlindAdmClaims{} claims cases use the two L0 archives, and every clinic base is an Opus Block~BC archive. The results are per case, not rates. The authors chose the brief's excerpts, wrote the implementation and chose the tools, having read the earlier challenges; the implementation was sealed before any tool ran and confirmed case by case by the fidelity reviewer. GPT-6's expectations are its readings of the registered rules.\xspace}  % r31.blind.app: r31 blind challenge: the appendix section over -
\newcommand{\BlindAppendixTextR}{\emph{This is neither the sealed challenge (Table~\ref{tab:challenge}) nor the post-hoc author-built checks of Appendix~\ref{app:posthoc}, and it changes neither result.} \emph{Design.} GPT-6 (ChatGPT, a new temporary chat with memory off) received a brief of verbatim excerpts of the registered rules (the claims pre-registration and the clinic addenda that govern Block~BC) and an archive schema (file list, what each log records, one type skeleton per file); the brief held no code, no paper text, no earlier case, class or finding, and no model outcome, and three redactions removed a historical defect label, a defect narrative and changelog identifiers. It returned \BlindSpecs{} case specifications (\BlindSpecsPerWorkflow{} per workflow: \BlindSpecClaimsCorrupt{} corruptions and \BlindSpecClaimsControls{} controls each), each with its expected verdict, its rule basis and any accepted alternative; they were parsed without edits, and GPT-6 marked \BlindAmbiguous{} as ambiguous. \emph{Implementation and seal.} The base-selection, exclusion and scoring rules were committed by digest at \BlindRulesUTC, before any answer text had been retrieved (the retrieval log records none until \BlindFirstTextUTC). The authors then implemented each specification by literal application of its named edits (a specification that could not be applied as written was to be excluded, not reinterpreted) on a copy of a counted prospective archive (claims: Blocks CLM-B and CLM-BS; clinic: Block~BC), editing every copy of a fact and recomputing recorded digests. The answer, specifications, cases, expectations and all implementation, run and comparison code were sealed at \BlindSealUTC; no tool under test had run on any case before then, so no case could be altered to make a tool fail. A second GPT-6 temporary chat---a model, not a human adjudicator---compared every implementation with its specification and judged \BlindAdmitted{} of the \BlindImplemented{} implemented ones faithful; cases it did not confirm were excluded under the frozen admission rule, and the fidelity claim remains the authors'; its decision was recorded at \BlindFidelityUTC. The authors checked every admitted expectation against the rule text and disputed none; expectations are copied verbatim and none was edited, and under the frozen rules a dispute would have been reported beside the case without changing any score. The run began at \BlindRunUTC, used no model and no world, and the tool and case files did not change during it. \emph{Exclusions (pre-declared rules).} Of the specifications, \BlindNoBase{} had no base archive meeting their stated requirement: \BlindNoBaseClinic{} clinic ones (\BlindNoBaseOffSucc{} need a successful OFF-A episode, and Block~BC has none) and \BlindNoBaseClaims{} claims one; the brief, being blind, did not say which outcomes each level contains, and the fidelity reviewer judged \BlindUnfaithful{} (\BlindUnfaithfulIDs) unfaithful; none of these ran. Admitted: \BlindAdmClaims{} claims cases (\BlindCorruptClaims{} corruptions, \BlindUncountedClaims{} of them expected uncounted, and \BlindControlsClaims{} controls) and \BlindAdmClinic{} clinic cases (\BlindCorruptClinic{} corruptions, all expected uncounted, and \BlindControlsClinic{} controls). \emph{Tools.} \emph{claims}: combined pipeline (classifier, void gate), evaluator with classifier, claims validity re-derivation (C8), independent scorer, simple raw-log baseline (r28), repaired raw-log checker (r29); \emph{clinic}: combined pipeline (driver row, void gate), evaluator with classifier (refresh), BC validity re-derivation, independent scorer, simple raw-log clinic baseline (r29). The clinic evaluator path re-applies what the harness computes from archived evidence, with the world readouts as archived. Two disclosed deviations: the runner crashed in its own bookkeeping on the case with a deleted trajectory before any claims tool had produced output; the one-line fix changed only that bookkeeping (both runner digests recorded; the tool files are identical across the two invocations), the claims part then ran once, and the clinic part, which had already run once, was not rerun; and the brief described the agent-attributed access log as the same list as the trajectory's, so three cases were implemented on the trajectory's copy with the slice re-derived, which the fidelity reviewer was told and confirmed.\par\paragraph{Results and every miss.} Table~\ref{tab:blind-tools} gives each tool; Table~\ref{tab:blind-cases} every case. The combined pipeline accepted all \BlindControls{} controls (\BlindControlsClaims{} claims, \BlindControlsClinic{} clinic) and, of the \BlindCorrupt{} corruptions, rejected or flagged \BlindPipeCaught{} (including the wrong-class case below), gave no verdict on \BlindPipeErr{} and counted none as clean: no false acceptance and \BlindPipeErr{} abstentions, which is not \BlindCorrupt/\BlindCorrupt{} detection. It missed three: on KC01, KC08 (missing trajectory, missing required artifact) the classifier alone returned the expected \code{harness\_error}, but the evaluator raised a file-not-found error, so the pipeline reached no verdict; on KC13 (missing required ON review panel) it rejected the case as \code{invalid\_intervention} rather than \code{observation\_not\_delivered}, because the evaluator's panel-geometry validity term precedes the delivery row. The claims validity re-derivation counted \BlindClaimsCEightFa{} corruptions as clean (KC06, KC07, KC09, KC11, KC12, KC13, KC14, KC15, KC20); each falls under a countedness row it does not re-derive by design, since it re-derives intervention validity only. The independent scorer counted \BlindClaimsScorerFa{} claims corruptions as clean (KC02, KC03, KC04, KC05, KC06, KC11, KC14, KC15, KC20): it does not read the stop reason, recorded infrastructure errors, read-target violations, per-call model identity, harness text across steps, access-log episode stamps or the arm payload. In the clinic, Block~BC's validity re-derivation and the scorer both counted LC07 (supplied-frame failure on silent arm) as clean: the validity script re-derives frame supply from the frame file, which the case left in place, and the scorer's input check gates only rows the driver counted; the operational driver voided the case as expected, and in a block that disagreement triggers the void gate. The simple raw-log baselines counted \BlindClaimsBaselineFa{} of the \BlindUncountedClaims{} claims corruptions expected uncounted as clean (the repaired checker the same cases) and \BlindClinicBaselineFa{} of the \BlindUncountedClinic{} clinic ones; none reads stop reasons, infrastructure errors, read targets, prompts, episode stamps or arm payloads. The clinic baseline accepted every control but never reports the booked-slot term I1 as passing, so it meets no exact expectation.\par\paragraph{Limits.} Coverage is uneven: the clinic side has \BlindCorruptClinic{} corruptions, all expected uncounted, and no outcome-invariant corruption, because every such specification needed a base outcome Block~BC does not contain; \BlindClaimsLZero{} of the \BlindAdmClaims{} claims cases use the two L0 archives, and every clinic base is an Opus Block~BC archive. The results are per case, not rates. The authors chose the brief's excerpts, wrote the implementation and chose the tools, having read the earlier challenges; the implementation was sealed before any tool ran, and a model, not an independent team, reviewed its fidelity. What was blind is exactly the case design: specifications and expected verdicts were written without the implementation, the paper, earlier cases or model outcomes. The controls are a constructed case set, not a false-positive-rate estimate, and claims and clinic counts are never pooled into a rate. GPT-6's expectations are its readings of the registered rules.\xspace}  % r32.blind_app: r32: the rule-only challenge's appendix section over -
\newcommand{\BlindBaseFA}{19\xspace}  % r31.blind.base_fa: r31 blind challenge: corruptions the simple raw-log baselines counted as clean over case
\newcommand{\BlindClaimsBaselineCaught}{3\xspace}  % r31.blind.claims.baseline_r28.caught: r31 blind challenge: claims baseline_r28: caught over case
\newcommand{\BlindClaimsBaselineErr}{1\xspace}  % r31.blind.claims.baseline_r28.err: r31 blind challenge: claims baseline_r28: err over case
\newcommand{\BlindClaimsBaselineFa}{14\xspace}  % r31.blind.claims.baseline_r28.fa: r31 blind challenge: claims baseline_r28: fa over case
\newcommand{\BlindClaimsBaselineMet}{12\xspace}  % r31.blind.claims.baseline_r28.met: r31 blind challenge: claims baseline_r28: met over case
\newcommand{\BlindClaimsBaselineOos}{2\xspace}  % r31.blind.claims.baseline_r28.oos: r31 blind challenge: claims baseline_r28: oos over case
\newcommand{\BlindClaimsCEightCaught}{6\xspace}  % r31.blind.claims.c8.caught: r31 blind challenge: claims c8: caught over case
\newcommand{\BlindClaimsCEightErr}{1\xspace}  % r31.blind.claims.c8.err: r31 blind challenge: claims c8: err over case
\newcommand{\BlindClaimsCEightFa}{9\xspace}  % r31.blind.claims.c8.fa: r31 blind challenge: claims c8: fa over case
\newcommand{\BlindClaimsCEightMet}{16\xspace}  % r31.blind.claims.c8.met: r31 blind challenge: claims c8: met over case
\newcommand{\BlindClaimsCEightOos}{4\xspace}  % r31.blind.claims.c8.oos: r31 blind challenge: claims c8: oos over case
\newcommand{\BlindClaimsEvalCaught}{18\xspace}  % r31.blind.claims.eval_classifier.caught: r31 blind challenge: claims eval_classifier: caught over case
\newcommand{\BlindClaimsEvalErr}{2\xspace}  % r31.blind.claims.eval_classifier.err: r31 blind challenge: claims eval_classifier: err over case
\newcommand{\BlindClaimsEvalFa}{0\xspace}  % r31.blind.claims.eval_classifier.fa: r31 blind challenge: claims eval_classifier: fa over case
\newcommand{\BlindClaimsEvalMet}{24\xspace}  % r31.blind.claims.eval_classifier.met: r31 blind challenge: claims eval_classifier: met over case
\newcommand{\BlindClaimsEvalOos}{0\xspace}  % r31.blind.claims.eval_classifier.oos: r31 blind challenge: claims eval_classifier: oos over case
\newcommand{\BlindClaimsLZero}{19\xspace}  % r31.blind.l0: r31 blind challenge: admitted claims cases built on an L0 archive over case
\newcommand{\BlindClaimsPipeCaught}{18\xspace}  % r31.blind.claims.pipeline.caught: r31 blind challenge: claims pipeline: caught over case
\newcommand{\BlindClaimsPipeErr}{2\xspace}  % r31.blind.claims.pipeline.err: r31 blind challenge: claims pipeline: err over case
\newcommand{\BlindClaimsPipeFa}{0\xspace}  % r31.blind.claims.pipeline.fa: r31 blind challenge: claims pipeline: fa over case
\newcommand{\BlindClaimsPipeMet}{24\xspace}  % r31.blind.claims.pipeline.met: r31 blind challenge: claims pipeline: met over case
\newcommand{\BlindClaimsPipeOos}{0\xspace}  % r31.blind.claims.pipeline.oos: r31 blind challenge: claims pipeline: oos over case
\newcommand{\BlindClaimsRepairedCaught}{3\xspace}  % r31.blind.claims.repaired_r29.caught: r31 blind challenge: claims repaired_r29: caught over case
\newcommand{\BlindClaimsRepairedErr}{1\xspace}  % r31.blind.claims.repaired_r29.err: r31 blind challenge: claims repaired_r29: err over case
\newcommand{\BlindClaimsRepairedFa}{14\xspace}  % r31.blind.claims.repaired_r29.fa: r31 blind challenge: claims repaired_r29: fa over case
\newcommand{\BlindClaimsRepairedMet}{12\xspace}  % r31.blind.claims.repaired_r29.met: r31 blind challenge: claims repaired_r29: met over case
\newcommand{\BlindClaimsRepairedOos}{2\xspace}  % r31.blind.claims.repaired_r29.oos: r31 blind challenge: claims repaired_r29: oos over case
\newcommand{\BlindClaimsScorerCaught}{10\xspace}  % r31.blind.claims.scorer.caught: r31 blind challenge: claims scorer: caught over case
\newcommand{\BlindClaimsScorerErr}{1\xspace}  % r31.blind.claims.scorer.err: r31 blind challenge: claims scorer: err over case
\newcommand{\BlindClaimsScorerFa}{9\xspace}  % r31.blind.claims.scorer.fa: r31 blind challenge: claims scorer: fa over case
\newcommand{\BlindClaimsScorerMet}{12\xspace}  % r31.blind.claims.scorer.met: r31 blind challenge: claims scorer: met over case
\newcommand{\BlindClaimsScorerOos}{0\xspace}  % r31.blind.claims.scorer.oos: r31 blind challenge: claims scorer: oos over case
\newcommand{\BlindClinicBaselineCaught}{1\xspace}  % r31.blind.clinic.baseline_r29.caught: r31 blind challenge: clinic baseline_r29: caught over case
\newcommand{\BlindClinicBaselineErr}{0\xspace}  % r31.blind.clinic.baseline_r29.err: r31 blind challenge: clinic baseline_r29: err over case
\newcommand{\BlindClinicBaselineFa}{5\xspace}  % r31.blind.clinic.baseline_r29.fa: r31 blind challenge: clinic baseline_r29: fa over case
\newcommand{\BlindClinicBaselineMet}{0\xspace}  % r31.blind.clinic.baseline_r29.met: r31 blind challenge: clinic baseline_r29: met over case
\newcommand{\BlindClinicBaselineOos}{0\xspace}  % r31.blind.clinic.baseline_r29.oos: r31 blind challenge: clinic baseline_r29: oos over case
\newcommand{\BlindClinicEvalCaught}{6\xspace}  % r31.blind.clinic.eval_classifier.caught: r31 blind challenge: clinic eval_classifier: caught over case
\newcommand{\BlindClinicEvalErr}{0\xspace}  % r31.blind.clinic.eval_classifier.err: r31 blind challenge: clinic eval_classifier: err over case
\newcommand{\BlindClinicEvalFa}{0\xspace}  % r31.blind.clinic.eval_classifier.fa: r31 blind challenge: clinic eval_classifier: fa over case
\newcommand{\BlindClinicEvalMet}{9\xspace}  % r31.blind.clinic.eval_classifier.met: r31 blind challenge: clinic eval_classifier: met over case
\newcommand{\BlindClinicEvalOos}{0\xspace}  % r31.blind.clinic.eval_classifier.oos: r31 blind challenge: clinic eval_classifier: oos over case
\newcommand{\BlindClinicPipeCaught}{6\xspace}  % r31.blind.clinic.pipeline.caught: r31 blind challenge: clinic pipeline: caught over case
\newcommand{\BlindClinicPipeErr}{0\xspace}  % r31.blind.clinic.pipeline.err: r31 blind challenge: clinic pipeline: err over case
\newcommand{\BlindClinicPipeFa}{0\xspace}  % r31.blind.clinic.pipeline.fa: r31 blind challenge: clinic pipeline: fa over case
\newcommand{\BlindClinicPipeMet}{9\xspace}  % r31.blind.clinic.pipeline.met: r31 blind challenge: clinic pipeline: met over case
\newcommand{\BlindClinicPipeOos}{0\xspace}  % r31.blind.clinic.pipeline.oos: r31 blind challenge: clinic pipeline: oos over case
\newcommand{\BlindClinicScorerCaught}{5\xspace}  % r31.blind.clinic.scorer.caught: r31 blind challenge: clinic scorer: caught over case
\newcommand{\BlindClinicScorerErr}{0\xspace}  % r31.blind.clinic.scorer.err: r31 blind challenge: clinic scorer: err over case
\newcommand{\BlindClinicScorerFa}{1\xspace}  % r31.blind.clinic.scorer.fa: r31 blind challenge: clinic scorer: fa over case
\newcommand{\BlindClinicScorerMet}{8\xspace}  % r31.blind.clinic.scorer.met: r31 blind challenge: clinic scorer: met over case
\newcommand{\BlindClinicScorerOos}{0\xspace}  % r31.blind.clinic.scorer.oos: r31 blind challenge: clinic scorer: oos over case
\newcommand{\BlindClinicVindCaught}{5\xspace}  % r31.blind.clinic.vi.caught: r31 blind challenge: clinic vi: caught over case
\newcommand{\BlindClinicVindErr}{0\xspace}  % r31.blind.clinic.vi.err: r31 blind challenge: clinic vi: err over case
\newcommand{\BlindClinicVindFa}{1\xspace}  % r31.blind.clinic.vi.fa: r31 blind challenge: clinic vi: fa over case
\newcommand{\BlindClinicVindMet}{8\xspace}  % r31.blind.clinic.vi.met: r31 blind challenge: clinic vi: met over case
\newcommand{\BlindClinicVindOos}{0\xspace}  % r31.blind.clinic.vi.oos: r31 blind challenge: clinic vi: oos over case
\newcommand{\BlindControls}{10\xspace}  % r31.blind.ctl: r31 blind challenge: valid controls admitted over case
\newcommand{\BlindControlsClaims}{7\xspace}  % r31.blind.claims.ctl: r31 blind challenge: claims controls admitted over case
\newcommand{\BlindControlsClinic}{3\xspace}  % r31.blind.clinic.ctl: r31 blind challenge: clinic controls admitted over case
\newcommand{\BlindCorrupt}{26\xspace}  % r31.blind.cor: r31 blind challenge: corruptions admitted over case
\newcommand{\BlindCorruptClaims}{20\xspace}  % r31.blind.claims.cor: r31 blind challenge: claims corruptions admitted over case
\newcommand{\BlindCorruptClinic}{6\xspace}  % r31.blind.clinic.cor: r31 blind challenge: clinic corruptions admitted over case
\newcommand{\BlindDisputes}{0\xspace}  % r31.blind.disputes: r31 blind challenge: admitted expectations the authors disputed over case
\newcommand{\BlindExcluded}{20\xspace}  % r31.blind.excl: r31 blind challenge: specifications excluded over case specification
\newcommand{\BlindFidelityUTC}{2026-09-24 19:08Z\xspace}  % r31.blind.fid_utc: r31 blind challenge: when the fidelity decision was recorded over -
\newcommand{\BlindFirstTextUTC}{2026-09-24 18:51Z\xspace}  % r32.blind.first_utc: r32: the first retrieval poll that found answer text over -
\newcommand{\BlindImplemented}{38\xspace}  % r31.blind.implemented: r31 blind challenge: specs implemented over case specification
\newcommand{\BlindMainParagraph}{\paragraph{A blind-constructed challenge.} Unlike the sealed and post-hoc cases, GPT-6 designed the case classes and expected verdicts from registered rules and archive schema alone; we implemented them on archive copies, a second GPT-6 chat checked fidelity, and each tool ran once on \BlindAdmitted{} cases. The pipeline accepted all \BlindControls{} controls and counted none of \BlindCorrupt{} corruptions as clean, but gave no verdict on two and the wrong class to one; the scorer counted \BlindScorerFA{} as clean, raw-log baselines \BlindBaseFA{} (Appendix~\ref{app:blind}).\xspace}  % r31.blind.main: r31 blind challenge: Section 6 paragraph over -
\newcommand{\BlindMainR}{\paragraph{Rule-only case-design challenge.} A fresh GPT-6 chat, given only registered-rule excerpts and the archive schema---no implementation code, paper, earlier cases or model outcomes---specified \BlindSpecs{} corruption and control cases with expected verdicts. We implemented them on archive copies under rules frozen before any answer text was retrieved; a second GPT-6 chat reviewed fidelity, and unconfirmed cases and cases without a base archive were excluded by the frozen rule, leaving \BlindAdmitted{} cases, run once. The combined pipeline accepted all \BlindControls{} controls; of \BlindCorrupt{} admitted corruptions (\BlindCorruptClaims{} claims, \BlindCorruptClinic{} clinic) it rejected or outcome-flagged \BlindPipeCaught (one under an unexpected validity class), gave no verdict on \BlindPipeErr and counted none as clean; the outcome scorer alone counted \BlindScorerFA{} as clean, the simple raw-log baselines \BlindBaseFA. Only the case design was blind: we chose the rule excerpts, implemented the cases and chose the tools, and clinic coverage is thin (\BlindCorruptClinic{} corruptions, none on an outcome invariant), so these are case-level results on this suite, not a detection rate or independent-team validation (Appendix~\ref{app:blind}).\xspace}  % r32.blind_main: r32: Section 6: the rule-only case-design challenge over -
\newcommand{\BlindMainThree}{\paragraph{Rule-only case-design challenge.} A fresh GPT-6 chat given only rule excerpts and the archive schema (no code, paper, earlier cases or outcomes) specified \BlindSpecs{} cases with expected verdicts. We implemented them on archive copies under frozen rules; a second chat reviewed fidelity, and \BlindAdmitted{} admitted cases ran once. The pipeline accepted all \BlindControls{} controls and, of \BlindCorrupt{} corruptions, caught \BlindPipeCaught{} (one under another class), gave no verdict on \BlindPipeErr{} and counted none as clean (outcome scorer alone: \BlindScorerFA; raw-log baselines: \BlindBaseFA). Only the case design was blind, and clinic coverage is thin (Appendix~\ref{app:blind}).\xspace}  % r34.ext.blind3: r34 external challenge: Section 6: the rule-only challenge (compact) over -
\newcommand{\BlindNoBase}{18\xspace}  % r31.blind.nobase: r31 blind challenge: specs with no base archive over case specification
\newcommand{\BlindNoBaseClaims}{1\xspace}  % r31.blind.claims.nobase: r31 blind challenge: claims specs with no base archive over case specification
\newcommand{\BlindNoBaseClinic}{17\xspace}  % r31.blind.clinic.nobase: r31 blind challenge: clinic specs with no base archive over case specification
\newcommand{\BlindNoBaseOffSucc}{13\xspace}  % r31.blind.off_succ: r31 blind challenge: clinic specs needing a successful OFF-A episode (Block BC has none) over case specification
\newcommand{\BlindPipeCaught}{24\xspace}  % r31.blind.pipe.caught: r31 blind challenge: pipeline, both workflows: caught over case
\newcommand{\BlindPipeCtlOk}{10\xspace}  % r31.blind.pipe.ctl_ok: r31 blind challenge: pipeline, both workflows: ctl_ok over case
\newcommand{\BlindPipeErr}{2\xspace}  % r31.blind.pipe.err: r31 blind challenge: pipeline, both workflows: err over case
\newcommand{\BlindPipeFA}{0\xspace}  % r31.blind.pipe.fa: r31 blind challenge: pipeline, both workflows: fa over case
\newcommand{\BlindPipeFR}{0\xspace}  % r31.blind.pipe.fr: r31 blind challenge: pipeline, both workflows: fr over case
\newcommand{\BlindPipeMet}{33\xspace}  % r31.blind.pipe.met: r31 blind challenge: pipeline, both workflows: met over case
\newcommand{\BlindPipeWrongClass}{1\xspace}  % r31.blind.pipe.wrong: r31 blind challenge: pipeline, both workflows: wrong over case
\newcommand{\BlindRulesUTC}{2026-09-24 18:44Z\xspace}  % r32.blind.rules_utc: r32: when the implementation and scoring rules were committed by digest over -
\newcommand{\BlindRunUTC}{2026-09-24 19:08Z\xspace}  % r31.blind.run_utc: r31 blind challenge: when the run started over -
\newcommand{\BlindScorerFA}{10\xspace}  % r31.blind.scorer_fa: r31 blind challenge: corruptions the independent scorer counted as clean (both workflows) over case
\newcommand{\BlindSealUTC}{2026-09-24 19:00Z\xspace}  % r31.blind.seal_utc: r31 blind challenge: when the lane was sealed over -
\newcommand{\BlindSpecClaimsControls}{8\xspace}  % r31.blind.claims.ctl_spec: r31 blind challenge: claims controls specified over case specification
\newcommand{\BlindSpecClaimsCorrupt}{20\xspace}  % r31.blind.claims.cor_spec: r31 blind challenge: claims corruptions specified over case specification
\newcommand{\BlindSpecClinicControls}{8\xspace}  % r31.blind.clinic.ctl_spec: r31 blind challenge: clinic controls specified over case specification
\newcommand{\BlindSpecClinicCorrupt}{20\xspace}  % r31.blind.clinic.cor_spec: r31 blind challenge: clinic corruptions specified over case specification
\newcommand{\BlindSpecs}{56\xspace}  % r31.blind.specs: r31 blind challenge: specifications GPT-6 returned over case specification
\newcommand{\BlindSpecsPerWorkflow}{28\xspace}  % r31.blind.specs_w: r31 blind challenge: specifications per workflow over case specification
\newcommand{\BlindUncountedClaims}{16\xspace}  % r31.blind.claims.unc: r31 blind challenge: claims corruptions GPT-6 expected uncounted over case
\newcommand{\BlindUncountedClinic}{6\xspace}  % r31.blind.clinic.unc: r31 blind challenge: clinic corruptions GPT-6 expected uncounted over case
\newcommand{\BlindUnfaithful}{2\xspace}  % r31.blind.unf: r31 blind challenge: specs the fidelity reviewer judged unfaithful over case specification
\newcommand{\BlindUnfaithfulIDs}{LC14, LC15\xspace}  % r31.blind.unf_ids: r31 blind challenge: the unfaithful specs over -
\newcommand{\BlindValidityFA}{10\xspace}  % r31.blind.vind_fa: r31 blind challenge: corruptions the validity re-derivations counted as clean (both workflows) over case
\newcommand{\BlockAtwoSEffect}{---\xspace}  % pending.AtwoS.effect: discordant-pair proportion (envos.stats.effect_size; NOT the net paired effect) over pair
\newcommand{\BlockAtwoSNNeg}{---\xspace}  % pending.AtwoS.n_neg: count over pair
\newcommand{\BlockAtwoSNPos}{---\xspace}  % pending.AtwoS.n_pos: count over pair
\newcommand{\BlockAtwoSNTied}{---\xspace}  % pending.AtwoS.n_tied: count over pair
\newcommand{\BlockAtwoSP}{---\xspace}  % pending.AtwoS.p: exact two-sided sign test over pair
\newcommand{\BlockAtwoSPairs}{---\xspace}  % pending.AtwoS.pairs: count over pair
\newcommand{\BlockAtwoSRows}{9\xspace}  % pending.AtwoS.rows: rows so far over rollout
\newcommand{\BlockAtwoSSCCap}{2\xspace}  % pending.AtwoS.S-C.Cap: count over counted rollout
\newcommand{\BlockAtwoSSCN}{4\xspace}  % pending.AtwoS.S-C.n: count over counted rollout
\newcommand{\BlockAtwoSSCPass}{2\xspace}  % pending.AtwoS.S-C.pass: count over counted rollout
\newcommand{\BlockAtwoSSCPassFrac}{2/4\xspace}  % pending.AtwoS.S-C.frac: k/n over counted rollout
\newcommand{\BlockAtwoSSCRevised}{0\xspace}  % pending.AtwoS.S-C.Revised: count over counted rollout
\newcommand{\BlockAtwoSSCStaleFlagged}{0\xspace}  % pending.AtwoS.S-C.StaleFlagged: count over counted rollout
\newcommand{\BlockAtwoSSCStaleUnflagged}{0\xspace}  % pending.AtwoS.S-C.StaleUnflagged: count over counted rollout
\newcommand{\BlockAtwoSSLtwoCap}{0\xspace}  % pending.AtwoS.S-L2.Cap: count over counted rollout
\newcommand{\BlockAtwoSSLtwoN}{4\xspace}  % pending.AtwoS.S-L2.n: count over counted rollout
\newcommand{\BlockAtwoSSLtwoPass}{4\xspace}  % pending.AtwoS.S-L2.pass: count over counted rollout
\newcommand{\BlockAtwoSSLtwoPassFrac}{4/4\xspace}  % pending.AtwoS.S-L2.frac: k/n over counted rollout
\newcommand{\BlockAtwoSSLtwoRevised}{0\xspace}  % pending.AtwoS.S-L2.Revised: count over counted rollout
\newcommand{\BlockAtwoSSLtwoStaleFlagged}{0\xspace}  % pending.AtwoS.S-L2.StaleFlagged: count over counted rollout
\newcommand{\BlockAtwoSSLtwoStaleUnflagged}{0\xspace}  % pending.AtwoS.S-L2.StaleUnflagged: count over counted rollout
\newcommand{\BlockAtwoSSLzeroCap}{0\xspace}  % pending.AtwoS.S-L0.Cap: count over counted rollout
\newcommand{\BlockAtwoSSLzeroN}{1\xspace}  % pending.AtwoS.S-L0.n: count over counted rollout
\newcommand{\BlockAtwoSSLzeroPass}{1\xspace}  % pending.AtwoS.S-L0.pass: count over counted rollout
\newcommand{\BlockAtwoSSLzeroPassFrac}{1/1\xspace}  % pending.AtwoS.S-L0.frac: k/n over counted rollout
\newcommand{\BlockAtwoSSLzeroRevised}{0\xspace}  % pending.AtwoS.S-L0.Revised: count over counted rollout
\newcommand{\BlockAtwoSSLzeroStaleFlagged}{0\xspace}  % pending.AtwoS.S-L0.StaleFlagged: count over counted rollout
\newcommand{\BlockAtwoSSLzeroStaleUnflagged}{0\xspace}  % pending.AtwoS.S-L0.StaleUnflagged: count over counted rollout
\newcommand{\BlockAtwoSStatus}{\texttt{complete}\xspace}  % pending.AtwoS.status: search-log status over -
\newcommand{\BlockAtwoSVoided}{0\xspace}  % pending.AtwoS.voided: count over rollout
\newcommand{\BlockBCConfig}{Claude CLI, frames by file read\xspace}  % r21.BC.config: invoker and frame-delivery channel, from the spec over -
\newcommand{\BlockBCContradictions}{0\xspace}  % r21.BC.Contradictions: Contradictions over counted rollout
\newcommand{\BlockBCControls}{3\xspace}  % r21.BC.controls: unpaired control rollouts in the spec over rollout
\newcommand{\BlockBCCounted}{51\xspace}  % r21.BC.counted: counted rollouts over rollout
\newcommand{\BlockBCCountedFail}{31\xspace}  % r21.BC.CountedFail: counted failures over counted rollout
\newcommand{\BlockBCCountedSucc}{20\xspace}  % r21.BC.CountedSucc: CountedSucc over counted rollout
\newcommand{\BlockBCCueOffBonfPaper}{1.00\xspace}  % fam.alias.BC.CueOff.b: alias over -
\newcommand{\BlockBCCueOffBothFail}{14\xspace}  % r21.BC.CueOff.BothFail: both failed over pair
\newcommand{\BlockBCCueOffBothPass}{0\xspace}  % r21.BC.CueOff.BothPass: both passed over pair
\newcommand{\BlockBCCueOffDir}{treatment\xspace}  % r21.BC.CueOff.Dir: direction of the discordance over pair
\newcommand{\BlockBCCueOffHarm}{0\xspace}  % r21.BC.CueOff.Harm: control passed, treatment failed over pair
\newcommand{\BlockBCCueOffHolmLocal}{0.5\xspace}  % r21.BC.CueOff.HolmLocal: block-local Holm over pair
\newcommand{\BlockBCCueOffHolmPaper}{1.00\xspace}  % fam.alias.BC.CueOff: alias over -
\newcommand{\BlockBCCueOffMinPairs}{13\xspace}  % r21.BC.CueOff.MinPairs: G1 minimum complete pairs of this contrast (min_pairs_by_contrast, else min_pairs) over pair
\newcommand{\BlockBCCueOffNet}{$+0.13$\xspace}  % r21.BC.CueOff.Net: net paired difference over pair
\newcommand{\BlockBCCueOffNetCI}{$+0.13$ [$-0.09$, $0.36$]\xspace}  % r21.BC.CueOff.NetCI: net paired difference, Newcombe method-10 marginal 95% interval over pair
\newcommand{\BlockBCCueOffP}{0.5\xspace}  % r21.BC.CueOff.P: exact two-sided sign test over pair
\newcommand{\BlockBCCueOffPairs}{16\xspace}  % r21.BC.CueOff.Pairs: complete pairs over pair
\newcommand{\BlockBCCueOffRescue}{2\xspace}  % r21.BC.CueOff.Rescue: control failed, treatment passed over pair
\newcommand{\BlockBCCueOffTie}{14\xspace}  % r21.BC.CueOff.Tie: both passed or both failed over pair
\newcommand{\BlockBCDecisionTerm}{50\xspace}  % r21.BC.DecisionTerm: DecisionTerm over counted rollout
\newcommand{\BlockBCDisposition}{completed\xspace}  % r21.BC.disposition: disposition text over -
\newcommand{\BlockBCEffect}{0.812\xspace}  % pending.BC.effect: discordant-pair proportion (envos.stats.effect_size; NOT the net paired effect) over pair
\newcommand{\BlockBCEndpointFull}{51\xspace}  % r21.BC.EndpointFull: EndpointFull over counted rollout
\newcommand{\BlockBCEndpointFullSucc}{20\xspace}  % r21.BC.EndpointFullSucc: EndpointFullSucc over counted rollout
\newcommand{\BlockBCEndpointUnresolved}{0\xspace}  % r21.BC.EndpointUnresolved: EndpointUnresolved over counted rollout
\newcommand{\BlockBCFRXCueACap}{0\xspace}  % pending.BC.FRX-CUE-A.Cap: count over counted rollout
\newcommand{\BlockBCFRXCueALinkFollowed}{1\xspace}  % r21.BC.FRXCueALinkFollowed: process measure followed_panel_link at FRX-CUE-A (descriptive) over rollout
\newcommand{\BlockBCFRXCueAN}{16\xspace}  % pending.BC.FRX-CUE-A.n: count over counted rollout
\newcommand{\BlockBCFRXCueAPass}{2\xspace}  % pending.BC.FRX-CUE-A.pass: count over counted rollout
\newcommand{\BlockBCFRXCueAPassFrac}{2/16\xspace}  % pending.BC.FRX-CUE-A.frac: k/n over counted rollout
\newcommand{\BlockBCFRXCueARecovered}{1\xspace}  % r21.BC.FRXCueARecovered: process measure bc_recovered at FRX-CUE-A (descriptive) over rollout
\newcommand{\BlockBCFRXCueARevised}{0\xspace}  % pending.BC.FRX-CUE-A.Revised: count over counted rollout
\newcommand{\BlockBCFRXCueAStaleFlagged}{1\xspace}  % pending.BC.FRX-CUE-A.StaleFlagged: count over counted rollout
\newcommand{\BlockBCFRXCueAStaleUnflagged}{0\xspace}  % pending.BC.FRX-CUE-A.StaleUnflagged: count over counted rollout
\newcommand{\BlockBCFRXLiveACap}{1\xspace}  % pending.BC.FRX-LIVE-A.Cap: count over counted rollout
\newcommand{\BlockBCFRXLiveAN}{16\xspace}  % pending.BC.FRX-LIVE-A.n: count over counted rollout
\newcommand{\BlockBCFRXLiveAPass}{15\xspace}  % pending.BC.FRX-LIVE-A.pass: count over counted rollout
\newcommand{\BlockBCFRXLiveAPassFrac}{15/16\xspace}  % pending.BC.FRX-LIVE-A.frac: k/n over counted rollout
\newcommand{\BlockBCFRXLiveARecovered}{15\xspace}  % r21.BC.FRXLiveARecovered: process measure bc_recovered at FRX-LIVE-A (descriptive) over rollout
\newcommand{\BlockBCFRXLiveARevised}{15\xspace}  % pending.BC.FRX-LIVE-A.Revised: count over counted rollout
\newcommand{\BlockBCFRXLiveAStaleFlagged}{0\xspace}  % pending.BC.FRX-LIVE-A.StaleFlagged: count over counted rollout
\newcommand{\BlockBCFRXLiveAStaleUnflagged}{0\xspace}  % pending.BC.FRX-LIVE-A.StaleUnflagged: count over counted rollout
\newcommand{\BlockBCFRXLiveICap}{0\xspace}  % pending.BC.FRX-LIVE-I.Cap: count over counted rollout
\newcommand{\BlockBCFRXLiveIN}{3\xspace}  % pending.BC.FRX-LIVE-I.n: count over counted rollout
\newcommand{\BlockBCFRXLiveIPass}{3\xspace}  % pending.BC.FRX-LIVE-I.pass: count over counted rollout
\newcommand{\BlockBCFRXLiveIPassFrac}{3/3\xspace}  % pending.BC.FRX-LIVE-I.frac: k/n over counted rollout
\newcommand{\BlockBCFRXLiveIRevised}{0\xspace}  % pending.BC.FRX-LIVE-I.Revised: count over counted rollout
\newcommand{\BlockBCFRXLiveIStaleFlagged}{0\xspace}  % pending.BC.FRX-LIVE-I.StaleFlagged: count over counted rollout
\newcommand{\BlockBCFRXLiveIStaleUnflagged}{0\xspace}  % pending.BC.FRX-LIVE-I.StaleUnflagged: count over counted rollout
\newcommand{\BlockBCFRXOffACap}{0\xspace}  % pending.BC.FRX-OFF-A.Cap: count over counted rollout
\newcommand{\BlockBCFRXOffAN}{16\xspace}  % pending.BC.FRX-OFF-A.n: count over counted rollout
\newcommand{\BlockBCFRXOffAPass}{0\xspace}  % pending.BC.FRX-OFF-A.pass: count over counted rollout
\newcommand{\BlockBCFRXOffAPassFrac}{0/16\xspace}  % pending.BC.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\BlockBCFRXOffARevised}{0\xspace}  % pending.BC.FRX-OFF-A.Revised: count over counted rollout
\newcommand{\BlockBCFRXOffAStaleFlagged}{3\xspace}  % pending.BC.FRX-OFF-A.StaleFlagged: count over counted rollout
\newcommand{\BlockBCFRXOffAStaleUnflagged}{13\xspace}  % pending.BC.FRX-OFF-A.StaleUnflagged: count over counted rollout
\newcommand{\BlockBCGzero}{ok\xspace}  % r21.BC.g0: G0 (ADDENDUM 18 section 6.5), from the generated report over -
\newcommand{\BlockBCGzeroWhy}{--\xspace}  % r21.BC.g0_why: G0 problems over -
\newcommand{\BlockBCInstancePhrase}{\BlockBCInstances frozen generated instances (seeds \BlockBCSeedList)\xspace}  % r21.BC.instance_phrase: the block's instances as a phrase that reads correctly whether or not its spec exists over -
\newcommand{\BlockBCInstances}{16\xspace}  % r21.BC.instances: paired instances over instance
\newcommand{\BlockBCInstancesWords}{sixteen\xspace}  % r21.BC.instances_words: in words over instance
\newcommand{\BlockBCLiveCueBonfPaper}{0.00293\xspace}  % fam.alias.BC.LiveCue.b: alias over -
\newcommand{\BlockBCLiveCueBothFail}{1\xspace}  % r21.BC.LiveCue.BothFail: both failed over pair
\newcommand{\BlockBCLiveCueBothPass}{2\xspace}  % r21.BC.LiveCue.BothPass: both passed over pair
\newcommand{\BlockBCLiveCueDir}{treatment\xspace}  % r21.BC.LiveCue.Dir: direction of the discordance over pair
\newcommand{\BlockBCLiveCueHarm}{0\xspace}  % r21.BC.LiveCue.Harm: control passed, treatment failed over pair
\newcommand{\BlockBCLiveCueHolmLocal}{0.000488\xspace}  % r21.BC.LiveCue.HolmLocal: block-local Holm over pair
\newcommand{\BlockBCLiveCueHolmPaper}{0.00293\xspace}  % fam.alias.BC.LiveCue: alias over -
\newcommand{\BlockBCLiveCueMinPairs}{13\xspace}  % r21.BC.LiveCue.MinPairs: G1 minimum complete pairs of this contrast (min_pairs_by_contrast, else min_pairs) over pair
\newcommand{\BlockBCLiveCueNet}{$+0.81$\xspace}  % r21.BC.LiveCue.Net: net paired difference over pair
\newcommand{\BlockBCLiveCueNetCI}{$+0.81$ [$0.49$, $0.92$]\xspace}  % r21.BC.LiveCue.NetCI: net paired difference, Newcombe method-10 marginal 95% interval over pair
\newcommand{\BlockBCLiveCueP}{0.000244\xspace}  % r21.BC.LiveCue.P: exact two-sided sign test over pair
\newcommand{\BlockBCLiveCuePairs}{16\xspace}  % r21.BC.LiveCue.Pairs: complete pairs over pair
\newcommand{\BlockBCLiveCueRescue}{13\xspace}  % r21.BC.LiveCue.Rescue: control failed, treatment passed over pair
\newcommand{\BlockBCLiveCueTie}{3\xspace}  % r21.BC.LiveCue.Tie: both passed or both failed over pair
\newcommand{\BlockBCLiveOffBonfPaper}{\textit{outside the family}\xspace}  % fam.alias.BC.LiveOff.b: not a paper-wide test over -
\newcommand{\BlockBCLiveOffBothFail}{1\xspace}  % r21.BC.LiveOff.BothFail: both failed over pair
\newcommand{\BlockBCLiveOffBothPass}{0\xspace}  % r21.BC.LiveOff.BothPass: both passed over pair
\newcommand{\BlockBCLiveOffDir}{treatment\xspace}  % r21.BC.LiveOff.Dir: direction of the discordance over pair
\newcommand{\BlockBCLiveOffHarm}{0\xspace}  % r21.BC.LiveOff.Harm: control passed, treatment failed over pair
\newcommand{\BlockBCLiveOffHolmLocal}{---\xspace}  % r21.BC.LiveOff.HolmLocal: not in a block-local family over pair
\newcommand{\BlockBCLiveOffHolmPaper}{\textit{outside the family}\xspace}  % fam.alias.BC.LiveOff: not a paper-wide test over -
\newcommand{\BlockBCLiveOffNet}{$+0.94$\xspace}  % r21.BC.LiveOff.Net: net paired difference over pair
\newcommand{\BlockBCLiveOffNetCI}{$+0.94$ [$0.64$, $0.99$]\xspace}  % r21.BC.LiveOff.NetCI: net paired difference, Newcombe method-10 marginal 95% interval over pair
\newcommand{\BlockBCLiveOffP}{6.1e-05\xspace}  % r21.BC.LiveOff.P: exact two-sided sign test over pair
\newcommand{\BlockBCLiveOffPairs}{16\xspace}  % r21.BC.LiveOff.Pairs: complete pairs over pair
\newcommand{\BlockBCLiveOffRescue}{15\xspace}  % r21.BC.LiveOff.Rescue: control failed, treatment passed over pair
\newcommand{\BlockBCLiveOffTie}{1\xspace}  % r21.BC.LiveOff.Tie: both passed or both failed over pair
\newcommand{\BlockBCMinPairs}{13\xspace}  % r21.BC.min_pairs: G1 minimum complete pairs over pair
\newcommand{\BlockBCModel}{Claude Opus~5\xspace}  % r21.BC.model: evaluated model over -
\newcommand{\BlockBCNNeg}{13\xspace}  % pending.BC.n_neg: count over pair
\newcommand{\BlockBCNPos}{0\xspace}  % pending.BC.n_pos: count over pair
\newcommand{\BlockBCNTied}{3\xspace}  % pending.BC.n_tied: count over pair
\newcommand{\BlockBCOffFail}{16\xspace}  % r21.BC.off_fail: FRX-OFF-A failures over instance
\newcommand{\BlockBCOffGate}{8\xspace}  % r21.BC.off_gate: R-D/R-E OFF-A failure gate over instance
\newcommand{\BlockBCOffPass}{0\xspace}  % r21.BC.off_pass: FRX-OFF-A successes over instance
\newcommand{\BlockBCOffPlanned}{16\xspace}  % r21.BC.off_planned: planned FRX-OFF-A rows (R-E states n of the planned rows) over rollout
\newcommand{\BlockBCOffReread}{0\xspace}  % r21.BC.OffReread: process measure source_visit_after_review at FRX-OFF-A (descriptive) over rollout
\newcommand{\BlockBCOrderWord}{frozen\xspace}  % r22.bc_order: 'frozen' only once ADDENDUM 18 is frozen over -
\newcommand{\BlockBCP}{0.000\xspace}  % pending.BC.p: exact two-sided sign test over pair
\newcommand{\BlockBCPairs}{16\xspace}  % pending.BC.pairs: count over pair
\newcommand{\BlockBCReadingBody}{Claude Opus~5 passed OFF-A \BlockBCFRXOffAPassFrac, CUE-A \BlockBCFRXCueAPassFrac and LIVE-A \BlockBCFRXLiveAPassFrac on \BlockBCInstances instances (Table~\ref{tab:tests} gives every contrast). At the registered block-local level, displaying the current location increased success relative to this cue-and-link panel. The CUE--OFF contrast did not reject; this does not establish absence of a cue effect. Contradiction, salience, and reduced verification effort remain possible explanations. The LIVE--CUE rejection survives the paper-wide Holm analysis over \HolmPaperM claim-bearing tests (adjusted $p=\BlockBCLiveCueHolmPaper$). The LIVE-I controls passed \BlockBCFRXLiveIPassFrac; nothing is attributed to the panel from unmatched controls. The independent scorer reconstructs appointment availability from archived rows; calendar compatibility is not re-derived but rests on stated design conditions (the generator and state preservation), whose checks are reported separately. Under that condition, every outcome term is resolved and agreeing with the evaluator on \BlockBCEndpointFull of \BlockBCCounted counted rollouts (Table~\ref{tab:coverage}).\xspace}  % r21.BC.body: main-text reading paragraph over -
\newcommand{\BlockBCReadingFull}{Over the \BlockBCInstances instances (seeds \BlockBCSeedList), Claude Opus~5 passed OFF-A \BlockBCFRXOffAPassFrac, CUE-A \BlockBCFRXCueAPassFrac and LIVE-A \BlockBCFRXLiveAPassFrac. LIVE versus CUE (primary): rescue \BlockBCLiveCueRescue, harm \BlockBCLiveCueHarm, tie \BlockBCLiveCueTie of \BlockBCLiveCuePairs pairs, net \BlockBCLiveCueNetCI (marginal 95\,\% interval), $p=\BlockBCLiveCueP$ (block-local Holm $p=\BlockBCLiveCueHolmLocal$). CUE versus OFF (key secondary): \BlockBCCueOffRescue/\BlockBCCueOffHarm/\BlockBCCueOffTie, net \BlockBCCueOffNetCI, $p=\BlockBCCueOffP$ (block-local Holm $p=\BlockBCCueOffHolmLocal$). LIVE versus OFF (supporting, descriptive, outside the paper-wide family): \BlockBCLiveOffRescue/\BlockBCLiveOffHarm/\BlockBCLiveOffTie, net \BlockBCLiveOffNetCI. At the registered block-local level, displaying the current location increased success relative to this cue-and-link panel. The CUE--OFF contrast did not reject; this does not establish absence of a cue effect. Contradiction, salience, and reduced verification effort remain possible explanations. The LIVE--CUE rejection survives the paper-wide Holm analysis over \HolmPaperM claim-bearing tests (adjusted $p=\BlockBCLiveCueHolmPaper$). The LIVE--OFF comparison is a supporting descriptive analysis; it supports neither a confirmatory replication claim nor a claim that the effect differs from Block~B. The LIVE-I controls passed \BlockBCFRXLiveIPassFrac; nothing is attributed to the panel from unmatched controls. The independent scorer reconstructs appointment availability from archived rows; calendar compatibility is not re-derived but rests on stated design conditions (the generator and state preservation), whose checks are reported separately. Under that condition, every outcome term is resolved and agreeing with the evaluator on \BlockBCEndpointFull of \BlockBCCounted counted rollouts (Table~\ref{tab:coverage}). Independent code re-derived this block's validity verdicts (\BlockBCVindPath), agreeing with the archive on \BlockBCVindAgree attempts. Strict recovery occurred in \BlockBCFRXCueARecovered of \BlockBCFRXCueAN CUE-A and \BlockBCFRXLiveARecovered of \BlockBCFRXLiveAN LIVE-A runs, and \BlockBCFRXCueALinkFollowed of \BlockBCFRXCueAN CUE-A runs followed the panel's link (descriptive; never a reading condition).\xspace}  % r21.BC.full: appendix reading paragraph over -
\newcommand{\BlockBCReadingIDs}{R-A, A19\xspace}  % r21.BC.reading_ids: registered reading ids selected by the mirrored rule over -
\newcommand{\BlockBCReadingShort}{at the block-local level the value display increased success relative to the cue-and-link panel; LIVE--CUE surviving the paper-wide Holm analysis\xspace}  % r21.BC.short: short reading over -
\newcommand{\BlockBCRegistered}{ADDENDUM~18\xspace}  % r21.BC.registered: where the block is registered, and whether that registration is frozen (heading present and .sha256 verifying) over -
\newcommand{\BlockBCReplaced}{2\xspace}  % r21.BC.replaced: attempts not counted over rollout
\newcommand{\BlockBCRows}{53\xspace}  % pending.BC.rows: rows so far over rollout
\newcommand{\BlockBCSConfig}{Claude CLI, frames by file read\xspace}  % r21.BCS.config: invoker and frame-delivery channel, from the spec over -
\newcommand{\BlockBCSContradictions}{\textit{incomplete}\xspace}  % r21.BCS.Contradictions: Contradictions over -
\newcommand{\BlockBCSControls}{3\xspace}  % r21.BCS.controls: unpaired control rollouts in the spec over rollout
\newcommand{\BlockBCSCounted}{\textit{incomplete}\xspace}  % r21.BCS.counted: incomplete over -
\newcommand{\BlockBCSCountedFail}{\textit{incomplete}\xspace}  % r21.BCS.CountedFail: counted failures over -
\newcommand{\BlockBCSCountedSucc}{\textit{incomplete}\xspace}  % r21.BCS.CountedSucc: CountedSucc over -
\newcommand{\BlockBCSCueOffBonfPaper}{\textit{not admissible}\xspace}  % fam.alias.BCS.CueOff.b: alias over -
\newcommand{\BlockBCSCueOffBothFail}{\textit{incomplete}\xspace}  % r21.BCS.CueOff.BothFail: both failed over pair
\newcommand{\BlockBCSCueOffBothPass}{\textit{incomplete}\xspace}  % r21.BCS.CueOff.BothPass: both passed over pair
\newcommand{\BlockBCSCueOffDir}{\textit{incomplete}\xspace}  % r21.BCS.CueOff.Dir: direction of the discordance over pair
\newcommand{\BlockBCSCueOffHarm}{\textit{incomplete}\xspace}  % r21.BCS.CueOff.Harm: control passed, treatment failed over pair
\newcommand{\BlockBCSCueOffHolmLocal}{\textit{incomplete}\xspace}  % r21.BCS.CueOff.HolmLocal: - over pair
\newcommand{\BlockBCSCueOffHolmPaper}{\textit{not admissible}\xspace}  % fam.alias.BCS.CueOff: alias over -
\newcommand{\BlockBCSCueOffMinPairs}{13\xspace}  % r21.BCS.CueOff.MinPairs: G1 minimum complete pairs of this contrast (min_pairs_by_contrast, else min_pairs) over pair
\newcommand{\BlockBCSCueOffNet}{\textit{incomplete}\xspace}  % r21.BCS.CueOff.Net: net paired difference over pair
\newcommand{\BlockBCSCueOffNetCI}{\textit{incomplete}\xspace}  % r21.BCS.CueOff.NetCI: net paired difference, Newcombe method-10 marginal 95% interval over pair
\newcommand{\BlockBCSCueOffP}{\textit{incomplete}\xspace}  % r21.BCS.CueOff.P: exact two-sided sign test over pair
\newcommand{\BlockBCSCueOffPairs}{\textit{incomplete}\xspace}  % r21.BCS.CueOff.Pairs: complete pairs over pair
\newcommand{\BlockBCSCueOffRescue}{\textit{incomplete}\xspace}  % r21.BCS.CueOff.Rescue: control failed, treatment passed over pair
\newcommand{\BlockBCSCueOffTie}{\textit{incomplete}\xspace}  % r21.BCS.CueOff.Tie: both passed or both failed over pair
\newcommand{\BlockBCSDecisionTerm}{\textit{incomplete}\xspace}  % r21.BCS.DecisionTerm: DecisionTerm over -
\newcommand{\BlockBCSDisposition}{incomplete at the registered experiment cutoff\xspace}  % r21.BCS.disposition: disposition text over -
\newcommand{\BlockBCSEffect}{\textit{incomplete}\xspace}  % pending.BCS.effect: discordant-pair proportion (envos.stats.effect_size; NOT the net paired effect) over pair
\newcommand{\BlockBCSEndpointFull}{\textit{incomplete}\xspace}  % r21.BCS.EndpointFull: EndpointFull over -
\newcommand{\BlockBCSEndpointFullSucc}{\textit{incomplete}\xspace}  % r21.BCS.EndpointFullSucc: EndpointFullSucc over -
\newcommand{\BlockBCSEndpointUnresolved}{\textit{incomplete}\xspace}  % r21.BCS.EndpointUnresolved: EndpointUnresolved over -
\newcommand{\BlockBCSFRXCueACap}{\textit{incomplete}\xspace}  % pending.BCS.FRX-CUE-A.Cap: count over counted rollout
\newcommand{\BlockBCSFRXCueALinkFollowed}{\textit{incomplete}\xspace}  % r21.BCS.FRXCueALinkFollowed: process measure followed_panel_link at FRX-CUE-A (descriptive) over rollout
\newcommand{\BlockBCSFRXCueAN}{\textit{incomplete}\xspace}  % pending.BCS.FRX-CUE-A.n: count over counted rollout
\newcommand{\BlockBCSFRXCueAPass}{\textit{incomplete}\xspace}  % pending.BCS.FRX-CUE-A.pass: count over counted rollout
\newcommand{\BlockBCSFRXCueAPassFrac}{\textit{incomplete}\xspace}  % pending.BCS.FRX-CUE-A.frac: k/n over counted rollout
\newcommand{\BlockBCSFRXCueARecovered}{\textit{incomplete}\xspace}  % r21.BCS.FRXCueARecovered: process measure bc_recovered at FRX-CUE-A (descriptive) over rollout
\newcommand{\BlockBCSFRXCueARevised}{\textit{incomplete}\xspace}  % pending.BCS.FRX-CUE-A.Revised: count over counted rollout
\newcommand{\BlockBCSFRXCueAStaleFlagged}{\textit{incomplete}\xspace}  % pending.BCS.FRX-CUE-A.StaleFlagged: count over counted rollout
\newcommand{\BlockBCSFRXCueAStaleUnflagged}{\textit{incomplete}\xspace}  % pending.BCS.FRX-CUE-A.StaleUnflagged: count over counted rollout
\newcommand{\BlockBCSFRXLiveACap}{\textit{incomplete}\xspace}  % pending.BCS.FRX-LIVE-A.Cap: count over counted rollout
\newcommand{\BlockBCSFRXLiveAN}{\textit{incomplete}\xspace}  % pending.BCS.FRX-LIVE-A.n: count over counted rollout
\newcommand{\BlockBCSFRXLiveAPass}{\textit{incomplete}\xspace}  % pending.BCS.FRX-LIVE-A.pass: count over counted rollout
\newcommand{\BlockBCSFRXLiveAPassFrac}{\textit{incomplete}\xspace}  % pending.BCS.FRX-LIVE-A.frac: k/n over counted rollout
\newcommand{\BlockBCSFRXLiveARecovered}{\textit{incomplete}\xspace}  % r21.BCS.FRXLiveARecovered: process measure bc_recovered at FRX-LIVE-A (descriptive) over rollout
\newcommand{\BlockBCSFRXLiveARevised}{\textit{incomplete}\xspace}  % pending.BCS.FRX-LIVE-A.Revised: count over counted rollout
\newcommand{\BlockBCSFRXLiveAStaleFlagged}{\textit{incomplete}\xspace}  % pending.BCS.FRX-LIVE-A.StaleFlagged: count over counted rollout
\newcommand{\BlockBCSFRXLiveAStaleUnflagged}{\textit{incomplete}\xspace}  % pending.BCS.FRX-LIVE-A.StaleUnflagged: count over counted rollout
\newcommand{\BlockBCSFRXLiveICap}{\textit{incomplete}\xspace}  % pending.BCS.FRX-LIVE-I.Cap: count over counted rollout
\newcommand{\BlockBCSFRXLiveIN}{\textit{incomplete}\xspace}  % pending.BCS.FRX-LIVE-I.n: count over counted rollout
\newcommand{\BlockBCSFRXLiveIPass}{\textit{incomplete}\xspace}  % pending.BCS.FRX-LIVE-I.pass: count over counted rollout
\newcommand{\BlockBCSFRXLiveIPassFrac}{\textit{incomplete}\xspace}  % pending.BCS.FRX-LIVE-I.frac: k/n over counted rollout
\newcommand{\BlockBCSFRXLiveIRevised}{\textit{incomplete}\xspace}  % pending.BCS.FRX-LIVE-I.Revised: count over counted rollout
\newcommand{\BlockBCSFRXLiveIStaleFlagged}{\textit{incomplete}\xspace}  % pending.BCS.FRX-LIVE-I.StaleFlagged: count over counted rollout
\newcommand{\BlockBCSFRXLiveIStaleUnflagged}{\textit{incomplete}\xspace}  % pending.BCS.FRX-LIVE-I.StaleUnflagged: count over counted rollout
\newcommand{\BlockBCSFRXOffACap}{\textit{incomplete}\xspace}  % pending.BCS.FRX-OFF-A.Cap: count over counted rollout
\newcommand{\BlockBCSFRXOffAN}{\textit{incomplete}\xspace}  % pending.BCS.FRX-OFF-A.n: count over counted rollout
\newcommand{\BlockBCSFRXOffAPass}{\textit{incomplete}\xspace}  % pending.BCS.FRX-OFF-A.pass: count over counted rollout
\newcommand{\BlockBCSFRXOffAPassFrac}{\textit{incomplete}\xspace}  % pending.BCS.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\BlockBCSFRXOffARevised}{\textit{incomplete}\xspace}  % pending.BCS.FRX-OFF-A.Revised: count over counted rollout
\newcommand{\BlockBCSFRXOffAStaleFlagged}{\textit{incomplete}\xspace}  % pending.BCS.FRX-OFF-A.StaleFlagged: count over counted rollout
\newcommand{\BlockBCSFRXOffAStaleUnflagged}{\textit{incomplete}\xspace}  % pending.BCS.FRX-OFF-A.StaleUnflagged: count over counted rollout
\newcommand{\BlockBCSGzero}{pending\xspace}  % r21.BCS.g0: G0 (ADDENDUM 18 section 6.5), from the generated report over -
\newcommand{\BlockBCSGzeroWhy}{--\xspace}  % r21.BCS.g0_why: G0 problems over -
\newcommand{\BlockBCSInstancePhrase}{\BlockBCSInstances frozen generated instances (seeds \BlockBCSSeedList)\xspace}  % r21.BCS.instance_phrase: the block's instances as a phrase that reads correctly whether or not its spec exists over -
\newcommand{\BlockBCSInstances}{16\xspace}  % r21.BCS.instances: paired instances over instance
\newcommand{\BlockBCSInstancesWords}{sixteen\xspace}  % r21.BCS.instances_words: in words over instance
\newcommand{\BlockBCSLiveCueBonfPaper}{\textit{not admissible}\xspace}  % fam.alias.BCS.LiveCue.b: alias over -
\newcommand{\BlockBCSLiveCueBothFail}{\textit{incomplete}\xspace}  % r21.BCS.LiveCue.BothFail: both failed over pair
\newcommand{\BlockBCSLiveCueBothPass}{\textit{incomplete}\xspace}  % r21.BCS.LiveCue.BothPass: both passed over pair
\newcommand{\BlockBCSLiveCueDir}{\textit{incomplete}\xspace}  % r21.BCS.LiveCue.Dir: direction of the discordance over pair
\newcommand{\BlockBCSLiveCueHarm}{\textit{incomplete}\xspace}  % r21.BCS.LiveCue.Harm: control passed, treatment failed over pair
\newcommand{\BlockBCSLiveCueHolmLocal}{\textit{incomplete}\xspace}  % r21.BCS.LiveCue.HolmLocal: - over pair
\newcommand{\BlockBCSLiveCueHolmPaper}{\textit{not admissible}\xspace}  % fam.alias.BCS.LiveCue: alias over -
\newcommand{\BlockBCSLiveCueMinPairs}{13\xspace}  % r21.BCS.LiveCue.MinPairs: G1 minimum complete pairs of this contrast (min_pairs_by_contrast, else min_pairs) over pair
\newcommand{\BlockBCSLiveCueNet}{\textit{incomplete}\xspace}  % r21.BCS.LiveCue.Net: net paired difference over pair
\newcommand{\BlockBCSLiveCueNetCI}{\textit{incomplete}\xspace}  % r21.BCS.LiveCue.NetCI: net paired difference, Newcombe method-10 marginal 95% interval over pair
\newcommand{\BlockBCSLiveCueP}{\textit{incomplete}\xspace}  % r21.BCS.LiveCue.P: exact two-sided sign test over pair
\newcommand{\BlockBCSLiveCuePairs}{\textit{incomplete}\xspace}  % r21.BCS.LiveCue.Pairs: complete pairs over pair
\newcommand{\BlockBCSLiveCueRescue}{\textit{incomplete}\xspace}  % r21.BCS.LiveCue.Rescue: control failed, treatment passed over pair
\newcommand{\BlockBCSLiveCueTie}{\textit{incomplete}\xspace}  % r21.BCS.LiveCue.Tie: both passed or both failed over pair
\newcommand{\BlockBCSLiveOffBonfPaper}{\textit{outside the family}\xspace}  % fam.alias.BCS.LiveOff.b: not a paper-wide test over -
\newcommand{\BlockBCSLiveOffBothFail}{\textit{incomplete}\xspace}  % r21.BCS.LiveOff.BothFail: both failed over pair
\newcommand{\BlockBCSLiveOffBothPass}{\textit{incomplete}\xspace}  % r21.BCS.LiveOff.BothPass: both passed over pair
\newcommand{\BlockBCSLiveOffDir}{\textit{incomplete}\xspace}  % r21.BCS.LiveOff.Dir: direction of the discordance over pair
\newcommand{\BlockBCSLiveOffHarm}{\textit{incomplete}\xspace}  % r21.BCS.LiveOff.Harm: control passed, treatment failed over pair
\newcommand{\BlockBCSLiveOffHolmLocal}{\textit{incomplete}\xspace}  % r21.BCS.LiveOff.HolmLocal: - over pair
\newcommand{\BlockBCSLiveOffHolmPaper}{\textit{outside the family}\xspace}  % fam.alias.BCS.LiveOff: not a paper-wide test over -
\newcommand{\BlockBCSLiveOffNet}{\textit{incomplete}\xspace}  % r21.BCS.LiveOff.Net: net paired difference over pair
\newcommand{\BlockBCSLiveOffNetCI}{\textit{incomplete}\xspace}  % r21.BCS.LiveOff.NetCI: net paired difference, Newcombe method-10 marginal 95% interval over pair
\newcommand{\BlockBCSLiveOffP}{\textit{incomplete}\xspace}  % r21.BCS.LiveOff.P: exact two-sided sign test over pair
\newcommand{\BlockBCSLiveOffPairs}{\textit{incomplete}\xspace}  % r21.BCS.LiveOff.Pairs: complete pairs over pair
\newcommand{\BlockBCSLiveOffRescue}{\textit{incomplete}\xspace}  % r21.BCS.LiveOff.Rescue: control failed, treatment passed over pair
\newcommand{\BlockBCSLiveOffTie}{\textit{incomplete}\xspace}  % r21.BCS.LiveOff.Tie: both passed or both failed over pair
\newcommand{\BlockBCSMinPairs}{13\xspace}  % r21.BCS.min_pairs: G1 minimum complete pairs over pair
\newcommand{\BlockBCSModel}{Claude Sonnet~5\xspace}  % r21.BCS.model: evaluated model over -
\newcommand{\BlockBCSNNeg}{\textit{incomplete}\xspace}  % pending.BCS.n_neg: count over pair
\newcommand{\BlockBCSNPos}{\textit{incomplete}\xspace}  % pending.BCS.n_pos: count over pair
\newcommand{\BlockBCSNTied}{\textit{incomplete}\xspace}  % pending.BCS.n_tied: count over pair
\newcommand{\BlockBCSOffFail}{\textit{incomplete}\xspace}  % r21.BCS.off_fail: incomplete over -
\newcommand{\BlockBCSOffGate}{8\xspace}  % r21.BCS.off_gate: R-D/R-E OFF-A failure gate over instance
\newcommand{\BlockBCSOffPass}{\textit{incomplete}\xspace}  % r21.BCS.off_pass: incomplete over -
\newcommand{\BlockBCSOffPlanned}{16\xspace}  % r21.BCS.off_planned: planned FRX-OFF-A rows (R-E states n of the planned rows) over rollout
\newcommand{\BlockBCSOffReread}{\textit{incomplete}\xspace}  % r21.BCS.OffReread: process measure source_visit_after_review at FRX-OFF-A (descriptive) over rollout
\newcommand{\BlockBCSP}{\textit{incomplete}\xspace}  % pending.BCS.p: exact two-sided sign test over pair
\newcommand{\BlockBCSPairs}{\textit{incomplete}\xspace}  % pending.BCS.pairs: count over pair
\newcommand{\BlockBCSReadingBody}{Block~BCS started but did not complete (\BlockBCSDisposition). It contributes no inferential result; its rows are listed in Appendix~\ref{app:bc} as a record only.\xspace}  % r21.BCS.body: main-text reading paragraph over -
\newcommand{\BlockBCSReadingFull}{Block~BCS started but did not complete (\BlockBCSDisposition). It contributes no inferential result; its rows are listed in Appendix~\ref{app:bc} as a record only.\xspace}  % r21.BCS.full: appendix reading paragraph over -
\newcommand{\BlockBCSReadingIDs}{INCOMPLETE\xspace}  % r21.BCS.reading_ids: registered reading ids selected by the mirrored rule over -
\newcommand{\BlockBCSReadingShort}{started but not completed (\BlockBCSDisposition); no inference\xspace}  % r21.BCS.short: short reading over -
\newcommand{\BlockBCSRegistered}{ADDENDUM~19\xspace}  % r21.BCS.registered: where the block is registered, and whether that registration is frozen (heading present and .sha256 verifying) over -
\newcommand{\BlockBCSReplaced}{\textit{incomplete}\xspace}  % r21.BCS.replaced: incomplete over -
\newcommand{\BlockBCSRows}{24\xspace}  % pending.BCS.rows: rows so far over rollout
\newcommand{\BlockBCSSeedList}{42--49, 51--55, 57--59\xspace}  % r21.BCS.seeds: exact seed list of the block's paired instances over seed
\newcommand{\BlockBCSShortForm}{Claude Sonnet~5 on the same instances (Block~BCS): \BlockBCSReadingShort.\xspace}  % r21.BCS.shortform: main-text short form over -
\newcommand{\BlockBCSState}{incomplete\xspace}  % r21.BCS.state: execution disposition (r21_state) over -
\newcommand{\BlockBCSStateCell}{incomplete at the registered cutoff: \BCSCellsCounted{} of \BCSCellsRegistered{} cells counted; no inference\xspace}  % r28.BCS.cell: r28: the block's state for Table 1 over -
\newcommand{\BlockBCSStatus}{\texttt{paused\_limit}\xspace}  % pending.BCS.status: search-log status over -
\newcommand{\BlockBCSVerdictFail}{\textit{incomplete}\xspace}  % r21.BCS.VerdictFail: VerdictFail over -
\newcommand{\BlockBCSVerdictSucc}{\textit{incomplete}\xspace}  % r21.BCS.VerdictSucc: VerdictSucc over -
\newcommand{\BlockBCSVindAgree}{\textit{incomplete}\xspace}  % r21.BCS.vind: validity re-derivation over -
\newcommand{\BlockBCSVindAgreeSlash}{\textit{incomplete}\xspace}  % r21.BCS.vind_slash: validity re-derivation over -
\newcommand{\BlockBCSVindPath}{\code{audit/\allowbreak{}failure\_\allowbreak{}mining/\allowbreak{}P3v2/\allowbreak{}VALIDITY\_\allowbreak{}INDEPENDENT\_\allowbreak{}blockBCS.json}\xspace}  % r21.BCS.vind_path: the expected independent validity re-derivation artifact over -
\newcommand{\BlockBCSVindStatus}{re-derived\xspace}  % r21.BCS.vind_status: whether audit/failure_mining/P3v2/VALIDITY_INDEPENDENT_blockBCS.json exists over -
\newcommand{\BlockBCSVoided}{3\xspace}  % pending.BCS.voided: count over rollout
\newcommand{\BlockBCSeedList}{42--49, 51--55, 57--59\xspace}  % r21.BC.seeds: exact seed list of the block's paired instances over seed
\newcommand{\BlockBCShortForm}{Claude Opus~5 on the same instances (Block~BC): OFF-A \BlockBCFRXOffAPassFrac, CUE-A \BlockBCFRXCueAPassFrac, LIVE-A \BlockBCFRXLiveAPassFrac; block-local Holm $p=\BlockBCLiveCueHolmLocal$ (LIVE--CUE) and $p=\BlockBCCueOffHolmLocal$ (CUE--OFF); \BlockBCReadingShort.\xspace}  % r21.BC.shortform: main-text short form over -
\newcommand{\BlockBCState}{complete\xspace}  % r21.BC.state: execution disposition (r21_state) over -
\newcommand{\BlockBCStateCell}{complete\xspace}  % r28.BC.cell: r28: the block's state for Table 1 over -
\newcommand{\BlockBCStatus}{\texttt{complete}\xspace}  % pending.BC.status: search-log status over -
\newcommand{\BlockBCVerdictFail}{31\xspace}  % r21.BC.VerdictFail: VerdictFail over counted rollout
\newcommand{\BlockBCVerdictSucc}{20\xspace}  % r21.BC.VerdictSucc: VerdictSucc over counted rollout
\newcommand{\BlockBCVindAgree}{53 of 53\xspace}  % r21.BC.vind: independent validity re-derivation, agreeing / all attempts over attempt
\newcommand{\BlockBCVindAgreeSlash}{53/53\xspace}  % r21.BC.vind_slash: the same, as a/b over attempt
\newcommand{\BlockBCVindPath}{\code{audit/\allowbreak{}failure\_\allowbreak{}mining/\allowbreak{}P3v2/\allowbreak{}VALIDITY\_\allowbreak{}INDEPENDENT\_\allowbreak{}blockBC.json}\xspace}  % r21.BC.vind_path: the expected independent validity re-derivation artifact over -
\newcommand{\BlockBCVindStatus}{re-derived\xspace}  % r21.BC.vind_status: whether audit/failure_mining/P3v2/VALIDITY_INDEPENDENT_blockBC.json exists over -
\newcommand{\BlockBCVoided}{2\xspace}  % pending.BC.voided: count over rollout
\newcommand{\BlockBEffect}{1.000\xspace}  % pending.B.effect: discordant-pair proportion (envos.stats.effect_size; NOT the net paired effect) over pair
\newcommand{\BlockBFFRXOffACap}{0\xspace}  % pending.BF.FRX-OFF-A.Cap: count over counted rollout
\newcommand{\BlockBFFRXOffAN}{4\xspace}  % pending.BF.FRX-OFF-A.n: count over counted rollout
\newcommand{\BlockBFFRXOffAPass}{0\xspace}  % pending.BF.FRX-OFF-A.pass: count over counted rollout
\newcommand{\BlockBFFRXOffAPassFrac}{0/4\xspace}  % pending.BF.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\BlockBFFRXOffARevised}{0\xspace}  % pending.BF.FRX-OFF-A.Revised: count over counted rollout
\newcommand{\BlockBFFRXOffAStaleFlagged}{1\xspace}  % pending.BF.FRX-OFF-A.StaleFlagged: count over counted rollout
\newcommand{\BlockBFFRXOffAStaleUnflagged}{3\xspace}  % pending.BF.FRX-OFF-A.StaleUnflagged: count over counted rollout
\newcommand{\BlockBFFRXOnICap}{0\xspace}  % pending.BF.FRX-ON-I.Cap: count over counted rollout
\newcommand{\BlockBFFRXOnIN}{1\xspace}  % pending.BF.FRX-ON-I.n: count over counted rollout
\newcommand{\BlockBFFRXOnIPass}{1\xspace}  % pending.BF.FRX-ON-I.pass: count over counted rollout
\newcommand{\BlockBFFRXOnIPassFrac}{1/1\xspace}  % pending.BF.FRX-ON-I.frac: k/n over counted rollout
\newcommand{\BlockBFFRXOnIRevised}{0\xspace}  % pending.BF.FRX-ON-I.Revised: count over counted rollout
\newcommand{\BlockBFFRXOnIStaleFlagged}{0\xspace}  % pending.BF.FRX-ON-I.StaleFlagged: count over counted rollout
\newcommand{\BlockBFFRXOnIStaleUnflagged}{0\xspace}  % pending.BF.FRX-ON-I.StaleUnflagged: count over counted rollout
\newcommand{\BlockBFRXOffACap}{0\xspace}  % pending.B.FRX-OFF-A.Cap: count over counted rollout
\newcommand{\BlockBFRXOffAN}{10\xspace}  % pending.B.FRX-OFF-A.n: count over counted rollout
\newcommand{\BlockBFRXOffAPass}{0\xspace}  % pending.B.FRX-OFF-A.pass: count over counted rollout
\newcommand{\BlockBFRXOffAPassFrac}{0/10\xspace}  % pending.B.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\BlockBFRXOffARevised}{0\xspace}  % pending.B.FRX-OFF-A.Revised: count over counted rollout
\newcommand{\BlockBFRXOffAStaleFlagged}{3\xspace}  % pending.B.FRX-OFF-A.StaleFlagged: count over counted rollout
\newcommand{\BlockBFRXOffAStaleUnflagged}{7\xspace}  % pending.B.FRX-OFF-A.StaleUnflagged: count over counted rollout
\newcommand{\BlockBFRXOnACap}{0\xspace}  % pending.B.FRX-ON-A.Cap: count over counted rollout
\newcommand{\BlockBFRXOnAN}{10\xspace}  % pending.B.FRX-ON-A.n: count over counted rollout
\newcommand{\BlockBFRXOnAPass}{10\xspace}  % pending.B.FRX-ON-A.pass: count over counted rollout
\newcommand{\BlockBFRXOnAPassFrac}{10/10\xspace}  % pending.B.FRX-ON-A.frac: k/n over counted rollout
\newcommand{\BlockBFRXOnARevised}{10\xspace}  % pending.B.FRX-ON-A.Revised: count over counted rollout
\newcommand{\BlockBFRXOnAStaleFlagged}{0\xspace}  % pending.B.FRX-ON-A.StaleFlagged: count over counted rollout
\newcommand{\BlockBFRXOnAStaleUnflagged}{0\xspace}  % pending.B.FRX-ON-A.StaleUnflagged: count over counted rollout
\newcommand{\BlockBFRXOnICap}{0\xspace}  % pending.B.FRX-ON-I.Cap: count over counted rollout
\newcommand{\BlockBFRXOnIN}{3\xspace}  % pending.B.FRX-ON-I.n: count over counted rollout
\newcommand{\BlockBFRXOnIPass}{3\xspace}  % pending.B.FRX-ON-I.pass: count over counted rollout
\newcommand{\BlockBFRXOnIPassFrac}{3/3\xspace}  % pending.B.FRX-ON-I.frac: k/n over counted rollout
\newcommand{\BlockBFRXOnIRevised}{0\xspace}  % pending.B.FRX-ON-I.Revised: count over counted rollout
\newcommand{\BlockBFRXOnIStaleFlagged}{0\xspace}  % pending.B.FRX-ON-I.StaleFlagged: count over counted rollout
\newcommand{\BlockBFRXOnIStaleUnflagged}{0\xspace}  % pending.B.FRX-ON-I.StaleUnflagged: count over counted rollout
\newcommand{\BlockBFRows}{5\xspace}  % pending.BF.rows: rows so far over rollout
\newcommand{\BlockBFStatus}{\texttt{complete}\xspace}  % pending.BF.status: search-log status over -
\newcommand{\BlockBFVoided}{0\xspace}  % pending.BF.voided: count over rollout
\newcommand{\BlockBGCConfig}{Codex CLI, frames inline\xspace}  % r21.BGC.config: invoker and frame-delivery channel, from the spec over -
\newcommand{\BlockBGCContradictions}{\textit{not run}\xspace}  % r21.BGC.Contradictions: Contradictions over -
\newcommand{\BlockBGCControls}{3\xspace}  % r21.BGC.controls: unpaired control rollouts in the spec over rollout
\newcommand{\BlockBGCCounted}{\textit{not run}\xspace}  % r21.BGC.counted: notrun over -
\newcommand{\BlockBGCCountedFail}{\textit{not run}\xspace}  % r21.BGC.CountedFail: counted failures over -
\newcommand{\BlockBGCCountedSucc}{\textit{not run}\xspace}  % r21.BGC.CountedSucc: CountedSucc over -
\newcommand{\BlockBGCCueOffBonfPaper}{\textit{not admissible}\xspace}  % fam.alias.BGC.CueOff.b: alias over -
\newcommand{\BlockBGCCueOffBothFail}{\textit{not run}\xspace}  % r21.BGC.CueOff.BothFail: both failed over pair
\newcommand{\BlockBGCCueOffBothPass}{\textit{not run}\xspace}  % r21.BGC.CueOff.BothPass: both passed over pair
\newcommand{\BlockBGCCueOffDir}{\textit{not run}\xspace}  % r21.BGC.CueOff.Dir: direction of the discordance over pair
\newcommand{\BlockBGCCueOffHarm}{\textit{not run}\xspace}  % r21.BGC.CueOff.Harm: control passed, treatment failed over pair
\newcommand{\BlockBGCCueOffHolmLocal}{\textit{not run}\xspace}  % r21.BGC.CueOff.HolmLocal: - over pair
\newcommand{\BlockBGCCueOffHolmPaper}{\textit{not admissible}\xspace}  % fam.alias.BGC.CueOff: alias over -
\newcommand{\BlockBGCCueOffMinPairs}{13\xspace}  % r21.BGC.CueOff.MinPairs: G1 minimum complete pairs of this contrast (min_pairs_by_contrast, else min_pairs) over pair
\newcommand{\BlockBGCCueOffNet}{\textit{not run}\xspace}  % r21.BGC.CueOff.Net: net paired difference over pair
\newcommand{\BlockBGCCueOffNetCI}{\textit{not run}\xspace}  % r21.BGC.CueOff.NetCI: net paired difference, Newcombe method-10 marginal 95% interval over pair
\newcommand{\BlockBGCCueOffP}{\textit{not run}\xspace}  % r21.BGC.CueOff.P: exact two-sided sign test over pair
\newcommand{\BlockBGCCueOffPairs}{\textit{not run}\xspace}  % r21.BGC.CueOff.Pairs: complete pairs over pair
\newcommand{\BlockBGCCueOffRescue}{\textit{not run}\xspace}  % r21.BGC.CueOff.Rescue: control failed, treatment passed over pair
\newcommand{\BlockBGCCueOffTie}{\textit{not run}\xspace}  % r21.BGC.CueOff.Tie: both passed or both failed over pair
\newcommand{\BlockBGCDecisionTerm}{\textit{not run}\xspace}  % r21.BGC.DecisionTerm: DecisionTerm over -
\newcommand{\BlockBGCDisposition}{launch preconditions unmet by the experiment cutoff\xspace}  % r21.BGC.disposition: disposition text over -
\newcommand{\BlockBGCEffect}{\textit{not run}\xspace}  % pending.BGC.effect: discordant-pair proportion (envos.stats.effect_size; NOT the net paired effect) over pair
\newcommand{\BlockBGCEndpointFull}{\textit{not run}\xspace}  % r21.BGC.EndpointFull: EndpointFull over -
\newcommand{\BlockBGCEndpointFullSucc}{\textit{not run}\xspace}  % r21.BGC.EndpointFullSucc: EndpointFullSucc over -
\newcommand{\BlockBGCEndpointUnresolved}{\textit{not run}\xspace}  % r21.BGC.EndpointUnresolved: EndpointUnresolved over -
\newcommand{\BlockBGCFRXCueALinkFollowed}{\textit{not run}\xspace}  % r21.BGC.FRXCueALinkFollowed: process measure followed_panel_link at FRX-CUE-A (descriptive) over rollout
\newcommand{\BlockBGCFRXCueAN}{\textit{not run}\xspace}  % pending.BGC.FRX-CUE-A.n: count over counted rollout
\newcommand{\BlockBGCFRXCueAPass}{\textit{not run}\xspace}  % pending.BGC.FRX-CUE-A.pass: count over counted rollout
\newcommand{\BlockBGCFRXCueAPassFrac}{\textit{not run}\xspace}  % pending.BGC.FRX-CUE-A.frac: k/n over counted rollout
\newcommand{\BlockBGCFRXCueARecovered}{\textit{not run}\xspace}  % r21.BGC.FRXCueARecovered: process measure bc_recovered at FRX-CUE-A (descriptive) over rollout
\newcommand{\BlockBGCFRXLiveAN}{\textit{not run}\xspace}  % pending.BGC.FRX-LIVE-A.n: count over counted rollout
\newcommand{\BlockBGCFRXLiveAPass}{\textit{not run}\xspace}  % pending.BGC.FRX-LIVE-A.pass: count over counted rollout
\newcommand{\BlockBGCFRXLiveAPassFrac}{\textit{not run}\xspace}  % pending.BGC.FRX-LIVE-A.frac: k/n over counted rollout
\newcommand{\BlockBGCFRXLiveARecovered}{\textit{not run}\xspace}  % r21.BGC.FRXLiveARecovered: process measure bc_recovered at FRX-LIVE-A (descriptive) over rollout
\newcommand{\BlockBGCFRXLiveIN}{\textit{not run}\xspace}  % pending.BGC.FRX-LIVE-I.n: count over counted rollout
\newcommand{\BlockBGCFRXLiveIPass}{\textit{not run}\xspace}  % pending.BGC.FRX-LIVE-I.pass: count over counted rollout
\newcommand{\BlockBGCFRXLiveIPassFrac}{\textit{not run}\xspace}  % pending.BGC.FRX-LIVE-I.frac: k/n over counted rollout
\newcommand{\BlockBGCFRXOffAN}{\textit{not run}\xspace}  % pending.BGC.FRX-OFF-A.n: count over counted rollout
\newcommand{\BlockBGCFRXOffAPass}{\textit{not run}\xspace}  % pending.BGC.FRX-OFF-A.pass: count over counted rollout
\newcommand{\BlockBGCFRXOffAPassFrac}{\textit{not run}\xspace}  % pending.BGC.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\BlockBGCFRXOffIN}{\textit{not run}\xspace}  % pending.BGC.FRX-OFF-I.n: count over counted rollout
\newcommand{\BlockBGCFRXOffIPass}{\textit{not run}\xspace}  % pending.BGC.FRX-OFF-I.pass: count over counted rollout
\newcommand{\BlockBGCFRXOffIPassFrac}{\textit{not run}\xspace}  % pending.BGC.FRX-OFF-I.frac: k/n over counted rollout
\newcommand{\BlockBGCGzero}{pending\xspace}  % r21.BGC.g0: G0 (ADDENDUM 18 section 6.5), from the generated report over -
\newcommand{\BlockBGCGzeroWhy}{--\xspace}  % r21.BGC.g0_why: G0 problems over -
\newcommand{\BlockBGCInstancePhrase}{\BlockBGCInstances frozen generated instances (seeds \BlockBGCSeedList)\xspace}  % r21.BGC.instance_phrase: the block's instances as a phrase that reads correctly whether or not its spec exists over -
\newcommand{\BlockBGCInstances}{16\xspace}  % r21.BGC.instances: paired instances over instance
\newcommand{\BlockBGCInstancesWords}{sixteen\xspace}  % r21.BGC.instances_words: in words over instance
\newcommand{\BlockBGCLiveCueBonfPaper}{\textit{not admissible}\xspace}  % fam.alias.BGC.LiveCue.b: alias over -
\newcommand{\BlockBGCLiveCueBothFail}{\textit{not run}\xspace}  % r21.BGC.LiveCue.BothFail: both failed over pair
\newcommand{\BlockBGCLiveCueBothPass}{\textit{not run}\xspace}  % r21.BGC.LiveCue.BothPass: both passed over pair
\newcommand{\BlockBGCLiveCueDir}{\textit{not run}\xspace}  % r21.BGC.LiveCue.Dir: direction of the discordance over pair
\newcommand{\BlockBGCLiveCueHarm}{\textit{not run}\xspace}  % r21.BGC.LiveCue.Harm: control passed, treatment failed over pair
\newcommand{\BlockBGCLiveCueHolmLocal}{\textit{not run}\xspace}  % r21.BGC.LiveCue.HolmLocal: - over pair
\newcommand{\BlockBGCLiveCueHolmPaper}{\textit{not admissible}\xspace}  % fam.alias.BGC.LiveCue: alias over -
\newcommand{\BlockBGCLiveCueMinPairs}{13\xspace}  % r21.BGC.LiveCue.MinPairs: G1 minimum complete pairs of this contrast (min_pairs_by_contrast, else min_pairs) over pair
\newcommand{\BlockBGCLiveCueNet}{\textit{not run}\xspace}  % r21.BGC.LiveCue.Net: net paired difference over pair
\newcommand{\BlockBGCLiveCueNetCI}{\textit{not run}\xspace}  % r21.BGC.LiveCue.NetCI: net paired difference, Newcombe method-10 marginal 95% interval over pair
\newcommand{\BlockBGCLiveCueP}{\textit{not run}\xspace}  % r21.BGC.LiveCue.P: exact two-sided sign test over pair
\newcommand{\BlockBGCLiveCuePairs}{\textit{not run}\xspace}  % r21.BGC.LiveCue.Pairs: complete pairs over pair
\newcommand{\BlockBGCLiveCueRescue}{\textit{not run}\xspace}  % r21.BGC.LiveCue.Rescue: control failed, treatment passed over pair
\newcommand{\BlockBGCLiveCueTie}{\textit{not run}\xspace}  % r21.BGC.LiveCue.Tie: both passed or both failed over pair
\newcommand{\BlockBGCLiveOffBonfPaper}{\textit{outside the family}\xspace}  % fam.alias.BGC.LiveOff.b: not a paper-wide test over -
\newcommand{\BlockBGCLiveOffBothFail}{\textit{not run}\xspace}  % r21.BGC.LiveOff.BothFail: both failed over pair
\newcommand{\BlockBGCLiveOffBothPass}{\textit{not run}\xspace}  % r21.BGC.LiveOff.BothPass: both passed over pair
\newcommand{\BlockBGCLiveOffDir}{\textit{not run}\xspace}  % r21.BGC.LiveOff.Dir: direction of the discordance over pair
\newcommand{\BlockBGCLiveOffHarm}{\textit{not run}\xspace}  % r21.BGC.LiveOff.Harm: control passed, treatment failed over pair
\newcommand{\BlockBGCLiveOffHolmLocal}{\textit{not run}\xspace}  % r21.BGC.LiveOff.HolmLocal: - over pair
\newcommand{\BlockBGCLiveOffHolmPaper}{\textit{outside the family}\xspace}  % fam.alias.BGC.LiveOff: not a paper-wide test over -
\newcommand{\BlockBGCLiveOffNet}{\textit{not run}\xspace}  % r21.BGC.LiveOff.Net: net paired difference over pair
\newcommand{\BlockBGCLiveOffNetCI}{\textit{not run}\xspace}  % r21.BGC.LiveOff.NetCI: net paired difference, Newcombe method-10 marginal 95% interval over pair
\newcommand{\BlockBGCLiveOffP}{\textit{not run}\xspace}  % r21.BGC.LiveOff.P: exact two-sided sign test over pair
\newcommand{\BlockBGCLiveOffPairs}{\textit{not run}\xspace}  % r21.BGC.LiveOff.Pairs: complete pairs over pair
\newcommand{\BlockBGCLiveOffRescue}{\textit{not run}\xspace}  % r21.BGC.LiveOff.Rescue: control failed, treatment passed over pair
\newcommand{\BlockBGCLiveOffTie}{\textit{not run}\xspace}  % r21.BGC.LiveOff.Tie: both passed or both failed over pair
\newcommand{\BlockBGCMinPairs}{13\xspace}  % r21.BGC.min_pairs: G1 minimum complete pairs over pair
\newcommand{\BlockBGCModel}{GPT-6\xspace}  % r21.BGC.model: evaluated model over -
\newcommand{\BlockBGCNNeg}{\textit{not run}\xspace}  % pending.BGC.n_neg: count over pair
\newcommand{\BlockBGCNPos}{\textit{not run}\xspace}  % pending.BGC.n_pos: count over pair
\newcommand{\BlockBGCNTied}{\textit{not run}\xspace}  % pending.BGC.n_tied: count over pair
\newcommand{\BlockBGCOffFail}{\textit{not run}\xspace}  % r21.BGC.off_fail: notrun over -
\newcommand{\BlockBGCOffGate}{8\xspace}  % r21.BGC.off_gate: R-D/R-E OFF-A failure gate over instance
\newcommand{\BlockBGCOffIFail}{\textit{not run}\xspace}  % r21.BGC.offi_fail: notrun over -
\newcommand{\BlockBGCOffIN}{\textit{not run}\xspace}  % r21.BGC.offi_n: notrun over -
\newcommand{\BlockBGCOffPass}{\textit{not run}\xspace}  % r21.BGC.off_pass: notrun over -
\newcommand{\BlockBGCOffPlanned}{16\xspace}  % r21.BGC.off_planned: planned FRX-OFF-A rows (R-E states n of the planned rows) over rollout
\newcommand{\BlockBGCOffReread}{\textit{not run}\xspace}  % r21.BGC.OffReread: process measure source_visit_after_review at FRX-OFF-A (descriptive) over rollout
\newcommand{\BlockBGCOffiOffaBonfPaper}{\textit{not admissible}\xspace}  % fam.alias.BGC.OffiOffa.b: alias over -
\newcommand{\BlockBGCOffiOffaBothFail}{\textit{not run}\xspace}  % r21.BGC.OffiOffa.BothFail: both failed over pair
\newcommand{\BlockBGCOffiOffaBothPass}{\textit{not run}\xspace}  % r21.BGC.OffiOffa.BothPass: both passed over pair
\newcommand{\BlockBGCOffiOffaDir}{\textit{not run}\xspace}  % r21.BGC.OffiOffa.Dir: direction of the discordance over pair
\newcommand{\BlockBGCOffiOffaHarm}{\textit{not run}\xspace}  % r21.BGC.OffiOffa.Harm: control passed, treatment failed over pair
\newcommand{\BlockBGCOffiOffaHolmLocal}{\textit{not run}\xspace}  % r21.BGC.OffiOffa.HolmLocal: - over pair
\newcommand{\BlockBGCOffiOffaHolmPaper}{\textit{not admissible}\xspace}  % fam.alias.BGC.OffiOffa: alias over -
\newcommand{\BlockBGCOffiOffaMinPairs}{8\xspace}  % r21.BGC.OffiOffa.MinPairs: G1 minimum complete pairs of this contrast (min_pairs_by_contrast, else min_pairs) over pair
\newcommand{\BlockBGCOffiOffaNet}{\textit{not run}\xspace}  % r21.BGC.OffiOffa.Net: net paired difference over pair
\newcommand{\BlockBGCOffiOffaNetCI}{\textit{not run}\xspace}  % r21.BGC.OffiOffa.NetCI: net paired difference, Newcombe method-10 marginal 95% interval over pair
\newcommand{\BlockBGCOffiOffaP}{\textit{not run}\xspace}  % r21.BGC.OffiOffa.P: exact two-sided sign test over pair
\newcommand{\BlockBGCOffiOffaPairs}{\textit{not run}\xspace}  % r21.BGC.OffiOffa.Pairs: complete pairs over pair
\newcommand{\BlockBGCOffiOffaRescue}{\textit{not run}\xspace}  % r21.BGC.OffiOffa.Rescue: control failed, treatment passed over pair
\newcommand{\BlockBGCOffiOffaTie}{\textit{not run}\xspace}  % r21.BGC.OffiOffa.Tie: both passed or both failed over pair
\newcommand{\BlockBGCP}{\textit{not run}\xspace}  % pending.BGC.p: exact two-sided sign test over pair
\newcommand{\BlockBGCPairs}{\textit{not run}\xspace}  % pending.BGC.pairs: count over pair
\newcommand{\BlockBGCReadingBody}{Block~BGC was not run (\BlockBGCDisposition). It contributes no inferential result; its paper-wide slots are non-rejection placeholders.\xspace}  % r21.BGC.body: main-text reading paragraph over -
\newcommand{\BlockBGCReadingFull}{Block~BGC was not run (\BlockBGCDisposition). It contributes no inferential result; its paper-wide slots are non-rejection placeholders.\xspace}  % r21.BGC.full: appendix reading paragraph over -
\newcommand{\BlockBGCReadingIDs}{NOTRUN\xspace}  % r21.BGC.reading_ids: registered reading ids selected by the mirrored rule over -
\newcommand{\BlockBGCReadingShort}{not run (\BlockBGCDisposition)\xspace}  % r21.BGC.short: short reading over -
\newcommand{\BlockBGCRegistered}{ADDENDUM~19\xspace}  % r21.BGC.registered: where the block is registered, and whether that registration is frozen (heading present and .sha256 verifying) over -
\newcommand{\BlockBGCReplaced}{\textit{not run}\xspace}  % r21.BGC.replaced: notrun over -
\newcommand{\BlockBGCRows}{\textit{terminal disposition not\_run\_preconditions\_unmet:manifest\_blockBGC,admission\_link\_blockBGC,inline\_contract\_dryrun\_BGC}\xspace}  % pending.BGC.rows: rows so far over rollout
\newcommand{\BlockBGCSeedList}{42--49, 51--55, 57--59\xspace}  % r21.BGC.seeds: exact seed list of the block's paired instances over seed
\newcommand{\BlockBGCShortForm}{GPT-6 on the same instances (Block~BGC): \BlockBGCReadingShort.\xspace}  % r21.BGC.shortform: main-text short form over -
\newcommand{\BlockBGCState}{notrun\xspace}  % r21.BGC.state: execution disposition (r21_state) over -
\newcommand{\BlockBGCStateCell}{not run: launch preconditions unmet by the experiment cutoff\xspace}  % r28.BGC.cell: r28: the block's state for Table 1 over -
\newcommand{\BlockBGCStatus}{\textit{terminal disposition not\_run\_preconditions\_unmet:manifest\_blockBGC,admission\_link\_blockBGC,inline\_contract\_dryrun\_BGC}\xspace}  % pending.BGC.status: search-log status over -
\newcommand{\BlockBGCVerdictFail}{\textit{not run}\xspace}  % r21.BGC.VerdictFail: VerdictFail over -
\newcommand{\BlockBGCVerdictSucc}{\textit{not run}\xspace}  % r21.BGC.VerdictSucc: VerdictSucc over -
\newcommand{\BlockBGCVindAgree}{\textit{not run}\xspace}  % r21.BGC.vind: validity re-derivation over -
\newcommand{\BlockBGCVindAgreeSlash}{\textit{not run}\xspace}  % r21.BGC.vind_slash: validity re-derivation over -
\newcommand{\BlockBGCVindPath}{\code{audit/\allowbreak{}failure\_\allowbreak{}mining/\allowbreak{}P3v2/\allowbreak{}VALIDITY\_\allowbreak{}INDEPENDENT\_\allowbreak{}blockBGC.json}\xspace}  % r21.BGC.vind_path: the expected independent validity re-derivation artifact over -
\newcommand{\BlockBGCVindStatus}{\textit{not re-derived}\xspace}  % r21.BGC.vind_status: whether audit/failure_mining/P3v2/VALIDITY_INDEPENDENT_blockBGC.json exists over -
\newcommand{\BlockBGtwoConfig}{Codex CLI, frames inline\xspace}  % r21.BGtwo.config: invoker and frame-delivery channel, from the spec over -
\newcommand{\BlockBGtwoContradictions}{\textit{not run}\xspace}  % r21.BGtwo.Contradictions: Contradictions over -
\newcommand{\BlockBGtwoControls}{3\xspace}  % r21.BGtwo.controls: unpaired control rollouts in the spec over rollout
\newcommand{\BlockBGtwoCounted}{\textit{not run}\xspace}  % r21.BGtwo.counted: notrun over -
\newcommand{\BlockBGtwoCountedFail}{\textit{not run}\xspace}  % r21.BGtwo.CountedFail: counted failures over -
\newcommand{\BlockBGtwoCountedSucc}{\textit{not run}\xspace}  % r21.BGtwo.CountedSucc: CountedSucc over -
\newcommand{\BlockBGtwoDecisionTerm}{\textit{not run}\xspace}  % r21.BGtwo.DecisionTerm: DecisionTerm over -
\newcommand{\BlockBGtwoDisposition}{fallback not triggered\xspace}  % r21.BGtwo.disposition: disposition text over -
\newcommand{\BlockBGtwoEffect}{\textit{not run}\xspace}  % pending.BGtwo.effect: discordant-pair proportion (envos.stats.effect_size; NOT the net paired effect) over pair
\newcommand{\BlockBGtwoEndpointFull}{\textit{not run}\xspace}  % r21.BGtwo.EndpointFull: EndpointFull over -
\newcommand{\BlockBGtwoEndpointFullSucc}{\textit{not run}\xspace}  % r21.BGtwo.EndpointFullSucc: EndpointFullSucc over -
\newcommand{\BlockBGtwoEndpointUnresolved}{\textit{not run}\xspace}  % r21.BGtwo.EndpointUnresolved: EndpointUnresolved over -
\newcommand{\BlockBGtwoFRXOffAN}{\textit{not run}\xspace}  % pending.BGtwo.FRX-OFF-A.n: count over counted rollout
\newcommand{\BlockBGtwoFRXOffAPass}{\textit{not run}\xspace}  % pending.BGtwo.FRX-OFF-A.pass: count over counted rollout
\newcommand{\BlockBGtwoFRXOffAPassFrac}{\textit{not run}\xspace}  % pending.BGtwo.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\BlockBGtwoFRXOnAN}{\textit{not run}\xspace}  % pending.BGtwo.FRX-ON-A.n: count over counted rollout
\newcommand{\BlockBGtwoFRXOnAPass}{\textit{not run}\xspace}  % pending.BGtwo.FRX-ON-A.pass: count over counted rollout
\newcommand{\BlockBGtwoFRXOnAPassFrac}{\textit{not run}\xspace}  % pending.BGtwo.FRX-ON-A.frac: k/n over counted rollout
\newcommand{\BlockBGtwoFRXOnIN}{\textit{not run}\xspace}  % pending.BGtwo.FRX-ON-I.n: count over counted rollout
\newcommand{\BlockBGtwoFRXOnIPass}{\textit{not run}\xspace}  % pending.BGtwo.FRX-ON-I.pass: count over counted rollout
\newcommand{\BlockBGtwoFRXOnIPassFrac}{\textit{not run}\xspace}  % pending.BGtwo.FRX-ON-I.frac: k/n over counted rollout
\newcommand{\BlockBGtwoInstancePhrase}{\BlockBGtwoInstances frozen generated instances (seeds \BlockBGtwoSeedList)\xspace}  % r21.BGtwo.instance_phrase: the block's instances as a phrase that reads correctly whether or not its spec exists over -
\newcommand{\BlockBGtwoInstances}{10\xspace}  % r21.BGtwo.instances: paired instances over instance
\newcommand{\BlockBGtwoInstancesWords}{ten\xspace}  % r21.BGtwo.instances_words: in words over instance
\newcommand{\BlockBGtwoModel}{GPT-6\xspace}  % r21.BGtwo.model: evaluated model over -
\newcommand{\BlockBGtwoNNeg}{\textit{not run}\xspace}  % pending.BGtwo.n_neg: count over pair
\newcommand{\BlockBGtwoNPos}{\textit{not run}\xspace}  % pending.BGtwo.n_pos: count over pair
\newcommand{\BlockBGtwoNTied}{\textit{not run}\xspace}  % pending.BGtwo.n_tied: count over pair
\newcommand{\BlockBGtwoOffFail}{\textit{not run}\xspace}  % r21.BGtwo.off_fail: notrun over -
\newcommand{\BlockBGtwoOffPass}{\textit{not run}\xspace}  % r21.BGtwo.off_pass: notrun over -
\newcommand{\BlockBGtwoOnOffBonfPaper}{\textit{not run}\xspace}  % fam.alias.BGtwo.OnOff.b: alternative not used over -
\newcommand{\BlockBGtwoOnOffBothFail}{\textit{not run}\xspace}  % r21.BGtwo.OnOff.BothFail: both failed over pair
\newcommand{\BlockBGtwoOnOffBothPass}{\textit{not run}\xspace}  % r21.BGtwo.OnOff.BothPass: both passed over pair
\newcommand{\BlockBGtwoOnOffDir}{\textit{not run}\xspace}  % r21.BGtwo.OnOff.Dir: direction of the discordance over pair
\newcommand{\BlockBGtwoOnOffHarm}{\textit{not run}\xspace}  % r21.BGtwo.OnOff.Harm: control passed, treatment failed over pair
\newcommand{\BlockBGtwoOnOffHolmLocal}{\textit{not run}\xspace}  % r21.BGtwo.OnOff.HolmLocal: - over pair
\newcommand{\BlockBGtwoOnOffHolmPaper}{\textit{not run}\xspace}  % fam.alias.BGtwo.OnOff: alternative not used over -
\newcommand{\BlockBGtwoOnOffNet}{\textit{not run}\xspace}  % r21.BGtwo.OnOff.Net: net paired difference over pair
\newcommand{\BlockBGtwoOnOffNetCI}{\textit{not run}\xspace}  % r21.BGtwo.OnOff.NetCI: net paired difference, Newcombe method-10 marginal 95% interval over pair
\newcommand{\BlockBGtwoOnOffP}{\textit{not run}\xspace}  % r21.BGtwo.OnOff.P: exact two-sided sign test over pair
\newcommand{\BlockBGtwoOnOffPairs}{\textit{not run}\xspace}  % r21.BGtwo.OnOff.Pairs: complete pairs over pair
\newcommand{\BlockBGtwoOnOffRescue}{\textit{not run}\xspace}  % r21.BGtwo.OnOff.Rescue: control failed, treatment passed over pair
\newcommand{\BlockBGtwoOnOffTie}{\textit{not run}\xspace}  % r21.BGtwo.OnOff.Tie: both passed or both failed over pair
\newcommand{\BlockBGtwoP}{\textit{not run}\xspace}  % pending.BGtwo.p: exact two-sided sign test over pair
\newcommand{\BlockBGtwoPairs}{\textit{not run}\xspace}  % pending.BGtwo.pairs: count over pair
\newcommand{\BlockBGtwoReadingBody}{Block~BG2 was not run (\BlockBGtwoDisposition).\xspace}  % r21.BGtwo.body: main-text reading paragraph over -
\newcommand{\BlockBGtwoReadingFull}{Block~BG2 was not run (\BlockBGtwoDisposition).\xspace}  % r21.BGtwo.full: appendix reading paragraph over -
\newcommand{\BlockBGtwoReadingIDs}{NOTRUN\xspace}  % r21.BGtwo.reading_ids: registered reading ids selected by the mirrored rule over -
\newcommand{\BlockBGtwoReadingShort}{not run (\BlockBGtwoDisposition)\xspace}  % r21.BGtwo.short: short reading over -
\newcommand{\BlockBGtwoRegistered}{ADDENDUM~19\xspace}  % r21.BGtwo.registered: where the block is registered, and whether that registration is frozen (heading present and .sha256 verifying) over -
\newcommand{\BlockBGtwoReplaced}{\textit{not run}\xspace}  % r21.BGtwo.replaced: notrun over -
\newcommand{\BlockBGtwoRows}{\textit{fallback not triggered}\xspace}  % pending.BGtwo.rows: rows so far over rollout
\newcommand{\BlockBGtwoSeedList}{20--29\xspace}  % r21.BGtwo.seeds: exact seed list of the block's paired instances over seed
\newcommand{\BlockBGtwoShortForm}{\xspace}  % r21.BGtwo.shortform: main-text short form over -
\newcommand{\BlockBGtwoState}{notrun\xspace}  % r21.BGtwo.state: execution disposition (r21_state) over -
\newcommand{\BlockBGtwoStateCell}{not run\xspace}  % r28.BGtwo.cell: r28: the block's state for Table 1 over -
\newcommand{\BlockBGtwoStatus}{\textit{fallback not triggered}\xspace}  % pending.BGtwo.status: search-log status over -
\newcommand{\BlockBGtwoVerdictFail}{\textit{not run}\xspace}  % r21.BGtwo.VerdictFail: VerdictFail over -
\newcommand{\BlockBGtwoVerdictSucc}{\textit{not run}\xspace}  % r21.BGtwo.VerdictSucc: VerdictSucc over -
\newcommand{\BlockBGtwoVindAgree}{\textit{not run}\xspace}  % r21.BGtwo.vind: validity re-derivation over -
\newcommand{\BlockBGtwoVindAgreeSlash}{\textit{not run}\xspace}  % r21.BGtwo.vind_slash: validity re-derivation over -
\newcommand{\BlockBGtwoVindPath}{\code{audit/\allowbreak{}failure\_\allowbreak{}mining/\allowbreak{}P3v2/\allowbreak{}VALIDITY\_\allowbreak{}INDEPENDENT\_\allowbreak{}blockBG2.json}\xspace}  % r21.BGtwo.vind_path: the expected independent validity re-derivation artifact over -
\newcommand{\BlockBGtwoVindStatus}{\textit{not re-derived}\xspace}  % r21.BGtwo.vind_status: whether audit/failure_mining/P3v2/VALIDITY_INDEPENDENT_blockBG2.json exists over -
\newcommand{\BlockBNNeg}{10\xspace}  % pending.B.n_neg: count over pair
\newcommand{\BlockBNPos}{0\xspace}  % pending.B.n_pos: count over pair
\newcommand{\BlockBNTied}{0\xspace}  % pending.B.n_tied: count over pair
\newcommand{\BlockBP}{0.002\xspace}  % pending.B.p: exact two-sided sign test over pair
\newcommand{\BlockBPairs}{10\xspace}  % pending.B.pairs: count over pair
\newcommand{\BlockBRFRXOffAN}{\textit{cancelled}\xspace}  % pending.BR.FRX-OFF-A.n: count over counted rollout
\newcommand{\BlockBRFRXOffAPass}{\textit{cancelled}\xspace}  % pending.BR.FRX-OFF-A.pass: count over counted rollout
\newcommand{\BlockBRFRXOffAPassFrac}{\textit{cancelled}\xspace}  % pending.BR.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\BlockBRRows}{\textit{cancelled}\xspace}  % pending.BR.rows: rows so far over rollout
\newcommand{\BlockBRSFRXOffAN}{\textit{cancelled}\xspace}  % pending.BRS.FRX-OFF-A.n: count over counted rollout
\newcommand{\BlockBRSFRXOffAPass}{\textit{cancelled}\xspace}  % pending.BRS.FRX-OFF-A.pass: count over counted rollout
\newcommand{\BlockBRSFRXOffAPassFrac}{\textit{cancelled}\xspace}  % pending.BRS.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\BlockBRSLtwoN}{\textit{cancelled}\xspace}  % pending.BR.S-L2.n: count over counted rollout
\newcommand{\BlockBRSLtwoPass}{\textit{cancelled}\xspace}  % pending.BR.S-L2.pass: count over counted rollout
\newcommand{\BlockBRSLtwoPassFrac}{\textit{cancelled}\xspace}  % pending.BR.S-L2.frac: k/n over counted rollout
\newcommand{\BlockBRSRows}{\textit{cancelled}\xspace}  % pending.BRS.rows: rows so far over rollout
\newcommand{\BlockBRSSLtwoN}{\textit{cancelled}\xspace}  % pending.BRS.S-L2.n: count over counted rollout
\newcommand{\BlockBRSSLtwoPass}{\textit{cancelled}\xspace}  % pending.BRS.S-L2.pass: count over counted rollout
\newcommand{\BlockBRSSLtwoPassFrac}{\textit{cancelled}\xspace}  % pending.BRS.S-L2.frac: k/n over counted rollout
\newcommand{\BlockBRSStatus}{\textit{cancelled}\xspace}  % pending.BRS.status: search-log status over -
\newcommand{\BlockBRStatus}{\textit{cancelled}\xspace}  % pending.BR.status: search-log status over -
\newcommand{\BlockBRows}{23\xspace}  % pending.B.rows: rows so far over rollout
\newcommand{\BlockBSEffect}{0.600\xspace}  % pending.BS.effect: discordant-pair proportion (envos.stats.effect_size; NOT the net paired effect) over pair
\newcommand{\BlockBSFRXOffACap}{2\xspace}  % pending.BS.FRX-OFF-A.Cap: count over counted rollout
\newcommand{\BlockBSFRXOffAN}{10\xspace}  % pending.BS.FRX-OFF-A.n: count over counted rollout
\newcommand{\BlockBSFRXOffAPass}{0\xspace}  % pending.BS.FRX-OFF-A.pass: count over counted rollout
\newcommand{\BlockBSFRXOffAPassFrac}{0/10\xspace}  % pending.BS.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\BlockBSFRXOffARevised}{0\xspace}  % pending.BS.FRX-OFF-A.Revised: count over counted rollout
\newcommand{\BlockBSFRXOffAStaleFlagged}{0\xspace}  % pending.BS.FRX-OFF-A.StaleFlagged: count over counted rollout
\newcommand{\BlockBSFRXOffAStaleUnflagged}{9\xspace}  % pending.BS.FRX-OFF-A.StaleUnflagged: count over counted rollout
\newcommand{\BlockBSFRXOnACap}{1\xspace}  % pending.BS.FRX-ON-A.Cap: count over counted rollout
\newcommand{\BlockBSFRXOnAN}{10\xspace}  % pending.BS.FRX-ON-A.n: count over counted rollout
\newcommand{\BlockBSFRXOnAPass}{6\xspace}  % pending.BS.FRX-ON-A.pass: count over counted rollout
\newcommand{\BlockBSFRXOnAPassFrac}{6/10\xspace}  % pending.BS.FRX-ON-A.frac: k/n over counted rollout
\newcommand{\BlockBSFRXOnARevised}{6\xspace}  % pending.BS.FRX-ON-A.Revised: count over counted rollout
\newcommand{\BlockBSFRXOnAStaleFlagged}{1\xspace}  % pending.BS.FRX-ON-A.StaleFlagged: count over counted rollout
\newcommand{\BlockBSFRXOnAStaleUnflagged}{0\xspace}  % pending.BS.FRX-ON-A.StaleUnflagged: count over counted rollout
\newcommand{\BlockBSFRXOnICap}{1\xspace}  % pending.BS.FRX-ON-I.Cap: count over counted rollout
\newcommand{\BlockBSFRXOnIN}{3\xspace}  % pending.BS.FRX-ON-I.n: count over counted rollout
\newcommand{\BlockBSFRXOnIPass}{2\xspace}  % pending.BS.FRX-ON-I.pass: count over counted rollout
\newcommand{\BlockBSFRXOnIPassFrac}{2/3\xspace}  % pending.BS.FRX-ON-I.frac: k/n over counted rollout
\newcommand{\BlockBSFRXOnIRevised}{0\xspace}  % pending.BS.FRX-ON-I.Revised: count over counted rollout
\newcommand{\BlockBSFRXOnIStaleFlagged}{0\xspace}  % pending.BS.FRX-ON-I.StaleFlagged: count over counted rollout
\newcommand{\BlockBSFRXOnIStaleUnflagged}{0\xspace}  % pending.BS.FRX-ON-I.StaleUnflagged: count over counted rollout
\newcommand{\BlockBSNNeg}{6\xspace}  % pending.BS.n_neg: count over pair
\newcommand{\BlockBSNPos}{0\xspace}  % pending.BS.n_pos: count over pair
\newcommand{\BlockBSNTied}{4\xspace}  % pending.BS.n_tied: count over pair
\newcommand{\BlockBSP}{0.031\xspace}  % pending.BS.p: exact two-sided sign test over pair
\newcommand{\BlockBSPairs}{10\xspace}  % pending.BS.pairs: count over pair
\newcommand{\BlockBSRows}{26\xspace}  % pending.BS.rows: rows so far over rollout
\newcommand{\BlockBSStatus}{\texttt{complete}\xspace}  % pending.BS.status: search-log status over -
\newcommand{\BlockBSVoided}{3\xspace}  % pending.BS.voided: count over rollout
\newcommand{\BlockBStatus}{\texttt{complete}\xspace}  % pending.B.status: search-log status over -
\newcommand{\BlockBVoided}{0\xspace}  % pending.B.voided: count over rollout
\newcommand{\BlockClmBAttempts}{24\xspace}  % clm.ClmB.Attempts: Attempts over -
\newcommand{\BlockClmBAuditGate}{passed\xspace}  % clm.ClmB.AuditGate: AuditGate over -
\newcommand{\BlockClmBAuditTerms}{4\xspace}  % clm.ClmB.AuditTerms: AuditTerms over -
\newcommand{\BlockClmBClmLzeroCap}{0\xspace}  % pending.ClmB.CLM-L0.Cap: count over counted rollout
\newcommand{\BlockClmBClmLzeroN}{1\xspace}  % pending.ClmB.CLM-L0.n: count over counted rollout
\newcommand{\BlockClmBClmLzeroPass}{1\xspace}  % pending.ClmB.CLM-L0.pass: count over counted rollout
\newcommand{\BlockClmBClmLzeroPassFrac}{1/1\xspace}  % pending.ClmB.CLM-L0.frac: k/n over counted rollout
\newcommand{\BlockClmBClmLzeroRevised}{0\xspace}  % pending.ClmB.CLM-L0.Revised: count over counted rollout
\newcommand{\BlockClmBClmLzeroStaleFlagged}{0\xspace}  % pending.ClmB.CLM-L0.StaleFlagged: count over counted rollout
\newcommand{\BlockClmBClmLzeroStaleUnflagged}{0\xspace}  % pending.ClmB.CLM-L0.StaleUnflagged: count over counted rollout
\newcommand{\BlockClmBClmOffACap}{0\xspace}  % pending.ClmB.CLM-OFF-A.Cap: count over counted rollout
\newcommand{\BlockClmBClmOffAN}{10\xspace}  % pending.ClmB.CLM-OFF-A.n: count over counted rollout
\newcommand{\BlockClmBClmOffAPass}{10\xspace}  % pending.ClmB.CLM-OFF-A.pass: count over counted rollout
\newcommand{\BlockClmBClmOffAPassFrac}{10/10\xspace}  % pending.ClmB.CLM-OFF-A.frac: k/n over counted rollout
\newcommand{\BlockClmBClmOffARevised}{0\xspace}  % pending.ClmB.CLM-OFF-A.Revised: count over counted rollout
\newcommand{\BlockClmBClmOffAStaleFlagged}{0\xspace}  % pending.ClmB.CLM-OFF-A.StaleFlagged: count over counted rollout
\newcommand{\BlockClmBClmOffAStaleUnflagged}{0\xspace}  % pending.ClmB.CLM-OFF-A.StaleUnflagged: count over counted rollout
\newcommand{\BlockClmBClmOnACap}{0\xspace}  % pending.ClmB.CLM-ON-A.Cap: count over counted rollout
\newcommand{\BlockClmBClmOnAN}{10\xspace}  % pending.ClmB.CLM-ON-A.n: count over counted rollout
\newcommand{\BlockClmBClmOnAPass}{10\xspace}  % pending.ClmB.CLM-ON-A.pass: count over counted rollout
\newcommand{\BlockClmBClmOnAPassFrac}{10/10\xspace}  % pending.ClmB.CLM-ON-A.frac: k/n over counted rollout
\newcommand{\BlockClmBClmOnARevised}{0\xspace}  % pending.ClmB.CLM-ON-A.Revised: count over counted rollout
\newcommand{\BlockClmBClmOnAStaleFlagged}{0\xspace}  % pending.ClmB.CLM-ON-A.StaleFlagged: count over counted rollout
\newcommand{\BlockClmBClmOnAStaleUnflagged}{0\xspace}  % pending.ClmB.CLM-ON-A.StaleUnflagged: count over counted rollout
\newcommand{\BlockClmBClmOnICap}{0\xspace}  % pending.ClmB.CLM-ON-I.Cap: count over counted rollout
\newcommand{\BlockClmBClmOnIN}{3\xspace}  % pending.ClmB.CLM-ON-I.n: count over counted rollout
\newcommand{\BlockClmBClmOnIPass}{3\xspace}  % pending.ClmB.CLM-ON-I.pass: count over counted rollout
\newcommand{\BlockClmBClmOnIPassFrac}{3/3\xspace}  % pending.ClmB.CLM-ON-I.frac: k/n over counted rollout
\newcommand{\BlockClmBClmOnIRevised}{0\xspace}  % pending.ClmB.CLM-ON-I.Revised: count over counted rollout
\newcommand{\BlockClmBClmOnIStaleFlagged}{0\xspace}  % pending.ClmB.CLM-ON-I.StaleFlagged: count over counted rollout
\newcommand{\BlockClmBClmOnIStaleUnflagged}{0\xspace}  % pending.ClmB.CLM-ON-I.StaleUnflagged: count over counted rollout
\newcommand{\BlockClmBConfig}{Claude CLI, frames by file read\xspace}  % r21.ClmB.config: invoker and frame-delivery channel, from the spec over -
\newcommand{\BlockClmBContradictions}{0\xspace}  % r21.ClmB.Contradictions: Contradictions over counted rollout
\newcommand{\BlockClmBControls}{4\xspace}  % r21.ClmB.controls: unpaired control rollouts in the spec over rollout
\newcommand{\BlockClmBControlsCredible}{credible\xspace}  % r21.ClmB.ControlsCredible: ControlsCredible over -
\newcommand{\BlockClmBCopyLimitControls}{not credible\xspace}  % clm.ClmB.CopyLimitControls: CopyLimitControls over -
\newcommand{\BlockClmBCopyLimitDerived}{not met\xspace}  % clm.ClmB.CopyLimitDerived: CopyLimitDerived over -
\newcommand{\BlockClmBCopyLimitHarm}{0\xspace}  % clm.ClmB.CopyLimitHarm: CopyLimitHarm over -
\newcommand{\BlockClmBCopyLimitOffFail}{10\xspace}  % clm.ClmB.CopyLimitOffFail: CopyLimitOffFail over -
\newcommand{\BlockClmBCopyLimitP}{0.0156\xspace}  % clm.ClmB.CopyLimitP: CopyLimitP over -
\newcommand{\BlockClmBCopyLimitReading}{R1\xspace}  % r21.ClmB.CopyLimitReading: CopyLimitReading over -
\newcommand{\BlockClmBCopyLimitRescue}{7\xspace}  % clm.ClmB.CopyLimitRescue: CopyLimitRescue over -
\newcommand{\BlockClmBCopyLimitTie}{3\xspace}  % clm.ClmB.CopyLimitTie: CopyLimitTie over -
\newcommand{\BlockClmBCopyLimitXupN}{3\xspace}  % clm.ClmB.CopyLimitXupN: CopyLimitXupN over -
\newcommand{\BlockClmBCopyLimitXupOn}{0\xspace}  % clm.ClmB.CopyLimitXupOn: CopyLimitXupOn over -
\newcommand{\BlockClmBCounted}{24\xspace}  % r21.ClmB.counted: counted rollouts over rollout
\newcommand{\BlockClmBCountedFail}{0\xspace}  % r21.ClmB.CountedFail: counted failures over counted rollout
\newcommand{\BlockClmBCountedSucc}{24\xspace}  % r21.ClmB.CountedSucc: CountedSucc over counted rollout
\newcommand{\BlockClmBDecideCheck}{registered decide() = mirror = stored reading\xspace}  % clm.ClmB.DecideCheck: DecideCheck over -
\newcommand{\BlockClmBDecisionTerm}{24\xspace}  % r21.ClmB.DecisionTerm: DecisionTerm over counted rollout
\newcommand{\BlockClmBDerivedGate}{met\xspace}  % r21.ClmB.DerivedGate: DerivedGate over -
\newcommand{\BlockClmBDisposition}{completed\xspace}  % r21.ClmB.disposition: disposition text over -
\newcommand{\BlockClmBEffect}{---\xspace}  % pending.ClmB.effect: discordant-pair proportion (envos.stats.effect_size; NOT the net paired effect) over pair
\newcommand{\BlockClmBEndpointFull}{24\xspace}  % r21.ClmB.EndpointFull: EndpointFull over counted rollout
\newcommand{\BlockClmBEndpointFullSucc}{24\xspace}  % r21.ClmB.EndpointFullSucc: EndpointFullSucc over counted rollout
\newcommand{\BlockClmBEndpointUnresolved}{0\xspace}  % r21.ClmB.EndpointUnresolved: EndpointUnresolved over counted rollout
\newcommand{\BlockClmBHolmSlot}{6\xspace}  % clm.ClmB.HolmSlot: HolmSlot over -
\newcommand{\BlockClmBInstancePhrase}{\BlockClmBInstances frozen generated instances (seeds \BlockClmBSeedList)\xspace}  % r21.ClmB.instance_phrase: the block's instances as a phrase that reads correctly whether or not its spec exists over -
\newcommand{\BlockClmBInstances}{10\xspace}  % r21.ClmB.instances: paired instances over instance
\newcommand{\BlockClmBInstancesWords}{ten\xspace}  % r21.ClmB.instances_words: in words over instance
\newcommand{\BlockClmBInterrupted}{0\xspace}  % clm.ClmB.Interrupted: Interrupted over -
\newcommand{\BlockClmBInterruptedWhere}{none\xspace}  % clm.ClmB.InterruptedWhere: InterruptedWhere over -
\newcommand{\BlockClmBInterruptedWhy}{none\xspace}  % clm.ClmB.InterruptedWhy: InterruptedWhy over -
\newcommand{\BlockClmBModel}{Claude Opus~5\xspace}  % r21.ClmB.model: evaluated model over -
\newcommand{\BlockClmBNNeg}{---\xspace}  % pending.ClmB.n_neg: count over pair
\newcommand{\BlockClmBNPos}{---\xspace}  % pending.ClmB.n_pos: count over pair
\newcommand{\BlockClmBNTied}{---\xspace}  % pending.ClmB.n_tied: count over pair
\newcommand{\BlockClmBOffBack}{8\xspace}  % clm.ClmB.OffBack: OffBack over -
\newcommand{\BlockClmBOffFail}{0\xspace}  % r21.ClmB.off_fail: CLM-OFF-A failures over instance
\newcommand{\BlockClmBOffPass}{10\xspace}  % r21.ClmB.off_pass: CLM-OFF-A successes over instance
\newcommand{\BlockClmBOffReread}{10\xspace}  % clm.ClmB.OffReread: OffReread over -
\newcommand{\BlockClmBOffStale}{0\xspace}  % clm.ClmB.OffStale: OffStale over -
\newcommand{\BlockClmBOnBack}{8\xspace}  % clm.ClmB.OnBack: OnBack over -
\newcommand{\BlockClmBOnFailCorrect}{0\xspace}  % clm.ClmB.OnFailCorrect: OnFailCorrect over -
\newcommand{\BlockClmBOnFailTerms}{none\xspace}  % clm.ClmB.OnFailTerms: OnFailTerms over -
\newcommand{\BlockClmBOnOffBonfPaper}{1.00\xspace}  % fam.alias.ClmB.OnOff.b: alias over -
\newcommand{\BlockClmBOnOffBothFail}{0\xspace}  % r21.ClmB.OnOff.BothFail: both failed over pair
\newcommand{\BlockClmBOnOffBothPass}{10\xspace}  % r21.ClmB.OnOff.BothPass: both passed over pair
\newcommand{\BlockClmBOnOffDir}{none\xspace}  % r21.ClmB.OnOff.Dir: direction of the discordance over pair
\newcommand{\BlockClmBOnOffHarm}{0\xspace}  % r21.ClmB.OnOff.Harm: control passed, treatment failed over pair
\newcommand{\BlockClmBOnOffHolmLocal}{---\xspace}  % r21.ClmB.OnOff.HolmLocal: not in a block-local family over pair
\newcommand{\BlockClmBOnOffHolmPaper}{1.00\xspace}  % fam.alias.ClmB.OnOff: alias over -
\newcommand{\BlockClmBOnOffNet}{$0.00$\xspace}  % r21.ClmB.OnOff.Net: net paired difference over pair
\newcommand{\BlockClmBOnOffNetCI}{$0.00$ [$-0.28$, $0.28$]\xspace}  % r21.ClmB.OnOff.NetCI: net paired difference, Newcombe method-10 marginal 95% interval over pair
\newcommand{\BlockClmBOnOffP}{1.00\xspace}  % r21.ClmB.OnOff.P: exact two-sided sign test over pair
\newcommand{\BlockClmBOnOffPairs}{10\xspace}  % r21.ClmB.OnOff.Pairs: complete pairs over pair
\newcommand{\BlockClmBOnOffRescue}{0\xspace}  % r21.ClmB.OnOff.Rescue: control failed, treatment passed over pair
\newcommand{\BlockClmBOnOffTie}{10\xspace}  % r21.ClmB.OnOff.Tie: both passed or both failed over pair
\newcommand{\BlockClmBOnReread}{10\xspace}  % clm.ClmB.OnReread: OnReread over -
\newcommand{\BlockClmBOrderWord}{frozen\xspace}  % r22.clm_order: 'frozen' only once the claims pre-registration is frozen over -
\newcommand{\BlockClmBP}{1.000\xspace}  % pending.ClmB.p: exact two-sided sign test over pair
\newcommand{\BlockClmBPairs}{10\xspace}  % pending.ClmB.pairs: count over pair
\newcommand{\BlockClmBPaperFamilyP}{1.00\xspace}  % clm.ClmB.PaperFamilyP: PaperFamilyP over -
\newcommand{\BlockClmBReadingBody}{Over \BlockClmBOnOffPairs sealed instance pairs (seeds \BlockClmBSeedList), Claude Opus~5 met the full approval endpoint on \BlockClmBClmOffAPassFrac without the panel and \BlockClmBClmOnAPassFrac with it; of the pairs, \BlockClmBOnOffRescue favoured the panel, \BlockClmBOnOffHarm the arm without it, and \BlockClmBOnOffTie neither; net \BlockClmBOnOffNetCI (marginal 95\,\% interval), $p=\BlockClmBOnOffP$. Controls: ON-I \BlockClmBClmOnIPassFrac, L0 \BlockClmBClmLzeroPassFrac. Without the panel, the agent succeeded on \BlockClmBOffPass/\BlockClmBClmOffAN instances under silent supersession; the registered rescue-opportunity threshold was not met. The scripted copy-limit shortcut, run on the same cells before any model, is assigned \BlockClmBCopyLimitReading under the same rules. Every outcome term the independent scorer re-derives is resolved and agreeing with the evaluator on \BlockClmBEndpointFull of \BlockClmBCounted counted rollouts. The standard-library validity re-derivation agrees with the archive on \BlockClmBVindAgree attempts.\xspace}  % r21.ClmB.body: main-text reading paragraph over -
\newcommand{\BlockClmBReadingFull}{Over \BlockClmBOnOffPairs sealed instance pairs (seeds \BlockClmBSeedList), Claude Opus~5 met the full approval endpoint on \BlockClmBClmOffAPassFrac without the panel and \BlockClmBClmOnAPassFrac with it; of the pairs, \BlockClmBOnOffRescue favoured the panel, \BlockClmBOnOffHarm the arm without it, and \BlockClmBOnOffTie neither; net \BlockClmBOnOffNetCI (marginal 95\,\% interval), $p=\BlockClmBOnOffP$. Controls: ON-I \BlockClmBClmOnIPassFrac, L0 \BlockClmBClmLzeroPassFrac. Without the panel, the agent succeeded on \BlockClmBOffPass/\BlockClmBClmOffAN instances under silent supersession; the registered rescue-opportunity threshold was not met. The scripted copy-limit shortcut, run on the same cells before any model, is assigned \BlockClmBCopyLimitReading under the same rules. Every outcome term the independent scorer re-derives is resolved and agreeing with the evaluator on \BlockClmBEndpointFull of \BlockClmBCounted counted rollouts. The standard-library validity re-derivation agrees with the archive on \BlockClmBVindAgree attempts.\xspace}  % r21.ClmB.full: appendix reading paragraph over -
\newcommand{\BlockClmBReadingIDs}{R2\xspace}  % r21.ClmB.reading_ids: registered reading ids selected by the mirrored rule over -
\newcommand{\BlockClmBReadingMain}{Over \BlockClmBOnOffPairs sealed instance pairs (seeds \BlockClmBSeedList), Claude Opus~5 met the full approval endpoint on \BlockClmBClmOffAPassFrac without the panel and \BlockClmBClmOnAPassFrac with it; of the pairs, \BlockClmBOnOffRescue favoured the panel, \BlockClmBOnOffHarm the arm without it, and \BlockClmBOnOffTie neither; net \BlockClmBOnOffNetCI (marginal 95\,\% interval), $p=\BlockClmBOnOffP$. Controls: ON-I \BlockClmBClmOnIPassFrac, L0 \BlockClmBClmLzeroPassFrac. Without the panel, the agent succeeded on \BlockClmBOffPass/\BlockClmBClmOffAN instances under silent supersession; the registered rescue-opportunity threshold was not met. The pre-registered derived-decision gate passed on all three threshold-crossing cases. Every outcome term the independent scorer re-derives is resolved and agreeing with the evaluator on \BlockClmBEndpointFull of \BlockClmBCounted counted rollouts. The standard-library validity re-derivation agrees with the archive on \BlockClmBVindAgree attempts.\xspace}  % r28.ClmB.main: r28: main-text reading paragraph (GPT-6 r20 page 6) over -
\newcommand{\BlockClmBReadingShort}{OFF-A succeeded often, below the rescue-opportunity threshold\xspace}  % r21.ClmB.short: short reading over -
\newcommand{\BlockClmBRegistered}{PRECOMMIT\_\allowbreak{}CLAIMS\xspace}  % r21.ClmB.registered: where the block is registered, and whether that registration is frozen (heading present and .sha256 verifying) over -
\newcommand{\BlockClmBReplaced}{0\xspace}  % r21.ClmB.replaced: attempts not counted over rollout
\newcommand{\BlockClmBReplacements}{0\xspace}  % r21.ClmB.Replacements: Replacements over -
\newcommand{\BlockClmBReplacementsSpent}{0\xspace}  % clm.ClmB.ReplacementsSpent: ReplacementsSpent over -
\newcommand{\BlockClmBRfourWhy}{--\xspace}  % r21.ClmB.r4why: why R4 over -
\newcommand{\BlockClmBRows}{24\xspace}  % pending.ClmB.rows: rows so far over rollout
\newcommand{\BlockClmBSAttempts}{25\xspace}  % clm.ClmBS.Attempts: Attempts over -
\newcommand{\BlockClmBSAuditGate}{passed\xspace}  % clm.ClmBS.AuditGate: AuditGate over -
\newcommand{\BlockClmBSAuditTerms}{4\xspace}  % clm.ClmBS.AuditTerms: AuditTerms over -
\newcommand{\BlockClmBSClmLzeroCap}{0\xspace}  % pending.ClmBS.CLM-L0.Cap: count over counted rollout
\newcommand{\BlockClmBSClmLzeroN}{1\xspace}  % pending.ClmBS.CLM-L0.n: count over counted rollout
\newcommand{\BlockClmBSClmLzeroPass}{1\xspace}  % pending.ClmBS.CLM-L0.pass: count over counted rollout
\newcommand{\BlockClmBSClmLzeroPassFrac}{1/1\xspace}  % pending.ClmBS.CLM-L0.frac: k/n over counted rollout
\newcommand{\BlockClmBSClmLzeroRevised}{0\xspace}  % pending.ClmBS.CLM-L0.Revised: count over counted rollout
\newcommand{\BlockClmBSClmLzeroStaleFlagged}{0\xspace}  % pending.ClmBS.CLM-L0.StaleFlagged: count over counted rollout
\newcommand{\BlockClmBSClmLzeroStaleUnflagged}{0\xspace}  % pending.ClmBS.CLM-L0.StaleUnflagged: count over counted rollout
\newcommand{\BlockClmBSClmOffACap}{0\xspace}  % pending.ClmBS.CLM-OFF-A.Cap: count over counted rollout
\newcommand{\BlockClmBSClmOffAN}{10\xspace}  % pending.ClmBS.CLM-OFF-A.n: count over counted rollout
\newcommand{\BlockClmBSClmOffAPass}{1\xspace}  % pending.ClmBS.CLM-OFF-A.pass: count over counted rollout
\newcommand{\BlockClmBSClmOffAPassFrac}{1/10\xspace}  % pending.ClmBS.CLM-OFF-A.frac: k/n over counted rollout
\newcommand{\BlockClmBSClmOffARevised}{0\xspace}  % pending.ClmBS.CLM-OFF-A.Revised: count over counted rollout
\newcommand{\BlockClmBSClmOffAStaleFlagged}{0\xspace}  % pending.ClmBS.CLM-OFF-A.StaleFlagged: count over counted rollout
\newcommand{\BlockClmBSClmOffAStaleUnflagged}{0\xspace}  % pending.ClmBS.CLM-OFF-A.StaleUnflagged: count over counted rollout
\newcommand{\BlockClmBSClmOnACap}{0\xspace}  % pending.ClmBS.CLM-ON-A.Cap: count over counted rollout
\newcommand{\BlockClmBSClmOnAN}{10\xspace}  % pending.ClmBS.CLM-ON-A.n: count over counted rollout
\newcommand{\BlockClmBSClmOnAPass}{9\xspace}  % pending.ClmBS.CLM-ON-A.pass: count over counted rollout
\newcommand{\BlockClmBSClmOnAPassFrac}{9/10\xspace}  % pending.ClmBS.CLM-ON-A.frac: k/n over counted rollout
\newcommand{\BlockClmBSClmOnARevised}{0\xspace}  % pending.ClmBS.CLM-ON-A.Revised: count over counted rollout
\newcommand{\BlockClmBSClmOnAStaleFlagged}{0\xspace}  % pending.ClmBS.CLM-ON-A.StaleFlagged: count over counted rollout
\newcommand{\BlockClmBSClmOnAStaleUnflagged}{0\xspace}  % pending.ClmBS.CLM-ON-A.StaleUnflagged: count over counted rollout
\newcommand{\BlockClmBSClmOnICap}{0\xspace}  % pending.ClmBS.CLM-ON-I.Cap: count over counted rollout
\newcommand{\BlockClmBSClmOnIN}{3\xspace}  % pending.ClmBS.CLM-ON-I.n: count over counted rollout
\newcommand{\BlockClmBSClmOnIPass}{3\xspace}  % pending.ClmBS.CLM-ON-I.pass: count over counted rollout
\newcommand{\BlockClmBSClmOnIPassFrac}{3/3\xspace}  % pending.ClmBS.CLM-ON-I.frac: k/n over counted rollout
\newcommand{\BlockClmBSClmOnIRevised}{0\xspace}  % pending.ClmBS.CLM-ON-I.Revised: count over counted rollout
\newcommand{\BlockClmBSClmOnIStaleFlagged}{0\xspace}  % pending.ClmBS.CLM-ON-I.StaleFlagged: count over counted rollout
\newcommand{\BlockClmBSClmOnIStaleUnflagged}{0\xspace}  % pending.ClmBS.CLM-ON-I.StaleUnflagged: count over counted rollout
\newcommand{\BlockClmBSConfig}{Claude CLI, frames by file read\xspace}  % r21.ClmBS.config: invoker and frame-delivery channel, from the spec over -
\newcommand{\BlockClmBSContradictions}{0\xspace}  % r21.ClmBS.Contradictions: Contradictions over counted rollout
\newcommand{\BlockClmBSControls}{4\xspace}  % r21.ClmBS.controls: unpaired control rollouts in the spec over rollout
\newcommand{\BlockClmBSControlsCredible}{credible\xspace}  % r21.ClmBS.ControlsCredible: ControlsCredible over -
\newcommand{\BlockClmBSCopyLimitControls}{not credible\xspace}  % clm.ClmBS.CopyLimitControls: CopyLimitControls over -
\newcommand{\BlockClmBSCopyLimitDerived}{not met\xspace}  % clm.ClmBS.CopyLimitDerived: CopyLimitDerived over -
\newcommand{\BlockClmBSCopyLimitHarm}{0\xspace}  % clm.ClmBS.CopyLimitHarm: CopyLimitHarm over -
\newcommand{\BlockClmBSCopyLimitOffFail}{10\xspace}  % clm.ClmBS.CopyLimitOffFail: CopyLimitOffFail over -
\newcommand{\BlockClmBSCopyLimitP}{0.0156\xspace}  % clm.ClmBS.CopyLimitP: CopyLimitP over -
\newcommand{\BlockClmBSCopyLimitReading}{R1\xspace}  % r21.ClmBS.CopyLimitReading: CopyLimitReading over -
\newcommand{\BlockClmBSCopyLimitRescue}{7\xspace}  % clm.ClmBS.CopyLimitRescue: CopyLimitRescue over -
\newcommand{\BlockClmBSCopyLimitTie}{3\xspace}  % clm.ClmBS.CopyLimitTie: CopyLimitTie over -
\newcommand{\BlockClmBSCopyLimitXupN}{3\xspace}  % clm.ClmBS.CopyLimitXupN: CopyLimitXupN over -
\newcommand{\BlockClmBSCopyLimitXupOn}{0\xspace}  % clm.ClmBS.CopyLimitXupOn: CopyLimitXupOn over -
\newcommand{\BlockClmBSCounted}{24\xspace}  % r21.ClmBS.counted: counted rollouts over rollout
\newcommand{\BlockClmBSCountedFail}{10\xspace}  % r21.ClmBS.CountedFail: counted failures over counted rollout
\newcommand{\BlockClmBSCountedSucc}{14\xspace}  % r21.ClmBS.CountedSucc: CountedSucc over counted rollout
\newcommand{\BlockClmBSDecideCheck}{registered decide() = mirror = stored reading\xspace}  % clm.ClmBS.DecideCheck: DecideCheck over -
\newcommand{\BlockClmBSDecisionTerm}{24\xspace}  % r21.ClmBS.DecisionTerm: DecisionTerm over counted rollout
\newcommand{\BlockClmBSDerivedGate}{met\xspace}  % r21.ClmBS.DerivedGate: DerivedGate over -
\newcommand{\BlockClmBSDisposition}{completed\xspace}  % r21.ClmBS.disposition: disposition text over -
\newcommand{\BlockClmBSEffect}{---\xspace}  % pending.ClmBS.effect: discordant-pair proportion (envos.stats.effect_size; NOT the net paired effect) over pair
\newcommand{\BlockClmBSEndpointFull}{24\xspace}  % r21.ClmBS.EndpointFull: EndpointFull over counted rollout
\newcommand{\BlockClmBSEndpointFullSucc}{14\xspace}  % r21.ClmBS.EndpointFullSucc: EndpointFullSucc over counted rollout
\newcommand{\BlockClmBSEndpointUnresolved}{0\xspace}  % r21.ClmBS.EndpointUnresolved: EndpointUnresolved over counted rollout
\newcommand{\BlockClmBSHolmSlot}{7\xspace}  % clm.ClmBS.HolmSlot: HolmSlot over -
\newcommand{\BlockClmBSInstancePhrase}{\BlockClmBSInstances frozen generated instances (seeds \BlockClmBSSeedList)\xspace}  % r21.ClmBS.instance_phrase: the block's instances as a phrase that reads correctly whether or not its spec exists over -
\newcommand{\BlockClmBSInstances}{10\xspace}  % r21.ClmBS.instances: paired instances over instance
\newcommand{\BlockClmBSInstancesWords}{ten\xspace}  % r21.ClmBS.instances_words: in words over instance
\newcommand{\BlockClmBSInterrupted}{1\xspace}  % clm.ClmBS.Interrupted: Interrupted over -
\newcommand{\BlockClmBSInterruptedWhere}{pair9 CLM-ON-A, attempt 0\xspace}  % clm.ClmBS.InterruptedWhere: InterruptedWhere over -
\newcommand{\BlockClmBSInterruptedWhy}{operationally interrupted before the archive was written\xspace}  % clm.ClmBS.InterruptedWhy: InterruptedWhy over -
\newcommand{\BlockClmBSModel}{Claude Sonnet~5\xspace}  % r21.ClmBS.model: evaluated model over -
\newcommand{\BlockClmBSNNeg}{---\xspace}  % pending.ClmBS.n_neg: count over pair
\newcommand{\BlockClmBSNPos}{---\xspace}  % pending.ClmBS.n_pos: count over pair
\newcommand{\BlockClmBSNTied}{---\xspace}  % pending.ClmBS.n_tied: count over pair
\newcommand{\BlockClmBSOffBack}{0\xspace}  % clm.ClmBS.OffBack: OffBack over -
\newcommand{\BlockClmBSOffFail}{9\xspace}  % r21.ClmBS.off_fail: CLM-OFF-A failures over instance
\newcommand{\BlockClmBSOffPass}{1\xspace}  % r21.ClmBS.off_pass: CLM-OFF-A successes over instance
\newcommand{\BlockClmBSOffReread}{1\xspace}  % clm.ClmBS.OffReread: OffReread over -
\newcommand{\BlockClmBSOffStale}{9\xspace}  % clm.ClmBS.OffStale: OffStale over -
\newcommand{\BlockClmBSOnBack}{10\xspace}  % clm.ClmBS.OnBack: OnBack over -
\newcommand{\BlockClmBSOnFailCorrect}{1\xspace}  % clm.ClmBS.OnFailCorrect: OnFailCorrect over -
\newcommand{\BlockClmBSOnFailTerms}{final-report\xspace}  % clm.ClmBS.OnFailTerms: OnFailTerms over -
\newcommand{\BlockClmBSOnOffBonfPaper}{0.0938\xspace}  % fam.alias.ClmBS.OnOff.b: alias over -
\newcommand{\BlockClmBSOnOffBothFail}{1\xspace}  % r21.ClmBS.OnOff.BothFail: both failed over pair
\newcommand{\BlockClmBSOnOffBothPass}{1\xspace}  % r21.ClmBS.OnOff.BothPass: both passed over pair
\newcommand{\BlockClmBSOnOffDir}{treatment\xspace}  % r21.ClmBS.OnOff.Dir: direction of the discordance over pair
\newcommand{\BlockClmBSOnOffHarm}{0\xspace}  % r21.ClmBS.OnOff.Harm: control passed, treatment failed over pair
\newcommand{\BlockClmBSOnOffHolmLocal}{---\xspace}  % r21.ClmBS.OnOff.HolmLocal: not in a block-local family over pair
\newcommand{\BlockClmBSOnOffHolmPaper}{0.0781\xspace}  % fam.alias.ClmBS.OnOff: alias over -
\newcommand{\BlockClmBSOnOffNet}{$+0.80$\xspace}  % r21.ClmBS.OnOff.Net: net paired difference over pair
\newcommand{\BlockClmBSOnOffNetCI}{$+0.80$ [$0.37$, $0.92$]\xspace}  % r21.ClmBS.OnOff.NetCI: net paired difference, Newcombe method-10 marginal 95% interval over pair
\newcommand{\BlockClmBSOnOffP}{0.00781\xspace}  % r21.ClmBS.OnOff.P: exact two-sided sign test over pair
\newcommand{\BlockClmBSOnOffPairs}{10\xspace}  % r21.ClmBS.OnOff.Pairs: complete pairs over pair
\newcommand{\BlockClmBSOnOffRescue}{8\xspace}  % r21.ClmBS.OnOff.Rescue: control failed, treatment passed over pair
\newcommand{\BlockClmBSOnOffTie}{2\xspace}  % r21.ClmBS.OnOff.Tie: both passed or both failed over pair
\newcommand{\BlockClmBSOnReread}{8\xspace}  % clm.ClmBS.OnReread: OnReread over -
\newcommand{\BlockClmBSP}{0.008\xspace}  % pending.ClmBS.p: exact two-sided sign test over pair
\newcommand{\BlockClmBSPairs}{10\xspace}  % pending.ClmBS.pairs: count over pair
\newcommand{\BlockClmBSPaperFamilyP}{0.00781\xspace}  % clm.ClmBS.PaperFamilyP: PaperFamilyP over -
\newcommand{\BlockClmBSReadingBody}{Over \BlockClmBSOnOffPairs sealed instance pairs (seeds \BlockClmBSSeedList), Claude Sonnet~5 met the full approval endpoint on \BlockClmBSClmOffAPassFrac without the panel and \BlockClmBSClmOnAPassFrac with it; of the pairs, \BlockClmBSOnOffRescue favoured the panel, \BlockClmBSOnOffHarm the arm without it, and \BlockClmBSOnOffTie neither; net \BlockClmBSOnOffNetCI (marginal 95\,\% interval), $p=\BlockClmBSOnOffP$. Controls: ON-I \BlockClmBSClmOnIPassFrac, L0 \BlockClmBSClmLzeroPassFrac. The review-step panel increased full-task success at the registered local level. The OFF-A failure categories and observed pre-commit revisions are reported separately (Appendix~\ref{app:claims}). The OFF-A--ON-A contrast rejects under its registered block-local analysis but not under the paper-wide Holm analysis (adjusted $p=\BlockClmBSOnOffHolmPaper$ over \HolmPaperM tests). The scripted copy-limit shortcut, run on the same cells before any model, is assigned \BlockClmBSCopyLimitReading under the same rules. Every outcome term the independent scorer re-derives is resolved and agreeing with the evaluator on \BlockClmBSEndpointFull of \BlockClmBSCounted counted rollouts. The standard-library validity re-derivation agrees with the archive on \BlockClmBSVindAgree attempts.\xspace}  % r21.ClmBS.body: main-text reading paragraph over -
\newcommand{\BlockClmBSReadingFull}{Over \BlockClmBSOnOffPairs sealed instance pairs (seeds \BlockClmBSSeedList), Claude Sonnet~5 met the full approval endpoint on \BlockClmBSClmOffAPassFrac without the panel and \BlockClmBSClmOnAPassFrac with it; of the pairs, \BlockClmBSOnOffRescue favoured the panel, \BlockClmBSOnOffHarm the arm without it, and \BlockClmBSOnOffTie neither; net \BlockClmBSOnOffNetCI (marginal 95\,\% interval), $p=\BlockClmBSOnOffP$. Controls: ON-I \BlockClmBSClmOnIPassFrac, L0 \BlockClmBSClmLzeroPassFrac. The review-step panel increased full-task success at the registered local level. The OFF-A failure categories and observed pre-commit revisions are reported separately (Appendix~\ref{app:claims}). The OFF-A--ON-A contrast rejects under its registered block-local analysis but not under the paper-wide Holm analysis (adjusted $p=\BlockClmBSOnOffHolmPaper$ over \HolmPaperM tests). The scripted copy-limit shortcut, run on the same cells before any model, is assigned \BlockClmBSCopyLimitReading under the same rules. Every outcome term the independent scorer re-derives is resolved and agreeing with the evaluator on \BlockClmBSEndpointFull of \BlockClmBSCounted counted rollouts. The standard-library validity re-derivation agrees with the archive on \BlockClmBSVindAgree attempts.\xspace}  % r21.ClmBS.full: appendix reading paragraph over -
\newcommand{\BlockClmBSReadingIDs}{R1\xspace}  % r21.ClmBS.reading_ids: registered reading ids selected by the mirrored rule over -
\newcommand{\BlockClmBSReadingMain}{Over \BlockClmBSOnOffPairs sealed instance pairs (seeds \BlockClmBSSeedList), Claude Sonnet~5 met the full approval endpoint on \BlockClmBSClmOffAPassFrac without the panel and \BlockClmBSClmOnAPassFrac with it; of the pairs, \BlockClmBSOnOffRescue favoured the panel, \BlockClmBSOnOffHarm the arm without it, and \BlockClmBSOnOffTie neither; net \BlockClmBSOnOffNetCI (marginal 95\,\% interval), $p=\BlockClmBSOnOffP$. Controls: ON-I \BlockClmBSClmOnIPassFrac, L0 \BlockClmBSClmLzeroPassFrac. The review-step panel increased full-task success at the registered local level. The OFF-A failure categories and observed pre-commit revisions are reported separately (Appendix~\ref{app:claims}). The pre-registered block-level paired test rejects; the later paper-wide family is reported only as a retrospective sensitivity analysis for the claims blocks (Appendix~\ref{app:multiplicity}). The pre-registered derived-decision gate passed on all three threshold-crossing cases. Every outcome term the independent scorer re-derives is resolved and agreeing with the evaluator on \BlockClmBSEndpointFull of \BlockClmBSCounted counted rollouts. The standard-library validity re-derivation agrees with the archive on \BlockClmBSVindAgree attempts.\xspace}  % r28.ClmBS.main: r28: main-text reading paragraph (GPT-6 r20 page 6) over -
\newcommand{\BlockClmBSReadingMainS}{Over \BlockClmBSOnOffPairs sealed instance pairs (seeds \BlockClmBSSeedList), Claude Sonnet~5 met the full approval endpoint on \BlockClmBSClmOffAPassFrac without the panel and \BlockClmBSClmOnAPassFrac with it; of the pairs, \BlockClmBSOnOffRescue favoured the panel, \BlockClmBSOnOffHarm the arm without it, and \BlockClmBSOnOffTie neither; net \BlockClmBSOnOffNetCI (marginal 95\,\% interval), $p=\BlockClmBSOnOffP$. Controls: ON-I \BlockClmBSClmOnIPassFrac, L0 \BlockClmBSClmLzeroPassFrac. The review-step panel increased full-task success at the registered local level. The OFF-A failure categories and observed pre-commit revisions are reported separately (Appendix~\ref{app:claims}). The OFF-A--ON-A contrast rejects under its registered block-local analysis but not under the paper-wide Holm analysis (adjusted $p=\BlockClmBSOnOffHolmPaper$ over \HolmPaperM tests). That family was finalized after the claims outcomes (Appendix~\ref{app:multiplicity}). The pre-registered derived-decision gate passed on all three threshold-crossing cases. Every outcome term the independent scorer re-derives is resolved and agreeing with the evaluator on \BlockClmBSEndpointFull of \BlockClmBSCounted counted rollouts. The standard-library validity re-derivation agrees with the archive on \BlockClmBSVindAgree attempts.\xspace}  % r37f.clmbs_main: r37 final reviews: CLM-BS's main-text reading over -
\newcommand{\BlockClmBSReadingShort}{the panel increased full-task success at the registered local level; OFF-A--ON-A not significant under the paper-wide Holm analysis\xspace}  % r21.ClmBS.short: short reading over -
\newcommand{\BlockClmBSRegistered}{PRECOMMIT\_\allowbreak{}CLAIMS ADDENDUM~1\xspace}  % r21.ClmBS.registered: where the block is registered, and whether that registration is frozen (heading present and .sha256 verifying) over -
\newcommand{\BlockClmBSReplaced}{1\xspace}  % r21.ClmBS.replaced: attempts not counted over rollout
\newcommand{\BlockClmBSReplacements}{0\xspace}  % r21.ClmBS.Replacements: Replacements over -
\newcommand{\BlockClmBSReplacementsSpent}{0\xspace}  % clm.ClmBS.ReplacementsSpent: ReplacementsSpent over -
\newcommand{\BlockClmBSRfourWhy}{--\xspace}  % r21.ClmBS.r4why: why R4 over -
\newcommand{\BlockClmBSRows}{25\xspace}  % pending.ClmBS.rows: rows so far over rollout
\newcommand{\BlockClmBSSeedList}{0--9\xspace}  % r21.ClmBS.seeds: exact seed list of the block's paired instances over seed
\newcommand{\BlockClmBSShortForm}{Claude Sonnet~5 on CLM-B's frozen slots (Block~CLM-BS): OFF-A \BlockClmBSClmOffAPassFrac, ON-A \BlockClmBSClmOnAPassFrac, $p=\BlockClmBSOnOffP$; \BlockClmBSReadingShort. The two models share instances, so their difference is descriptive.\xspace}  % r21.ClmBS.shortform: main-text short form over -
\newcommand{\BlockClmBSStaleRescues}{8\xspace}  % clm.ClmBS.StaleRescues: StaleRescues over -
\newcommand{\BlockClmBSState}{complete\xspace}  % r21.ClmBS.state: execution disposition (r21_state) over -
\newcommand{\BlockClmBSStateCell}{complete\xspace}  % r28.ClmBS.cell: r28: the block's state for Table 1 over -
\newcommand{\BlockClmBSStatus}{\texttt{complete}\xspace}  % pending.ClmBS.status: search-log status over -
\newcommand{\BlockClmBSStepCap}{0\xspace}  % clm.ClmBS.StepCap: StepCap over -
\newcommand{\BlockClmBSStoredCIDiffers}{True\xspace}  % clm.ClmBS.StoredCIDiffers: StoredCIDiffers over -
\newcommand{\BlockClmBSStoredNetCI}{$+0.80$ [$0.39$, $0.91$]\xspace}  % clm.ClmBS.StoredNetCI: StoredNetCI over -
\newcommand{\BlockClmBSUncounted}{1\xspace}  % clm.ClmBS.Uncounted: Uncounted over -
\newcommand{\BlockClmBSVerdictFail}{10\xspace}  % r21.ClmBS.VerdictFail: VerdictFail over counted rollout
\newcommand{\BlockClmBSVerdictSucc}{14\xspace}  % r21.ClmBS.VerdictSucc: VerdictSucc over counted rollout
\newcommand{\BlockClmBSVindAgree}{25 of 25\xspace}  % r21.ClmBS.vind: independent validity re-derivation, agreeing / all attempts over attempt
\newcommand{\BlockClmBSVindAgreeSlash}{25/25\xspace}  % r21.ClmBS.vind_slash: the same, as a/b over attempt
\newcommand{\BlockClmBSVindCountedValid}{24 of 24\xspace}  % clm.ClmBS.VindCountedValid: VindCountedValid over -
\newcommand{\BlockClmBSVindPath}{\code{audit/\allowbreak{}failure\_\allowbreak{}mining/\allowbreak{}CLAIMS/\allowbreak{}VALIDITY\_\allowbreak{}INDEPENDENT\_\allowbreak{}blockCLMBS.json}\xspace}  % r21.ClmBS.vind_path: the expected independent validity re-derivation artifact over -
\newcommand{\BlockClmBSVindStatus}{re-derived\xspace}  % r21.ClmBS.vind_status: whether audit/failure_mining/CLAIMS/VALIDITY_INDEPENDENT_blockCLMBS.json exists over -
\newcommand{\BlockClmBSVoided}{1\xspace}  % pending.ClmBS.voided: count over rollout
\newcommand{\BlockClmBSXupN}{3\xspace}  % r21.ClmBS.XupN: XupN over -
\newcommand{\BlockClmBSXupOn}{3\xspace}  % r21.ClmBS.XupOn: XupOn over -
\newcommand{\BlockClmBSeedList}{0--9\xspace}  % r21.ClmB.seeds: exact seed list of the block's paired instances over seed
\newcommand{\BlockClmBShortForm}{Claude Opus~5 on CLM-B's frozen slots (Block~CLM-B): OFF-A \BlockClmBClmOffAPassFrac, ON-A \BlockClmBClmOnAPassFrac, $p=\BlockClmBOnOffP$; \BlockClmBReadingShort. The two models share instances, so their difference is descriptive.\xspace}  % r21.ClmB.shortform: main-text short form over -
\newcommand{\BlockClmBStaleRescues}{0\xspace}  % clm.ClmB.StaleRescues: StaleRescues over -
\newcommand{\BlockClmBState}{complete\xspace}  % r21.ClmB.state: execution disposition (r21_state) over -
\newcommand{\BlockClmBStateCell}{complete\xspace}  % r28.ClmB.cell: r28: the block's state for Table 1 over -
\newcommand{\BlockClmBStatus}{\texttt{complete}\xspace}  % pending.ClmB.status: search-log status over -
\newcommand{\BlockClmBStepCap}{0\xspace}  % clm.ClmB.StepCap: StepCap over -
\newcommand{\BlockClmBStoredCIDiffers}{False\xspace}  % clm.ClmB.StoredCIDiffers: StoredCIDiffers over -
\newcommand{\BlockClmBStoredNetCI}{$0.00$ [$-0.28$, $0.28$]\xspace}  % clm.ClmB.StoredNetCI: StoredNetCI over -
\newcommand{\BlockClmBUncounted}{0\xspace}  % clm.ClmB.Uncounted: Uncounted over -
\newcommand{\BlockClmBVerdictFail}{0\xspace}  % r21.ClmB.VerdictFail: VerdictFail over counted rollout
\newcommand{\BlockClmBVerdictSucc}{24\xspace}  % r21.ClmB.VerdictSucc: VerdictSucc over counted rollout
\newcommand{\BlockClmBVindAgree}{24 of 24\xspace}  % r21.ClmB.vind: independent validity re-derivation, agreeing / all attempts over attempt
\newcommand{\BlockClmBVindAgreeSlash}{24/24\xspace}  % r21.ClmB.vind_slash: the same, as a/b over attempt
\newcommand{\BlockClmBVindCountedValid}{24 of 24\xspace}  % clm.ClmB.VindCountedValid: VindCountedValid over -
\newcommand{\BlockClmBVindPath}{\code{audit/\allowbreak{}failure\_\allowbreak{}mining/\allowbreak{}CLAIMS/\allowbreak{}VALIDITY\_\allowbreak{}INDEPENDENT\_\allowbreak{}blockCLMB.json}\xspace}  % r21.ClmB.vind_path: the expected independent validity re-derivation artifact over -
\newcommand{\BlockClmBVindStatus}{re-derived\xspace}  % r21.ClmB.vind_status: whether audit/failure_mining/CLAIMS/VALIDITY_INDEPENDENT_blockCLMB.json exists over -
\newcommand{\BlockClmBVoided}{0\xspace}  % pending.ClmB.voided: count over rollout
\newcommand{\BlockClmBXupN}{3\xspace}  % r21.ClmB.XupN: XupN over -
\newcommand{\BlockClmBXupOn}{3\xspace}  % r21.ClmB.XupOn: XupOn over -
\newcommand{\BlockPoneMACCCap}{0\xspace}  % pending.PoneM.AC-C.Cap: count over counted rollout
\newcommand{\BlockPoneMACCN}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-C.n: count over counted rollout
\newcommand{\BlockPoneMACCPass}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-C.pass: count over counted rollout
\newcommand{\BlockPoneMACCPassFrac}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-C.frac: k/n over counted rollout
\newcommand{\BlockPoneMACCRevised}{0\xspace}  % pending.PoneM.AC-C.Revised: count over counted rollout
\newcommand{\BlockPoneMACCStaleFlagged}{0\xspace}  % pending.PoneM.AC-C.StaleFlagged: count over counted rollout
\newcommand{\BlockPoneMACCStaleUnflagged}{0\xspace}  % pending.PoneM.AC-C.StaleUnflagged: count over counted rollout
\newcommand{\BlockPoneMACLfourCap}{0\xspace}  % pending.PoneM.AC-L4.Cap: count over counted rollout
\newcommand{\BlockPoneMACLfourN}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-L4.n: count over counted rollout
\newcommand{\BlockPoneMACLfourPass}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-L4.pass: count over counted rollout
\newcommand{\BlockPoneMACLfourPassFrac}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-L4.frac: k/n over counted rollout
\newcommand{\BlockPoneMACLfourRevised}{0\xspace}  % pending.PoneM.AC-L4.Revised: count over counted rollout
\newcommand{\BlockPoneMACLfourStaleFlagged}{0\xspace}  % pending.PoneM.AC-L4.StaleFlagged: count over counted rollout
\newcommand{\BlockPoneMACLfourStaleUnflagged}{0\xspace}  % pending.PoneM.AC-L4.StaleUnflagged: count over counted rollout
\newcommand{\BlockPoneMACLthreeCap}{0\xspace}  % pending.PoneM.AC-L3.Cap: count over counted rollout
\newcommand{\BlockPoneMACLthreeN}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-L3.n: count over counted rollout
\newcommand{\BlockPoneMACLthreePass}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-L3.pass: count over counted rollout
\newcommand{\BlockPoneMACLthreePassFrac}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-L3.frac: k/n over counted rollout
\newcommand{\BlockPoneMACLthreePlusCap}{0\xspace}  % pending.PoneM.AC-L3+.Cap: count over counted rollout
\newcommand{\BlockPoneMACLthreePlusN}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-L3+.n: count over counted rollout
\newcommand{\BlockPoneMACLthreePlusPass}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-L3+.pass: count over counted rollout
\newcommand{\BlockPoneMACLthreePlusPassFrac}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-L3+.frac: k/n over counted rollout
\newcommand{\BlockPoneMACLthreePlusRevised}{0\xspace}  % pending.PoneM.AC-L3+.Revised: count over counted rollout
\newcommand{\BlockPoneMACLthreePlusStaleFlagged}{0\xspace}  % pending.PoneM.AC-L3+.StaleFlagged: count over counted rollout
\newcommand{\BlockPoneMACLthreePlusStaleUnflagged}{0\xspace}  % pending.PoneM.AC-L3+.StaleUnflagged: count over counted rollout
\newcommand{\BlockPoneMACLthreeRevised}{0\xspace}  % pending.PoneM.AC-L3.Revised: count over counted rollout
\newcommand{\BlockPoneMACLthreeStaleFlagged}{0\xspace}  % pending.PoneM.AC-L3.StaleFlagged: count over counted rollout
\newcommand{\BlockPoneMACLthreeStaleUnflagged}{0\xspace}  % pending.PoneM.AC-L3.StaleUnflagged: count over counted rollout
\newcommand{\BlockPoneMACLtwoCap}{0\xspace}  % pending.PoneM.AC-L2.Cap: count over counted rollout
\newcommand{\BlockPoneMACLtwoN}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-L2.n: count over counted rollout
\newcommand{\BlockPoneMACLtwoPass}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-L2.pass: count over counted rollout
\newcommand{\BlockPoneMACLtwoPassFrac}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-L2.frac: k/n over counted rollout
\newcommand{\BlockPoneMACLtwoRevised}{0\xspace}  % pending.PoneM.AC-L2.Revised: count over counted rollout
\newcommand{\BlockPoneMACLtwoStaleFlagged}{0\xspace}  % pending.PoneM.AC-L2.StaleFlagged: count over counted rollout
\newcommand{\BlockPoneMACLtwoStaleUnflagged}{0\xspace}  % pending.PoneM.AC-L2.StaleUnflagged: count over counted rollout
\newcommand{\BlockPoneMACLzeroCap}{0\xspace}  % pending.PoneM.AC-L0.Cap: count over counted rollout
\newcommand{\BlockPoneMACLzeroN}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-L0.n: count over counted rollout
\newcommand{\BlockPoneMACLzeroPass}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-L0.pass: count over counted rollout
\newcommand{\BlockPoneMACLzeroPassFrac}{\textit{unevaluable}\xspace}  % pending.PoneM.AC-L0.frac: k/n over counted rollout
\newcommand{\BlockPoneMACLzeroRevised}{0\xspace}  % pending.PoneM.AC-L0.Revised: count over counted rollout
\newcommand{\BlockPoneMACLzeroStaleFlagged}{0\xspace}  % pending.PoneM.AC-L0.StaleFlagged: count over counted rollout
\newcommand{\BlockPoneMACLzeroStaleUnflagged}{0\xspace}  % pending.PoneM.AC-L0.StaleUnflagged: count over counted rollout
\newcommand{\BlockPoneMRows}{4\xspace}  % pending.PoneM.rows: rows so far over rollout
\newcommand{\BlockPoneMSACCN}{\textit{never started}\xspace}  % pending.PoneMS.AC-C.n: count over counted rollout
\newcommand{\BlockPoneMSACCPass}{\textit{never started}\xspace}  % pending.PoneMS.AC-C.pass: count over counted rollout
\newcommand{\BlockPoneMSACCPassFrac}{\textit{never started}\xspace}  % pending.PoneMS.AC-C.frac: k/n over counted rollout
\newcommand{\BlockPoneMSACLfourN}{\textit{never started}\xspace}  % pending.PoneMS.AC-L4.n: count over counted rollout
\newcommand{\BlockPoneMSACLfourPass}{\textit{never started}\xspace}  % pending.PoneMS.AC-L4.pass: count over counted rollout
\newcommand{\BlockPoneMSACLfourPassFrac}{\textit{never started}\xspace}  % pending.PoneMS.AC-L4.frac: k/n over counted rollout
\newcommand{\BlockPoneMSACLthreeN}{\textit{never started}\xspace}  % pending.PoneMS.AC-L3.n: count over counted rollout
\newcommand{\BlockPoneMSACLthreePass}{\textit{never started}\xspace}  % pending.PoneMS.AC-L3.pass: count over counted rollout
\newcommand{\BlockPoneMSACLthreePassFrac}{\textit{never started}\xspace}  % pending.PoneMS.AC-L3.frac: k/n over counted rollout
\newcommand{\BlockPoneMSACLthreePlusN}{\textit{never started}\xspace}  % pending.PoneMS.AC-L3+.n: count over counted rollout
\newcommand{\BlockPoneMSACLthreePlusPass}{\textit{never started}\xspace}  % pending.PoneMS.AC-L3+.pass: count over counted rollout
\newcommand{\BlockPoneMSACLthreePlusPassFrac}{\textit{never started}\xspace}  % pending.PoneMS.AC-L3+.frac: k/n over counted rollout
\newcommand{\BlockPoneMSACLtwoN}{\textit{never started}\xspace}  % pending.PoneMS.AC-L2.n: count over counted rollout
\newcommand{\BlockPoneMSACLtwoPass}{\textit{never started}\xspace}  % pending.PoneMS.AC-L2.pass: count over counted rollout
\newcommand{\BlockPoneMSACLtwoPassFrac}{\textit{never started}\xspace}  % pending.PoneMS.AC-L2.frac: k/n over counted rollout
\newcommand{\BlockPoneMSACLzeroN}{\textit{never started}\xspace}  % pending.PoneMS.AC-L0.n: count over counted rollout
\newcommand{\BlockPoneMSACLzeroPass}{\textit{never started}\xspace}  % pending.PoneMS.AC-L0.pass: count over counted rollout
\newcommand{\BlockPoneMSACLzeroPassFrac}{\textit{never started}\xspace}  % pending.PoneMS.AC-L0.frac: k/n over counted rollout
\newcommand{\BlockPoneMSRows}{\textit{never started}\xspace}  % pending.PoneMS.rows: rows so far over rollout
\newcommand{\BlockPoneMSStatus}{\textit{never started}\xspace}  % pending.PoneMS.status: search-log status over -
\newcommand{\BlockPoneMStatus}{\texttt{paused\_infra}\xspace}  % pending.PoneM.status: search-log status over -
\newcommand{\BlockPoneMVoided}{3\xspace}  % pending.PoneM.voided: count over rollout
\newcommand{\BlockPtwoSPtwoCN}{\textit{failed admission}\xspace}  % pending.PtwoS.P2-C.n: count over counted rollout
\newcommand{\BlockPtwoSPtwoCPass}{\textit{failed admission}\xspace}  % pending.PtwoS.P2-C.pass: count over counted rollout
\newcommand{\BlockPtwoSPtwoCPassFrac}{\textit{failed admission}\xspace}  % pending.PtwoS.P2-C.frac: k/n over counted rollout
\newcommand{\BlockPtwoSPtwoLoneN}{\textit{failed admission}\xspace}  % pending.PtwoS.P2-L1.n: count over counted rollout
\newcommand{\BlockPtwoSPtwoLonePass}{\textit{failed admission}\xspace}  % pending.PtwoS.P2-L1.pass: count over counted rollout
\newcommand{\BlockPtwoSPtwoLonePassFrac}{\textit{failed admission}\xspace}  % pending.PtwoS.P2-L1.frac: k/n over counted rollout
\newcommand{\BlockPtwoSPtwoLzeroN}{\textit{failed admission}\xspace}  % pending.PtwoS.P2-L0.n: count over counted rollout
\newcommand{\BlockPtwoSPtwoLzeroPass}{\textit{failed admission}\xspace}  % pending.PtwoS.P2-L0.pass: count over counted rollout
\newcommand{\BlockPtwoSPtwoLzeroPassFrac}{\textit{failed admission}\xspace}  % pending.PtwoS.P2-L0.frac: k/n over counted rollout
\newcommand{\BlockPtwoSRows}{\textit{failed admission}\xspace}  % pending.PtwoS.rows: rows so far over rollout
\newcommand{\BlockPtwoSSPtwoCN}{\textit{failed admission}\xspace}  % pending.PtwoSS.P2-C.n: count over counted rollout
\newcommand{\BlockPtwoSSPtwoCPass}{\textit{failed admission}\xspace}  % pending.PtwoSS.P2-C.pass: count over counted rollout
\newcommand{\BlockPtwoSSPtwoCPassFrac}{\textit{failed admission}\xspace}  % pending.PtwoSS.P2-C.frac: k/n over counted rollout
\newcommand{\BlockPtwoSSPtwoLoneN}{\textit{failed admission}\xspace}  % pending.PtwoSS.P2-L1.n: count over counted rollout
\newcommand{\BlockPtwoSSPtwoLonePass}{\textit{failed admission}\xspace}  % pending.PtwoSS.P2-L1.pass: count over counted rollout
\newcommand{\BlockPtwoSSPtwoLonePassFrac}{\textit{failed admission}\xspace}  % pending.PtwoSS.P2-L1.frac: k/n over counted rollout
\newcommand{\BlockPtwoSSPtwoLzeroN}{\textit{failed admission}\xspace}  % pending.PtwoSS.P2-L0.n: count over counted rollout
\newcommand{\BlockPtwoSSPtwoLzeroPass}{\textit{failed admission}\xspace}  % pending.PtwoSS.P2-L0.pass: count over counted rollout
\newcommand{\BlockPtwoSSPtwoLzeroPassFrac}{\textit{failed admission}\xspace}  % pending.PtwoSS.P2-L0.frac: k/n over counted rollout
\newcommand{\BlockPtwoSSRows}{\textit{failed admission}\xspace}  % pending.PtwoSS.rows: rows so far over rollout
\newcommand{\BlockPtwoSSStatus}{\textit{failed admission}\xspace}  % pending.PtwoSS.status: search-log status over -
\newcommand{\BlockPtwoSStatus}{\textit{failed admission}\xspace}  % pending.PtwoS.status: search-log status over -
\newcommand{\BonfPaperAtwo}{1.00\xspace}  % fam.Atwo.bonf: min(1, m p) over -
\newcommand{\BonfPaperB}{0.0234\xspace}  % fam.B.bonf: min(1, m p) over -
\newcommand{\BonfPaperBCCueOff}{1.00\xspace}  % fam.BCCueOff.bonf: min(1, m p) over -
\newcommand{\BonfPaperBCLiveCue}{0.00293\xspace}  % fam.BCLiveCue.bonf: min(1, m p) over -
\newcommand{\BonfPaperBCSCueOff}{\textit{not admissible}\xspace}  % fam.BCSCueOff.bonf: min(1, m p) over -
\newcommand{\BonfPaperBCSLiveCue}{\textit{not admissible}\xspace}  % fam.BCSLiveCue.bonf: min(1, m p) over -
\newcommand{\BonfPaperBGCCueOff}{\textit{not admissible}\xspace}  % fam.BGCCueOff.bonf: min(1, m p) over -
\newcommand{\BonfPaperBGCOffiOffa}{\textit{not admissible}\xspace}  % fam.BGCOffiOffa.bonf: min(1, m p) over -
\newcommand{\BonfPaperBS}{0.375\xspace}  % fam.BS.bonf: min(1, m p) over -
\newcommand{\BonfPaperClmB}{1.00\xspace}  % fam.ClmB.bonf: min(1, m p) over -
\newcommand{\BonfPaperClmBS}{0.0938\xspace}  % fam.ClmBS.bonf: min(1, m p) over -
\newcommand{\BonfPaperSlotTen}{\textit{not admissible}\xspace}  % fam.SlotTen.bonf: min(1, m p) over -
\newcommand{\CarrySentence}{The prospective claims and BC blocks, not Block~B, carry the paper's model-effect conclusions.\xspace}  % r27.carry: r27: which blocks carry the conclusions, from block status over -
\newcommand{\CensusFrameUnread}{80\xspace}  % r29.cs.unread: r29 lane C interface census (post hoc) over tool call
\newcommand{\CensusNonReadOpus}{21\xspace}  % r29.cs.nr_opus: r29 lane C interface census (post hoc) over tool call
\newcommand{\CensusNonReadSonnet}{338\xspace}  % r29.cs.nr_sonnet: r29 lane C interface census (post hoc) over tool call
\newcommand{\CensusReadChars}{300\xspace}  % r29.cs.read_chars: Read result text archived per call over character
\newcommand{\CensusReadViolations}{0\xspace}  % r29.cs.viol: r29 lane C interface census (post hoc) over step
\newcommand{\CensusSteps}{654\xspace}  % r29.cs.steps: r29 lane C interface census (post hoc) over step
\newcommand{\CertAtwoChecksMax}{50\xspace}  % cert.a2.max: max checks over certificate
\newcommand{\CertAtwoChecksMin}{32\xspace}  % cert.a2.min: min checks over certificate
\newcommand{\CertChecksMax}{50\xspace}  % cert.max: max checks over certificate
\newcommand{\CertChecksMin}{32\xspace}  % cert.min: min checks over certificate
\newcommand{\CertChecksTotal}{277\xspace}  % cert.total: sum over the seven certificates over check
\newcommand{\CertDistinctChecks}{65\xspace}  % cert.distinct: distinct over check name
\newcommand{\CertFRXOffAChecks}{40\xspace}  % cert.FRX-OFF-A.checks: count over check
\newcommand{\CertFRXOffAFailed}{0\xspace}  % cert.FRX-OFF-A.failed: count over check
\newcommand{\CertFRXOffAIssued}{2026-09-18\xspace}  % cert.FRX-OFF-A.issued: issue date over -
\newcommand{\CertFRXOffAMonitorErrors}{0\xspace}  % cert.FRX-OFF-A.monitor: count over check
\newcommand{\CertFRXOffIChecks}{37\xspace}  % cert.FRX-OFF-I.checks: count over check
\newcommand{\CertFRXOffIFailed}{0\xspace}  % cert.FRX-OFF-I.failed: count over check
\newcommand{\CertFRXOffIIssued}{2026-09-18\xspace}  % cert.FRX-OFF-I.issued: issue date over -
\newcommand{\CertFRXOffIMonitorErrors}{0\xspace}  % cert.FRX-OFF-I.monitor: count over check
\newcommand{\CertFRXOnAChecks}{41\xspace}  % cert.FRX-ON-A.checks: count over check
\newcommand{\CertFRXOnAFailed}{0\xspace}  % cert.FRX-ON-A.failed: count over check
\newcommand{\CertFRXOnAIssued}{2026-09-18\xspace}  % cert.FRX-ON-A.issued: issue date over -
\newcommand{\CertFRXOnAMonitorErrors}{0\xspace}  % cert.FRX-ON-A.monitor: count over check
\newcommand{\CertFRXOnIChecks}{37\xspace}  % cert.FRX-ON-I.checks: count over check
\newcommand{\CertFRXOnIFailed}{0\xspace}  % cert.FRX-ON-I.failed: count over check
\newcommand{\CertFRXOnIIssued}{2026-09-18\xspace}  % cert.FRX-ON-I.issued: issue date over -
\newcommand{\CertFRXOnIMonitorErrors}{0\xspace}  % cert.FRX-ON-I.monitor: count over check
\newcommand{\CertGovAtwoMax}{48\xspace}  % cert.gov.a2.max: max checks, certificates that governed Block A2 over certificate
\newcommand{\CertGovAtwoMin}{30\xspace}  % cert.gov.a2.min: min checks, certificates that governed Block A2 over certificate
\newcommand{\CertGovChecksMax}{50\xspace}  % cert.gov.max: max checks over governing certificates over certificate
\newcommand{\CertGovChecksMin}{30\xspace}  % cert.gov.min: min checks over governing certificates over certificate
\newcommand{\CertGovN}{9\xspace}  % cert.gov.n: certificates that governed a model block over certificate
\newcommand{\CertGovUnrecorded}{3\xspace}  % cert.gov.unrecorded: governing certificates whose sha256 prefix no addendum records over certificate
\newcommand{\CertN}{7\xspace}  % cert.n: count over certificate
\newcommand{\CertSCChecks}{40\xspace}  % cert.S-C.checks: count over check
\newcommand{\CertSCFailed}{0\xspace}  % cert.S-C.failed: count over check
\newcommand{\CertSCIssued}{2026-09-22\xspace}  % cert.S-C.issued: issue date over -
\newcommand{\CertSCMonitorErrors}{0\xspace}  % cert.S-C.monitor: count over check
\newcommand{\CertSLtwoChecks}{50\xspace}  % cert.S-L2.checks: count over check
\newcommand{\CertSLtwoFailed}{0\xspace}  % cert.S-L2.failed: count over check
\newcommand{\CertSLtwoIssued}{2026-09-22\xspace}  % cert.S-L2.issued: issue date over -
\newcommand{\CertSLtwoMonitorErrors}{0\xspace}  % cert.S-L2.monitor: count over check
\newcommand{\CertSLzeroChecks}{32\xspace}  % cert.S-L0.checks: count over check
\newcommand{\CertSLzeroFailed}{0\xspace}  % cert.S-L0.failed: count over check
\newcommand{\CertSLzeroIssued}{2026-09-22\xspace}  % cert.S-L0.issued: issue date over -
\newcommand{\CertSLzeroMonitorErrors}{0\xspace}  % cert.S-L0.monitor: count over check
\newcommand{\CertVersionsN}{10\xspace}  % cert.versions.n: certificate files listed (governing or not) over certificate
\newcommand{\ChallengeAppendixText}{Built by a different model (GPT-6, through the Codex CLI) from real Block~A2, B and BS episodes, with its expectations written per tool before its harness: \ChallengeN{} cases, \ChallengeValid{} valid controls and \ChallengeCorrupt{} corruptions, one per defect class. It is unseen only by the Claude agents that wrote and ran the pipeline, not by its builder: our brief named the defect classes, and the builder could read the whole repository (the code under test, the protocol and the paper), so its cases are white-box to it. Its seal record (\ChallengeSealSha) and the \ChallengeSealFiles{} file digests it holds are those ADDENDUM~19 \S7 froze before any Claude agent read the challenge (\S7 discloses that a Claude agent's repository-wide search printed lines of its comparison and expectation-writing scripts, never its expectations); the build re-verifies them, and every one of the \ChallengeFirstRunFiles{} outputs against the hash list written at the run before anyone read them (\ChallengeFirstRunSha). This is its first and only run, and its first output is the result: no case-specific patch was made (the \ChallengeToolSources{} tool source files its run manifest pins are byte-identical now, so no patch followed), no expectation was edited, and the misses are reported, not repaired. Three tools ran on every case, and no invocation ended in a tool error or was skipped. The sealed sentence at the head of this paragraph gives the registered pipeline's numbers, the outcome scorer's and the validity re-derivation's jointly; Section~\ref{sec:caught} reports each layer, and Table~\ref{tab:challenge} gives each tool per case class. The \ChallengeMissed{} misses, as its comparison output words them: (1)~\texttt{C01\_\allowbreak{}success\_\allowbreak{}without\_\allowbreak{}delivery} (success-before-validity: notice), the validity re-derivation: ``validity: valid (expected observation\_\allowbreak{}not\_\allowbreak{}delivered)''; (2)~\texttt{C02\_\allowbreak{}panel\_\allowbreak{}without\_\allowbreak{}delivery} (missing intervention panel delivery), the validity re-derivation: ``validity: valid (expected observation\_\allowbreak{}not\_\allowbreak{}delivered)''; (3)~\texttt{C08\_\allowbreak{}commit\_\allowbreak{}before\_\allowbreak{}change} (commit before change), the validity re-derivation: ``validity: valid (expected invalid\_\allowbreak{}intervention); registered\_\allowbreak{}validity: valid (expected invalid\_\allowbreak{}intervention)''; (4)~\texttt{C15\_\allowbreak{}truncated\_\allowbreak{}trajectory} (truncated trajectory), the validity re-derivation: ``registered\_\allowbreak{}validity: valid (expected delivery\_\allowbreak{}ambiguous/\allowbreak{}verifier\_\allowbreak{}failure/\allowbreak{}infra\_\allowbreak{}failure)''. Under the rules as implemented the validity re-derivation missed three (C01, C02, C08), under the rules as registered two (C08, C15); one (C08) under both. The evaluator's archived verdict path met \ChallengeEvalMet{} of its frozen expectations and missed \ChallengeEvalMissed{} (it met \ChallengeEvalValidMet{} of the \ChallengeValid{} valid controls and \ChallengeEvalCorruptMet{} of the \ChallengeCorrupt{} corruptions); these misses stand as failed expectations. Architecturally, its archive-replay entry point re-derives the delivery checkpoints from the raw logs and re-runs the classifier, but keeps the archived run-validity and invariant claims, which the corruptions leave in place; its verdict equalled the archived one on every case; this is why the outcome scorer and the validity re-derivation are separate layers. The challenge bounds defect detection on one family; it does not establish universal correctness, and it selects no cell and gates no block.\xspace}  % chal.appendix: the challenge, in the appendix over -
\newcommand{\ChallengeClause}{A second, sealed archive challenge built by a different model met \ChallengeMet of \ChallengeN frozen expectations on its first and only run (\ChallengeCorruptRejected of \ChallengeCorruptInstantiated instantiated corruptions rejected; \ChallengeValidAccepted of \ChallengeValidInstantiated valid cases accepted); its \ChallengeMissed misses are listed in Appendix~\ref{app:certificates} as its comparison output words them.\xspace}  % chal.clause: challenge sentence over -
\newcommand{\ChallengeCorrupt}{18\xspace}  % chal.corrupt: corruptions over case
\newcommand{\ChallengeCorruptClasses}{18\xspace}  % chal.classes: corruption classes over class
\newcommand{\ChallengeCorruptInstantiated}{18\xspace}  % chal.corrupt_instantiated: corruption cases on which neither registered tool errored over case
\newcommand{\ChallengeCorruptRejected}{14\xspace}  % chal.corrupt_rejected: instantiated corruptions both registered tools met (rejected as expected) over case
\newcommand{\ChallengeEvalCorruptMet}{0\xspace}  % chal.evaluator.corrupt_met: evaluator: corruptions met over case
\newcommand{\ChallengeEvalMet}{10\xspace}  % chal.evaluator.met: evaluator: cases met over case
\newcommand{\ChallengeEvalMissed}{18\xspace}  % chal.r27.eval_missed: evaluator: cases not met over case
\newcommand{\ChallengeEvalValidMet}{10\xspace}  % chal.evaluator.valid_met: evaluator: valid met over case
\newcommand{\ChallengeFirstRunFiles}{337\xspace}  % chal.first_run_files: first-run outputs the hash list names, all verified over file
\newcommand{\ChallengeFirstRunSha}{\texttt{9d0c898bc8bb}\xspace}  % chal.first_run_sha: sha256 prefix of the first-run hash list over -
\newcommand{\ChallengeGptParagraph}{To test the auditing machinery without tuning to the observed model blocks, we ran once a \ChallengeN-case archive challenge constructed independently, with expectations sealed by digest before the run and the first-run outputs locked. The independent outcome scorer met all \ChallengeN{} frozen expectations. The standard-library validity re-derivation met \ChallengeVindMet{} of \ChallengeN: it failed to reject two cases with missing observation delivery, one commit-before-change case, and one truncated-trajectory case. The evaluator's archived verdict path met \ChallengeEvalMet{} of \ChallengeN{} expectations. We do not repair, rerun, or reinterpret these misses for this challenge. The result therefore does not establish verifier soundness; it bounds what each auditing layer currently detects. In particular, it provides strong evidence for the independent outcome scorer on this suite, exposes four concrete blind spots in the independent validity reconstruction, and shows that the evaluator's own archived verdicts are not a substitute for re-derivation from raw evidence.\xspace}  % chal.r27.para: r27 challenge text (scorer 28/28, validity 24/28, evaluator 10/28) over -
\newcommand{\ChallengeLedgerClause}{These are the registered pipeline's numbers, the outcome scorer's and the validity re-derivation's jointly (a case is met only if both meet it); by tool, the outcome scorer met \ChallengeScorerMet, the validity re-derivation \ChallengeVindMet{} and the evaluator's archive replay \ChallengeEvalMet{} of the \ChallengeN{} (Table~\ref{tab:challenge}), and the misses are reported, not repaired.\xspace}  % chal.ledger: the challenge by tool, beside the sealed sentence over -
\newcommand{\ChallengeLimitClause}{the second challenge (unseen by the pipeline's Claude authors, white-box to its builder) ran once on \ChallengeN{} constructed cases of one family, with its misses reported rather than repaired\xspace}  % r22.chal_limit: challenge status, for the limits over -
\newcommand{\ChallengeMainParagraph}{To stress-test the auditing layers without tuning to model outcomes, a separate model constructed \ChallengeN{} archive cases and sealed per-tool expectations before a single run; the cases were unseen by the Claude agents that developed and ran the pipeline, but white-box to their builder. The independent outcome scorer met \ChallengeScorerMet/\ChallengeN{} frozen expectations. Independent validity re-derivation met \ChallengeVindMet/\ChallengeN, missing two delivery faults, one commit-before-change case and one truncated trajectory; evaluator replay met \ChallengeEvalMet/\ChallengeN{} because it preserves archived validity and invariant claims. We neither repaired nor reran the challenge. These results bound the tested layers on this constructed suite; they do not establish verifier soundness.\xspace}  % chal.r28.main: r28 challenge paragraph (scorer 28/28, validity 24/28, evaluator 10/28) over -
\newcommand{\ChallengeMainR}{A separate model built a run-once \ChallengeN-case challenge whose per-tool expectations were sealed before its one run; the cases were unseen by the Claude agents that built and ran the pipeline but white-box to their builder. The outcome scorer met \ChallengeScorerMet/\ChallengeN{} frozen expectations, validity re-derivation \ChallengeVindMet/\ChallengeN{} and archived evaluator replay \ChallengeEvalMet/\ChallengeN; misses were neither repaired nor rerun (Table~\ref{tab:layers}, Appendix~\ref{app:certificates}). This bounds these layers on that constructed suite but is not blind validation.\xspace}  % r32.chal: r32: Section 6: the sealed challenge (compressed) over -
\newcommand{\ChallengeMainThree}{\paragraph{Sealed challenge.} A separate model built a run-once \ChallengeN-case challenge, white-box to its builder but unseen by the Claude agents that built the pipeline; the outcome scorer met \ChallengeScorerMet/\ChallengeN{} sealed expectations, validity re-derivation \ChallengeVindMet/\ChallengeN{} and archived evaluator replay \ChallengeEvalMet/\ChallengeN, unrepaired (Table~\ref{tab:layers}, Appendix~\ref{app:certificates}); not blind validation.\xspace}  % r34.ext.chal3: r34 external challenge: Section 6: the sealed challenge (compact) over -
\newcommand{\ChallengeMet}{24\xspace}  % chal.met: cases whose frozen expectations both registered tools met over case
\newcommand{\ChallengeMissed}{4\xspace}  % chal.missed: cases not met by the registered pipeline over case
\newcommand{\ChallengeN}{28\xspace}  % chal.n: sealed cases over case
\newcommand{\ChallengeRetainedSentence}{All four validity misses are retained as failed expectations and identified as future regression targets only after the sealed result; the sealed score remains \ChallengeMet/\ChallengeN.\xspace}  % chal.r27.retained: r27 challenge text (scorer 28/28, validity 24/28, evaluator 10/28) over -
\newcommand{\ChallengeRiskFourSentence}{EnvOS is intentionally reported as a composition of bounded checks rather than a soundness guarantee: the sealed challenge exposed four blind spots in independent validity reconstruction and eighteen in the evaluator's archived verdict path; these misses are part of the result, not excluded from it.\xspace}  % chal.r27.risk4: r27 challenge text (scorer 28/28, validity 24/28, evaluator 10/28) over -
\newcommand{\ChallengeScorerCorruptMet}{18\xspace}  % chal.reward_audit.corrupt_met: reward_audit: corruptions met over case
\newcommand{\ChallengeScorerMet}{28\xspace}  % chal.reward_audit.met: reward_audit: cases met over case
\newcommand{\ChallengeScorerValidMet}{10\xspace}  % chal.reward_audit.valid_met: reward_audit: valid met over case
\newcommand{\ChallengeSealFiles}{7\xspace}  % chal.seal_files: sealed files whose digests ADDENDUM 19 section 7 records over file
\newcommand{\ChallengeSealSha}{\texttt{b9f9000f0393}\xspace}  % chal.seal: sha256 prefix of the challenge seal record over -
\newcommand{\ChallengeToolErrors}{0\xspace}  % chal.tool_errors: tool errors, SKIPPED included, over every tool over invocation
\newcommand{\ChallengeToolSources}{7\xspace}  % chal.sources: tool source files the run manifest pins over file
\newcommand{\ChallengeToolSourcesSame}{7\xspace}  % chal.sources_same: of those, byte-identical now (a patch after the run would show here) over file
\newcommand{\ChallengeValid}{10\xspace}  % chal.valid: valid controls over case
\newcommand{\ChallengeValidAccepted}{10\xspace}  % chal.valid_accepted: instantiated valid controls both registered tools met (accepted) over case
\newcommand{\ChallengeValidInstantiated}{10\xspace}  % chal.valid_instantiated: valid controls on which neither registered tool errored over case
\newcommand{\ChallengeVindCorruptMet}{14\xspace}  % chal.validity_independent.corrupt_met: validity_independent: corruptions met over case
\newcommand{\ChallengeVindGaps}{missing observation delivery (2); commit before change (1); truncated trajectory (1)\xspace}  % chal.r27.vind_gaps: r27 challenge text (scorer 28/28, validity 24/28, evaluator 10/28) over -
\newcommand{\ChallengeVindMet}{24\xspace}  % chal.validity_independent.met: validity_independent: cases met over case
\newcommand{\ChallengeVindMissed}{4\xspace}  % chal.r27.vind_missed: validity re-derivation: cases not met over case
\newcommand{\ChallengeVindValidMet}{10\xspace}  % chal.validity_independent.valid_met: validity_independent: valid met over case
\newcommand{\ClmActionBudget}{40\xspace}  % spec.clm_max_steps: the claims blocks' declared budget over action
\newcommand{\ClmAnchorSentence}{\ClmOpusInstrSentence{} Sonnet~5 rarely did so (\BlockClmBSOffReread{} of \BlockClmBSClmOffAN{} OFF-A runs), and re-exposing the live policy record before approval increased its success from \BlockClmBSClmOffAPassFrac{} to \BlockClmBSClmOnAPassFrac\xspace}  % r25.anchor: generated sentence (opus_all=True sonnet_rare=True sonnet_R1=True) over -
\newcommand{\ClmBSPaperHolmR}{\xspace}  % r32.clmbs_holm: r32: CLM-BS's paper-wide Holm standing as arithmetic over -
\newcommand{\ClmBoundarySentence}{In this claims workflow, behavior separates at re-verification: Opus re-read the authoritative record after the change in all \BlockClmBClmOffAN{} OFF-A episodes, whereas Sonnet did so in \BlockClmBSOffReread/\BlockClmBSClmOffAN; review-step re-exposure increased Sonnet success from \BlockClmBSClmOffAPassFrac{} to \BlockClmBSClmOnAPassFrac{} (net \BlockClmBSOnOffNetCI, exact paired $p=\BlockClmBSOnOffP$). We treat this as a within-task behavioral boundary: a hypothesis consistent with these observations, not a separately identified mechanism and not a model-wide capability claim.\xspace}  % r25.boundary: generated sentence (opus_all=True sonnet_rare=True sonnet_R1=True) over -
\newcommand{\ClmBundleFiles}{29\xspace}  % clm.bundle_n: files CLAIMS_BUNDLE_SHA256SUMS.txt lists, every one present and verifying (asserted by claims_bundle) over file
\newcommand{\ClmBundleSha}{\texttt{063b7ae44e11}\xspace}  % clm.bundle_sha: sha256 prefix of CLAIMS_BUNDLE_SHA256SUMS.txt over -
\newcommand{\ClmConclSentence}{In claims approval, Opus re-read the changed policy record in all \BlockClmBClmOffAN{} OFF-A runs and succeeded \BlockClmBClmOffAPassFrac{} without review-step re-exposure; Sonnet succeeded on \BlockClmBSClmOffAPassFrac{} OFF-A and \BlockClmBSClmOnAPassFrac{} ON-A under the same fixed instruction. These are within-configuration effects, not model-wide capability claims.\xspace}  % r25.concl: generated sentence (opus_all=True sonnet_rare=True sonnet_R1=True) over -
\newcommand{\ClmContribution}{A prospective second-workflow result, a test of task-level reuse rather than environment-level transfer: under one fixed instruction Opus~5 re-verified without re-exposure, and the same review-step re-exposure raised Sonnet~5's success from \BlockClmBSClmOffAPassFrac{} to \BlockClmBSClmOnAPassFrac\xspace}  % r25.contrib: generated sentence (opus_all=True sonnet_rare=True sonnet_R1=True) over -
\newcommand{\ClmCopyLimitTally}{10 OFF-A failures, 7 rescues, 0 harms, 3 ties\xspace}  % r29.cs.copy: the copy-limit baseline recomputed from the table over -
\newcommand{\ClmCountedTotal}{48\xspace}  % clm.counted_total: counted rollouts of the admissible claims blocks over counted rollout
\newcommand{\ClmGAbstractR}{A separately pre-registered follow-up with a non-Anthropic configuration (Gemini 3.1 Pro Preview) did not meet the registered effect criterion (0/10 to 5/10, exact p = 0.0625).\xspace}  % clmg.abstract: r32 CLM-BG: the registered abstract sentence (s8.3) over -
\newcommand{\ClmGAddendumSha}{\texttt{bf3999dbd602e432}\xspace}  % clmg.sha: r32 CLM-BG: ADDENDUM G's sha256 (first 16 hex) over -
\newcommand{\ClmGAttempts}{25\xspace}  % clmg.attempts: r32 CLM-BG: attempts over attempt
\newcommand{\ClmGBlockedSteps}{0\xspace}  % clmg.gbad: r32 CLM-BG: provider-blocked or empty-reply steps (s3.3), all arms over step
\newcommand{\ClmGBuildCutoff}{23:00Z\xspace}  % clmg.cutoff: r32 CLM-BG: the registered hard build cutoff over -
\newcommand{\ClmGCaption}{Gemini 3.1 Pro Preview received each frame inline in a stateless REST request with no tools; the Claude models were instructed to read each frame file with their file-read tool. Provider, model, invoker and image-delivery channel differ together; rows describe model–invoker configurations, not vendor effects.\xspace}  % clmg.caption: r32 CLM-BG: the mandatory mixed-table caption (s7.4) over -
\newcommand{\ClmGChecks}{42\xspace}  % clmg.gx_checks: r32 CLM-BG: lane GX's offline re-derivation checks (all pass) over -
\newcommand{\ClmGConclR}{The prospective claims and BC experiments, not the historical predecessor blocks, carry the model-effect conclusions (Section~\ref{sec:experiments}). In claims approval Opus succeeded \BlockClmBClmOffAPassFrac{} without review-step re-exposure, and for Sonnet the panel increased full-task success at the registered local level; in clinic booking, at the block-local level the value display increased success relative to the cue-and-link panel (block-local Holm $p=\BlockBCLiveCueHolmLocal$ for LIVE--CUE, $p=\BlockBCCueOffHolmLocal$ for CUE--OFF). \ConclNullClause{} A separately pre-registered follow-up with a non-Anthropic configuration (Gemini 3.1 Pro Preview) did not meet the registered effect criterion (0/10 to 5/10, exact p = 0.0625). The auditing challenges and raw-log comparisons show concretely that intervention, delivery and scoring checks can disagree on the same corrupted archive, motivating explicit testing of each layer rather than assuming evaluator correctness.\xspace}  % clmg.concl: r32 CLM-BG: the conclusion with the registered CLM-BG sentence over -
\newcommand{\ClmGControls}{credible\xspace}  % clmg.controls: r32 CLM-BG: control credibility over -
\newcommand{\ClmGCopyLimit}{R1 (7/0/3, $p=0.0156$; controls not credible)\xspace}  % clmg.copy: r32 CLM-BG: the copy-limit baseline's reading over -
\newcommand{\ClmGCounted}{24\xspace}  % clmg.counted: r32 CLM-BG: counted rollouts over rollout
\newcommand{\ClmGEndpointFull}{24\xspace}  % clmg.endpoint: r32 CLM-BG: counted rows whose four terms the independent scorer re-derives and agree with the evaluator over rollout
\newcommand{\ClmGFirstReqUTC}{21:47Z\xspace}  % clmg.first: r32 CLM-BG: first task request over -
\newcommand{\ClmGFrameReadB}{357/357\xspace}  % clmg.fb_b: r32 CLM-BG: CLM-B policy steps with an executed frame Read (pinned before any CLM-BG rollout) over -
\newcommand{\ClmGFrameReadBS}{217/297\xspace}  % clmg.fb_bs: r32 CLM-BG: CLM-BS policy steps with an executed frame Read (pinned before any CLM-BG rollout) over -
\newcommand{\ClmGFrozenUTC}{2026-09-24 21:36Z\xspace}  % clmg.frozen: r32 CLM-BG: ADDENDUM G's FROZEN time over -
\newcommand{\ClmGGenConfig}{temperature 1.0, top-$p$ 0.95, top-$k$ 64, thinking level ``high'', high media resolution\xspace}  % clmg.gen: r32 CLM-BG: the pinned generation settings over -
\newcommand{\ClmGHarm}{0\xspace}  % clmg.harm: r32 CLM-BG: harms over pair
\newcommand{\ClmGIncidentEpisode}{41 of 48\xspace}  % clmg.inc_ep: r32 CLM-BG: the certification episode the pre-send check stopped at over -
\newcommand{\ClmGIncidentFrames}{3 of 915\xspace}  % clmg.inc_fr: r32 CLM-BG: archived certification frames matching the key pattern over -
\newcommand{\ClmGInfraStep}{22\xspace}  % clmg.infra_step: r32 CLM-BG: the step of the uncounted attempt's provider error over -
\newcommand{\ClmGJournalRows}{626\xspace}  % clmg.journal: r32 CLM-BG: journaled task requests (each with image and text digests) over request
\newcommand{\ClmGLastReqUTC}{23:34Z\xspace}  % clmg.last: r32 CLM-BG: last task request over -
\newcommand{\ClmGLaunches}{1\xspace}  % clmg.launches: r32 CLM-BG: launches over launch
\newcommand{\ClmGLimitR}{All prospective inferential claims of the paper rest on Claude-model blocks; the only non-Anthropic block (CLM-BG) is a separately registered configuration follow-up on reused instances.\xspace}  % clmg.limit: r32 CLM-BG: the fixed limitations sentence (s8.1, every outcome) over -
\newcommand{\ClmGLzeroBack}{0\xspace}  % clmg.Lzero.back: r32 CLM-BG: CLM-L0 returns from the review step over rollout
\newcommand{\ClmGLzeroLabels}{correct 1\xspace}  % clmg.Lzero.labels: r32 CLM-BG: CLM-L0 evaluator labels over -
\newcommand{\ClmGLzeroPassFrac}{1/1\xspace}  % clmg.Lzero.frac: r32 CLM-BG: CLM-L0 successes / counted over -
\newcommand{\ClmGLzeroReread}{0\xspace}  % clmg.Lzero.reread: r32 CLM-BG: CLM-L0 policy re-reads after the change over rollout
\newcommand{\ClmGLzeroStepCap}{0\xspace}  % clmg.Lzero.cap: r32 CLM-BG: CLM-L0 step-cap terminations over rollout
\newcommand{\ClmGLzeroWilson}{[0.21, 1.00]\xspace}  % clmg.Lzero.wilson: r32 CLM-BG: CLM-L0 Wilson 95% (z = 1.96) over -
\newcommand{\ClmGMaxSteps}{40\xspace}  % clmg.maxsteps: r32 CLM-BG: step budget over step
\newcommand{\ClmGModel}{Gemini 3.1 Pro Preview (\texttt{gemini-3.1-pro-preview})\xspace}  % clmg.model: r32 CLM-BG: the model id over -
\newcommand{\ClmGModelVersion}{\texttt{3.1-pro-preview-01-2026}\xspace}  % clmg.version: r32 CLM-BG: models.get version before and after the block over -
\newcommand{\ClmGNetCI}{$+0.50$ [$0.12$, $0.76$]\xspace}  % clmg.netci: r32 CLM-BG: net difference, Newcombe method 10 over -
\newcommand{\ClmGOffABack}{0\xspace}  % clmg.OffA.back: r32 CLM-BG: CLM-OFF-A returns from the review step over rollout
\newcommand{\ClmGOffALabels}{no commit 1, stale approval 9\xspace}  % clmg.OffA.labels: r32 CLM-BG: CLM-OFF-A evaluator labels over -
\newcommand{\ClmGOffAPassFrac}{0/10\xspace}  % clmg.OffA.frac: r32 CLM-BG: CLM-OFF-A successes / counted over -
\newcommand{\ClmGOffAReread}{0\xspace}  % clmg.OffA.reread: r32 CLM-BG: CLM-OFF-A policy re-reads after the change over rollout
\newcommand{\ClmGOffAStepCap}{1\xspace}  % clmg.OffA.cap: r32 CLM-BG: CLM-OFF-A step-cap terminations over rollout
\newcommand{\ClmGOffAWilson}{[0.00, 0.28]\xspace}  % clmg.OffA.wilson: r32 CLM-BG: CLM-OFF-A Wilson 95% (z = 1.96) over -
\newcommand{\ClmGOffFail}{10\xspace}  % clmg.offfail: r32 CLM-BG: OFF-A failures over pair
\newcommand{\ClmGOnABack}{9\xspace}  % clmg.OnA.back: r32 CLM-BG: CLM-ON-A returns from the review step over rollout
\newcommand{\ClmGOnALabels}{correct 5, no commit 5\xspace}  % clmg.OnA.labels: r32 CLM-BG: CLM-ON-A evaluator labels over -
\newcommand{\ClmGOnAPassFrac}{5/10\xspace}  % clmg.OnA.frac: r32 CLM-BG: CLM-ON-A successes / counted over -
\newcommand{\ClmGOnAReread}{6\xspace}  % clmg.OnA.reread: r32 CLM-BG: CLM-ON-A policy re-reads after the change over rollout
\newcommand{\ClmGOnAStepCap}{5\xspace}  % clmg.OnA.cap: r32 CLM-BG: CLM-ON-A step-cap terminations over rollout
\newcommand{\ClmGOnAWilson}{[0.24, 0.76]\xspace}  % clmg.OnA.wilson: r32 CLM-BG: CLM-ON-A Wilson 95% (z = 1.96) over -
\newcommand{\ClmGOnIBack}{0\xspace}  % clmg.OnI.back: r32 CLM-BG: CLM-ON-I returns from the review step over rollout
\newcommand{\ClmGOnILabels}{correct 3\xspace}  % clmg.OnI.labels: r32 CLM-BG: CLM-ON-I evaluator labels over -
\newcommand{\ClmGOnIPassFrac}{3/3\xspace}  % clmg.OnI.frac: r32 CLM-BG: CLM-ON-I successes / counted over -
\newcommand{\ClmGOnIReread}{0\xspace}  % clmg.OnI.reread: r32 CLM-BG: CLM-ON-I policy re-reads after the change over rollout
\newcommand{\ClmGOnIStepCap}{0\xspace}  % clmg.OnI.cap: r32 CLM-BG: CLM-ON-I step-cap terminations over rollout
\newcommand{\ClmGOnIWilson}{[0.44, 1.00]\xspace}  % clmg.OnI.wilson: r32 CLM-BG: CLM-ON-I Wilson 95% (z = 1.96) over -
\newcommand{\ClmGP}{0.0625\xspace}  % clmg.p: r32 CLM-BG: exact two-sided sign test (nominal within-block p) over -
\newcommand{\ClmGPairs}{10\xspace}  % clmg.pairs: r32 CLM-BG: paired instances over pair
\newcommand{\ClmGPolicySteps}{603\xspace}  % clmg.gsteps: r32 CLM-BG: policy steps of the counted rollouts over step
\newcommand{\ClmGPriorResultUTC}{2026-09-24 04:06Z\xspace}  % clmg.prior: r32 CLM-BG: when the CLM-B/CLM-BS results were generated over -
\newcommand{\ClmGReading}{R3\xspace}  % clmg.reading: r32 CLM-BG: reading by the registered decide() over -
\newcommand{\ClmGReplacements}{1\xspace}  % clmg.repl: r32 CLM-BG: reserve replacements spent over attempt
\newcommand{\ClmGReplacementsMax}{6\xspace}  % clmg.replmax: r32 CLM-BG: the registered reserve over attempt
\newcommand{\ClmGRescue}{5\xspace}  % clmg.rescue: r32 CLM-BG: rescues (ON-A pass, OFF-A fail) over pair
\newcommand{\ClmGRescuedOff}{stale approval 5\xspace}  % clmg.rescoff: r32 CLM-BG: OFF-A labels of the rescued pairs over -
\newcommand{\ClmGResultsR}{On the ten registered reused claims instances, under the frozen Gemini 3.1 Pro Preview configuration, OFF-A failed on 10/10 instances, but review-step re-exposure did not meet the registered effect criterion (5 rescues, 0 harms, 5 ties; exact paired p = 0.0625); the effect is not shown for these instances under this configuration at this budget, and this is not evidence of no effect.\xspace}  % clmg.results: r32 CLM-BG: the registered Results paragraph (s8.2) over -
\newcommand{\ClmGStaleRescues}{5\xspace}  % clmg.stale_rescues: r32 CLM-BG: stale-approval rescues over pair
\newcommand{\ClmGTie}{5\xspace}  % clmg.tie: r32 CLM-BG: ties over pair
\newcommand{\ClmGTrigFired}{OFF-A 10/10, ON-A 10/10, ON-I 3/3\xspace}  % clmg.trig: r32 CLM-BG: trigger fired per arm (s6 (a)) over -
\newcommand{\ClmGTrigOnly}{10 pairs, 5 rescues, 0 harms\xspace}  % clmg.trigonly: r32 CLM-BG: triggered-only sensitivity: pairs, rescues, harms (s6 (b)) over -
\newcommand{\ClmGTsaCutoff}{23:30Z\xspace}  % clmg.tsa_cut: r32 CLM-BG: the registered external-timestamp deadline over -
\newcommand{\ClmGTsaUTC}{21:36:27Z\xspace}  % clmg.tsa: r32 CLM-BG: the RFC 3161 token time (FreeTSA) over -
\newcommand{\ClmGVindAgree}{25\xspace}  % clmg.vind: r32 CLM-BG: validity re-derivation: attempts agreeing over attempt
\newcommand{\ClmGVindValid}{24\xspace}  % clmg.vind_valid: r32 CLM-BG: validity re-derivation: counted rows valid over rollout
\newcommand{\ClmGXupOn}{1/3\xspace}  % clmg.xup: r32 CLM-BG: ON-A successes on the threshold-crossing-increase pairs over -
\newcommand{\ClmInstanceControls}{ON-I at seeds 0 (1400.00, copy-limit pass), 1 (1550.00, copy-limit pass) and 4 (3856.18, copy-limit fail); L0 at seed 5 (2240.59, copy-limit fail)\xspace}  % r29.cs.controls: control cells: correct approvals over -
\newcommand{\ClmInstrChecked}{48\xspace}  % r29.cs.instr_n: counted trajectories the instruction is byte-checked on over episode
\newcommand{\ClmInstrExample}{CLM-BS, OFF-A, seed~0\xspace}  % r29.cs.instr_ex: the printed request's episode over -
\newcommand{\ClmInstrRequestSha}{18cd71847bed\xspace}  % r29.cs.instr_sha: the printed step-0 request's digest prefix over -
\newcommand{\ClmInstructionPhrase}{as it stands when you approve\xspace}  % clm.phrase: the instruction phrase PRECOMMIT_CLAIMS section 2 keeps and discloses (quoted from the frozen file) over -
\newcommand{\ClmLanguageRule}{The claims task shares the scaffold, harness, invoker and vendor with the clinic task: it is a second decision rule for the same intervention, not an independent environment, and no cue or announcement was varied in it.\xspace}  % r21.clm_language: the language rule (always) over -
\newcommand{\ClmLooseParserText}{\emph{Report-format sensitivity.} One CLM-BS ON-A episode (seed~9) approved the correct amount and failed only the report term, because its single reply line starts with prose before \code{RESULT:}, which the frozen parser requires at the start of a line. Under a looser reading that accepts \code{RESULT:} anywhere in the line, the pair would be a further rescue (9 discordant pairs, exact $p=0.00391$); the registered, stricter reading is the one reported.\xspace}  % r29.ep.loose: the report-format sensitivity (post hoc) over -
\newcommand{\ClmNewFiles}{28\xspace}  % reuse.new_files: new_files over -
\newcommand{\ClmNewLines}{10187\xspace}  % reuse.new_file_lines: new_file_lines over -
\newcommand{\ClmNoForceSentence}{Opus's \BlockClmBClmOffAPassFrac{} OFF performance is evidence that silent supersession does not mechanically force failure under this task.\xspace}  % r25.noforce: generated sentence (opus_all=True sonnet_rare=True sonnet_R1=True) over -
\newcommand{\ClmOpusInstrSentence}{Under an instruction defining correctness by the policy value ``\ClmInstructionPhrase,'' Opus~5 re-read the policy record after the silent change in all \BlockClmBClmOffAN{} OFF-A runs and succeeded without review-step re-exposure.\xspace}  % r27.opus_instr: generated sentence (opus_all=True sonnet_rare=True sonnet_R1=True) over -
\newcommand{\ClmOpusMain}{Opus succeeded \BlockClmBClmOffAPassFrac{} in both OFF-A and ON-A; because every OFF-A instance already succeeded, the registered rescue-opportunity gate was not met and no panel-effect claim is made for Opus. Opus requested the policy record after the change in all \BlockClmBClmOffAN{} OFF-A runs, versus \BlockClmBSOffReread/\BlockClmBSClmOffAN{} for Sonnet; these process counts are descriptive, and the instruction itself may encourage checking.\xspace}  % r28.opus: r28: the Opus paragraph (GPT-6 r20) over -
\newcommand{\ClmOrderClause}{In CLM-BS the arm run first and the arm run second each succeeded on 5 of 10 pairs (by order: Appendix~\ref{app:claimsspec}); five pairs per order cannot exclude a period effect.\xspace}  % r29.cs.order: Section 3.4: order-specific split over -
\newcommand{\ClmPageTextCap}{3000\xspace}  % r29.cs.page_cap: page text cap per prompt (prompt layout) over character
\newcommand{\ClmRegisteredROne}{The certified evaluation protocol transfers to a second domain with a derived decision, and the review-step intervention increases full-task success\xspace}  % clm.r1_registered: PRECOMMIT_CLAIMS section 7, R1, verbatim over -
\newcommand{\ClmReuseAddedLines}{at most 1357 added or changed\xspace}  % reuse.shared_lines_added_or_changed_upper_bound: shared_lines_added_or_changed_upper_bound over -
\newcommand{\ClmReuseClause}{\ClmReuseUnchanged of \ClmReuseShared shared components are byte-identical to their clinic-pinned versions, the others gained \ClmReuseAddedLines lines, and \ClmNewFiles new files (\ClmNewLines lines) implement the task, its checks and its audits.\xspace}  % reuse.clause: reuse sentence over -
\newcommand{\ClmReuseShared}{23\xspace}  % reuse.shared_files: shared_files over -
\newcommand{\ClmReuseUnchanged}{12\xspace}  % reuse.shared_unchanged: shared_unchanged over -
\newcommand{\ClmRuleText}{a block with more than 6 replacements or failed readiness gives reading R4 and no result; the rescue question is open only if OFF-A fails on at least 5 pairs (else R2); R1 needs $p<0.05$, more rescues than harms and a minimum number of rescues, which together require at least 6 (else R3); controls are credible only if every L0 control passes and at least 2 ON-I controls pass; the derived-decision gate needs ON-A to pass on at least 2 threshold-crossing-increase pairs\xspace}  % r22.clm_rule: claims decision thresholds (probed from claims_decide) over -
\newcommand{\ClmScorerScope}{The independent scorer's scope covers all \BlockClmBSAuditTerms{} registered outcome terms.\xspace}  % r32.clm_scope: r32: the claims scorer re-derives every registered term (not only a subset) over -
\newcommand{\ClmVerifiedClause}{an independent scorer re-derived every outcome term of all \ClmCountedTotal{} counted claims rollouts, each resolved and agreeing with the evaluator, and independent code re-derived every validity verdict\xspace}  % clm.verified_clause: full only if, on every admissible claims block, every term of every counted rollout is resolved and agreeing, with no contradiction and every validity verdict re-derived in agreement over -
\newcommand{\ClmWorkedInstance}{For example, at seed~1 the claim is for 2769.51 with a deductible of 75.00, so 2694.51 is eligible; the limit reads 1550.00 when the agent first opens the policy record and is 3050.00 at approval, so the correct approval is 2694.51, the stale one 1550.00, and copying the displayed limit gives 1550.00 without the panel and 3050.00 with it (instruction and all instances: Appendix~\ref{app:claimsspec}).\xspace}  % r29.cs.worked: a worked numerical instance (threshold crossing) over -
\newcommand{\ConclNullClause}{These contrasts estimate within-configuration effects; unrejected comparisons do not establish absence or equivalence.\xspace}  % r21.concl_fixed: conclusion, fixed over -
\newcommand{\ConclR}{The prospective claims and BC experiments, not the historical predecessor blocks, carry the model-effect conclusions. In claims approval, Opus re-read the changed policy record after the intervention in all \BlockClmBClmOffAN{} OFF-A runs and succeeded \BlockClmBClmOffAPassFrac{} without review-step re-exposure; under the same fixed instruction, Sonnet succeeded on \BlockClmBSClmOffAPassFrac{} OFF-A and \BlockClmBSClmOnAPassFrac{} ON-A, and for Sonnet the panel increased full-task success at the registered local level. In clinic booking, Opus succeeded on \BlockBCFRXOffAPassFrac{} no-panel, \BlockBCFRXCueAPassFrac{} cue-and-link and \BlockBCFRXLiveAPassFrac{} current-value instances; at the block-local level the value display increased success relative to the cue-and-link panel (block-local Holm $p=\BlockBCLiveCueHolmLocal$ for LIVE--CUE and $p=\BlockBCCueOffHolmLocal$ for CUE--OFF). \ConclNullClause{} The auditing challenge and raw-log comparisons further show that such claims depend on testing the evaluator's intervention, delivery and scoring machinery rather than assuming it is correct.\xspace}  % r31.concl: r31: the conclusion over -
\newcommand{\ConclThree}{The prospective claims and clinic experiments, not the historical predecessor blocks, carry the model-effect conclusions (Section~\ref{sec:experiments}). In clinic booking, at the block-local level the value display increased success relative to the cue-and-link panel (LIVE--CUE block-local Holm $p=\BlockBCLiveCueHolmLocal$, paper-wide $p=\BlockBCLiveCueHolmPaper$; CUE--OFF block-local $p=\BlockBCCueOffHolmLocal$). In claims approval Opus succeeded \BlockClmBClmOffAPassFrac{} without review-step re-exposure, and for Sonnet the panel increased full-task success at the registered local level (block-local $p=\BlockClmBSOnOffP$; retrospective paper-wide Holm $p=\HolmPaperClmBS$). \ConclNullClause{} The auditing challenges and the post-hoc, author-built raw-log comparisons show concretely that intervention, delivery and scoring checks can disagree on the same corrupted archive, so each layer must be tested rather than assumed correct.\xspace}  % r37f.concl: r37 final reviews: the conclusion over -
\newcommand{\ConclTwo}{The prospective claims and BC experiments, not the historical predecessor blocks, carry the model-effect conclusions (Section~\ref{sec:experiments}). In claims approval Opus succeeded \BlockClmBClmOffAPassFrac{} without review-step re-exposure, and for Sonnet the panel increased full-task success at the registered local level; in clinic booking, at the block-local level the value display increased success relative to the cue-and-link panel (block-local Holm $p=\BlockBCLiveCueHolmLocal$ for LIVE--CUE, $p=\BlockBCCueOffHolmLocal$ for CUE--OFF). \ConclNullClause{} The auditing challenges and raw-log comparisons show concretely that intervention, delivery and scoring checks can disagree on the same corrupted archive, motivating explicit testing of each layer rather than assuming evaluator correctness.\xspace}  % r32.concl: r32: the conclusion over -
\newcommand{\ContribBCTail}{ (iv) A prospective clinic decomposition of cue versus value (Section~\ref{sec:bc}): \BlockBCReadingShort.\xspace}  % r28.contrib_bc: r28: the contributions' BC item, by state over -
\newcommand{\ContribTwoR}{two prospectively frozen studies (Section~\ref{sec:experiments}): in a derived claims decision, for Sonnet~5 the panel increased full-task success at the registered local level, while Opus~5 succeeded on \BlockClmBClmOffAPassFrac{} OFF-A instances without the panel; in clinic booking, at the block-local level the value display increased success relative to the cue-and-link panel\xspace}  % r31.contrib: r31: contribution (ii) over -
\newcommand{\ContribTwoS}{two prospectively frozen studies (Section~\ref{sec:experiments}): in clinic booking, at the block-local level the value display increased success relative to the cue-and-link panel (paper-wide Holm $p=\BlockBCLiveCueHolmPaper$); in a derived claims decision, for Sonnet~5 the panel increased full-task success at the registered local level (a block-local test; retrospective paper-wide Holm $p=\HolmPaperClmBS$), while Opus~5 succeeded on \BlockClmBClmOffAPassFrac{} no-panel instances\xspace}  % r37f.contrib: r37 final reviews: contribution (ii) over -
\newcommand{\CorrElevenRows}{5\xspace}  % rules.corr11.rows: A2 rows re-derived by ADDENDUM 11 over rollout
\newcommand{\CorrElevenSig}{4\xspace}  % rules.corr11.sig: signature changes over rollout
\newcommand{\CorrSixteenFlips}{7\xspace}  % rules.corr16.flips: checkpoints flipped false->true by ADDENDUM 16's delivery redefinition over rollout
\newcommand{\CorrSixteenSig}{4\xspace}  % rules.corr16.sig: signature changes over rollout
\newcommand{\CorrTenCounterfactual}{25\xspace}  % rules.corr10.counterfactual: silent-arm model failures the pre-ADDENDUM-10 classifier would have voided over counted rollout
\newcommand{\CountedFailN}{32\xspace}  % slot.n_fail: counted failures over counted failure
\newcommand{\CountedSuccessN}{46\xspace}  % slot.n_success: counted successes over counted success
\newcommand{\CovAllResolved}{32\xspace}  % cov.all_resolved: episodes with all five invariants resolved and agreeing over counted model episode
\newcommand{\CovAttempts}{82\xspace}  % cov.attempts: run directories audited over model attempt
\newcommand{\CovAttributionGap}{18\xspace}  % cov.attribution_gap: counted rows the scorer's search-log attribution could not attach over counted model episode
\newcommand{\CovCertIOneUnresolved}{41\xspace}  % cov.cert.i1_unresolved: I1 unresolved under the current nearest-slot rule over certification episode
\newcommand{\CovCertIThreeUnresolved}{15\xspace}  % cov.cert.i3_unresolved: I3 unresolved (null and modal_bypass policies) over certification episode
\newcommand{\CovCertPaperIOneUnresolved}{0\xspace}  % cov.cert.paper_i1_unresolved: I1 unresolved in the audit the paper cites (before the nearest-slot rule) over certification episode
\newcommand{\CovCertRuns}{76\xspace}  % cov.cert.runs: rescored over certification episode
\newcommand{\CovClinicFalse}{27\xspace}  % cov.clinic_false: clinic term resolved wrong over counted model episode
\newcommand{\CovClinicNoRow}{5\xspace}  % cov.clinic_norow: clinic term unresolved: no single booked row for the patient over counted model episode
\newcommand{\CovClinicResolved}{73\xspace}  % cov.clinic_resolved: clinic term resolved (every counted episode with a booked row) over counted model episode
\newcommand{\CovClinicTrue}{46\xspace}  % cov.clinic_true: clinic term resolved correct over counted model episode
\newcommand{\CovEpisodes}{78\xspace}  % cov.episodes: episodes audited over counted model episode
\newcommand{\CovIOneAgree}{32\xspace}  % cov.i1_agree: I1 resolved and agreeing over counted model episode
\newcommand{\CovIOneUnresolved}{46\xspace}  % cov.i1_unresolved: I1 unresolved over counted model episode
\newcommand{\CovInjectionContradictions}{1\xspace}  % cov.injection: counted contradictions (injection audit, not an invariant) over finding
\newcommand{\CovInvContradictions}{0\xspace}  % cov.inv_contradictions: invariant contradictions over counted model episodes over finding
\newcommand{\CovOtherUnresolved}{0\xspace}  % cov.other_unresolved: unresolved on I2--I5 over counted model episode
\newcommand{\CovSlotEvidence}{0\xspace}  % cov.slot_evidence: trajectories carrying the valid-slot evidence the nearest-slot term needs over trajectory
\newcommand{\CovUncountedContradictions}{12\xspace}  % cov.uncounted: contradictions on the uncounted (harness_error) episodes, reported but excluded from the gate over finding
\newcommand{\CovVerdictIndependent}{no\xspace}  % cov.verdict_independent: whether any script re-derives validity verdicts without the evaluator's code over -
\newcommand{\DefectAEvidence}{\xspace}  % defect.1: evidence present over -
\newcommand{\DefectARows}{1\xspace}  % defect.1.rows: rows of the archived search log scored under the defect over rollout
\newcommand{\DefectBEvidence}{\xspace}  % defect.2: evidence present over -
\newcommand{\DefectBRows}{1\xspace}  % defect.2.rows: rows of the archived search log scored under the defect over rollout
\newcommand{\DefectCEvidence}{\xspace}  % defect.3: evidence present over -
\newcommand{\DefectCRows}{11\xspace}  % defect.3.rows: rows of the archived search log scored under the defect over rollout
\newcommand{\DefectDEvidence}{\xspace}  % defect.4: evidence present over -
\newcommand{\DefectDRows}{3\xspace}  % defect.4.rows: rows of the archived search log scored under the defect over rollout
\newcommand{\DefectEEvidence}{\xspace}  % defect.5: evidence present over -
\newcommand{\DefectERows}{0\xspace}  % defect.5.rows: rows of the archived search log scored under the defect over rollout
\newcommand{\DefectEightAuditAtwo}{19\xspace}  % rules.d8.a2: of which Block A2 attempts over episode
\newcommand{\DefectEightAuditB}{5\xspace}  % rules.d8.b: of which early Block B rows over episode
\newcommand{\DefectEightAuditClaimed}{22\xspace}  % rules.d8.claimed: the count ADDENDUM 11 states over episode
\newcommand{\DefectEightAuditRuns}{24\xspace}  % rules.d8.runs: runs in the audit ADDENDUM 11 cites over episode
\newcommand{\DefectFEvidence}{\xspace}  % defect.6: evidence present over -
\newcommand{\DefectFRows}{0\xspace}  % defect.6.rows: rows of the archived search log scored under the defect over rollout
\newcommand{\DefectGEvidence}{\xspace}  % defect.7: evidence present over -
\newcommand{\DefectGRows}{0\xspace}  % defect.7.rows: rows of the archived search log scored under the defect over rollout
\newcommand{\DefectHEvidence}{\xspace}  % defect.8: evidence present over -
\newcommand{\DefectHRows}{5\xspace}  % defect.8.rows: rows of the archived search log scored under the defect over rollout
\newcommand{\DefectIEvidence}{\xspace}  % defect.9: evidence present over -
\newcommand{\DefectIRows}{3\xspace}  % defect.9.rows: rows of the archived search log scored under the defect over rollout
\newcommand{\DefectJEvidence}{\xspace}  % defect.10: evidence present over -
\newcommand{\DefectJRows}{3\xspace}  % defect.10.rows: rows of the archived search log scored under the defect over rollout
\newcommand{\DefectKEvidence}{\xspace}  % defect.11: evidence present over -
\newcommand{\DefectKRows}{3\xspace}  % defect.11.rows: rows of the archived search log scored under the defect over rollout
\newcommand{\DefectScorerEarlyIndex}{4\xspace}  % defects.scorer_early_index: index, in the defect table, of the scorer-placed-the-event-early defect over -
\newcommand{\DiscBCNew}{16\xspace}  % disc.bc_new: Block BC's instance triples, frozen spec over triple
\newcommand{\DiscBCOld}{10\xspace}  % disc.bc_old: Block BC's instance triples in the pre-image spec (FREEZE_r21/preimage) over triple
\newcommand{\DiscDeadlineNew}{09:00\xspace}  % disc.deadline_new: ADDENDUM 19 branch deadline before/after the round-4 amendment over UTC time
\newcommand{\DiscDeadlineOld}{06:00\xspace}  % disc.deadline_old: ADDENDUM 19 branch deadline before/after the round-4 amendment over UTC time
\newcommand{\DiscInterruptedWord}{One\xspace}  % disc.interrupted: CLM-BS attempts interrupted (ledger) over attempt
\newcommand{\DiscTemplatesWord}{Two\xspace}  % disc.templates: sealed templates that said 'randomized' in the round-3 pre-image and 'counterbalanced' now over template
\newcommand{\DiscTimeoutNew}{120\xspace}  % disc.timeout_new: docker-exec transport timeout before/after the round-4 amendment (FREEZE_r21/CODE_FINAL.md) over second
\newcommand{\DiscTimeoutOld}{30\xspace}  % disc.timeout_old: docker-exec transport timeout before/after the round-4 amendment (FREEZE_r21/CODE_FINAL.md) over second
\newcommand{\DispositionBlocks}{15\xspace}  % disp.blocks: registered blocks with a disposition over block
\newcommand{\DistractorIsNewClinic}{6\xspace}  % neutral.distractor_new: instances whose distractor appointment is at the instance's NEW clinic over instance
\newcommand{\DistractorNewRows}{23\xspace}  % neutral.rows_new: counted rows whose delivered distractor page carried the instance's new clinic over counted rollout
\newcommand{\EndToEndSentence}{The six stages have been executed end-to-end, including independent audits, on both prospective workflows.\xspace}  % r28.e2e: r28: which workflows ran end to end (GPT-6 r20) over -
\newcommand{\ExtAppendixText}{\emph{This challenge differs from the rule-only one (Appendix~\ref{app:blind}) in one respect that matters: the authors neither implemented nor reviewed the cases.} \emph{Constructor and sandbox.} One headless Gemini CLI call (\code{gemini-3.1-pro-preview}, default approval mode; it could neither run a shell nor write files) worked in a sandbox holding only: the four rule and schema files of the rule-only challenge's brief (byte copies, same redactions), \ExtBasesOffered{} byte-verified copies of counted base archives (\ExtClaimsBasesOffered{} claims, three each from CLM-B, CLM-BS and CLM-BG, including failed episodes; \ExtClinicBasesOffered{} Block~BC clinic ones), and an instruction file asking for at least 20 corruptions and 8 unusual-but-valid controls per workflow, a stdlib-only generator that edits every copy of a changed fact and recomputes recorded digests, and an expectation file. The sandbox held no code of ours, no earlier case, class or finding, no paper and no outcome table; a leak check of the instructions, prompt and every base file found no case identifier, tool name or earlier-round label outside verbatim rule text. \emph{Instantiation and seal.} The agent returned the generator and \ExtDesigned{} expectations between markers; both were saved byte for byte and the generator ran once, unedited. It built \ExtRun{} cases; \ExtExcludedIDs{} is excluded because its own generation raised, and no repair round was used. The cases, expectations, transcript, runner and scorer were sealed at \ExtSealUTC, before any tool under test touched any case (the only earlier tool run was a loader smoke test on unmodified base copies). The run began at \ExtRunUTC, used no model and no world; tool and case files did not change during it. The runner is the rule-only challenge's with only its loader adapted, and the scoring functions are that challenge's, copied verbatim. \par\paragraph{Results.} Table~\ref{tab:external-tools} gives each tool. Against the simple raw-log baselines (claims: the r28 baseline; clinic: the r29 baseline) the pipeline caught \ExtClaimsPipeOnly{} claims corruptions the baseline missed and the baseline none the pipeline missed; in the clinic \ExtClinicPipeOnly{} against \ExtClinicBaseOnly{} (EB12, whose edit added a key the schema lacks; the baseline scores it only because it never reports the booked-slot term I1 as passing). Every miss: the pipeline counted EA08, EA09, EA19, EA20 (claims) and EB01, EB03, EB10, EB12, EB14, EB16, EB17, EB18 (clinic) as clean. EB14 and EB18 are undisputed gaps: EB14 changed a collateral appointment's status only in the final state rows, disagreeing with the archived I3 pass, and EB18 set the trajectory's event-log target version equal to its source version while the event log and step copies were unchanged; the pipeline does not cross-check these copies. Three claims misses (EA08, EA19, EA20) edit only an archived derived verdict, which the pipeline silently re-derives instead of flagging the disagreement. It gave no verdict on EA01 and EA18 (a deleted trajectory or claims file: the evaluator raised), and rejected EA11, EB05, EB08, EB09, EB19, EB20 under a class other than the registered one (clinic: the void gate's \code{G0\_void} where the rules name the infrastructure or harness verdict). It did not count EA26, EA27, EB27, controls that change one copy of a fact: the scorer reported the disagreement and the void gate voided the case, whereas the agent expected them counted. \emph{Disputes (scores unchanged).} Written after scoring from a mechanical diff of each case against its base: six edit only a derived field that the refresh re-derives or the rules say is never read (EA08, EA19, EA20, EB03, EB10, EB17); three equal their base (EA09, EA28, EB28); three expect an outcome the unchanged evidence contradicts (EA24, EB24, EB25); two add a key the schema lacks (EB12, EB26); two set a stop reason the rules do not register (EB01, EB16); two are controls that change one copy of a fact, against the instructions (EA26, EA27); one is a control the rules leave open (EB27). On the undisputed cases alone the pipeline caught \ExtClaimsUndPipeCaught/\ExtClaimsUndCor{} claims corruptions with \ExtClaimsUndPipeFA{} counted as clean and \ExtClaimsUndPipeErr{} without verdict (baseline \ExtClaimsUndBaseCaught{} and \ExtClaimsUndBaseFA), and \ExtClinicUndPipeCaught/\ExtClinicUndCor{} clinic ones with \ExtClinicUndPipeFA{} counted as clean (baseline \ExtClinicUndBaseCaught{} and \ExtClinicUndBaseFA), accepting every undisputed control.\par\paragraph{Limits.} The design is shallow: one call, one base per workflow (a CLM-B Opus success and a Block~BC success) although several were requested, one-to-three-word case descriptions, and no case marked ambiguous; \ExtDisputes{} of \ExtDesigned{} expectations are disputable. Most corruptions flip a single field the harness records (stop reason, infrastructure errors, read-target violations, episode marker, a policy-input fault or digest) that the operational validity table reads by design; the raw-log baselines were built to audit intervention validity and the I1/I2 terms and do not read those fields, so part of the gap reflects their narrower scope, and a baseline that reads the validity-table fields was not tested. The constructor is an LLM agent, not an independent research team, and Gemini is also a policy under test elsewhere in this paper (CLM-BG, the same model); the authors chose the rule excerpts, the base archives, the instructions and the tools. The results are per case on this suite, not detection rates, and claims and clinic counts are not pooled.\xspace}  % r34.ext.app: r34 external challenge: the appendix section over -
\newcommand{\ExtBasesOffered}{15\xspace}  % r34.ext.bases_offered: r34 external challenge: base-archive copies in the sandbox over archive
\newcommand{\ExtClaimsBaseCaught}{1\xspace}  % r34.ext.claims.baseline_r28.caught: r34 external challenge: claims baseline_r28: caught over case
\newcommand{\ExtClaimsBaseErr}{2\xspace}  % r34.ext.claims.baseline_r28.err: r34 external challenge: claims baseline_r28: err over case
\newcommand{\ExtClaimsBaseFA}{15\xspace}  % r34.ext.claims.baseline_r28.fa: r34 external challenge: claims baseline_r28: fa over case
\newcommand{\ExtClaimsBaseFR}{0\xspace}  % r34.ext.claims.baseline_r28.fr: r34 external challenge: claims baseline_r28: fr over case
\newcommand{\ExtClaimsBaseMet}{6\xspace}  % r34.ext.claims.baseline_r28.met: r34 external challenge: claims baseline_r28: met over case
\newcommand{\ExtClaimsBaseOnly}{0\xspace}  % r34.ext.claims.pv.base: r34 external challenge: claims: caught by the simple baseline only over case
\newcommand{\ExtClaimsBaseWrong}{0\xspace}  % r34.ext.claims.baseline_r28.wrong: r34 external challenge: claims baseline_r28: rejected, other class over case
\newcommand{\ExtClaimsBasesOffered}{9\xspace}  % r34.ext.claims.bases: r34 external challenge: claims base copies offered over archive
\newcommand{\ExtClaimsCEightCaught}{3\xspace}  % r34.ext.claims.c8.caught: r34 external challenge: claims c8: caught over case
\newcommand{\ExtClaimsCEightErr}{1\xspace}  % r34.ext.claims.c8.err: r34 external challenge: claims c8: err over case
\newcommand{\ExtClaimsCEightFA}{12\xspace}  % r34.ext.claims.c8.fa: r34 external challenge: claims c8: fa over case
\newcommand{\ExtClaimsCEightFR}{0\xspace}  % r34.ext.claims.c8.fr: r34 external challenge: claims c8: fr over case
\newcommand{\ExtClaimsCEightMet}{15\xspace}  % r34.ext.claims.c8.met: r34 external challenge: claims c8: met over case
\newcommand{\ExtClaimsCEightWrong}{0\xspace}  % r34.ext.claims.c8.wrong: r34 external challenge: claims c8: rejected, other class over case
\newcommand{\ExtClaimsCor}{20\xspace}  % r34.ext.claims.cor: r34 external challenge: claims corruptions run over case
\newcommand{\ExtClaimsCtl}{8\xspace}  % r34.ext.claims.ctl: r34 external challenge: claims controls run over case
\newcommand{\ExtClaimsEvalCaught}{14\xspace}  % r34.ext.claims.eval_classifier.caught: r34 external challenge: claims eval_classifier: caught over case
\newcommand{\ExtClaimsEvalErr}{2\xspace}  % r34.ext.claims.eval_classifier.err: r34 external challenge: claims eval_classifier: err over case
\newcommand{\ExtClaimsEvalFA}{4\xspace}  % r34.ext.claims.eval_classifier.fa: r34 external challenge: claims eval_classifier: fa over case
\newcommand{\ExtClaimsEvalFR}{0\xspace}  % r34.ext.claims.eval_classifier.fr: r34 external challenge: claims eval_classifier: fr over case
\newcommand{\ExtClaimsEvalMet}{15\xspace}  % r34.ext.claims.eval_classifier.met: r34 external challenge: claims eval_classifier: met over case
\newcommand{\ExtClaimsEvalWrong}{1\xspace}  % r34.ext.claims.eval_classifier.wrong: r34 external challenge: claims eval_classifier: rejected, other class over case
\newcommand{\ExtClaimsPipeCaught}{14\xspace}  % r34.ext.claims.pipeline.caught: r34 external challenge: claims pipeline: caught over case
\newcommand{\ExtClaimsPipeErr}{2\xspace}  % r34.ext.claims.pipeline.err: r34 external challenge: claims pipeline: err over case
\newcommand{\ExtClaimsPipeFA}{4\xspace}  % r34.ext.claims.pipeline.fa: r34 external challenge: claims pipeline: fa over case
\newcommand{\ExtClaimsPipeFR}{2\xspace}  % r34.ext.claims.pipeline.fr: r34 external challenge: claims pipeline: fr over case
\newcommand{\ExtClaimsPipeMet}{14\xspace}  % r34.ext.claims.pipeline.met: r34 external challenge: claims pipeline: met over case
\newcommand{\ExtClaimsPipeOnly}{13\xspace}  % r34.ext.claims.pv.pipe: r34 external challenge: claims: caught by the pipeline only over case
\newcommand{\ExtClaimsPipeWrong}{1\xspace}  % r34.ext.claims.pipeline.wrong: r34 external challenge: claims pipeline: rejected, other class over case
\newcommand{\ExtClaimsRepCaught}{2\xspace}  % r34.ext.claims.repaired_r29.caught: r34 external challenge: claims repaired_r29: caught over case
\newcommand{\ExtClaimsRepErr}{2\xspace}  % r34.ext.claims.repaired_r29.err: r34 external challenge: claims repaired_r29: err over case
\newcommand{\ExtClaimsRepFA}{15\xspace}  % r34.ext.claims.repaired_r29.fa: r34 external challenge: claims repaired_r29: fa over case
\newcommand{\ExtClaimsRepFR}{1\xspace}  % r34.ext.claims.repaired_r29.fr: r34 external challenge: claims repaired_r29: fr over case
\newcommand{\ExtClaimsRepMet}{4\xspace}  % r34.ext.claims.repaired_r29.met: r34 external challenge: claims repaired_r29: met over case
\newcommand{\ExtClaimsRepWrong}{0\xspace}  % r34.ext.claims.repaired_r29.wrong: r34 external challenge: claims repaired_r29: rejected, other class over case
\newcommand{\ExtClaimsScorerCaught}{8\xspace}  % r34.ext.claims.scorer.caught: r34 external challenge: claims scorer: caught over case
\newcommand{\ExtClaimsScorerErr}{1\xspace}  % r34.ext.claims.scorer.err: r34 external challenge: claims scorer: err over case
\newcommand{\ExtClaimsScorerFA}{11\xspace}  % r34.ext.claims.scorer.fa: r34 external challenge: claims scorer: fa over case
\newcommand{\ExtClaimsScorerFR}{2\xspace}  % r34.ext.claims.scorer.fr: r34 external challenge: claims scorer: fr over case
\newcommand{\ExtClaimsScorerMet}{5\xspace}  % r34.ext.claims.scorer.met: r34 external challenge: claims scorer: met over case
\newcommand{\ExtClaimsScorerWrong}{4\xspace}  % r34.ext.claims.scorer.wrong: r34 external challenge: claims scorer: rejected, other class over case
\newcommand{\ExtClaimsUndBaseCaught}{1\xspace}  % r34.ext.claims.u.baseline_r28.caught: r34 external challenge: claims undisputed, baseline_r28: caught over case
\newcommand{\ExtClaimsUndBaseCtlOk}{4\xspace}  % r34.ext.claims.u.baseline_r28.ctl_ok: r34 external challenge: claims undisputed, baseline_r28: ctl_ok over case
\newcommand{\ExtClaimsUndBaseErr}{2\xspace}  % r34.ext.claims.u.baseline_r28.err: r34 external challenge: claims undisputed, baseline_r28: err over case
\newcommand{\ExtClaimsUndBaseFA}{11\xspace}  % r34.ext.claims.u.baseline_r28.fa: r34 external challenge: claims undisputed, baseline_r28: fa over case
\newcommand{\ExtClaimsUndCor}{16\xspace}  % r34.ext.claims.u.n: r34 external challenge: claims: undisputed corruptions over case
\newcommand{\ExtClaimsUndCtl}{4\xspace}  % r34.ext.claims.u.ctl: r34 external challenge: claims: undisputed controls over case
\newcommand{\ExtClaimsUndPipeCaught}{14\xspace}  % r34.ext.claims.u.pipeline.caught: r34 external challenge: claims undisputed, pipeline: caught over case
\newcommand{\ExtClaimsUndPipeCtlOk}{4\xspace}  % r34.ext.claims.u.pipeline.ctl_ok: r34 external challenge: claims undisputed, pipeline: ctl_ok over case
\newcommand{\ExtClaimsUndPipeErr}{2\xspace}  % r34.ext.claims.u.pipeline.err: r34 external challenge: claims undisputed, pipeline: err over case
\newcommand{\ExtClaimsUndPipeFA}{0\xspace}  % r34.ext.claims.u.pipeline.fa: r34 external challenge: claims undisputed, pipeline: fa over case
\newcommand{\ExtClinicBaseCaught}{3\xspace}  % r34.ext.clinic.baseline_r29.caught: r34 external challenge: clinic baseline_r29: caught over case
\newcommand{\ExtClinicBaseErr}{0\xspace}  % r34.ext.clinic.baseline_r29.err: r34 external challenge: clinic baseline_r29: err over case
\newcommand{\ExtClinicBaseFA}{15\xspace}  % r34.ext.clinic.baseline_r29.fa: r34 external challenge: clinic baseline_r29: fa over case
\newcommand{\ExtClinicBaseFR}{0\xspace}  % r34.ext.clinic.baseline_r29.fr: r34 external challenge: clinic baseline_r29: fr over case
\newcommand{\ExtClinicBaseMet}{0\xspace}  % r34.ext.clinic.baseline_r29.met: r34 external challenge: clinic baseline_r29: met over case
\newcommand{\ExtClinicBaseOnly}{1\xspace}  % r34.ext.clinic.pv.base: r34 external challenge: clinic: caught by the simple baseline only over case
\newcommand{\ExtClinicBaseWrong}{0\xspace}  % r34.ext.clinic.baseline_r29.wrong: r34 external challenge: clinic baseline_r29: rejected, other class over case
\newcommand{\ExtClinicBasesOffered}{6\xspace}  % r34.ext.clinic.bases: r34 external challenge: clinic base copies offered over archive
\newcommand{\ExtClinicCor}{19\xspace}  % r34.ext.clinic.cor: r34 external challenge: clinic corruptions run over case
\newcommand{\ExtClinicCtl}{8\xspace}  % r34.ext.clinic.ctl: r34 external challenge: clinic controls run over case
\newcommand{\ExtClinicEvalCaught}{4\xspace}  % r34.ext.clinic.eval_classifier.caught: r34 external challenge: clinic eval_classifier: caught over case
\newcommand{\ExtClinicEvalErr}{0\xspace}  % r34.ext.clinic.eval_classifier.err: r34 external challenge: clinic eval_classifier: err over case
\newcommand{\ExtClinicEvalFA}{15\xspace}  % r34.ext.clinic.eval_classifier.fa: r34 external challenge: clinic eval_classifier: fa over case
\newcommand{\ExtClinicEvalFR}{0\xspace}  % r34.ext.clinic.eval_classifier.fr: r34 external challenge: clinic eval_classifier: fr over case
\newcommand{\ExtClinicEvalMet}{7\xspace}  % r34.ext.clinic.eval_classifier.met: r34 external challenge: clinic eval_classifier: met over case
\newcommand{\ExtClinicEvalWrong}{0\xspace}  % r34.ext.clinic.eval_classifier.wrong: r34 external challenge: clinic eval_classifier: rejected, other class over case
\newcommand{\ExtClinicPipeCaught}{11\xspace}  % r34.ext.clinic.pipeline.caught: r34 external challenge: clinic pipeline: caught over case
\newcommand{\ExtClinicPipeErr}{0\xspace}  % r34.ext.clinic.pipeline.err: r34 external challenge: clinic pipeline: err over case
\newcommand{\ExtClinicPipeFA}{8\xspace}  % r34.ext.clinic.pipeline.fa: r34 external challenge: clinic pipeline: fa over case
\newcommand{\ExtClinicPipeFR}{1\xspace}  % r34.ext.clinic.pipeline.fr: r34 external challenge: clinic pipeline: fr over case
\newcommand{\ExtClinicPipeMet}{7\xspace}  % r34.ext.clinic.pipeline.met: r34 external challenge: clinic pipeline: met over case
\newcommand{\ExtClinicPipeOnly}{9\xspace}  % r34.ext.clinic.pv.pipe: r34 external challenge: clinic: caught by the pipeline only over case
\newcommand{\ExtClinicPipeWrong}{5\xspace}  % r34.ext.clinic.pipeline.wrong: r34 external challenge: clinic pipeline: rejected, other class over case
\newcommand{\ExtClinicScorerCaught}{5\xspace}  % r34.ext.clinic.scorer.caught: r34 external challenge: clinic scorer: caught over case
\newcommand{\ExtClinicScorerErr}{0\xspace}  % r34.ext.clinic.scorer.err: r34 external challenge: clinic scorer: err over case
\newcommand{\ExtClinicScorerFA}{14\xspace}  % r34.ext.clinic.scorer.fa: r34 external challenge: clinic scorer: fa over case
\newcommand{\ExtClinicScorerFR}{1\xspace}  % r34.ext.clinic.scorer.fr: r34 external challenge: clinic scorer: fr over case
\newcommand{\ExtClinicScorerMet}{6\xspace}  % r34.ext.clinic.scorer.met: r34 external challenge: clinic scorer: met over case
\newcommand{\ExtClinicScorerWrong}{0\xspace}  % r34.ext.clinic.scorer.wrong: r34 external challenge: clinic scorer: rejected, other class over case
\newcommand{\ExtClinicUndBaseCaught}{2\xspace}  % r34.ext.clinic.u.baseline_r29.caught: r34 external challenge: clinic undisputed, baseline_r29: caught over case
\newcommand{\ExtClinicUndBaseCtlOk}{3\xspace}  % r34.ext.clinic.u.baseline_r29.ctl_ok: r34 external challenge: clinic undisputed, baseline_r29: ctl_ok over case
\newcommand{\ExtClinicUndBaseErr}{0\xspace}  % r34.ext.clinic.u.baseline_r29.err: r34 external challenge: clinic undisputed, baseline_r29: err over case
\newcommand{\ExtClinicUndBaseFA}{10\xspace}  % r34.ext.clinic.u.baseline_r29.fa: r34 external challenge: clinic undisputed, baseline_r29: fa over case
\newcommand{\ExtClinicUndCor}{13\xspace}  % r34.ext.clinic.u.n: r34 external challenge: clinic: undisputed corruptions over case
\newcommand{\ExtClinicUndCtl}{3\xspace}  % r34.ext.clinic.u.ctl: r34 external challenge: clinic: undisputed controls over case
\newcommand{\ExtClinicUndPipeCaught}{11\xspace}  % r34.ext.clinic.u.pipeline.caught: r34 external challenge: clinic undisputed, pipeline: caught over case
\newcommand{\ExtClinicUndPipeCtlOk}{3\xspace}  % r34.ext.clinic.u.pipeline.ctl_ok: r34 external challenge: clinic undisputed, pipeline: ctl_ok over case
\newcommand{\ExtClinicUndPipeErr}{0\xspace}  % r34.ext.clinic.u.pipeline.err: r34 external challenge: clinic undisputed, pipeline: err over case
\newcommand{\ExtClinicUndPipeFA}{2\xspace}  % r34.ext.clinic.u.pipeline.fa: r34 external challenge: clinic undisputed, pipeline: fa over case
\newcommand{\ExtClinicVindCaught}{6\xspace}  % r34.ext.clinic.vi.caught: r34 external challenge: clinic vi: caught over case
\newcommand{\ExtClinicVindErr}{0\xspace}  % r34.ext.clinic.vi.err: r34 external challenge: clinic vi: err over case
\newcommand{\ExtClinicVindFA}{9\xspace}  % r34.ext.clinic.vi.fa: r34 external challenge: clinic vi: fa over case
\newcommand{\ExtClinicVindFR}{0\xspace}  % r34.ext.clinic.vi.fr: r34 external challenge: clinic vi: fr over case
\newcommand{\ExtClinicVindMet}{17\xspace}  % r34.ext.clinic.vi.met: r34 external challenge: clinic vi: met over case
\newcommand{\ExtClinicVindWrong}{1\xspace}  % r34.ext.clinic.vi.wrong: r34 external challenge: clinic vi: rejected, other class over case
\newcommand{\ExtConstructorModel}{gemini-3.1-pro-preview\xspace}  % r34.ext.model: r34 external challenge: the constructor's served model (Gemini CLI session log) over -
\newcommand{\ExtContrib}{, one also built by an external agent\xspace}  % r34.ext.contrib: r34 external challenge: contribution (iii)'s clause over -
\newcommand{\ExtControls}{16\xspace}  % r34.ext.ctl: r34 external challenge: controls run, both workflows over case
\newcommand{\ExtCorTotal}{39\xspace}  % r37f.cor: r37: external challenge, admitted corruptions, both workflows over case
\newcommand{\ExtDesigned}{56\xspace}  % r34.ext.designed: r34 external challenge: cases the external agent designed over case
\newcommand{\ExtDisputes}{19\xspace}  % r34.ext.disputes: r34 external challenge: expectations the authors dispute (scores unchanged) over case
\newcommand{\ExtExcluded}{1\xspace}  % r34.ext.excl: r34 external challenge: cases whose generation raised over case
\newcommand{\ExtExcludedIDs}{EB11\xspace}  % r34.ext.excl_ids: r34 external challenge: the excluded cases over -
\newcommand{\ExtMainR}{\paragraph{External challenge.} A Gemini CLI agent given only the rules, schema and \ExtBasesOffered{} archive copies designed \ExtDesigned{} cases \emph{and} wrote their generator, which we ran unread, sealed and scored once per tool. The pipeline caught \ExtClaimsPipeCaught/\ExtClaimsCor{} claims and \ExtClinicPipeCaught/\ExtClinicCor{} clinic corruptions (raw-log baselines \ExtClaimsBaseCaught, \ExtClinicBaseCaught), counted \ExtClaimsPipeFA{} and \ExtClinicPipeFA{} as clean (baselines \ExtClaimsBaseFA, \ExtClinicBaseFA) and rejected \ExtPipeFR{} of \ExtControls{} controls (baselines $\le$1). We dispute \ExtDisputes{} expectations; it used one base per workflow, and an LLM agent is no independent team (Appendix~\ref{app:external}).\xspace}  % r34.ext.main: r34 external challenge: Section 6 paragraph over -
\newcommand{\ExtPipeFATotal}{12\xspace}  % r37f.pc_fa: r37: external challenge, corruptions the pipeline counted as clean, both workflows over case
\newcommand{\ExtPipeFR}{3\xspace}  % r34.ext.pipe_fr: r34 external challenge: controls the pipeline did not count, both workflows over case
\newcommand{\ExtRun}{55\xspace}  % r34.ext.run: r34 external challenge: cases its generator built and every tool ran on over case
\newcommand{\ExtRunUTC}{2026-09-25 09:59:09Z\xspace}  % r34.ext.run_utc: r34 external challenge: when the one tool run started over -
\newcommand{\ExtSealUTC}{2026-09-25 09:59:06Z\xspace}  % r34.ext.seal_utc: r34 external challenge: when the cases were sealed over -
\newcommand{\FailFullyVerified}{32\xspace}  % slot.fail_verified: counted failures with all five invariants independently resolved over counted failure
\newcommand{\FeasAtwoN}{34\xspace}  % feas.A2.n: count over scripted episode
\newcommand{\FeasAtwoOk}{34\xspace}  % feas.A2.ok: count ok over scripted episode
\newcommand{\FeasAtwoPolicies}{3\xspace}  % feas.A2.policies: distinct over scripted policy
\newcommand{\FeasAtwoRefStepsMax}{26\xspace}  % feas.A2.ref_steps_max: max actions over scripted reference episode
\newcommand{\FeasAtwoRefStepsMin}{25\xspace}  % feas.A2.ref_steps_min: min actions over scripted reference episode
\newcommand{\FeasAtwoSeedHi}{15\xspace}  % feas.A2.seed_hi: max over seed
\newcommand{\FeasAtwoSeedLo}{8\xspace}  % feas.A2.seed_lo: min over seed
\newcommand{\FeasBN}{44\xspace}  % feas.B.n: count over scripted episode
\newcommand{\FeasBOffAReferenceN}{10\xspace}  % feas.B.offA.reference_n: count over scripted episode
\newcommand{\FeasBOffAReferenceSolved}{10\xspace}  % feas.B.offA.reference_solved: count at dense 1.0 over scripted episode
\newcommand{\FeasBOk}{44\xspace}  % feas.B.ok: count ok over scripted episode
\newcommand{\FeasBPolicies}{5\xspace}  % feas.B.policies: distinct over scripted policy
\newcommand{\FeasBSeedHi}{29\xspace}  % feas.B.seed_hi: max over seed
\newcommand{\FeasBSeedLo}{20\xspace}  % feas.B.seed_lo: min over seed
\newcommand{\FigResultsCaption}{\textbf{Counted rollouts per paired instance.} (a) The prospective claims blocks, without (OFF-A) and with (ON-A) the review-step policy panel, by model; (b) Block~BC, no panel / cue-and-link / value panel (Figure~\ref{fig:bcarms}). Columns are instances $1,\ldots,n$ (generator seeds: Appendices~\ref{app:bc}--\ref{app:claims}); row totals at the right. Filled: evaluator pass; open: failure, shaped by signature.\xspace}  % r29.bc.figcap: Figure 3's caption, by BC state over -
\newcommand{\FigResultsCaptionTwo}{\textbf{Counted rollouts per paired instance.} (a) The Claude claims blocks (CLM-BG: Figure~\ref{fig:clmg}), without (OFF-A) and with (ON-A) the review-step policy panel, by model; (b) Block~BC, no panel / cue-and-link / value panel (Figure~\ref{fig:bcarms}). Columns are instances $1,\ldots,n$ (generator seeds: Appendices~\ref{app:bc}--\ref{app:claims}); row totals at the right. Filled: evaluator pass; open: failure, shaped by signature.\xspace}  % clmg.figcap: r32 CLM-BG: Figure 3's caption with CLM-BG's pointer over -
\newcommand{\FreezeStatusText}{ADDENDA~18 and~19 and the claims pre-registration are frozen (each file verifies against its sha256 record) and the interpretation templates are sealed\xspace}  % r22.freeze_text: freeze/seal status of every prospective registration (heading present and .sha256 verifying; seal matching) over -
\newcommand{\FreshBaseMiss}{12\xspace}  % r29.fr.base_miss: r29 lane A fresh sealed cases (post hoc) over case
\newcommand{\FreshBases}{24\xspace}  % r29.fr.bases: r29 lane A fresh sealed cases (post hoc) over case
\newcommand{\FreshCorr}{15\xspace}  % r29.fr.cor: r29 lane A fresh sealed cases (post hoc) over case
\newcommand{\FreshCtl}{9\xspace}  % r29.fr.ctl: r29 lane A fresh sealed cases (post hoc) over case
\newcommand{\FreshN}{24\xspace}  % r29.fr.n: r29 lane A fresh sealed cases (post hoc) over case
\newcommand{\FreshPipeMiss}{7\xspace}  % r29.fr.pipe_miss: r29 lane A fresh sealed cases (post hoc) over case
\newcommand{\FreshPipeWrong}{1\xspace}  % r29.fr.pipe_wrong: r29 lane A fresh sealed cases (post hoc) over case
\newcommand{\FreshReconFR}{0\xspace}  % r29.fr.recon_fr: r29 lane A fresh sealed cases (post hoc) over case
\newcommand{\FreshReconMiss}{0\xspace}  % r29.fr.recon_miss: r29 lane A fresh sealed cases (post hoc) over case
\newcommand{\FreshRepMiss}{6\xspace}  % r29.fr.rep_miss: r29 lane A fresh sealed cases (post hoc) over case
\newcommand{\FreshRunUTC}{10:03:34Z\xspace}  % r29.fr.run_utc: the one run over -
\newcommand{\FreshSealUTC}{10:03:30Z\xspace}  % r29.fr.seal_utc: fresh cases sealed over -
\newcommand{\FreshSummarySentence}{In summary (moved from the main text), on these \FreshN{} post-hoc, author-built fresh cases with expectations sealed before their single run, the reconstruction missed none of \FreshCorr{} corruptions, the frozen pipeline \FreshPipeMiss{} (truncation, stale pages, access-log duplicate commits) and the repaired raw-log checker \FreshRepMiss{} (panel delivery, commit ordering). ``Fresh'' means unused archive bases, not independent or blind evidence: the cases were built by the authors after the fault classes were known.\xspace}  % r29.ep.fresh_summary: Appendix D: the fresh-case numbers, qualified (moved from Section 6) over -
\newcommand{\HeldoutCertified}{no\xspace}  % held.certified: battery status over -
\newcommand{\HeldoutCorrupt}{5\xspace}  % held.corrupt: corruptions (a non-empty expected-failing set) over mutation case
\newcommand{\HeldoutCorruptInstantiated}{5\xspace}  % held.corrupt_inst: corruptions the harness instantiated over mutation case
\newcommand{\HeldoutCorruptRejected}{5\xspace}  % held.corrupt_rejected: instantiated corruptions rejected over mutation case
\newcommand{\HeldoutExtraInvariant}{\code{final\_report\_correct}\xspace}  % held.extra_inv: invariant that also failed on the history-row case, beyond the frozen expectation over -
\newcommand{\HeldoutFalseAccept}{0\xspace}  % held.false_accept: instantiated corruptions accepted over mutation case
\newcommand{\HeldoutFalseReject}{0\xspace}  % held.false_reject: instantiated valid cases rejected over mutation case
\newcommand{\HeldoutMet}{8\xspace}  % held.met: frozen expectations met (battery `passed`) over mutation case
\newcommand{\HeldoutMissed}{2\xspace}  % held.missed: frozen expectations not met over mutation case
\newcommand{\HeldoutMonitorErrors}{1\xspace}  % held.monitor: cases ending in MONITOR_ERROR (not a pass) over mutation case
\newcommand{\HeldoutN}{10\xspace}  % held.n: cases in the sealed held-out set over mutation case
\newcommand{\HeldoutRunDate}{2026-09-23\xspace}  % held.date: date of the single run over -
\newcommand{\HeldoutValid}{5\xspace}  % held.valid: valid, invariant-preserving cases (expected-failing empty) over mutation case
\newcommand{\HeldoutValidAccepted}{4\xspace}  % held.valid_accepted: instantiated valid cases accepted over mutation case
\newcommand{\HeldoutValidInstantiated}{4\xspace}  % held.valid_inst: valid cases the harness instantiated over mutation case
\newcommand{\HeldoutValidNotInstantiated}{1\xspace}  % held.valid_not_inst: valid cases the harness could not instantiate over mutation case
\newcommand{\HistReplacedN}{four\xspace}  % hist.replaced: historical attempts not counted and replaced (A2, B, BS, BF, A2S); equal to the independent re-derivation's uncounted attempts, all of them harness errors over attempt
\newcommand{\HistoryWindow}{48\xspace}  % repro.history: history window of the task module (echoes every earlier action) over action
\newcommand{\HolmAtwoP}{1\xspace}  % holm.A2: RETROSPECTIVE Holm-adjusted p over the 3 pre-declared primary tests (not pre-registered) over pair
\newcommand{\HolmBCProspectiveSentence}{Block~BC's family was frozen before any BC outcome, so its registered block-local Holm adjustment is retained as prospective multiplicity control.\xspace}  % r27.holm_bc: r27: BC's block-local Holm, by timing over -
\newcommand{\HolmBP}{0.00586\xspace}  % holm.B: RETROSPECTIVE Holm-adjusted p over the 3 pre-declared primary tests (not pre-registered) over pair
\newcommand{\HolmBSP}{0.0625\xspace}  % holm.BS: RETROSPECTIVE Holm-adjusted p over the 3 pre-declared primary tests (not pre-registered) over pair
\newcommand{\HolmClaimsRetroSentence}{The claims contrasts were individually pre-registered before rollout; because the paper-wide family was finalized only after those outcomes existed, its adjustment of the claims tests is retrospective and is reported as a sensitivity analysis, not prospective multiplicity control.\xspace}  % r27.holm_clm: r27: the claims tests' paper-wide Holm, by timing over -
\newcommand{\HolmFamily}{3\xspace}  % holm.m: size of the retrospective Holm family over test
\newcommand{\HolmFixedClause}{fixed in the frozen ADDENDUM~19\xspace}  % r22.holm_fixed: the paper-wide family's fixing, from its status over -
\newcommand{\HolmMainSentence}{Each prospective block uses its pre-registered local test and multiplicity rule. Appendix~\ref{app:multiplicity} additionally reports a fixed \HolmPaperMWords-slot paper-wide Holm sensitivity family. Because that family was finalized after the claims outcomes existed, its adjustment of the claims and historical tests is retrospective; BC's block-local Holm family was frozen before any BC outcome and is its prospective multiplicity control.\xspace}  % r28.holm_main: r28: the main-text multiplicity paragraph (GPT-6 r20), by timing over -
\newcommand{\HolmPaperAtwo}{1.00\xspace}  % fam.Atwo.holm: paper-wide Holm-adjusted p (retrospective for historical slots) over -
\newcommand{\HolmPaperB}{0.0215\xspace}  % fam.B.holm: paper-wide Holm-adjusted p (retrospective for historical slots) over -
\newcommand{\HolmPaperBBound}{0.0234\xspace}  % fam.b_bonf: Block B's paper-wide Bonferroni bound over -
\newcommand{\HolmPaperBCCueOff}{1.00\xspace}  % fam.BCCueOff.holm: paper-wide Holm-adjusted p (retrospective for historical slots) over -
\newcommand{\HolmPaperBCLiveCue}{0.00293\xspace}  % fam.BCLiveCue.holm: paper-wide Holm-adjusted p (retrospective for historical slots) over -
\newcommand{\HolmPaperBCPairs}{16\xspace}  % fam.n_bc: BC triples, from the spec over pair
\newcommand{\HolmPaperBCSCueOff}{\textit{not admissible}\xspace}  % fam.BCSCueOff.holm: paper-wide Holm-adjusted p (retrospective for historical slots) over -
\newcommand{\HolmPaperBCSLiveCue}{\textit{not admissible}\xspace}  % fam.BCSLiveCue.holm: paper-wide Holm-adjusted p (retrospective for historical slots) over -
\newcommand{\HolmPaperBGCCueOff}{\textit{not admissible}\xspace}  % fam.BGCCueOff.holm: paper-wide Holm-adjusted p (retrospective for historical slots) over -
\newcommand{\HolmPaperBGCOffiOffa}{\textit{not admissible}\xspace}  % fam.BGCOffiOffa.holm: paper-wide Holm-adjusted p (retrospective for historical slots) over -
\newcommand{\HolmPaperBS}{0.281\xspace}  % fam.BS.holm: paper-wide Holm-adjusted p (retrospective for historical slots) over -
\newcommand{\HolmPaperBSMin}{0.0625\xspace}  % fam.bs_min: lowest adjusted p Block BS can reach: A2's p = 1 occupies a later rank, so BS's multiplier is at least 2 over -
\newcommand{\HolmPaperClmB}{1.00\xspace}  % fam.ClmB.holm: paper-wide Holm-adjusted p (retrospective for historical slots) over -
\newcommand{\HolmPaperClmBNeed}{---\xspace}  % fam.ClmB.need: not a local rejection over test
\newcommand{\HolmPaperClmBS}{0.0781\xspace}  % fam.ClmBS.holm: paper-wide Holm-adjusted p (retrospective for historical slots) over -
\newcommand{\HolmPaperClmBSNeed}{four\xspace}  % fam.ClmBS.need: further smaller family p-values the slot needs before (m - rank) p <= alpha can hold (necessary) over test
\newcommand{\HolmPaperFirst}{0.00417\xspace}  % fam.first: first Holm threshold alpha/m over -
\newcommand{\HolmPaperFirstSplits}{$k{:}0$ for $k=9,\ldots,16$ and $k{:}1$ for $k=12,\ldots,15$\xspace}  % fam.first_splits: every favourable split of at most 16 pairs that passes the first Holm step over pair split
\newcommand{\HolmPaperHiAtwo}{1.00\xspace}  % r32.holm.Atwo.hi: highest paper-wide Holm-adjusted p the slot can take (every unresolved slot at p = 1) over -
\newcommand{\HolmPaperHiB}{0.0215\xspace}  % r32.holm.B.hi: highest paper-wide Holm-adjusted p the slot can take (every unresolved slot at p = 1) over -
\newcommand{\HolmPaperHiBCCueOff}{1.00\xspace}  % r32.holm.BCCueOff.hi: highest paper-wide Holm-adjusted p the slot can take (every unresolved slot at p = 1) over -
\newcommand{\HolmPaperHiBCLiveCue}{0.00293\xspace}  % r32.holm.BCLiveCue.hi: highest paper-wide Holm-adjusted p the slot can take (every unresolved slot at p = 1) over -
\newcommand{\HolmPaperHiBS}{0.281\xspace}  % r32.holm.BS.hi: highest paper-wide Holm-adjusted p the slot can take (every unresolved slot at p = 1) over -
\newcommand{\HolmPaperHiClmB}{1.00\xspace}  % r32.holm.ClmB.hi: highest paper-wide Holm-adjusted p the slot can take (every unresolved slot at p = 1) over -
\newcommand{\HolmPaperHiClmBS}{0.0781\xspace}  % r32.holm.ClmBS.hi: highest paper-wide Holm-adjusted p the slot can take (every unresolved slot at p = 1) over -
\newcommand{\HolmPaperLoAtwo}{1.00\xspace}  % r32.holm.Atwo.lo: lowest paper-wide Holm-adjusted p the slot can take (every unresolved slot at p = 0) over -
\newcommand{\HolmPaperLoB}{0.0215\xspace}  % r32.holm.B.lo: lowest paper-wide Holm-adjusted p the slot can take (every unresolved slot at p = 0) over -
\newcommand{\HolmPaperLoBCCueOff}{1.00\xspace}  % r32.holm.BCCueOff.lo: lowest paper-wide Holm-adjusted p the slot can take (every unresolved slot at p = 0) over -
\newcommand{\HolmPaperLoBCLiveCue}{0.00293\xspace}  % r32.holm.BCLiveCue.lo: lowest paper-wide Holm-adjusted p the slot can take (every unresolved slot at p = 0) over -
\newcommand{\HolmPaperLoBS}{0.281\xspace}  % r32.holm.BS.lo: lowest paper-wide Holm-adjusted p the slot can take (every unresolved slot at p = 0) over -
\newcommand{\HolmPaperLoClmB}{1.00\xspace}  % r32.holm.ClmB.lo: lowest paper-wide Holm-adjusted p the slot can take (every unresolved slot at p = 0) over -
\newcommand{\HolmPaperLoClmBS}{0.0781\xspace}  % r32.holm.ClmBS.lo: lowest paper-wide Holm-adjusted p the slot can take (every unresolved slot at p = 0) over -
\newcommand{\HolmPaperM}{12\xspace}  % fam.m: size of the paper-wide Holm family (fixed before any new block ran) over test
\newcommand{\HolmPaperMWords}{twelve\xspace}  % fam.m_words: in words over test
\newcommand{\HolmPaperPendingN}{0\xspace}  % fam.pending_n: unresolved slots of the family over test
\newcommand{\HolmPaperPendingWords}{0\xspace}  % fam.pending_words: in words over test
\newcommand{\HolmPaperRCAdjusted}{0.0469\xspace}  % fam.rc_adjusted: Holm-adjusted p of two balanced adjacent gains at the latest ranks that let them pass over -
\newcommand{\HolmPaperRCText}{Under ordered outcomes, the adjacent gains divide at most 16 favorable discordances. Neither 8--0 contrast passes the first Holm threshold, but both can survive later steps if sufficiently many other family tests reject: with six smaller family $p$-values rejecting first, two 8--0 contrasts ($p=0.00781$ each) have Holm-adjusted $p=0.0469$. Paper-wide support therefore depends on the complete family.\xspace}  % fam.rc_text: the ordered-gains fact for the spec's size over -
\newcommand{\HolmPaperRejected}{2\xspace}  % fam.rejected: paper-wide Holm rejections over test
\newcommand{\HolmPaperSlotTen}{\textit{not admissible}\xspace}  % fam.SlotTen.holm: paper-wide Holm-adjusted p (retrospective for historical slots) over -
\newcommand{\HolmPaperSource}{ADDENDUM~19 \S5\xspace}  % fam.source: where the family is fixed; 'draft' until ADDENDUM 19 is in the verified frozen pre-registration over -
\newcommand{\HolmPaperStatus}{12 of 12 resolved\xspace}  % fam.status: slots resolved so far over slot
\newcommand{\HolmPaperSurvivalFacts}{(7) Every slot of the family is resolved; the adjusted values are in Table~\ref{tab:tests}.\xspace}  % r32.holm_facts: r32: appendix fact (7): attainable Holm ranges over -
\newcommand{\IndepClinicAtwoSC}{8\xspace}  % slot.cell.A2.S-C.clinic: A2 S-C: evaluator successes whose booked clinic the independent scorer confirms over counted success
\newcommand{\IndepClinicAtwoSLtwo}{7\xspace}  % slot.cell.A2.S-L2.clinic: A2 S-L2: evaluator successes whose booked clinic the independent scorer confirms over counted success
\newcommand{\IndepClinicAtwoSLzero}{2\xspace}  % slot.cell.A2.S-L0.clinic: A2 S-L0: evaluator successes whose booked clinic the independent scorer confirms over counted success
\newcommand{\IndepClinicAtwoSSC}{2\xspace}  % slot.cell.A2S.S-C.clinic: A2S S-C: evaluator successes whose booked clinic the independent scorer confirms over counted success
\newcommand{\IndepClinicAtwoSSLtwo}{4\xspace}  % slot.cell.A2S.S-L2.clinic: A2S S-L2: evaluator successes whose booked clinic the independent scorer confirms over counted success
\newcommand{\IndepClinicAtwoSSLzero}{1\xspace}  % slot.cell.A2S.S-L0.clinic: A2S S-L0: evaluator successes whose booked clinic the independent scorer confirms over counted success
\newcommand{\IndepClinicBFFRXOffA}{0\xspace}  % slot.cell.BF.FRX-OFF-A.clinic: BF FRX-OFF-A: evaluator successes whose booked clinic the independent scorer confirms over counted success
\newcommand{\IndepClinicBFFRXOnI}{1\xspace}  % slot.cell.BF.FRX-ON-I.clinic: BF FRX-ON-I: evaluator successes whose booked clinic the independent scorer confirms over counted success
\newcommand{\IndepClinicBFRXOffA}{0\xspace}  % slot.cell.B.FRX-OFF-A.clinic: B FRX-OFF-A: evaluator successes whose booked clinic the independent scorer confirms over counted success
\newcommand{\IndepClinicBFRXOnA}{10\xspace}  % slot.cell.B.FRX-ON-A.clinic: B FRX-ON-A: evaluator successes whose booked clinic the independent scorer confirms over counted success
\newcommand{\IndepClinicBFRXOnI}{3\xspace}  % slot.cell.B.FRX-ON-I.clinic: B FRX-ON-I: evaluator successes whose booked clinic the independent scorer confirms over counted success
\newcommand{\IndepClinicBSFRXOffA}{0\xspace}  % slot.cell.BS.FRX-OFF-A.clinic: BS FRX-OFF-A: evaluator successes whose booked clinic the independent scorer confirms over counted success
\newcommand{\IndepClinicBSFRXOnA}{6\xspace}  % slot.cell.BS.FRX-ON-A.clinic: BS FRX-ON-A: evaluator successes whose booked clinic the independent scorer confirms over counted success
\newcommand{\IndepClinicBSFRXOnI}{2\xspace}  % slot.cell.BS.FRX-ON-I.clinic: BS FRX-ON-I: evaluator successes whose booked clinic the independent scorer confirms over counted success
\newcommand{\IndepFullAtwoSC}{0\xspace}  % slot.cell.A2.S-C.full: A2 S-C: evaluator successes with all five invariants independently resolved over counted success
\newcommand{\IndepFullAtwoSLtwo}{0\xspace}  % slot.cell.A2.S-L2.full: A2 S-L2: evaluator successes with all five invariants independently resolved over counted success
\newcommand{\IndepFullAtwoSLzero}{0\xspace}  % slot.cell.A2.S-L0.full: A2 S-L0: evaluator successes with all five invariants independently resolved over counted success
\newcommand{\IndepFullAtwoSSC}{0\xspace}  % slot.cell.A2S.S-C.full: A2S S-C: evaluator successes with all five invariants independently resolved over counted success
\newcommand{\IndepFullAtwoSSLtwo}{0\xspace}  % slot.cell.A2S.S-L2.full: A2S S-L2: evaluator successes with all five invariants independently resolved over counted success
\newcommand{\IndepFullAtwoSSLzero}{0\xspace}  % slot.cell.A2S.S-L0.full: A2S S-L0: evaluator successes with all five invariants independently resolved over counted success
\newcommand{\IndepFullBFFRXOffA}{0\xspace}  % slot.cell.BF.FRX-OFF-A.full: BF FRX-OFF-A: evaluator successes with all five invariants independently resolved over counted success
\newcommand{\IndepFullBFFRXOnI}{0\xspace}  % slot.cell.BF.FRX-ON-I.full: BF FRX-ON-I: evaluator successes with all five invariants independently resolved over counted success
\newcommand{\IndepFullBFRXOffA}{0\xspace}  % slot.cell.B.FRX-OFF-A.full: B FRX-OFF-A: evaluator successes with all five invariants independently resolved over counted success
\newcommand{\IndepFullBFRXOnA}{0\xspace}  % slot.cell.B.FRX-ON-A.full: B FRX-ON-A: evaluator successes with all five invariants independently resolved over counted success
\newcommand{\IndepFullBFRXOnI}{0\xspace}  % slot.cell.B.FRX-ON-I.full: B FRX-ON-I: evaluator successes with all five invariants independently resolved over counted success
\newcommand{\IndepFullBSFRXOffA}{0\xspace}  % slot.cell.BS.FRX-OFF-A.full: BS FRX-OFF-A: evaluator successes with all five invariants independently resolved over counted success
\newcommand{\IndepFullBSFRXOnA}{0\xspace}  % slot.cell.BS.FRX-ON-A.full: BS FRX-ON-A: evaluator successes with all five invariants independently resolved over counted success
\newcommand{\IndepFullBSFRXOnI}{0\xspace}  % slot.cell.BS.FRX-ON-I.full: BS FRX-ON-I: evaluator successes with all five invariants independently resolved over counted success
\newcommand{\InjAckStep}{16\xspace}  % coh.inj_ack: A2S S-C s10: notice dismissed over step
\newcommand{\InjCommitStep}{41\xspace}  % coh.inj_commit: A2S S-C s10: commit (trajectory step) over step
\newcommand{\InjRepeatStep}{20\xspace}  % coh.inj_repeat: A2S S-C s10: notice shown again over step
\newcommand{\InjSeed}{10\xspace}  % coh.inj_seed: the episode's seed over seed
\newcommand{\InstructionSha}{\texttt{66260588}\xspace}  % pre.instruction_sha: sha256 prefix of the task module's default instruction text (TASK['instruction']), as pinned in the manifest over -
\newcommand{\IntroResultsR}{In claims approval, Opus re-read the authoritative record after the silent change in all \BlockClmBClmOffAN{} OFF-A episodes and succeeded \BlockClmBClmOffAPassFrac{} without a review-step panel. Sonnet did so in \BlockClmBSOffReread/\BlockClmBSClmOffAN{} OFF-A episodes and succeeded on \BlockClmBSClmOffAPassFrac{} without versus \BlockClmBSClmOnAPassFrac{} with review-step re-exposure (\BlockClmBSOnOffRescue{} rescues, \BlockClmBSOnOffHarm{} harms, \BlockClmBSOnOffTie{} ties; $p=\BlockClmBSOnOffP$): for Sonnet, the panel increased full-task success at the registered local level. The instruction defines correctness by the policy value ``\ClmInstructionPhrase,'' which may itself encourage checking. In clinic booking, Opus succeeded on \BlockBCFRXOffAPassFrac{} no-panel, \BlockBCFRXCueAPassFrac{} cue-and-link and \BlockBCFRXLiveAPassFrac{} current-value instances; the prospective LIVE--CUE contrast gives \BlockBCLiveCueRescue{} rescues, \BlockBCLiveCueHarm{} harms and \BlockBCLiveCueTie{} ties (block-local Holm $p=\BlockBCLiveCueHolmLocal$), and CUE--OFF has block-local Holm $p=\BlockBCCueOffHolmLocal$. At the registered block-local level, displaying the current location increased success relative to this cue-and-link panel. The CUE--OFF contrast did not reject; this does not establish absence of a cue effect. Contradiction, salience, and reduced verification effort remain possible explanations.\xspace}  % r31.intro: r31: the introduction's prospective-results paragraph over -
\newcommand{\IntroResultsS}{In clinic booking, Opus succeeded on \BlockBCFRXOffAPassFrac{} instances with no panel, \BlockBCFRXCueAPassFrac{} with a cue-and-link panel and \BlockBCFRXLiveAPassFrac{} with the current value shown. The pre-registered primary contrast, value versus cue (LIVE--CUE), gives \BlockBCLiveCueRescue{} rescues, \BlockBCLiveCueHarm{} harms and \BlockBCLiveCueTie{} ties (block-local Holm $p=\BlockBCLiveCueHolmLocal$, paper-wide Holm $p=\BlockBCLiveCueHolmPaper$); cue versus no panel (CUE--OFF) has block-local Holm $p=\BlockBCCueOffHolmLocal$. At the registered block-local level, displaying the current location increased success relative to this cue-and-link panel. The CUE--OFF contrast did not reject; this does not establish absence of a cue effect. Contradiction, salience, and reduced verification effort remain possible explanations. In claims approval, Opus re-read the changed record in all \BlockClmBClmOffAN{} no-panel episodes and succeeded on \BlockClmBClmOffAPassFrac; Sonnet re-read it in \BlockClmBSOffReread/\BlockClmBSClmOffAN{} and succeeded on \BlockClmBSClmOffAPassFrac{} without versus \BlockClmBSClmOnAPassFrac{} with review-step re-exposure (\BlockClmBSOnOffRescue{} rescues, \BlockClmBSOnOffHarm{} harms, \BlockClmBSOnOffTie{} ties; $p=\BlockClmBSOnOffP$): for Sonnet, the panel increased full-task success at the registered local level. That $p$ is its registered block-local test; the \HolmPaperMWords-test paper-wide Holm family, finalized after the claims outcomes, adjusts it to $p=\HolmPaperClmBS$. The instruction defines correctness by the policy value ``\ClmInstructionPhrase,'' which may itself encourage checking.\xspace}  % r37f.intro: r37 final reviews: the introduction's prospective-results paragraph over -
\newcommand{\KPairs}{8\xspace}  % spec.k: count over pair
\newcommand{\LambdaShape}{0.5\xspace}  % man.lambda: shaping weight over -
\newcommand{\LeakAuditWhere}{it is in the supplement\xspace}  % supp.leak_where: whether the leak-audit record ships over -
\newcommand{\LeakBrowserAttempts}{8\xspace}  % leak.browser_attempts: count over attempt
\newcommand{\LeakCanaries}{5\xspace}  % leak.canaries: count over canary
\newcommand{\LeakCanaryList}{a partial trajectory, the event log, a certificate, the pre-registration and a file on the orchestration volume inside the portal container\xspace}  % leak.canary_list: the canary keys, in prose over canary
\newcommand{\LeakDate}{2026-09-21\xspace}  % leak.date: date over -
\newcommand{\LeakDocumentedChannels}{3\xspace}  % leak.documented_channels: count of documented, permitted channels over channel
\newcommand{\LeakLeakedFrom}{0\xspace}  % leak.leaked_from: count over channel
\newcommand{\LeakModelReads}{5\xspace}  % leak.model_reads: count over read
\newcommand{\LeakOsAttempts}{15\xspace}  % leak.os_attempts: count over attempt
\newcommand{\LeakPolicyUser}{\texttt{envos-policy}\xspace}  % leak.policy_user: unix user over -
\newcommand{\LeakVerdict}{\textsc{pass}\xspace}  % leak.verdict: verdict over -
\newcommand{\LiveUsedN}{0\xspace}  % r22.live_used: manuscript macros (transitively) read from a live entry over macro
\newcommand{\LiveUsedText}{no macro the manuscript uses is read from a live entry\xspace}  % r22.live_used_text: the live-entry check, stated over -
\newcommand{\MBClaimsScopeBase}{6\xspace}  % r29.mb.claims.scope_base: r29 lane B matched comparison (post hoc) over case
\newcommand{\MBClaimsScopeN}{12\xspace}  % r29.mb.claims.scope_n: r29 lane B matched comparison (post hoc) over case
\newcommand{\MBClaimsScopeProt}{10\xspace}  % r29.mb.claims.scope_prot: r29 lane B matched comparison (post hoc) over case
\newcommand{\MBClinicBaseCtlAcc}{9\xspace}  % r29.mb.clinic.base_acc: r29 lane B matched comparison (post hoc) over case
\newcommand{\MBClinicBaseFR}{\code{V08}\xspace}  % r29.mb.clinic_base_fr: clinic baseline false rejections over -
\newcommand{\MBClinicBaseLines}{143\xspace}  % r29.mb.clinic.base_lines: r29 lane B matched comparison (post hoc) over line
\newcommand{\MBClinicBaseRej}{11\xspace}  % r29.mb.clinic.base_rej: r29 lane B matched comparison (post hoc) over case
\newcommand{\MBClinicCorr}{18\xspace}  % r29.mb.clinic.cor: r29 lane B matched comparison (post hoc) over case
\newcommand{\MBClinicCtl}{10\xspace}  % r29.mb.clinic.ctl: r29 lane B matched comparison (post hoc) over case
\newcommand{\MBClinicImplRej}{15\xspace}  % r29.mb.clinic.impl_rej: r29 lane B matched comparison (post hoc) over case
\newcommand{\MBClinicJoint}{14\xspace}  % r29.mb.clinic.joint: r29 lane B matched comparison (post hoc) over case
\newcommand{\MBClinicProtCtlAcc}{10\xspace}  % r29.mb.clinic.prot_acc: r29 lane B matched comparison (post hoc) over case
\newcommand{\MBClinicRegRej}{16\xspace}  % r29.mb.clinic.reg_rej: r29 lane B matched comparison (post hoc) over case
\newcommand{\MBClinicScopeBase}{11\xspace}  % r29.mb.clinic.scope_base: r29 lane B matched comparison (post hoc) over case
\newcommand{\MBClinicScopeN}{12\xspace}  % r29.mb.clinic.scope_n: r29 lane B matched comparison (post hoc) over case
\newcommand{\MBClinicScopeProt}{11\xspace}  % r29.mb.clinic.scope_prot: r29 lane B matched comparison (post hoc) over case
\newcommand{\MBClinicTopSourceN}{14\xspace}  % r29.mb.clinic.top_src: r29 lane B matched comparison (post hoc) over case
\newcommand{\MBDevBC}{16\xspace}  % r29.mb.clinic.dev_bc: r29 lane B matched comparison (post hoc) over archive
\newcommand{\MBDevN}{92\xspace}  % r29.mb.clinic.dev_n: r29 lane B matched comparison (post hoc) over archive
\newcommand{\MBRunUTC}{10:01Z\xspace}  % r29.mb.run_utc: clinic baseline's one run over -
\newcommand{\MBSealUTC}{2026-09-24 10:00Z\xspace}  % r29.mb.seal_utc: clinic baseline sealed over -
\newcommand{\ManifestBPaths}{29\xspace}  % man.b.paths: count of pinned digests over repo path
\newcommand{\ManifestImages}{2\xspace}  % man.images: count of pinned image ids over container image
\newcommand{\ManifestPaths}{29\xspace}  % man.paths: count of pinned digests over repo path
\newcommand{\ManifestShaAtwo}{\texttt{b66756ff}\xspace}  % man.sha: sha256 prefix over -
\newcommand{\MatchedAppendixText}{\paragraph{The same comparison on both workflows.} After the sealed challenge and the check above, we asked what the protocol adds over a fair simple checker on \emph{identical} evidence and scored properties. For clinic we wrote \code{clinic\_baseline.py} (\MBClinicBaseLines{} lines, standard library), the counterpart of the claims baseline: it asks whether the session row changed exactly once, after its old location was served in the same login session and inside the agent's own recorded request, and whether any served page contradicts the change (on L0, whether nothing changed); whether exactly one commit and one patient row followed the change; whether the booked clinic equals the session's location at the commit (the nearest-slot term is not archived, so it reports fail or unresolved, never pass); and whether the report matches the committed record. It does not check delivery, the arm served, collateral rows, the confirm state or archive completeness. It was developed only on \MBDevN{} clinic-family run archives that are not sources of any challenge case, sealed (with the table's decision definitions) at \MBSealUTC, and run once on the challenge's cases at \MBRunUTC; nothing was tuned afterwards. Before writing it, its author had read the challenge's expected verdicts, the sealed tools' recorded outputs and the unmodified control archives, but not the mutation code. \emph{Disclosure:} \MBDevBC{} of the \MBDevN{} development archives were Block~BC archives written while that block was running; the development check compared the baseline only with their archived evaluator scores, no number from them appears in this paper, and BC's reading is selected mechanically by its frozen rule. The sealed challenge's joint figure, \MBClinicJoint{} of \MBClinicCorr{} corruptions, is the set both validity readings reject; the protocol rows of Table~\ref{tab:matched} take one reading at a time. The claims baseline's in-scope misses reflect implementation choices a careful checker need not make (nearest-request attribution, timestamp ordering, no event log, counting history rows rather than change requests); the clinic baseline, which reads more raw sources, matched the protocol within its scope. The added value this shows is breadth of checked properties and, on claims, a more robust causal chain than one simple checker; it does not show that a simple checker cannot match the causal chain.\xspace}  % r29.mb.app: Appendix: the matched comparison over -
\newcommand{\MatchedCaption}{\textbf{The protocol against a simple raw-log baseline} (post hoc, author-built, not blind; separate from Table~\ref{tab:layers}). Same raw evidence and scored properties. Controls accepted; corruptions rejected (not counted, or counted with the corrupted invariant flagged), in brackets those in the baseline's declared scope. Clinic protocol rows are derived from the sealed tools' recorded outputs; the claims pipeline voids \code{C09b} as invalid rather than failing its single-commit term. Every case: Appendix~\ref{app:posthoc}.\xspace}  % r29.mb.caption: the matched table's caption over -
\newcommand{\MatchedLimitClause}{the raw-log baseline comparisons are post hoc and author-built (most corruptions from one archive: \MBClinicTopSourceN/\MBClinicCorr{} clinic, \ValTopSourceN/\ValCorrupt{} claims), so incremental coverage is case by case, not a rate; the reconstruction and repaired checker were written knowing the fault classes and read the same archives: independent code, not independent evidence\xspace}  % r29.mb.limit: Limitations: the matched comparison's scope over -
\newcommand{\MatchedMainFour}{\paragraph{Against a simple raw-log baseline.} This comparison is post hoc, author-built and not blind: after the sealed result, which stands unchanged, we wrote a simple checker rebuilding each verdict from the same raw state, access log and served pages, with the pipeline in view, and sealed each before its one run (Table~\ref{tab:matched}). No protocol path rejected a control; the clinic baseline rejected one. Within the baseline's declared scope both rejected \MBClinicScopeProt{} of \MBClinicScopeN{} clinic corruptions; on claims the pipeline rejected \MBClaimsScopeProt{} and the baseline \MBClaimsScopeBase{} of \MBClaimsScopeN. A careful simple checker thus reproduced most narrow clinic checks; \envos adds breadth (delivery, served arm, collateral state) that such a checker could be extended to cover, and the baseline alone caught one case (Appendix~\ref{app:posthoc}). As we built both cases and checkers, only the external challenge above tests independent construction, and there the pipeline counted \ExtClaimsPipeFA{} of \ExtClaimsCor{} claims and \ExtClinicPipeFA{} of \ExtClinicCor{} clinic corruptions as clean.\xspace}  % r37f.matched4: r37 final reviews: Section 6: the post-hoc baseline comparison over -
\newcommand{\MatchedMainParagraph}{\paragraph{Against a simple raw-log baseline (post hoc, author-built, not blind).} After the sealed result, which stands unchanged, we compared the protocol with a simple checker that rebuilds each verdict from the same raw world state, access log and served pages, on the same cases and scored properties (Table~\ref{tab:matched}): the sealed challenge's clinic cases, their recorded outputs re-tabulated, not re-run, and \ValCases{} claims cases we built; we wrote expectations and baselines with the pipeline in view and sealed each before its one run. No protocol path rejected a control; the clinic baseline rejected one (a space before a report's colon). Within the baseline's declared scope both rejected \MBClinicScopeProt{} of \MBClinicScopeN{} clinic corruptions; on claims the pipeline rejected \MBClaimsScopeProt{} and the baseline \MBClaimsScopeBase{} of \MBClaimsScopeN, the baseline crediting the change to the nearest request and ordering events by timestamp. On clinic, a carefully written simple checker therefore reproduced most of the narrow causal-chain checks within its declared scope. EnvOS's additional coverage is primarily systematic breadth (delivery, served arm, collateral state, report consistency and completeness), while on claims the operational pipeline also reconstructs more of the causal ordering than this simple baseline. This comparison does not show that a simple checker could not be extended to match that coverage; the baseline alone caught one case (a duplicate commit in the access log only, which the claims single-commit term accepts).\xspace}  % r29.mb.main: Section 6: the matched comparison (post hoc) over -
\newcommand{\MatchedMainThree}{\paragraph{Against a simple raw-log baseline (post hoc, author-built, not blind).} After the sealed result, which stands unchanged, we compared the protocol with a simple checker rebuilding each verdict from the same raw state, access log and served pages (Table~\ref{tab:matched}; written with the pipeline in view, each sealed before its one run). No protocol path rejected a control; the clinic baseline rejected one. Within the baseline's declared scope both rejected \MBClinicScopeProt{} of \MBClinicScopeN{} clinic corruptions; on claims the pipeline rejected \MBClaimsScopeProt{} and the baseline \MBClaimsScopeBase{} of \MBClaimsScopeN. A carefully written simple checker thus reproduced most narrow clinic checks; EnvOS adds breadth (delivery, served arm, collateral state), which a simple checker might be extended to match; the baseline alone caught one case (Appendix~\ref{app:posthoc}).\xspace}  % r34.ext.matched3: r34 external challenge: Section 6: the post-hoc baseline comparison (compact) over -
\newcommand{\MemoCarryFrac}{19/19\xspace}  % audit.memo_carry: k/n over counted rollout
\newcommand{\MemoMaxChars}{300\xspace}  % repro.memo_max: memo truncation (NOTE_MAX_CHARS) over character
\newcommand{\MinRejectDiscordant}{6\xspace}  % stat.min_reject_discordant: smallest one-way discordant count with p < alpha = 0.05 (2 * 0.5^d) over pair
\newcommand{\ModelAttempts}{82\xspace}  % rules.attempts: attempts in the five current model-block logs over rollout
\newcommand{\ModelCounted}{78\xspace}  % rules.counted: counted rows in the five current model-block logs over counted rollout
\newcommand{\ModelRunDirs}{82\xspace}  % rules.run_dirs: run directories on disk, each matching exactly one log row over run directory
\newcommand{\MutationDevChecks}{11\xspace}  % mut.dev.checks: count over mutation check
\newcommand{\MutationDevFailed}{0\xspace}  % mut.dev.failed: count over mutation check
\newcommand{\MutationsDev}{11\xspace}  % mut.dev.n: count over mutation
\newcommand{\MutationsDevControls}{2\xspace}  % mut.dev.controls: count of positive controls (a reference episode must still pass) over mutation
\newcommand{\MutationsDevCorruptions}{9\xspace}  % mut.dev.corruptions: count of corruptions the checker must reject over mutation
\newcommand{\MutationsHeldout}{10\xspace}  % mut.heldout.n: count (sealed by sha256) over corrupted world
\newcommand{\MutationsHeldoutSha}{\texttt{d1ac0f83}\xspace}  % mut.heldout.sha: sha256 prefix over -
\newcommand{\NDefectsBlockB}{4\xspace}  % defects.blockB: count over defect
\newcommand{\NDefectsModelAttributable}{7\xspace}  % defects.pre_rollout: count over defect
\newcommand{\NDefectsTotal}{11\xspace}  % defects.total: count over defect
\newcommand{\NDefectsTotalWords}{Eleven\xspace}  % defects.total_words: defects, in words over defect
\newcommand{\NFamiliesEndToEnd}{2\xspace}  % r21.families: clinic (historical blocks, audited) + claims iff CLM-B completed, eligible, independently scored and re-derived over task family
\newcommand{\NFamiliesEndToEndWords}{two\xspace}  % r21.families_words: in words over task family
\newcommand{\NeutralCertFiles}{10\xspace}  % neutral.cert_files: certificate files whose filler check ran on the module's own instance S-train-0 over certificate
\newcommand{\NeutralInstances}{18\xspace}  % neutral.instances: evaluated instances (seeds with a counted row) over instance
\newcommand{\NeutralMailCalendarHits}{0\xspace}  % neutral.hits: instances whose intake mail or calendar entry names a clinic over instance
\newcommand{\NewcombeCorrectedSha}{\texttt{54f6d791e7c4}\xspace}  % erratum.nc.module: sha256 prefix of the corrected envos/stats.py the recomputation imported over -
\newcommand{\NewcombeErratumApplies}{0\xspace}  % erratum.nc.applies: intervals whose counts have ad > bc (the only case the correction changes) over interval
\newcommand{\NewcombeErratumChanged}{0\xspace}  % erratum.nc.changed: recomputed intervals that differ from the printed ones at 4 decimals over interval
\newcommand{\NewcombeErratumMaxDiff}{below $10^{-9}$\xspace}  % erratum.nc.maxdiff: largest absolute change of any bound over -
\newcommand{\NewcombeErratumN}{5\xspace}  % erratum.nc.n: historical Newcombe intervals recomputed over interval
\newcommand{\NewcombeErratumNWords}{five\xspace}  % erratum.nc.n_words: in words over interval
\newcommand{\NonReadCallsFable}{1\xspace}  % repro.nonread_fable: Fable non-Read tool calls over tool call
\newcommand{\NonReadCallsOpus}{6\xspace}  % repro.nonread_opus: Opus non-Read tool calls over tool call
\newcommand{\NonReadCallsSonnet}{1591\xspace}  % repro.nonread_sonnet: Sonnet tool calls other than Read (names archived; whether each ran is not) over tool call
\newcommand{\NonReadClaimsClause}{in the historical blocks Sonnet~5 emitted \NonReadCallsSonnet; in the claims blocks Opus~5 emitted \CensusNonReadOpus{} and Sonnet~5 \CensusNonReadSonnet, Appendix~\ref{app:claimsspec}\xspace}  % r29.cs.nonread_clause: limitations: the claims census over -
\newcommand{\NonReadStepsSonnet}{801\xspace}  % repro.nonread_sonnet_steps: steps with one over policy step
\newcommand{\OfflineTestsPassed}{578\xspace}  % pre.offline_tests: count (latest addendum) over test
\newcommand{\OrigBSAgainst}{0\xspace}  % rules.Orig.BS.against: discordant against over pair
\newcommand{\OrigBSFRXOffAFrac}{0/10\xspace}  % rules.Orig.BS.FRX-OFF-A: BS FRX-OFF-A under original_screenshot_rule: observed k/n (voided rows unobserved, not imputed) over counted rollout
\newcommand{\OrigBSFRXOnAFrac}{6/7\xspace}  % rules.Orig.BS.FRX-ON-A: BS FRX-ON-A under original_screenshot_rule: observed k/n (voided rows unobserved, not imputed) over counted rollout
\newcommand{\OrigBSFRXOnIFrac}{0/1\xspace}  % rules.Orig.BS.FRX-ON-I: BS FRX-ON-I under original_screenshot_rule: observed k/n (voided rows unobserved, not imputed) over counted rollout
\newcommand{\OrigBSFor}{6\xspace}  % rules.Orig.BS.for: discordant in the hypothesised direction over pair
\newcommand{\OrigBSP}{0.0312\xspace}  % rules.Orig.BS.p: exact two-sided sign test over pair
\newcommand{\OrigBSPairs}{7\xspace}  % rules.Orig.BS.pairs: BS pairs observed under original_screenshot_rule over pair
\newcommand{\OrigBSTied}{1\xspace}  % rules.Orig.BS.tied: tied over pair
\newcommand{\OrigBSUnobserved}{5\xspace}  % rules.Orig.BS.unobserved: BS rows original_screenshot_rule would have voided (outcome of their replacements unobserved) over counted rollout
\newcommand{\OrigLitBSAgainst}{0\xspace}  % rules.OrigLit.BS.against: discordant against over pair
\newcommand{\OrigLitBSFRXOffAFrac}{0/10\xspace}  % rules.OrigLit.BS.FRX-OFF-A: BS FRX-OFF-A under original_screenshot_rule_literal: observed k/n (voided rows unobserved, not imputed) over counted rollout
\newcommand{\OrigLitBSFRXOnAFrac}{6/6\xspace}  % rules.OrigLit.BS.FRX-ON-A: BS FRX-ON-A under original_screenshot_rule_literal: observed k/n (voided rows unobserved, not imputed) over counted rollout
\newcommand{\OrigLitBSFRXOnIFrac}{0/0\xspace}  % rules.OrigLit.BS.FRX-ON-I: BS FRX-ON-I under original_screenshot_rule_literal: observed k/n (voided rows unobserved, not imputed) over counted rollout
\newcommand{\OrigLitBSFor}{6\xspace}  % rules.OrigLit.BS.for: discordant in the hypothesised direction over pair
\newcommand{\OrigLitBSP}{0.0312\xspace}  % rules.OrigLit.BS.p: exact two-sided sign test over pair
\newcommand{\OrigLitBSPairs}{6\xspace}  % rules.OrigLit.BS.pairs: BS pairs observed under original_screenshot_rule_literal over pair
\newcommand{\OrigLitBSTied}{0\xspace}  % rules.OrigLit.BS.tied: tied over pair
\newcommand{\OrigLitBSUnobserved}{7\xspace}  % rules.OrigLit.BS.unobserved: BS rows original_screenshot_rule_literal would have voided (outcome of their replacements unobserved) over counted rollout
\newcommand{\OswClmBLzeroFailed}{0\xspace}  % osw.ClmB.Lzero.Failed: OSWorld-2.0-style Failed for L0 over counted rollout
\newcommand{\OswClmBLzeroHandled}{0\xspace}  % osw.ClmB.Lzero.Handled: OSWorld-2.0-style Handled for L0 over counted rollout
\newcommand{\OswClmBLzeroN}{1\xspace}  % osw.ClmB.Lzero.N: OSWorld-2.0-style N for L0 over counted rollout
\newcommand{\OswClmBLzeroPartial}{4/4 (1.00)\xspace}  % osw.ClmB.Lzero.Partial: OSWorld-2.0-style Partial for L0 over counted rollout
\newcommand{\OswClmBLzeroSucc}{1\xspace}  % osw.ClmB.Lzero.Succ: OSWorld-2.0-style Succ for L0 over counted rollout
\newcommand{\OswClmBLzeroUntested}{1\xspace}  % osw.ClmB.Lzero.Untested: OSWorld-2.0-style Untested for L0 over counted rollout
\newcommand{\OswClmBOffAFailed}{0\xspace}  % osw.ClmB.OffA.Failed: OSWorld-2.0-style Failed for OFF-A over counted rollout
\newcommand{\OswClmBOffAHandled}{10\xspace}  % osw.ClmB.OffA.Handled: OSWorld-2.0-style Handled for OFF-A over counted rollout
\newcommand{\OswClmBOffAN}{10\xspace}  % osw.ClmB.OffA.N: OSWorld-2.0-style N for OFF-A over counted rollout
\newcommand{\OswClmBOffAPartial}{40/40 (1.00)\xspace}  % osw.ClmB.OffA.Partial: OSWorld-2.0-style Partial for OFF-A over counted rollout
\newcommand{\OswClmBOffASucc}{10\xspace}  % osw.ClmB.OffA.Succ: OSWorld-2.0-style Succ for OFF-A over counted rollout
\newcommand{\OswClmBOffAUntested}{0\xspace}  % osw.ClmB.OffA.Untested: OSWorld-2.0-style Untested for OFF-A over counted rollout
\newcommand{\OswClmBOnAFailed}{0\xspace}  % osw.ClmB.OnA.Failed: OSWorld-2.0-style Failed for ON-A over counted rollout
\newcommand{\OswClmBOnAHandled}{10\xspace}  % osw.ClmB.OnA.Handled: OSWorld-2.0-style Handled for ON-A over counted rollout
\newcommand{\OswClmBOnAN}{10\xspace}  % osw.ClmB.OnA.N: OSWorld-2.0-style N for ON-A over counted rollout
\newcommand{\OswClmBOnAPartial}{40/40 (1.00)\xspace}  % osw.ClmB.OnA.Partial: OSWorld-2.0-style Partial for ON-A over counted rollout
\newcommand{\OswClmBOnASucc}{10\xspace}  % osw.ClmB.OnA.Succ: OSWorld-2.0-style Succ for ON-A over counted rollout
\newcommand{\OswClmBOnAUntested}{0\xspace}  % osw.ClmB.OnA.Untested: OSWorld-2.0-style Untested for ON-A over counted rollout
\newcommand{\OswClmBOnIFailed}{0\xspace}  % osw.ClmB.OnI.Failed: OSWorld-2.0-style Failed for ON-I over counted rollout
\newcommand{\OswClmBOnIHandled}{0\xspace}  % osw.ClmB.OnI.Handled: OSWorld-2.0-style Handled for ON-I over counted rollout
\newcommand{\OswClmBOnIN}{3\xspace}  % osw.ClmB.OnI.N: OSWorld-2.0-style N for ON-I over counted rollout
\newcommand{\OswClmBOnIPartial}{12/12 (1.00)\xspace}  % osw.ClmB.OnI.Partial: OSWorld-2.0-style Partial for ON-I over counted rollout
\newcommand{\OswClmBOnISucc}{3\xspace}  % osw.ClmB.OnI.Succ: OSWorld-2.0-style Succ for ON-I over counted rollout
\newcommand{\OswClmBOnIUntested}{3\xspace}  % osw.ClmB.OnI.Untested: OSWorld-2.0-style Untested for ON-I over counted rollout
\newcommand{\OswClmBSLzeroFailed}{0\xspace}  % osw.ClmBS.Lzero.Failed: OSWorld-2.0-style Failed for L0 over counted rollout
\newcommand{\OswClmBSLzeroHandled}{0\xspace}  % osw.ClmBS.Lzero.Handled: OSWorld-2.0-style Handled for L0 over counted rollout
\newcommand{\OswClmBSLzeroN}{1\xspace}  % osw.ClmBS.Lzero.N: OSWorld-2.0-style N for L0 over counted rollout
\newcommand{\OswClmBSLzeroPartial}{4/4 (1.00)\xspace}  % osw.ClmBS.Lzero.Partial: OSWorld-2.0-style Partial for L0 over counted rollout
\newcommand{\OswClmBSLzeroSucc}{1\xspace}  % osw.ClmBS.Lzero.Succ: OSWorld-2.0-style Succ for L0 over counted rollout
\newcommand{\OswClmBSLzeroUntested}{1\xspace}  % osw.ClmBS.Lzero.Untested: OSWorld-2.0-style Untested for L0 over counted rollout
\newcommand{\OswClmBSOffAFailed}{9\xspace}  % osw.ClmBS.OffA.Failed: OSWorld-2.0-style Failed for OFF-A over counted rollout
\newcommand{\OswClmBSOffAHandled}{1\xspace}  % osw.ClmBS.OffA.Handled: OSWorld-2.0-style Handled for OFF-A over counted rollout
\newcommand{\OswClmBSOffAN}{10\xspace}  % osw.ClmBS.OffA.N: OSWorld-2.0-style N for OFF-A over counted rollout
\newcommand{\OswClmBSOffAPartial}{30/40 (0.75)\xspace}  % osw.ClmBS.OffA.Partial: OSWorld-2.0-style Partial for OFF-A over counted rollout
\newcommand{\OswClmBSOffASucc}{1\xspace}  % osw.ClmBS.OffA.Succ: OSWorld-2.0-style Succ for OFF-A over counted rollout
\newcommand{\OswClmBSOffAUntested}{0\xspace}  % osw.ClmBS.OffA.Untested: OSWorld-2.0-style Untested for OFF-A over counted rollout
\newcommand{\OswClmBSOnAFailed}{0\xspace}  % osw.ClmBS.OnA.Failed: OSWorld-2.0-style Failed for ON-A over counted rollout
\newcommand{\OswClmBSOnAHandled}{10\xspace}  % osw.ClmBS.OnA.Handled: OSWorld-2.0-style Handled for ON-A over counted rollout
\newcommand{\OswClmBSOnAN}{10\xspace}  % osw.ClmBS.OnA.N: OSWorld-2.0-style N for ON-A over counted rollout
\newcommand{\OswClmBSOnAPartial}{39/40 (0.98)\xspace}  % osw.ClmBS.OnA.Partial: OSWorld-2.0-style Partial for ON-A over counted rollout
\newcommand{\OswClmBSOnASucc}{9\xspace}  % osw.ClmBS.OnA.Succ: OSWorld-2.0-style Succ for ON-A over counted rollout
\newcommand{\OswClmBSOnAUntested}{0\xspace}  % osw.ClmBS.OnA.Untested: OSWorld-2.0-style Untested for ON-A over counted rollout
\newcommand{\OswClmBSOnIFailed}{0\xspace}  % osw.ClmBS.OnI.Failed: OSWorld-2.0-style Failed for ON-I over counted rollout
\newcommand{\OswClmBSOnIHandled}{0\xspace}  % osw.ClmBS.OnI.Handled: OSWorld-2.0-style Handled for ON-I over counted rollout
\newcommand{\OswClmBSOnIN}{3\xspace}  % osw.ClmBS.OnI.N: OSWorld-2.0-style N for ON-I over counted rollout
\newcommand{\OswClmBSOnIPartial}{12/12 (1.00)\xspace}  % osw.ClmBS.OnI.Partial: OSWorld-2.0-style Partial for ON-I over counted rollout
\newcommand{\OswClmBSOnISucc}{3\xspace}  % osw.ClmBS.OnI.Succ: OSWorld-2.0-style Succ for ON-I over counted rollout
\newcommand{\OswClmBSOnIUntested}{3\xspace}  % osw.ClmBS.OnI.Untested: OSWorld-2.0-style Untested for ON-I over counted rollout
\newcommand{\OswNoGoR}{A pre-registered screenshot-only coordinate-action crossover of the claims workflow stopped at its engineering admission gate before any model rollout: viewport fit failed (18 of 144 page checks did not fit) and legibility failed (4 of 404 values unrecovered at $1536\times864$). It therefore contributes no behavioral evidence, and interface robustness remains untested.\xspace}  % r31.osw: r31: the screenshot-only crossover's registered gate, with its counts (limitations; never a result) over -
\newcommand{\OswNoGoSentence}{A registered screenshot-only variant of the claims workflow stopped at its harness-certification gate before any model rollout (viewport fit and legibility failed at $1536\times864$), so screenshot-only use is untested.\xspace}  % r30.osw_nogo: r30: the screenshot-only crossover's registered G1 gate (limitations clause, never a result) over -
\newcommand{\PSignBOneAgainst}{0.021\xspace}  % pre.b_p_one_against: exact two-sided sign test, 9 vs 1, as stated in ADDENDUM 5 over pair
\newcommand{\PSignEightZero}{0.0078\xspace}  % stat.p_8_0: exact two-sided sign test, 8 vs 0 over pair
\newcommand{\PSignKZero}{0.0078\xspace}  % stat.p_k_0: exact two-sided sign test, 8 vs 0 (every pair one way) over pair
\newcommand{\PSignMinRejectZero}{0.0312\xspace}  % stat.p_minreject_0: exact two-sided sign test, 6 vs 0 over pair
\newcommand{\PSignNineOne}{0.021\xspace}  % stat.p_9_1: exact two-sided sign test, 9 vs 1 over pair
\newcommand{\PSignPreMinZero}{0.0156\xspace}  % stat.p_premin_0: exact two-sided sign test, 7 vs 0 (the pre-registered threshold) over pair
\newcommand{\PSignSevenZero}{0.0156\xspace}  % stat.p_7_0: exact two-sided sign test, 7 vs 0 over pair
\newcommand{\PSignSixZero}{0.0312\xspace}  % stat.p_6_0: exact two-sided sign test, 6 vs 0 over pair
\newcommand{\PairedAtwoCtrlOnly}{1\xspace}  % paired.A2.ctrl_only: only S-C succeeded over pair
\newcommand{\PairedAtwoN}{8\xspace}  % paired.A2.n: count of complete pairs over pair
\newcommand{\PairedAtwoNet}{$-0.13$\xspace}  % paired.A2.net: net paired difference P(treatment) - P(control), ties in the denominator over pair
\newcommand{\PairedAtwoNetCI}{$-0.13$ [$-0.47$, $0.22$]\xspace}  % paired.A2.net_ci: net paired difference with Newcombe (1998, method 10) hybrid-score 95% interval (not exact) over pair
\newcommand{\PairedAtwoP}{1\xspace}  % paired.A2.p: exact two-sided sign test on the discordant pairs over pair
\newcommand{\PairedAtwoSCtrlOnly}{0\xspace}  % paired.A2S.ctrl_only: only S-C succeeded over pair
\newcommand{\PairedAtwoSN}{4\xspace}  % paired.A2S.n: count of complete pairs over pair
\newcommand{\PairedAtwoSNet}{$+0.50$\xspace}  % paired.A2S.net: net paired difference P(treatment) - P(control), ties in the denominator over pair
\newcommand{\PairedAtwoSNetCI}{$+0.50$ [$-0.10$, $0.85$]\xspace}  % paired.A2S.net_ci: net paired difference with Newcombe (1998, method 10) hybrid-score 95% interval (not exact) over pair
\newcommand{\PairedAtwoSP}{0.5\xspace}  % paired.A2S.p: exact two-sided sign test on the discordant pairs (DESCRIPTIVE: no registered test) over pair
\newcommand{\PairedAtwoSTieBoth}{2\xspace}  % paired.A2S.tie_both: both arms succeeded over pair
\newcommand{\PairedAtwoSTieNeither}{0\xspace}  % paired.A2S.tie_neither: neither arm succeeded over pair
\newcommand{\PairedAtwoSTreatOnly}{2\xspace}  % paired.A2S.treat_only: only S-L2 succeeded over pair
\newcommand{\PairedAtwoTieBoth}{7\xspace}  % paired.A2.tie_both: both arms succeeded over pair
\newcommand{\PairedAtwoTieNeither}{0\xspace}  % paired.A2.tie_neither: neither arm succeeded over pair
\newcommand{\PairedAtwoTreatOnly}{0\xspace}  % paired.A2.treat_only: only S-L2 succeeded over pair
\newcommand{\PairedBCtrlOnly}{0\xspace}  % paired.B.ctrl_only: only FRX-OFF-A succeeded over pair
\newcommand{\PairedBN}{10\xspace}  % paired.B.n: count of complete pairs over pair
\newcommand{\PairedBNet}{$+1.00$\xspace}  % paired.B.net: net paired difference P(treatment) - P(control), ties in the denominator over pair
\newcommand{\PairedBNetCI}{$+1.00$ [$0.61$, $1.00$]\xspace}  % paired.B.net_ci: net paired difference with Newcombe (1998, method 10) hybrid-score 95% interval (not exact) over pair
\newcommand{\PairedBP}{0.00195\xspace}  % paired.B.p: exact two-sided sign test on the discordant pairs over pair
\newcommand{\PairedBSCtrlOnly}{0\xspace}  % paired.BS.ctrl_only: only FRX-OFF-A succeeded over pair
\newcommand{\PairedBSN}{10\xspace}  % paired.BS.n: count of complete pairs over pair
\newcommand{\PairedBSNet}{$+0.60$\xspace}  % paired.BS.net: net paired difference P(treatment) - P(control), ties in the denominator over pair
\newcommand{\PairedBSNetCI}{$+0.60$ [$0.20$, $0.83$]\xspace}  % paired.BS.net_ci: net paired difference with Newcombe (1998, method 10) hybrid-score 95% interval (not exact) over pair
\newcommand{\PairedBSNoCapCtrlOnly}{0\xspace}  % paired.BS.nocap.ctrl_only: only FRX-OFF-A succeeded over pair
\newcommand{\PairedBSNoCapN}{8\xspace}  % paired.BS.nocap.n: BS pairs with no action-cap arm over pair
\newcommand{\PairedBSNoCapNetCI}{$+0.63$ [$0.17$, $0.86$]\xspace}  % paired.BS.nocap.net_ci: net paired difference and Newcombe interval without action-cap pairs (retrospective) over pair
\newcommand{\PairedBSNoCapP}{0.0625\xspace}  % paired.BS.nocap.p: exact sign test without action-cap pairs over pair
\newcommand{\PairedBSNoCapTies}{3\xspace}  % paired.BS.nocap.ties: tied over pair
\newcommand{\PairedBSNoCapTreatOnly}{5\xspace}  % paired.BS.nocap.treat_only: only FRX-ON-A succeeded over pair
\newcommand{\PairedBSP}{0.0312\xspace}  % paired.BS.p: exact two-sided sign test on the discordant pairs over pair
\newcommand{\PairedBSTieBoth}{0\xspace}  % paired.BS.tie_both: both arms succeeded over pair
\newcommand{\PairedBSTieNeither}{4\xspace}  % paired.BS.tie_neither: neither arm succeeded over pair
\newcommand{\PairedBSTreatOnly}{6\xspace}  % paired.BS.treat_only: only FRX-ON-A succeeded over pair
\newcommand{\PairedBTieBoth}{0\xspace}  % paired.B.tie_both: both arms succeeded over pair
\newcommand{\PairedBTieNeither}{0\xspace}  % paired.B.tie_neither: neither arm succeeded over pair
\newcommand{\PairedBTreatOnly}{10\xspace}  % paired.B.treat_only: only FRX-ON-A succeeded over pair
\newcommand{\PreAddenda}{19\xspace}  % pre.addenda: count over addendum
\newcommand{\PreBudgetCounted}{18\xspace}  % pre.budget_counted: pre-registered counted budget over rollout
\newcommand{\PreControlFloor}{6/8\xspace}  % pre.control_floor: headline floor (§1 stopping rules) over counted control rollout
\newcommand{\PreMinDiscordant}{7\xspace}  % pre.min_discordant: pre-registered minimum one-way discordant pairs (§1) over pair
\newcommand{\PrecommitSha}{\texttt{c280ce46}\xspace}  % pre.sha: sha256 prefix (current freeze) over -
\newcommand{\PrecommitTaskTextSha}{\texttt{cdce6a1d}\xspace}  % pre.task_text_sha: sha256 prefix of the §4 task text block (instance seed 0) as frozen over -
\newcommand{\PrecommitUnmappedChars}{0\xspace}  % pre.unmapped_chars: count of non-ASCII characters in the pre-registration with no transliteration (must be 0) over character
\newcommand{\ProspCounted}{99\xspace}  % abs.prosp_counted: prospective counted rollouts under an independent audit over counted rollout
\newcommand{\ProspEndpointFull}{99\xspace}  % abs.prosp_full: prospective counted rollouts with every outcome term resolved and agreeing with the evaluator over counted rollout
\newcommand{\ProtocolFreezeClause}{The finalized protocol is frozen for the prospective blocks: \FreezeStatusText.\xspace}  % r22.protocol_clause: the protocol's freeze, stated from its status over -
\newcommand{\ProtocolFreezeSentence}{For each prospective block, the task definition, validity rules, analysis, code manifest, and interpretation templates were hash-frozen before the first rollout; later departures are reported rather than silently incorporated.\xspace}  % r28.freeze: r28: the introduction's freeze sentence (GPT-6 r20) over -
\newcommand{\ProtocolVersion}{2\xspace}  % man.protocol_version: protocol version over -
\newcommand{\PthreeCertCChecks}{40\xspace}  % p3.cert.P3-C: count over check
\newcommand{\PthreeCertLtwoChecks}{60\xspace}  % p3.cert.P3-L2: count over check
\newcommand{\PthreeCertLzeroChecks}{38\xspace}  % p3.cert.P3-L0: count over check
\newcommand{\PthreeCleanFable}{1/1\xspace}  % p3.Fable.clean: pass count over rollout
\newcommand{\PthreeCleanOpus}{1/1\xspace}  % p3.Opus.clean: pass count over rollout
\newcommand{\PthreeControlFable}{1/1\xspace}  % p3.Fable.control: pass count over rollout
\newcommand{\PthreeControlOpus}{1/1\xspace}  % p3.Opus.control: pass count over rollout
\newcommand{\PthreeFailFable}{3/3\xspace}  % p3.Fable.fail: failure count at P3-L2 over rollout
\newcommand{\PthreeFailOpus}{3/3\xspace}  % p3.Opus.fail: failure count at P3-L2 over rollout
\newcommand{\PthreeLtwoNFable}{3\xspace}  % p3.Fable.l2_n: count at P3-L2 over rollout
\newcommand{\PthreeLtwoNOpus}{3\xspace}  % p3.Opus.l2_n: count at P3-L2 over rollout
\newcommand{\PthreeRollouts}{10\xspace}  % p3.rollouts: count over rollout
\newcommand{\PtwoRecertFailed}{P2-C 8; P2-L0 9; P2-L1 18\xspace}  % disp.p2_failed: failed checks of the rejected P2 re-certification over check
\newcommand{\QconfigNote}{\xspace}  % r21.qconfig: mixed-vendor caption, printed only once admission passed and a GPT-6 row is reported over -
\newcommand{\QuoteAFiveSig}{This is a practical-effect guard only; significance comes solely from the pre-declared exact two-sided sign test at alpha = 0.05, positive = OFF failed and ON passed.\xspace}  % r22.q_a5: ADDENDUM 5, minimum effect, verbatim over -
\newcommand{\QuoteAFiveUnchanged}{every interpretation rule of S0-S6\xspace}  % r22.q_a5u: ADDENDUM 5, 'Unchanged', verbatim over -
\newcommand{\QuoteASeventeen}{The rescue contrast is decided by the primary test and is unaffected.\xspace}  % r22.q_a17: ADDENDUM 17, verbatim over -
\newcommand{\QuoteSSix}{The finding is claimed only if the primary test rejects at alpha = 0.05 AND every kept failing run's signature is \code{STALE\_\allowbreak{}APPLIED\_\allowbreak{}UNFLAGGED} AND C2 AND C3 hold in every kept run.\xspace}  % r22.q_s6: S6, first rule, verbatim over -
\newcommand{\ReadingRuleSha}{\texttt{b23e52dbffcf}\xspace}  % r21.rule_sha: sha256 prefix over the source of every function the interpretation depends on over -
\newcommand{\ReadingSealStatus}{sealed\xspace}  % r21.seal: whether the templates carry a seal record over -
\newcommand{\ReadingTemplatesSha}{\texttt{af62f98dba4e}\xspace}  % r21.templates_sha: sha256 prefix of readings/templates.tex over -
\newcommand{\RederiveWhat}{validity verdicts and outcome terms\xspace}  % r21.rederive_what: scope of the independent re-derivation claim: prospective blocks only once every reported block has both its validity re-derivation and its scorer audit over -
\newcommand{\RederiveWhatR}{validity verdicts and the outcome terms supported by archived evidence\xspace}  % r32.rederive: r32: the abstract's re-derivation scope over -
\newcommand{\RelatedClaimsAnchor}{The prospective claims blocks do not show this for Opus~5, which succeeded on \BlockClmBClmOffAPassFrac{} silent-change instances without the panel; there the panel contrast is Sonnet~5's (\BlockClmBSClmOffAPassFrac{} without, \BlockClmBSClmOnAPassFrac{} with), for this task and interface.\xspace}  % r29.rel.anchor: Appendix U: the prospective anchor (blind GPT-6 Pro r29, p. 52) over -
\newcommand{\ReproBCSentence}{ The anonymous supplement includes the raw text archives, search logs, results, independent scorer outputs and validity re-derivations for every prospective block reported in the main text, including BC; a no-model reproduction target recomputes the cells of Table~\ref{tab:results}, the per-instance grids of Figure~\ref{fig:results}, all registered paired tests and the associated audit counts from those packaged artifacts.\xspace}  % r31.repro: r31: the reproducibility statement's r23 sentence (true only for a rebuilt package) over -
\newcommand{\ReproCliVersion}{\code{2.1.274}\xspace}  % repro.cli_version: policy CLI version over -
\newcommand{\ReproFrameRead}{2305\xspace}  % repro.frame_read: steps on which the model Read the frame over policy step
\newcommand{\ReproModelAgree}{2548\xspace}  % repro.model_agree: steps whose CLI init model equals the requested id over policy step
\newcommand{\ReproSteps}{2548\xspace}  % repro.steps: archived model steps over the 82 attempts over policy step
\newcommand{\RequeryOffAFrac}{0/24\xspace}  % audit.requery_off: k/n over counted rollout
\newcommand{\RequeryOnAOpusFrac}{10/10\xspace}  % audit.requery_on_opus: k/n over counted rollout
\newcommand{\ReserveBlock}{6\xspace}  % spec.reserve_block: replacement reserve per block over rollout
\newcommand{\ReserveCell}{2\xspace}  % spec.reserve_cell: replacement reserve per cell over rollout
\newcommand{\ReservePauseAfter}{2\xspace}  % spec.pause_after: infra-invalid attempts before the block pauses over rollout
\newcommand{\RewardGamma}{1\xspace}  % spec.gamma: discount, as stated in reward_v2.py over -
\newcommand{\RewardVersion}{2\xspace}  % man.reward_version: reward version over -
\newcommand{\RiskOneSentence}{Both prospective applications were frozen before their first model rollout and are complete; Block~BCS, Sonnet~5 on BC's instances, was incomplete at its registered experiment cutoff.\xspace}  % r27.risk1: r27: GPT-6 r19 risk 1, generated from block status over -
\newcommand{\RiskTwoSentence}{Our estimand is a paired effect on the frozen generated instances, not a population-wide failure rate: Sonnet produced eight OFF-fail/ON-pass pairs, zero pairs in the opposite direction, and two ties (net and marginal 95\,\% CI \BlockClmBSOnOffNetCI); we make no claim about the prevalence of this behavior across tasks or agents.\xspace}  % r27.risk2: r27: GPT-6 r19 risk 2, counts from the ledger over -
\newcommand{\RuleMatrixRows}{13\xspace}  % rules.matrix_rows: rows of the rule matrix over rule
\newcommand{\ScorerAuditDate}{2026-09-21\xspace}  % scorer.audit_utc: audit date over -
\newcommand{\ScorerAuditRecordsDigest}{False\xspace}  % scorer.audit_records_digest: whether REWARD_AUDIT.json records a digest of the auditor (it records the path only) over -
\newcommand{\ScorerBehaviour}{2\xspace}  % scorer.behaviour: count over finding
\newcommand{\ScorerBypassStop}{\texttt{step\_cap}\xspace}  % scorer.bypass_stop: stop reason of the modal_bypass episodes with unresolved terms over -
\newcommand{\ScorerContradictions}{0\xspace}  % scorer.contradictions: count over finding
\newcommand{\ScorerEvaluatorImports}{0\xspace}  % scorer.evaluator_imports: count of imports from src/envos in the scorer source over import statement
\newcommand{\ScorerInvariants}{5\xspace}  % scorer.invariants: count over invariant
\newcommand{\ScorerNullSteps}{1\xspace}  % scorer.null_steps: max actions of a null-policy episode with unresolved terms over action
\newcommand{\ScorerRunsAudited}{76\xspace}  % scorer.runs: count over certification episode
\newcommand{\ScorerRunsUnresolvedBypass}{2\xspace}  % scorer.runs_unresolved.modal_bypass: count with an unresolved term on the modal_bypass policy over certification episode
\newcommand{\ScorerRunsUnresolvedNull}{13\xspace}  % scorer.runs_unresolved.null: count with an unresolved term on the null policy over certification episode
\newcommand{\ScorerRunsWithUnresolved}{15\xspace}  % scorer.runs_unresolved: count with an unresolved term over certification episode
\newcommand{\ScorerSourceSha}{\texttt{a113a2a8}\xspace}  % scorer.source_sha: sha256 prefix of the scorer source checked over -
\newcommand{\ScorerUnresolved}{46\xspace}  % scorer.unresolved: count over finding
\newcommand{\ScorerUnresolvedBypass}{6\xspace}  % scorer.unresolved.modal_bypass: count of unresolved terms on the modal_bypass policy over finding
\newcommand{\ScorerUnresolvedNull}{40\xspace}  % scorer.unresolved.null: count of unresolved terms on the null policy over finding
\newcommand{\SecFiveOpenR}{Both prospective workflows were frozen before their first rollout, and their primary blocks completed under their registered gates. Block~BCS, a separately pre-registered replication with Claude Sonnet~5 on BC's instances, was incomplete at its registered experiment cutoff, after a disclosed operator-caused halt (Appendix~\ref{app:disclosures}), and contributes no inferential result.\xspace}  % r31.sec5: r31: Section 5's status sentence over -
\newcommand{\SecFiveOpenThree}{Both prospective workflows were frozen before their first rollout, and their primary blocks completed under their registered gates. Each block is one model on one workflow: in claims approval CLM-B (Claude Opus~5) and CLM-BS (Claude Sonnet~5), with the Gemini follow-up CLM-BG; in clinic booking BC (Opus~5). BCS, a separately pre-registered Sonnet replication of BC on the same instances, was incomplete at its registered experiment cutoff, after a disclosed operator-caused halt (Appendix~\ref{app:disclosures}), and contributes no inferential result.\xspace}  % r37f.sec5: r37 final reviews: Section 5's status sentence over -
\newcommand{\SecFiveOpenTwo}{The two primary prospective applications, CLM-B/CLM-BS in claims approval and BC in clinic booking, were frozen before their first rollout and completed under their registered gates. BCS, a separately pre-registered Sonnet replication of BC on the same instances, was incomplete at its registered experiment cutoff, after a disclosed operator-caused halt (Appendix~\ref{app:disclosures}), and contributes no inferential result.\xspace}  % r32.sec5: r32: Section 5's status sentence over -
\newcommand{\SensAtwoBudgetAgainst}{1\xspace}  % sens.A2.budget.against: count over pair
\newcommand{\SensAtwoBudgetFor}{0\xspace}  % sens.A2.budget.for: count over pair
\newcommand{\SensAtwoBudgetP}{1\xspace}  % sens.A2.budget.p: exact two-sided sign test over pair
\newcommand{\SensAtwoBudgetPairs}{8\xspace}  % sens.A2.budget.pairs: count over pair
\newcommand{\SensAtwoBudgetSCFrac}{8/8\xspace}  % sens.A2.budget.S-C.frac: k/n over counted rollout
\newcommand{\SensAtwoBudgetSLtwoFrac}{7/8\xspace}  % sens.A2.budget.S-L2.frac: k/n over counted rollout
\newcommand{\SensAtwoBudgetSLzeroFrac}{2/2\xspace}  % sens.A2.budget.S-L0.frac: k/n over counted rollout
\newcommand{\SensAtwoDeliveryAgainst}{1\xspace}  % sens.A2.delivery.against: count over pair
\newcommand{\SensAtwoDeliveryFor}{0\xspace}  % sens.A2.delivery.for: count over pair
\newcommand{\SensAtwoDeliveryP}{1\xspace}  % sens.A2.delivery.p: exact two-sided sign test over pair
\newcommand{\SensAtwoDeliveryPairs}{8\xspace}  % sens.A2.delivery.pairs: count over pair
\newcommand{\SensAtwoDeliverySCFrac}{8/8\xspace}  % sens.A2.delivery.S-C.frac: k/n over counted rollout
\newcommand{\SensAtwoDeliverySLtwoFrac}{7/8\xspace}  % sens.A2.delivery.S-L2.frac: k/n over counted rollout
\newcommand{\SensAtwoDeliverySLzeroFrac}{2/2\xspace}  % sens.A2.delivery.S-L0.frac: k/n over counted rollout
\newcommand{\SensAtwoJointAgainst}{1\xspace}  % sens.A2.joint.against: count over pair
\newcommand{\SensAtwoJointFor}{0\xspace}  % sens.A2.joint.for: count over pair
\newcommand{\SensAtwoJointP}{1\xspace}  % sens.A2.joint.p: exact two-sided sign test over pair
\newcommand{\SensAtwoJointPairs}{8\xspace}  % sens.A2.joint.pairs: count over pair
\newcommand{\SensAtwoJointSCFrac}{8/8\xspace}  % sens.A2.joint.S-C.frac: k/n over counted rollout
\newcommand{\SensAtwoJointSLtwoFrac}{7/8\xspace}  % sens.A2.joint.S-L2.frac: k/n over counted rollout
\newcommand{\SensAtwoJointSLzeroFrac}{2/2\xspace}  % sens.A2.joint.S-L0.frac: k/n over counted rollout
\newcommand{\SensAtwoMatchesResultFile}{yes\xspace}  % sens.A2.matches: consistency check over -
\newcommand{\SensAtwoReportedAgainst}{1\xspace}  % sens.A2.as_reported.against: count over pair
\newcommand{\SensAtwoReportedFor}{0\xspace}  % sens.A2.as_reported.for: count over pair
\newcommand{\SensAtwoReportedP}{1\xspace}  % sens.A2.as_reported.p: exact two-sided sign test over pair
\newcommand{\SensAtwoReportedPairs}{8\xspace}  % sens.A2.as_reported.pairs: count over pair
\newcommand{\SensAtwoReportedSCFrac}{8/8\xspace}  % sens.A2.as_reported.S-C.frac: k/n over counted rollout
\newcommand{\SensAtwoReportedSLtwoFrac}{7/8\xspace}  % sens.A2.as_reported.S-L2.frac: k/n over counted rollout
\newcommand{\SensAtwoReportedSLzeroFrac}{2/2\xspace}  % sens.A2.as_reported.S-L0.frac: k/n over counted rollout
\newcommand{\SensAtwoSBudgetAgainst}{0\xspace}  % sens.A2S.budget.against: count over pair
\newcommand{\SensAtwoSBudgetFor}{0\xspace}  % sens.A2S.budget.for: count over pair
\newcommand{\SensAtwoSBudgetP}{1\xspace}  % sens.A2S.budget.p: exact two-sided sign test over pair
\newcommand{\SensAtwoSBudgetPairs}{2\xspace}  % sens.A2S.budget.pairs: count over pair
\newcommand{\SensAtwoSBudgetSCFrac}{2/2\xspace}  % sens.A2S.budget.S-C.frac: k/n over counted rollout
\newcommand{\SensAtwoSBudgetSLtwoFrac}{2/2\xspace}  % sens.A2S.budget.S-L2.frac: k/n over counted rollout
\newcommand{\SensAtwoSBudgetSLzeroFrac}{1/1\xspace}  % sens.A2S.budget.S-L0.frac: k/n over counted rollout
\newcommand{\SensAtwoSDeliveryAgainst}{0\xspace}  % sens.A2S.delivery.against: count over pair
\newcommand{\SensAtwoSDeliveryFor}{2\xspace}  % sens.A2S.delivery.for: count over pair
\newcommand{\SensAtwoSDeliveryP}{0.5\xspace}  % sens.A2S.delivery.p: exact two-sided sign test over pair
\newcommand{\SensAtwoSDeliveryPairs}{4\xspace}  % sens.A2S.delivery.pairs: count over pair
\newcommand{\SensAtwoSDeliverySCFrac}{2/4\xspace}  % sens.A2S.delivery.S-C.frac: k/n over counted rollout
\newcommand{\SensAtwoSDeliverySLtwoFrac}{4/4\xspace}  % sens.A2S.delivery.S-L2.frac: k/n over counted rollout
\newcommand{\SensAtwoSDeliverySLzeroFrac}{1/1\xspace}  % sens.A2S.delivery.S-L0.frac: k/n over counted rollout
\newcommand{\SensAtwoSJointAgainst}{0\xspace}  % sens.A2S.joint.against: count over pair
\newcommand{\SensAtwoSJointFor}{0\xspace}  % sens.A2S.joint.for: count over pair
\newcommand{\SensAtwoSJointP}{1\xspace}  % sens.A2S.joint.p: exact two-sided sign test over pair
\newcommand{\SensAtwoSJointPairs}{2\xspace}  % sens.A2S.joint.pairs: count over pair
\newcommand{\SensAtwoSJointSCFrac}{2/2\xspace}  % sens.A2S.joint.S-C.frac: k/n over counted rollout
\newcommand{\SensAtwoSJointSLtwoFrac}{2/2\xspace}  % sens.A2S.joint.S-L2.frac: k/n over counted rollout
\newcommand{\SensAtwoSJointSLzeroFrac}{1/1\xspace}  % sens.A2S.joint.S-L0.frac: k/n over counted rollout
\newcommand{\SensAtwoSMatchesResultFile}{yes\xspace}  % sens.A2S.matches: consistency check over -
\newcommand{\SensAtwoSReportedAgainst}{0\xspace}  % sens.A2S.as_reported.against: count over pair
\newcommand{\SensAtwoSReportedFor}{2\xspace}  % sens.A2S.as_reported.for: count over pair
\newcommand{\SensAtwoSReportedP}{0.5\xspace}  % sens.A2S.as_reported.p: exact two-sided sign test over pair
\newcommand{\SensAtwoSReportedPairs}{4\xspace}  % sens.A2S.as_reported.pairs: count over pair
\newcommand{\SensAtwoSReportedSCFrac}{2/4\xspace}  % sens.A2S.as_reported.S-C.frac: k/n over counted rollout
\newcommand{\SensAtwoSReportedSLtwoFrac}{4/4\xspace}  % sens.A2S.as_reported.S-L2.frac: k/n over counted rollout
\newcommand{\SensAtwoSReportedSLzeroFrac}{1/1\xspace}  % sens.A2S.as_reported.S-L0.frac: k/n over counted rollout
\newcommand{\SensBBudgetAgainst}{0\xspace}  % sens.B.budget.against: count over pair
\newcommand{\SensBBudgetFRXOffAFrac}{0/10\xspace}  % sens.B.budget.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\SensBBudgetFRXOnAFrac}{10/10\xspace}  % sens.B.budget.FRX-ON-A.frac: k/n over counted rollout
\newcommand{\SensBBudgetFRXOnIFrac}{3/3\xspace}  % sens.B.budget.FRX-ON-I.frac: k/n over counted rollout
\newcommand{\SensBBudgetFor}{10\xspace}  % sens.B.budget.for: count over pair
\newcommand{\SensBBudgetP}{0.00195\xspace}  % sens.B.budget.p: exact two-sided sign test over pair
\newcommand{\SensBBudgetPairs}{10\xspace}  % sens.B.budget.pairs: count over pair
\newcommand{\SensBCBudgetAgainst}{0\xspace}  % sens.BC.budget.against: count over pair
\newcommand{\SensBCBudgetFRXCueAFrac}{2/15\xspace}  % sens.BC.budget.FRX-CUE-A.frac: k/n over counted rollout
\newcommand{\SensBCBudgetFRXLiveAFrac}{15/15\xspace}  % sens.BC.budget.FRX-LIVE-A.frac: k/n over counted rollout
\newcommand{\SensBCBudgetFRXLiveIFrac}{3/3\xspace}  % sens.BC.budget.FRX-LIVE-I.frac: k/n over counted rollout
\newcommand{\SensBCBudgetFRXOffAFrac}{0/16\xspace}  % sens.BC.budget.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\SensBCBudgetFor}{13\xspace}  % sens.BC.budget.for: count over pair
\newcommand{\SensBCBudgetP}{0.000244\xspace}  % sens.BC.budget.p: exact two-sided sign test over pair
\newcommand{\SensBCBudgetPairs}{15\xspace}  % sens.BC.budget.pairs: count over pair
\newcommand{\SensBCDeliveryAgainst}{0\xspace}  % sens.BC.delivery.against: count over pair
\newcommand{\SensBCDeliveryFRXCueAFrac}{2/16\xspace}  % sens.BC.delivery.FRX-CUE-A.frac: k/n over counted rollout
\newcommand{\SensBCDeliveryFRXLiveAFrac}{15/16\xspace}  % sens.BC.delivery.FRX-LIVE-A.frac: k/n over counted rollout
\newcommand{\SensBCDeliveryFRXLiveIFrac}{3/3\xspace}  % sens.BC.delivery.FRX-LIVE-I.frac: k/n over counted rollout
\newcommand{\SensBCDeliveryFRXOffAFrac}{0/16\xspace}  % sens.BC.delivery.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\SensBCDeliveryFor}{13\xspace}  % sens.BC.delivery.for: count over pair
\newcommand{\SensBCDeliveryP}{0.000244\xspace}  % sens.BC.delivery.p: exact two-sided sign test over pair
\newcommand{\SensBCDeliveryPairs}{16\xspace}  % sens.BC.delivery.pairs: count over pair
\newcommand{\SensBCJointAgainst}{0\xspace}  % sens.BC.joint.against: count over pair
\newcommand{\SensBCJointFRXCueAFrac}{2/15\xspace}  % sens.BC.joint.FRX-CUE-A.frac: k/n over counted rollout
\newcommand{\SensBCJointFRXLiveAFrac}{15/15\xspace}  % sens.BC.joint.FRX-LIVE-A.frac: k/n over counted rollout
\newcommand{\SensBCJointFRXLiveIFrac}{3/3\xspace}  % sens.BC.joint.FRX-LIVE-I.frac: k/n over counted rollout
\newcommand{\SensBCJointFRXOffAFrac}{0/16\xspace}  % sens.BC.joint.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\SensBCJointFor}{13\xspace}  % sens.BC.joint.for: count over pair
\newcommand{\SensBCJointP}{0.000244\xspace}  % sens.BC.joint.p: exact two-sided sign test over pair
\newcommand{\SensBCJointPairs}{15\xspace}  % sens.BC.joint.pairs: count over pair
\newcommand{\SensBCMatchesResultFile}{yes\xspace}  % sens.BC.matches: consistency check over -
\newcommand{\SensBCReportedAgainst}{0\xspace}  % sens.BC.as_reported.against: count over pair
\newcommand{\SensBCReportedFRXCueAFrac}{2/16\xspace}  % sens.BC.as_reported.FRX-CUE-A.frac: k/n over counted rollout
\newcommand{\SensBCReportedFRXLiveAFrac}{15/16\xspace}  % sens.BC.as_reported.FRX-LIVE-A.frac: k/n over counted rollout
\newcommand{\SensBCReportedFRXLiveIFrac}{3/3\xspace}  % sens.BC.as_reported.FRX-LIVE-I.frac: k/n over counted rollout
\newcommand{\SensBCReportedFRXOffAFrac}{0/16\xspace}  % sens.BC.as_reported.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\SensBCReportedFor}{13\xspace}  % sens.BC.as_reported.for: count over pair
\newcommand{\SensBCReportedP}{0.000244\xspace}  % sens.BC.as_reported.p: exact two-sided sign test over pair
\newcommand{\SensBCReportedPairs}{16\xspace}  % sens.BC.as_reported.pairs: count over pair
\newcommand{\SensBDeliveryAgainst}{0\xspace}  % sens.B.delivery.against: count over pair
\newcommand{\SensBDeliveryFRXOffAFrac}{0/10\xspace}  % sens.B.delivery.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\SensBDeliveryFRXOnAFrac}{10/10\xspace}  % sens.B.delivery.FRX-ON-A.frac: k/n over counted rollout
\newcommand{\SensBDeliveryFRXOnIFrac}{3/3\xspace}  % sens.B.delivery.FRX-ON-I.frac: k/n over counted rollout
\newcommand{\SensBDeliveryFor}{10\xspace}  % sens.B.delivery.for: count over pair
\newcommand{\SensBDeliveryP}{0.00195\xspace}  % sens.B.delivery.p: exact two-sided sign test over pair
\newcommand{\SensBDeliveryPairs}{10\xspace}  % sens.B.delivery.pairs: count over pair
\newcommand{\SensBFBudgetFRXOffAFrac}{0/4\xspace}  % sens.BF.budget.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\SensBFBudgetFRXOnIFrac}{1/1\xspace}  % sens.BF.budget.FRX-ON-I.frac: k/n over counted rollout
\newcommand{\SensBFDeliveryFRXOffAFrac}{0/4\xspace}  % sens.BF.delivery.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\SensBFDeliveryFRXOnIFrac}{1/1\xspace}  % sens.BF.delivery.FRX-ON-I.frac: k/n over counted rollout
\newcommand{\SensBFJointFRXOffAFrac}{0/4\xspace}  % sens.BF.joint.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\SensBFJointFRXOnIFrac}{1/1\xspace}  % sens.BF.joint.FRX-ON-I.frac: k/n over counted rollout
\newcommand{\SensBFMatchesResultFile}{yes\xspace}  % sens.BF.matches: consistency check over -
\newcommand{\SensBFReportedFRXOffAFrac}{0/4\xspace}  % sens.BF.as_reported.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\SensBFReportedFRXOnIFrac}{1/1\xspace}  % sens.BF.as_reported.FRX-ON-I.frac: k/n over counted rollout
\newcommand{\SensBJointAgainst}{0\xspace}  % sens.B.joint.against: count over pair
\newcommand{\SensBJointFRXOffAFrac}{0/10\xspace}  % sens.B.joint.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\SensBJointFRXOnAFrac}{10/10\xspace}  % sens.B.joint.FRX-ON-A.frac: k/n over counted rollout
\newcommand{\SensBJointFRXOnIFrac}{3/3\xspace}  % sens.B.joint.FRX-ON-I.frac: k/n over counted rollout
\newcommand{\SensBJointFor}{10\xspace}  % sens.B.joint.for: count over pair
\newcommand{\SensBJointP}{0.00195\xspace}  % sens.B.joint.p: exact two-sided sign test over pair
\newcommand{\SensBJointPairs}{10\xspace}  % sens.B.joint.pairs: count over pair
\newcommand{\SensBMatchesResultFile}{yes\xspace}  % sens.B.matches: consistency check over -
\newcommand{\SensBReportedAgainst}{0\xspace}  % sens.B.as_reported.against: count over pair
\newcommand{\SensBReportedFRXOffAFrac}{0/10\xspace}  % sens.B.as_reported.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\SensBReportedFRXOnAFrac}{10/10\xspace}  % sens.B.as_reported.FRX-ON-A.frac: k/n over counted rollout
\newcommand{\SensBReportedFRXOnIFrac}{3/3\xspace}  % sens.B.as_reported.FRX-ON-I.frac: k/n over counted rollout
\newcommand{\SensBReportedFor}{10\xspace}  % sens.B.as_reported.for: count over pair
\newcommand{\SensBReportedP}{0.00195\xspace}  % sens.B.as_reported.p: exact two-sided sign test over pair
\newcommand{\SensBReportedPairs}{10\xspace}  % sens.B.as_reported.pairs: count over pair
\newcommand{\SensBSBudgetAgainst}{0\xspace}  % sens.BS.budget.against: count over pair
\newcommand{\SensBSBudgetFRXOffAFrac}{0/8\xspace}  % sens.BS.budget.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\SensBSBudgetFRXOnAFrac}{5/8\xspace}  % sens.BS.budget.FRX-ON-A.frac: k/n over counted rollout
\newcommand{\SensBSBudgetFRXOnIFrac}{2/2\xspace}  % sens.BS.budget.FRX-ON-I.frac: k/n over counted rollout
\newcommand{\SensBSBudgetFor}{5\xspace}  % sens.BS.budget.for: count over pair
\newcommand{\SensBSBudgetP}{0.0625\xspace}  % sens.BS.budget.p: exact two-sided sign test over pair
\newcommand{\SensBSBudgetPairs}{8\xspace}  % sens.BS.budget.pairs: count over pair
\newcommand{\SensBSDeliveryAgainst}{0\xspace}  % sens.BS.delivery.against: count over pair
\newcommand{\SensBSDeliveryFRXOffAFrac}{0/9\xspace}  % sens.BS.delivery.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\SensBSDeliveryFRXOnAFrac}{6/9\xspace}  % sens.BS.delivery.FRX-ON-A.frac: k/n over counted rollout
\newcommand{\SensBSDeliveryFRXOnIFrac}{2/2\xspace}  % sens.BS.delivery.FRX-ON-I.frac: k/n over counted rollout
\newcommand{\SensBSDeliveryFor}{6\xspace}  % sens.BS.delivery.for: count over pair
\newcommand{\SensBSDeliveryP}{0.0312\xspace}  % sens.BS.delivery.p: exact two-sided sign test over pair
\newcommand{\SensBSDeliveryPairs}{9\xspace}  % sens.BS.delivery.pairs: count over pair
\newcommand{\SensBSJointAgainst}{0\xspace}  % sens.BS.joint.against: count over pair
\newcommand{\SensBSJointFRXOffAFrac}{0/8\xspace}  % sens.BS.joint.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\SensBSJointFRXOnAFrac}{5/8\xspace}  % sens.BS.joint.FRX-ON-A.frac: k/n over counted rollout
\newcommand{\SensBSJointFRXOnIFrac}{2/2\xspace}  % sens.BS.joint.FRX-ON-I.frac: k/n over counted rollout
\newcommand{\SensBSJointFor}{5\xspace}  % sens.BS.joint.for: count over pair
\newcommand{\SensBSJointP}{0.0625\xspace}  % sens.BS.joint.p: exact two-sided sign test over pair
\newcommand{\SensBSJointPairs}{8\xspace}  % sens.BS.joint.pairs: count over pair
\newcommand{\SensBSMatchesResultFile}{yes\xspace}  % sens.BS.matches: consistency check over -
\newcommand{\SensBSReportedAgainst}{0\xspace}  % sens.BS.as_reported.against: count over pair
\newcommand{\SensBSReportedFRXOffAFrac}{0/10\xspace}  % sens.BS.as_reported.FRX-OFF-A.frac: k/n over counted rollout
\newcommand{\SensBSReportedFRXOnAFrac}{6/10\xspace}  % sens.BS.as_reported.FRX-ON-A.frac: k/n over counted rollout
\newcommand{\SensBSReportedFRXOnIFrac}{2/3\xspace}  % sens.BS.as_reported.FRX-ON-I.frac: k/n over counted rollout
\newcommand{\SensBSReportedFor}{6\xspace}  % sens.BS.as_reported.for: count over pair
\newcommand{\SensBSReportedP}{0.0312\xspace}  % sens.BS.as_reported.p: exact two-sided sign test over pair
\newcommand{\SensBSReportedPairs}{10\xspace}  % sens.BS.as_reported.pairs: count over pair
\newcommand{\SessionVersionFrom}{1\xspace}  % spec.version_from: from_version of every counted changed run's event log over row version
\newcommand{\SessionVersionTo}{2\xspace}  % spec.version_to: to_version of every counted changed run's event log over row version
\newcommand{\SilentPoolCommittedStale}{23\xspace}  % silent.pool.committed_stale: count over counted rollout
\newcommand{\SilentPoolFlagged}{4\xspace}  % silent.pool.flagged: count over counted rollout
\newcommand{\SilentPoolInstanceCI}{0.00--0.28\xspace}  % silent.pool.ci_instance: Wilson 95% on instances with any success over instance
\newcommand{\SilentPoolInstances}{10\xspace}  % silent.pool.instances: distinct instances (seeds) under the pooled silent arm; identical instance fingerprints across models over instance
\newcommand{\SilentPoolInstancesWords}{ten\xspace}  % silent.pool.instances_words: the same count in words over instance
\newcommand{\SilentPoolModels}{3\xspace}  % silent.pool.models: count over model
\newcommand{\SilentPoolModelsWords}{three\xspace}  % silent.pool.models_words: the same count in words over model
\newcommand{\SilentPoolN}{24\xspace}  % silent.pool.n: count over every silent arm over counted rollout
\newcommand{\SilentPoolNoCommit}{1\xspace}  % silent.pool.no_commit: count over counted rollout
\newcommand{\SilentPoolRolloutCI}{0.00--0.14\xspace}  % silent.pool.ci_rollout: Wilson 95% treating the pooled rollouts as independent (too narrow; shared instances) over counted rollout
\newcommand{\SilentPoolUnflagged}{19\xspace}  % silent.pool.unflagged: count over counted rollout
\newcommand{\SlotAllRecords}{1\xspace}  % slot.all_records: attempts that opened every seed record before committing over model attempt
\newcommand{\SlotBRescues}{10\xspace}  % slot.b_rescues: Block B FRX-ON-A successes (Opus's rescues) over counted success
\newcommand{\SlotBRescuesClinic}{10\xspace}  % slot.b_rescues_clinic: of which the booked clinic is independently confirmed over counted success
\newcommand{\SlotBRescuesVerified}{0\xspace}  % slot.b_rescues_verified: of which all five invariants are independently resolved over counted success
\newcommand{\SlotCommitted}{73\xspace}  % slot.committed: attempts with a commit (POST /new/2), every one with the slot submission POST /new/1 between its last occupancy read and the commit over model attempt
\newcommand{\SlotComplete}{0\xspace}  % slot.attempts_complete: attempts whose same-episode slot evidence is complete (offered and occupied sets, no write between) over model attempt
\newcommand{\SlotFPCommitStep}{36\xspace}  % slot.fp.commit: first step whose appointment-row count grows over step
\newcommand{\SlotFPLastRead}{26\xspace}  % slot.fp.last_read: last occupancy-establishing read over step
\newcommand{\SlotFPRunLabel}{A2, S-L2, seed 15, attempt 1\xspace}  % slot.fp.label: the one run over -
\newcommand{\SlotFPSupported}{1\xspace}  % slot.fp.supported: of which the committed slot equals the nearest available slot the evidence supports over counted success
\newcommand{\SlotFPSupportedWords}{one\xspace}  % slot.fp.supported_words: the same count in words over counted success
\newcommand{\SlotFPWrites}{2\xspace}  % slot.fp.writes: writes between read and commit over request
\newcommand{\SlotOneRecord}{78\xspace}  % slot.one_record: attempts that opened exactly one seed record over model attempt
\newcommand{\SlotSeedRecords}{4\xspace}  % slot.seed_records: appointments in the portal before the episode (not all on the requested date) over seed appointment
\newcommand{\SlotSuccessComplete}{0\xspace}  % slot.success_complete: counted successes whose slot term is decidable from same-episode evidence over counted success
\newcommand{\SlotSuccessCompleteFP}{1\xspace}  % slot.fp.complete: counted successes whose occupancy evidence is complete under the post-hoc fingerprint rule over counted success
\newcommand{\SonnetPanelShotSuccess}{6\xspace}  % rules.sonnet.shot_success: Sonnet FRX-ON-A rows with the screenshot opened at the panel step, all successes over counted rollout
\newcommand{\SonnetPanelTextFail}{3\xspace}  % rules.sonnet.text_fail: Sonnet FRX-ON-A rows with the panel as text only, all failures over counted rollout
\newcommand{\StackBArms}{32\xspace}  % stackb.arms: distinct (task, arm) rows of atlas.csv (every arm ran on Opus 5) over arm
\newcommand{\StackBControlArms}{5\xspace}  % stackb.ctrl: atlas.csv kind = control (clean baselines, cosmetic) over arm
\newcommand{\StackBEnvsWords}{three\xspace}  % stackb.envs: distinct tasks of atlas.csv, in words over environment
\newcommand{\StackBKMax}{7\xspace}  % stackb.kmax: most Opus rollouts on one arm over rollout
\newcommand{\StackBKMin}{1\xspace}  % stackb.kmin: fewest Opus rollouts on one arm over rollout
\newcommand{\StackBKThreeArms}{24\xspace}  % stackb.k3: arms with exactly three Opus rollouts over arm
\newcommand{\StackBOpusRollouts}{93\xspace}  % stackb.opus_rollouts: sum of atlas.csv k (= rows of runs.csv) over rollout
\newcommand{\StackBPhenArms}{27\xspace}  % stackb.phen: atlas.csv kind = phenomenon over arm
\newcommand{\StackBRescoreField}{93\xspace}  % stackb.rescore_field: archived Opus rollouts whose run-info.json carries the import re-score record (rescore_drift) over rollout
\newcommand{\StackBRescoreFlips}{2\xspace}  % stackb.rescore_flips: archived Opus rollouts whose stored FAIL was re-scored PASS at import over rollout
\newcommand{\StackBSharedArms}{22\xspace}  % stackb.shared: arms run on both models over arm
\newcommand{\StackBSonnetArms}{23\xspace}  % stackb.son_arms: arms with Sonnet 5 rollouts over arm
\newcommand{\StackBSonnetOnlyArms}{1\xspace}  % stackb.son_only: Sonnet arms with no Opus run over arm
\newcommand{\StackBUnionArms}{33\xspace}  % stackb.union: arms run on either model over arm
\newcommand{\SuccessFullyVerified}{0\xspace}  % slot.success_verified: counted successes with all five invariants independently resolved over counted success
\newcommand{\SupersededBlockCounted}{8\xspace}  % pre.superseded_counted: counted rows of the superseded Block A search log over rollout
\newcommand{\SupersededBlockCountedAddendum}{9\xspace}  % pre.superseded_counted_addendum: counted rows as ADDENDUM 3's prose states them (erratum: the log has SupersededBlockCounted) over rollout
\newcommand{\SupersededBlockEpisodes}{12\xspace}  % pre.superseded_episodes: attempts in the superseded Block A search log (ADDENDUM 3 states the same number) over rollout
\newcommand{\SupersededBlockInfra}{1\xspace}  % pre.superseded_infra: infra_rejected rows over rollout
\newcommand{\SupersededBlockNotTriggered}{3\xspace}  % pre.superseded_not_triggered: not_triggered rows of the superseded Block A search log over rollout
\newcommand{\SuppArchiveTextExcluded}{1377\xspace}  % supp.archtext: text files of the archived pre-image certification runs left out for size over file
\newcommand{\SuppBCRuns}{53\xspace}  % supp.bc_runs: r31: run directories of Block BC (complete) packaged, every one its search log references over run directory
\newcommand{\SuppBCRunsInFlight}{0\xspace}  % supp.bc_inflight: run directories of Block BC (running) captured by the package, not analysed over run directory
\newcommand{\SuppBCSRuns}{24\xspace}  % supp.bcs_runs: r34: run directories of Block BCS (terminal) packaged, every one its search log references over run directory
\newcommand{\SuppBCSRunsKeptOut}{0\xspace}  % supp.bcs_kept_out: r31: run directories of Block BCS (running) kept out of the package over run directory
\newcommand{\SuppBCSStatus}{stopped_cutoff\xspace}  % supp.bcs_status: r31: Block BCS's search-log status when the package was built (in-flight evidence kept out by rule) over -
\newcommand{\SuppClaimsAfter}{\xspace}  % supp.claims_after: whether the claims bundle is in the packaged supplement (and, r26, the challenge output after it) over -
\newcommand{\SuppClaimsAttemptDirs}{49\xspace}  % supp.claims_attempts: claims model attempt archives packaged (every attempt, counted or not) over attempt directory
\newcommand{\SuppCodeObjects}{123\xspace}  % supp.code_objects: pinned code versions packaged under code_snapshots/ over file
\newcommand{\SuppContents}{the environment, task-module, certifier, scorer, harness, invoker and test sources; the pre-registrations, certificates, block specifications, release manifests and search logs; the text records of all \SuppRuns historical model episodes (trajectory, access log, event log, checkpoints, classification); the leak-audit records; the held-out battery run with its reference runs' text records and every checker version it records; the r19/r20 archive re-analyses behind Appendices~\ref{app:rules}--\ref{app:certificates} with the two earlier scorer runs they compare against; the r21 plans and reviews and the cross-vendor admission record; the Stack~B corpus files (\SuppStackBFiles, identities rewritten); the sealed archive challenge after its one run (cases, sealed expectations, seal record, first-run outputs under their hash list, comparison code and result, run log); the claims blocks' frozen evidence bundle (\ClmBundleFiles files) and the raw archive of every claims model attempt (\SuppClaimsAttemptDirs attempt directories: trajectory, archived prompts, database snapshots, access and event logs, checkpoints, classification); Block~CLM-BG's evidence (ADDENDUM~G with its freeze, external-timestamp, admission and incident records; the request journal, audits and every attempt's text archive; the invoker and its tests; no API key); every code version a release manifest or the held-out run pins (\SuppCodeObjects files), except the pins listed as permanently missing below; the clinic portal's database snapshot and the five smaller world data snapshots; the text of the P1, P2, P3, P4 and ambiguous-commit archives and of the scripted feasibility episodes; the complete evidence of Block~BC (search log, result, report, independent-scorer and validity re-derivation records, deploy checks, certificate text and the text records of all \SuppBCRuns{} run directories its search log references); the complete evidence of Block~BCS, which stopped unfinished at its registered launch cutoff (search log, report, independent-scorer and validity re-derivation records, deploy checks and the text records of all \SuppBCSRuns{} run directories its search log references); six demo videos; the post-hoc, author-built checks of Appendix~\ref{app:posthoc} with their inputs and outputs; the screenshot-only crossover's admission-gate records (its NO-GO); the generated historical-provenance file; a reproduction script that, from the extracted supplement with no network, world or model, recomputes Table~\ref{tab:results}'s cells and Figure~\ref{fig:results}'s per-instance grids for the claims blocks and Block~BC from their raw run archives (per-arm counts, paired tallies, exact sign tests, Holm adjustments, Newcombe intervals, audit counts) with the scorer, validity and readings code at their pinned digests, re-runs Block~BC's independent scorer and validity re-derivation, re-runs the sealed challenge's unmodified comparison on its shipped first-run outputs, re-runs the archive re-analyses behind the historical tables and re-runs the ledger's verification; and this paper's build files\xspace}  % supp.contents: what the packaged supplement contains over -
\newcommand{\SuppEpisodeFrames}{0\xspace}  % supp.ep_frames: 1 if every screenshot frame of every Block A2/A2S/B/BS/BF model episode ships over -
\newcommand{\SuppFiles}{24399\xspace}  % supp.files: files packaged over file
\newcommand{\SuppFramesExcluded}{12241\xspace}  % supp.frames: screenshot frames of the P1/P3/ambiguous-commit archives left out for size over file
\newcommand{\SuppFramesShipped}{0\xspace}  % supp.frames_any: r31: screenshot-frame files packaged (every frame group) over file
\newcommand{\SuppIrrecoverablePins}{2\xspace}  % supp.irrecoverable_pins: release-manifest pins no surviving copy can supply over pin
\newcommand{\SuppIrrecoverableText}{two code versions pinned by the archived pre-image Block~A manifest (the harness \texttt{e4e215d1} and the task module \texttt{1eeaab16})\xspace}  % supp.irrecoverable_text: the irrecoverable pins, stated over -
\newcommand{\SuppKeptOut}{copies of this paper taken before an integration, tool caches, the world's environment file, a world database backup, the transcripts of external-model consultations, the job files and the packaging script\xspace}  % supp.kept_out: kept out of the package by rule over -
\newcommand{\SuppLeftOutSize}{the 7878 screenshot-frame files of Block~BC's model episodes, the 444 screenshot-frame files of Block~BCS's model episodes, the 3503 screenshot-frame files (305 distinct images; no reproduction target reads them) of the claims model attempts, the 347 screenshot-frame files of the CLM-BG attempts, the 765 screenshot-frame files of CLM-BG's admission and certification runs, the 1477 screenshot-frame files of the historical Blocks~B, BS and BF, the 598 screenshot-frame files of the historical Blocks~A2 and A2S, the 352 screenshot-frame files (52 distinct images) of the held-out battery's scripted reference runs, the 12241 screenshot frames of the P1, P3 and ambiguous-commit archives, 8 demo videos, 4 larger world data snapshots and the 1377 text files of the three archived pre-image certification runs (their top-level records ship)\xspace}  % supp.left_out: packaged-path candidates left out for size, by group over path
\newcommand{\SuppNotSelectedFrames}{40943\xspace}  % supp.not_selected: frames never selected for the package (scripted-policy, development, superseded/void attempts) over file
\newcommand{\SuppNotYet}{any record of the registered clinic blocks that were not run (Block~BGC's disposition record ships)\xspace}  % supp.not_yet: prospective records not yet produced over -
\newcommand{\SuppOmitted}{Every other audit artifact the appendices cite is packaged.\xspace}  % supp.omitted: existing artifacts the supplement omits (packaging, recoverable) over -
\newcommand{\SuppRecordsShip}{the frozen pre-registrations, the release manifests and the ledger (\code{claims.json}) of the paper build the package was made from ship as files in the supplement\xspace}  % supp.records_ship: 1 if the frozen registrations, the manifests and the ledger ship in the supplement over -
\newcommand{\SuppReproBCSStatus}{stopped_cutoff\xspace}  % r28.repro.bcs: Block BCS's status in the offline run (checked only once complete) over -
\newcommand{\SuppReproChalChecks}{31\xspace}  % r28.repro.chal_checks: challenge target checks in the offline run over check
\newcommand{\SuppReproChalOk}{31\xspace}  % r28.repro.chal_ok: challenge target checks passed over check
\newcommand{\SuppReproClaimsChecks}{85\xspace}  % r28.repro.claims_checks: claims target checks in the offline run over check
\newcommand{\SuppReproClaimsOk}{85\xspace}  % r28.repro.claims_ok: claims target checks passed over check
\newcommand{\SuppReproLedgerN}{2319\xspace}  % r28.repro.ledger_n: ledger entries the packaged claims.py --verify re-derived in the offline run over entry
\newcommand{\SuppReproProsChecks}{174\xspace}  % r28.repro.pros_checks: prospective target checks in the offline run over check
\newcommand{\SuppReproProsOk}{174\xspace}  % r28.repro.pros_ok: prospective target checks passed over check
\newcommand{\SuppReproResult}{In one offline run of this package (no network, world or model), the claims target passed all \SuppReproClaimsChecks{} of its checks, every recomputed count, test, interval, reading and audit count equal to this ledger's entry, and the challenge target all \SuppReproChalChecks{}, the re-run comparison's output identical to the shipped result; the packaged ledger's verification re-derived all \SuppReproLedgerN{} of its entries. Its prospective target passed all \SuppReproProsChecks{} of its checks: Table~\ref{tab:results}'s cells and Figure~\ref{fig:results}'s per-instance grids for the claims blocks and Block~BC, Block~BC's paired tests, Holm adjustments, Newcombe intervals and audit counts, recomputed from the raw run directories, equal this ledger's entries; for Block~BCS, which stopped unfinished at its registered cutoff and reports no test, its independent scorer and validity re-derivation were re-run and equal their records, and its attempts, counted cells and per-instance table were recomputed. All \SuppReproTablesOk{} historical archive re-analysis re-derivations reproduced; every generated table (61 files) re-renders byte for byte from the shipped records.\xspace}  % r28.repro.text: what the offline run of the package established over -
\newcommand{\SuppReproTablesFail}{0\xspace}  % r28.repro.tables_fail: archive re-analysis re-derivations whose re-derived records differ from the shipped ones over target
\newcommand{\SuppReproTablesN}{9\xspace}  % r28.repro.tables_n: archive re-analysis re-derivation targets in the default reproduction over target
\newcommand{\SuppReproTablesOk}{9\xspace}  % r28.repro.tables_ok: archive re-analysis re-derivations that reproduced over target
\newcommand{\SuppRewritten}{2545\xspace}  % supp.rewritten: packaged files with identity strings rewritten (original sha256 recorded) over file
\newcommand{\SuppRuns}{82\xspace}  % supp.runs: P3v2 model run archives packaged over run directory
\newcommand{\SuppStackBFiles}{149\xspace}  % supp.stackb: Stack B corpus files packaged (identities rewritten) over file
\newcommand{\SuppSummary}{the environment, task-module, certifier, scorer, harness, invoker and test sources; the pre-registrations, certificates, block specifications, release manifests and search logs; the raw text archives of the historical, claims (CLM-BG included) and Blocks~BC and~BCS model episodes (no screenshot frame ships, for size); the held-out battery and the sealed archive challenge after its one run; and a reproduction script that needs no network, world or model\xspace}  % supp.summary: the supplement in one clause (reproducibility statement) over -
\newcommand{\SuppVideosExcluded}{8\xspace}  % supp.videos: videos left out for size over file
\newcommand{\SuppVideosPackaged}{6\xspace}  % supp.videos_in: demo videos packaged over file
\newcommand{\SuppWorldSnapshotsExcluded}{4\xspace}  % supp.worlds: world data snapshots left out for size over file
\newcommand{\SuppZipMB}{94.6\xspace}  % supp.mb: zip size over MB
\newcommand{\SweepAgree}{48\xspace}  % r29.sweepagree: r29 lane A per-episode reconstruction (post hoc) over episode
\newcommand{\SweepArmed}{46\xspace}  % r29.sweeparmed: r29 lane A per-episode reconstruction (post hoc) over episode
\newcommand{\SweepBad}{0\xspace}  % r29.sweepbad: r29 lane A per-episode reconstruction (post hoc) over episode
\newcommand{\SweepCseventeenChecked}{31\xspace}  % r29.sweepcseventeenchecked: r29 lane A per-episode reconstruction (post hoc) over episode
\newcommand{\SweepCseventeenVacuous}{15\xspace}  % r29.sweepcseventeenvacuous: r29 lane A per-episode reconstruction (post hoc) over episode
\newcommand{\SweepGapCommit}{22.4 to 199.7 s (median 75.6)\xspace}  % r29.ep.gap_commit: change to the committing request, armed episodes over -
\newcommand{\SweepGapFire}{11.6 to 54.5 s (median 19.9)\xspace}  % r29.ep.gap_fire: last old-limit serve to the change, armed episodes over -
\newcommand{\SweepN}{48\xspace}  % r29.sweepn: r29 lane A per-episode reconstruction (post hoc) over episode
\newcommand{\SweepOldFrameUnread}{1\xspace}  % r29.sweepoldframeunread: r29 lane A per-episode reconstruction (post hoc) over episode
\newcommand{\SweepSentence}{A post-hoc reconstruction importing no pipeline code found no fault of the tested classes in the raw archives of all \SweepN{} counted claims episodes (success and label equal to the frozen log on \SweepAgree/\SweepN); on \FreshN{} fresh sealed cases it missed none of \FreshCorr{} corruptions, the frozen pipeline \FreshPipeMiss{} (truncation, stale pages, access-log duplicate commits) and a repaired raw-log checker \FreshRepMiss{} (panel delivery, commit ordering); these tools are ours, written knowing the fault classes (Appendices~\ref{app:posthoc}, \ref{app:claimsspec}).\xspace}  % r29.ep.sentence: Section 6: the 48-episode sweep and the fresh cases, one sentence over -
\newcommand{\SweepVacuousBreakdown}{9 OFF-A, 4 ON-I and 2 ON-A\xspace}  % r29.ep.c17_vac_by: armed episodes with no post-change policy page, by arm over -
\newcommand{\TabMainOmitted}{7\xspace}  % tab.main.omitted: counted FRX-ON-I controls, not in Table 1 over counted rollout
\newcommand{\TabMainShown}{71\xspace}  % tab.main.shown: counted rollouts in Table 1 (every counted cell except the silent inapplicable controls) over counted rollout
\newcommand{\TestsHistClinic}{31\xspace}  % slot.tests.clinic: of those, booked clinic independently confirmed over counted success
\newcommand{\TestsHistFull}{0\xspace}  % slot.tests.full: of those, all five invariants independently resolved over counted success
\newcommand{\TestsHistSucc}{31\xspace}  % slot.tests.succ: evaluator successes in the paired arms of the three historical claim-bearing tests over counted success
\newcommand{\TransferFixtures}{6\xspace}  % transfer.fixtures: count over fixture
\newcommand{\TransferFixturesCorrected}{2\xspace}  % transfer.fixtures_corrected: fixtures whose source or corruption changed between v1 and v2 (no expectation changed) over fixture
\newcommand{\TransferMet}{4\xspace}  % transfer.met: count over fixture
\newcommand{\TransferMissed}{2\xspace}  % transfer.missed: count over fixture
\newcommand{\TransferSpecEntries}{11\xspace}  % transfer.spec_entries: count over spec entry
\newcommand{\TransferTermsChanged}{3\xspace}  % transfer.terms_changed: count over scoring term
\newcommand{\TransferTermsReused}{22\xspace}  % transfer.terms_reused: count over scoring term
\newcommand{\TransferTermsTotal}{25\xspace}  % transfer.terms_total: count over scoring term
\newcommand{\TransferValidUnresolved}{7\xspace}  % transfer.valid_unresolved: unresolved terms on each untouched valid archive over scoring term
\newcommand{\VFirstCurrent}{46\xspace}  % coh.vf_current: counted successes of the five current blocks over success row
\newcommand{\VFirstSuperseded}{7\xspace}  % coh.vf_superseded: counted successes of the superseded Block A over success row
\newcommand{\VFirstVoidAtwo}{6\xspace}  % coh.vf_void_a2: of which Block A2 over success row
\newcommand{\VFirstVoidBS}{2\xspace}  % coh.vf_void_bs: of which Block BS over success row
\newcommand{\VFirstVoidCurrent}{8\xspace}  % coh.vf_void_current: of the voidable, current over success row
\newcommand{\VFirstVoidList}{A2 S-L2 s9; A2 S-L2 s11; A2 S-C s12; A2 S-C s13; A2 S-C s14; A2 S-C s15; BS FRX-ON-I s21; BS FRX-ON-I s22\xspace}  % coh.vf_void_list: the current voidable success rows, named over success row
\newcommand{\VFirstVoidSuperseded}{1\xspace}  % coh.vf_void_sup: of the voidable, superseded Block A over success row
\newcommand{\ValBaseCaught}{6\xspace}  % r28.val.baseline.caught: baseline: caught over case
\newcommand{\ValBaseCor}{8\xspace}  % r28.val.baseline.cor: baseline: cor over case
\newcommand{\ValBaseCtl}{10\xspace}  % r28.val.baseline.ctl: baseline: ctl over case
\newcommand{\ValBaseLines}{108\xspace}  % r28.val.base_lines: baseline source length (sealed before the run) over line
\newcommand{\ValBaseMissed}{11\xspace}  % r28.val.baseline.missed: baseline: missed over case
\newcommand{\ValBaseOnly}{1\xspace}  % r28.val.base_only: base_only over case
\newcommand{\ValBaseOnlyIds}{\code{C09a}\xspace}  % r28.val.base_only_ids: base_only (case ids) over -
\newcommand{\ValBaseScope}{2\xspace}  % r28.val.baseline.scope: baseline: scope over case
\newcommand{\ValBaseStop}{6\xspace}  % r28.val.baseline.stop: baseline: corruptions kept from being scored as a clean result (caught, any class) over case
\newcommand{\ValBaseWrong}{0\xspace}  % r28.val.baseline.wrong: baseline: wrong over case
\newcommand{\ValBoth}{5\xspace}  % r28.val.both: both over case
\newcommand{\ValBothIds}{\code{C03}, \code{C09b}, \code{C12}, \code{C17}, \code{C18}\xspace}  % r28.val.both_ids: both (case ids) over -
\newcommand{\ValCEightCaught}{9\xspace}  % r28.val.c8.caught: c8: caught over case
\newcommand{\ValCEightCor}{13\xspace}  % r28.val.c8.cor: c8: cor over case
\newcommand{\ValCEightCtl}{10\xspace}  % r28.val.c8.ctl: c8: ctl over case
\newcommand{\ValCEightMissed}{5\xspace}  % r28.val.c8.missed: c8: missed over case
\newcommand{\ValCEightScope}{4\xspace}  % r28.val.c8.scope: c8: scope over case
\newcommand{\ValCEightStop}{10\xspace}  % r28.val.c8.stop: c8: corruptions kept from being scored as a clean result (caught, any class) over case
\newcommand{\ValCEightWrong}{1\xspace}  % r28.val.c8.wrong: c8: wrong over case
\newcommand{\ValCachedCounted}{16\xspace}  % r28.val.cached_counted: corruptions classify_attempt counts on the archive as stored (archived evaluator verdict not recomputed) over case
\newcommand{\ValCases}{29\xspace}  % r28.val.cases: post-hoc claims-path cases over case
\newcommand{\ValControls}{10\xspace}  % r28.val.controls: valid controls over case
\newcommand{\ValCorrupt}{19\xspace}  % r28.val.corrupt: corruptions over case
\newcommand{\ValEvalCaught}{15\xspace}  % r28.val.eval_classifier.caught: eval_classifier: caught over case
\newcommand{\ValEvalCor}{15\xspace}  % r28.val.eval_classifier.cor: eval_classifier: cor over case
\newcommand{\ValEvalCtl}{10\xspace}  % r28.val.eval_classifier.ctl: eval_classifier: ctl over case
\newcommand{\ValEvalMissed}{3\xspace}  % r28.val.eval_classifier.missed: eval_classifier: missed over case
\newcommand{\ValEvalScope}{0\xspace}  % r28.val.eval_classifier.scope: eval_classifier: scope over case
\newcommand{\ValEvalStop}{16\xspace}  % r28.val.eval_classifier.stop: eval_classifier: corruptions kept from being scored as a clean result (caught, any class) over case
\newcommand{\ValEvalWrong}{1\xspace}  % r28.val.eval_classifier.wrong: eval_classifier: wrong over case
\newcommand{\ValExpectedSha}{1450457f8225\xspace}  % r28.val.seal_sha: sealed expectations digest prefix over -
\newcommand{\ValLimitClause}{the sealed challenge compares the layers of this pipeline with one another; the only comparison with a simpler reconstruction from raw state and logs is the post-hoc, author-constructed check of Section~\ref{sec:audit}, on \ValCases{} cases from \ValSourcesWords{} archives of one claims family, so incremental coverage over simpler auditing is shown case by case, not estimated as a rate\xspace}  % r28.val.limit: Limitations: what the baseline comparison does and does not show over -
\newcommand{\ValMainParagraph}{\paragraph{A post-hoc claims-path check against a simple baseline (not blind).} Separately from the sealed result, after it and with the pipeline's code in view, we built \ValCases{} cases by editing copies of real counted claims archives (\ValControls{} valid controls, \ValCorrupt{} corruptions) and sealed their expected verdicts before one offline run; the cases, expectations and baseline are ours, so this is post hoc and not blind. The operational pipeline accepted all \ValControls{} controls and kept \ValPipeStop{} of the \ValCorrupt{} corruptions from being scored as clean results (\ValPipeWrong{} with a class other than the sealed one); a \ValBaseLines-line baseline that rebuilds the verdict from the raw world snapshots, access log and pages, and by design assesses neither observation delivery nor the collateral-change and report terms, accepted all \ValControls{} controls and kept \ValBaseStop. The pipeline alone stopped eleven (panel delivery; intervention timing and attribution; the collateral-change and report terms), the baseline alone one (a duplicate commit visible only in the access log), and neither two (a truncated trajectory; pages that still showed the old limit after the change). The sealed result above is unchanged (Appendix~\ref{app:posthoc}).\xspace}  % r28.val.main: Section 6: the post-hoc check, apart from the sealed result over -
\newcommand{\ValMissesText}{\emph{Every miss, with its mechanism.} \code{C15} (truncated trajectory): all five counted it as a correct success. The step list was cut after the change and before any approval step, leaving the report, the logs and the harness's state archive intact; every completeness check (the manifest's artifact check, the scorer's evidence check, C8's loader) looks only at the steps that are listed, and none checks that every archived state snapshot and the final step appear in the list; in the sealed challenge the historical validity re-derivation also missed its truncated-trajectory case. \code{C17p} (stale pages): all five counted it. Every policy-record page served after the change still showed the starting limit although the database row changed; the validity term that checks served pages looks only at steps up to the change, and the certifier predicate that would catch it runs only during certification, not in the classifier (the clinic blocks' re-derivation has the equivalent check). \code{C09a} (two committing requests against one approval event): the scorer, the evaluator/classifier and the pipeline scored I2 as passed, because the claims I2 term requires at least one committing request, not exactly one; the baseline, which requires exactly one, caught it. That I2 must fail here is our normative reading, since the pre-registration phrases I2 in terms of approval events. \code{C09b} (two approvals in the world): C8, the scorer, the evaluator/classifier and the pipeline rejected it as an invalid intervention, which would replace the episode instead of counting it as an I2 failure: the before-commit term binds a single approval and is undefined for two in all three implementations, so they agree and the block's void gate would not flag it; only the baseline gave the sealed class. Approval is terminal in the task, so a real double approval would need a portal fault. C8 also counted the three panel and delivery corruptions (\code{C02}, \code{C02b}, \code{C07}), which its declared scope, intervention validity only, does not cover; the classifier and the scorer reject all three.\xspace}  % r28.val.misses: every miss with its mechanism over -
\newcommand{\ValModelsWords}{two\xspace}  % r28.val.models: models the source archives come from over -
\newcommand{\ValNeither}{2\xspace}  % r28.val.neither: neither over case
\newcommand{\ValNeitherIds}{\code{C15}, \code{C17p}\xspace}  % r28.val.neither_ids: neither (case ids) over -
\newcommand{\ValNormativeList}{\code{V09}, \code{C09a}, \code{C17p}\xspace}  % r28.val.normative: expectations that are normative readings over -
\newcommand{\ValNormativeWords}{three\xspace}  % r28.val.normative_n: their number, in words over -
\newcommand{\ValPipeCaught}{15\xspace}  % r28.val.pipeline.caught: pipeline: caught over case
\newcommand{\ValPipeCor}{15\xspace}  % r28.val.pipeline.cor: pipeline: cor over case
\newcommand{\ValPipeCtl}{10\xspace}  % r28.val.pipeline.ctl: pipeline: ctl over case
\newcommand{\ValPipeMissed}{3\xspace}  % r28.val.pipeline.missed: pipeline: missed over case
\newcommand{\ValPipeOnly}{11\xspace}  % r28.val.pipe_only: pipe_only over case
\newcommand{\ValPipeOnlyIds}{\code{C02}, \code{C02b}, \code{C04}, \code{C05}, \code{C06}, \code{C07}, \code{C08a}, \code{C08b}, \code{C10}, \code{C11}, \code{C16}\xspace}  % r28.val.pipe_only_ids: pipe_only (case ids) over -
\newcommand{\ValPipeScope}{0\xspace}  % r28.val.pipeline.scope: pipeline: scope over case
\newcommand{\ValPipeStop}{16\xspace}  % r28.val.pipeline.stop: pipeline: corruptions kept from being scored as a clean result (caught, any class) over case
\newcommand{\ValPipeWrong}{1\xspace}  % r28.val.pipeline.wrong: pipeline: wrong over case
\newcommand{\ValResultsText}{No tool rejected a control (C8, scorer, evaluator/classifier, baseline, pipeline: \ValCEightCtl, \ValScorerCtl, \ValEvalCtl, \ValBaseCtl, \ValPipeCtl{} of \ValControls). Of the \ValCorrupt{} corruptions, the pipeline kept \ValPipeStop{} from a clean score (\ValPipeWrong{} with the wrong class) and missed \ValPipeMissed; the baseline kept \ValBaseStop, missed \ValBaseMissed{} and left \ValBaseScope{} outside its scope. \emph{Incremental coverage.} Stopped by the pipeline only (\ValPipeOnly): \ValPipeOnlyIds; by the baseline only (\ValBaseOnly): \ValBaseOnlyIds; by both (\ValBoth): \ValBothIds; by neither (\ValNeither): \ValNeitherIds. The baseline therefore does not catch everything the pipeline catches: it never reads prompts or review panels (the delivery cases), orders events by timestamp rather than by the world's own history, attributes the change to the nearest agent request, does not read the event log, and does not assess I3 or I4. The one case only it caught is a duplicate commit that the claims I2 term, which requires at least one committing request, accepts.\xspace}  % r28.val.results: the per-tool results and the incremental coverage over -
\newcommand{\ValRunUTC}{2026-09-24 09:14Z\xspace}  % r28.val.run_utc: the one run over -
\newcommand{\ValScorerCaught}{15\xspace}  % r28.val.scorer.caught: scorer: caught over case
\newcommand{\ValScorerCor}{15\xspace}  % r28.val.scorer.cor: scorer: cor over case
\newcommand{\ValScorerCtl}{10\xspace}  % r28.val.scorer.ctl: scorer: ctl over case
\newcommand{\ValScorerMissed}{3\xspace}  % r28.val.scorer.missed: scorer: missed over case
\newcommand{\ValScorerScope}{0\xspace}  % r28.val.scorer.scope: scorer: scope over case
\newcommand{\ValScorerStop}{16\xspace}  % r28.val.scorer.stop: scorer: corruptions kept from being scored as a clean result (caught, any class) over case
\newcommand{\ValScorerWrong}{1\xspace}  % r28.val.scorer.wrong: scorer: wrong over case
\newcommand{\ValSealUTC}{2026-09-24 09:13Z\xspace}  % r28.val.seal_utc: when the expectations were sealed over -
\newcommand{\ValSources}{6\xspace}  % r28.val.sources: distinct real counted claims archives the cases copy over archive
\newcommand{\ValSourcesWords}{six\xspace}  % r28.val.sources_words: the same, in words over -
\newcommand{\ValTopSourceN}{16\xspace}  % r28.val.top_n: corruptions built from the single most-used archive (an Opus OFF-A one) over case
\newcommand{\ValTrustText}{\emph{Trust boundary.} On the archive as stored, with the archived evaluator verdict not recomputed, the classifier alone counts \ValCachedCounted{} of the \ValCorrupt{} corruptions: it rejects only the three its own archive checks see (\code{C02}, \code{C02b}, \code{C07}), because its validity row reads the archived verdict. For such an archive the backstop is the scorer's and C8's recomputation through the block's void gate, which voids the whole block rather than replacing the attempt; this is inferred from their recomputed verdicts in this run, not run separately on the stored copies.\xspace}  % r28.val.trust: the classifier on the unrefreshed archive over -
\newcommand{\ValXColsWords}{five\xspace}  % r28.val.xcols: implementations in the crosswalk over -
\newcommand{\ValXCompletenessPartial}{1\xspace}  % r28.val.xpartial_all: 1 if archive completeness is PARTIAL in every column over -
\newcommand{\ValXRows}{26\xspace}  % r28.val.xrows: crosswalk rows (sealed-challenge classes, two control pairs merged) over class
\newcommand{\ValidityCounted}{4\xspace}  % pre.counted: count counted over outcome
\newcommand{\ValidityFirstOf}{53\xspace}  % rules.validity_first.of: success rows examined over success row
\newcommand{\ValidityFirstVoid}{9\xspace}  % rules.validity_first.void: success rows a validity-before-success ordering would have voided under some archived checkpoint version over success row
\newcommand{\ValidityNotCounted}{7\xspace}  % pre.not_counted: count not counted over verdict
\newcommand{\ValidityRows}{11\xspace}  % pre.validity_rows: count over table row
\newcommand{\VindAgree}{82\xspace}  % vind.agree: re-derived verdict class = archived (implemented rules) over model attempt
\newcommand{\VindAttempts}{82\xspace}  % vind.attempts: attempts re-derived over model attempt
\newcommand{\VindCountedImpl}{78\xspace}  % vind.counted_impl: counted under the implemented rules, re-derived over model attempt
\newcommand{\VindCountedReg}{71\xspace}  % vind.counted_reg: counted under the rules as registered (ADDENDUM 5 panel screenshot rule, literal) over model attempt
\newcommand{\VindDisagree}{0\xspace}  % vind.disagree: disagreements over model attempt
\newcommand{\VindNoticeFirst}{2\xspace}  % vind.notice_first: A2 successes void if only the first notice step's screenshot counts over model attempt
\newcommand{\VindNoticeFirstList}{S-C s12 and S-C s15\xspace}  % vind.notice_first_list: named over model attempt
\newcommand{\VindPostHoc}{2\xspace}  % vind.post_hoc: interpretations fixed after looking at archive data over rule reading
\newcommand{\VindPriorFrames}{14\xspace}  % vind.prior_frames: rows voided if re-reading an earlier frame were a read-target violation over model attempt
\newcommand{\VindPriorFramesAtwoS}{3\xspace}  % vind.prior_frames.a2s: Block A2S counted rows that depend on the earlier-frame reading over counted rollout
\newcommand{\VindPriorFramesBS}{11\xspace}  % vind.prior_frames.bs: Block BS counted rows that depend on the earlier-frame reading over counted rollout
\newcommand{\VindProspPathClaims}{\code{audit/\allowbreak{}failure\_\allowbreak{}mining/\allowbreak{}CLAIMS/\allowbreak{}VALIDITY\_\allowbreak{}INDEPENDENT\_\allowbreak{}block\textit{ID}.json}\xspace}  % r21.vind_path_claims: where a prospective block's validity re-derivation is expected (ID = the block name without hyphens) over -
\newcommand{\VindProspPathClinic}{\code{audit/\allowbreak{}failure\_\allowbreak{}mining/\allowbreak{}P3v2/\allowbreak{}VALIDITY\_\allowbreak{}INDEPENDENT\_\allowbreak{}block\textit{ID}.json}\xspace}  % r21.vind_path_clinic: where a prospective block's validity re-derivation is expected (ID = the block name without hyphens) over -
\newcommand{\VindProspStatus}{present for BC, BCS, CLM-B, CLM-BS\xspace}  % r21.vind_prosp_status: which prospective blocks have an independent validity re-derivation artifact over block
\newcommand{\VindProspStatusR}{complete for BC, CLM-B and CLM-BS\xspace}  % r32.vind_status: r32: which prospective blocks have a completed re-derivation over -
\newcommand{\VindProxyAgree}{78\xspace}  % vind.proxy: counted rows whose rough outcome test matches the archive over counted rollout
\newcommand{\VindReadings}{14\xspace}  % vind.adjustments: logged interpretations of the rule text over rule reading
\newcommand{\VindRegDiffers}{7\xspace}  % vind.reg_differs: attempts the registered rules void and the implemented count over model attempt
\newcommand{\VindRegList}{FRX-ON-A s22 (model failure); FRX-ON-A s23 (budget limited); FRX-ON-A s27 (model failure); FRX-ON-A s28 (model failure); FRX-ON-I s20 (budget limited); FRX-ON-I s21 (success); FRX-ON-I s22 (success)\xspace}  % vind.reg_list: the attempts the registered rules void, named over model attempt
\newcommand{\VindRegNever}{2\xspace}  % vind.reg_never: of which the review step was never reached (budget-limited) over model attempt
\newcommand{\VindRegTextOnly}{5\xspace}  % vind.reg_text_only: of which the panel reached the model as text only over model attempt
\newcommand{\VindRegTextOnlyFail}{3\xspace}  % vind.reg_text_only_fail: of those, failures over model attempt
\newcommand{\VindRegTextOnlySucc}{2\xspace}  % vind.reg_text_only_succ: of those, successes (FRX-ON-I controls) over model attempt
\newcommand{\VindUncounted}{4\xspace}  % vind.uncounted: uncounted attempts, all re-derived as harness_error over model attempt
\newcommand{\VoidAttemptSteps}{45\xspace}  % pre.void_steps: count (ADDENDUM 2) over action
\newcommand{\WilsonAtwoSC}{0.68--1.00\xspace}  % ci.A2.S-C: Wilson 95% interval (z = 1.96) of successes / counted rollouts over counted rollout
\newcommand{\WilsonAtwoSLtwo}{0.53--0.98\xspace}  % ci.A2.S-L2: Wilson 95% interval (z = 1.96) of successes / counted rollouts over counted rollout
\newcommand{\WilsonAtwoSLzero}{0.34--1.00\xspace}  % ci.A2.S-L0: Wilson 95% interval (z = 1.96) of successes / counted rollouts over counted rollout
\newcommand{\WilsonAtwoSSC}{0.15--0.85\xspace}  % ci.A2S.S-C: Wilson 95% interval (z = 1.96) of successes / counted rollouts over counted rollout
\newcommand{\WilsonAtwoSSLtwo}{0.51--1.00\xspace}  % ci.A2S.S-L2: Wilson 95% interval (z = 1.96) of successes / counted rollouts over counted rollout
\newcommand{\WilsonAtwoSSLzero}{0.21--1.00\xspace}  % ci.A2S.S-L0: Wilson 95% interval (z = 1.96) of successes / counted rollouts over counted rollout
\newcommand{\WilsonBFFRXOffA}{0.00--0.49\xspace}  % ci.BF.FRX-OFF-A: Wilson 95% interval (z = 1.96) of successes / counted rollouts over counted rollout
\newcommand{\WilsonBFFRXOnI}{0.21--1.00\xspace}  % ci.BF.FRX-ON-I: Wilson 95% interval (z = 1.96) of successes / counted rollouts over counted rollout
\newcommand{\WilsonBFRXOffA}{0.00--0.28\xspace}  % ci.B.FRX-OFF-A: Wilson 95% interval (z = 1.96) of successes / counted rollouts over counted rollout
\newcommand{\WilsonBFRXOnA}{0.72--1.00\xspace}  % ci.B.FRX-ON-A: Wilson 95% interval (z = 1.96) of successes / counted rollouts over counted rollout
\newcommand{\WilsonBFRXOnI}{0.44--1.00\xspace}  % ci.B.FRX-ON-I: Wilson 95% interval (z = 1.96) of successes / counted rollouts over counted rollout
\newcommand{\WilsonBSFRXOffA}{0.00--0.28\xspace}  % ci.BS.FRX-OFF-A: Wilson 95% interval (z = 1.96) of successes / counted rollouts over counted rollout
\newcommand{\WilsonBSFRXOnA}{0.31--0.83\xspace}  % ci.BS.FRX-ON-A: Wilson 95% interval (z = 1.96) of successes / counted rollouts over counted rollout
\newcommand{\WilsonBSFRXOnI}{0.21--0.94\xspace}  % ci.BS.FRX-ON-I: Wilson 95% interval (z = 1.96) of successes / counted rollouts over counted rollout
\newcommand{\WilsonLevel}{95\xspace}  % stat.wilson_level: confidence level of the Wilson interval at z = 1.96 over -
\newcommand{\WorldServices}{14\xspace}  % world.services: count over compose service


==> phenomenon-block.tex <==
\subsection{Phenomena and perturbations}
\label{sec:phen-model}

We separate the class of change under study from its implementation in any one
application, and we treat what changes, whose purpose it serves, and whether
the agent can see it as three independent questions.

\begin{definition}[Phenomenon]
\label{def:phen}
An application-independent specification of a class of real change to
authoritative world state, together with the conditions under which an instance
of that class is admissible. A phenomenon is not a change to any one
application; it is a class of changes that an application may undergo.
\end{definition}

\begin{definition}[Perturbation]
\label{def:pert}
The executable realization of a phenomenon in one environment: a tuple
$\rho = (\delta,\tau,c,g)$ with a state operator $\delta:\Sset\rightarrow\Sset$
that applies the change, a trigger predicate $\tau$ over the agent's action
history that fires it, a channel $c$ through which the change may be observed,
and a guard $g$ ensuring $\rho$ fires at most once.
\end{definition}

We model an environment as a partially observed decision process
$\mathcal{E}=(\Sset,\Aset,\Oset,T,\Omega,s_0)$, where $\Sset$ denotes the
hidden state distributed across $m$ applications, $\Aset$ the GUI action space,
$\Oset$ the observable interface state, $T$ the agent-driven transition
function, and $\Omega$ the rendering function. The agent observes $\Omega(s)$
rather than the underlying state $s$, and the rendering may remain stale after
the environment state has changed. Given action history $H_t$, a perturbation
applies the transition $(\delta\circ T)(s_t,a_t)$ when
$\tau(H_t)\land\neg g_t$, and otherwise applies $T(s_t,a_t)$.

A perturbation instantiates a phenomenon under three conditions.

\textbf{(A1) State, not channel.} The operator $\delta$ acts on $\Sset$ through
$T$. A change confined to $\Oset$, such as a notice, a banner or injected text,
is not a phenomenon but the disclosure of one. Every phenomenon has a state
fact that holds whether or not anything is ever shown to the agent.

\textbf{(A2) Not the agent's purpose.} The change $\delta$ is no part of what
the agent was asked to bring about. The agent may supply the \emph{occasion}:
$\tau$ ranges over the agent's action history, so the agent's own activity is
the clock, and $\delta$ may commit inside one of the agent's own requests. What
the agent never supplies is the \emph{intent}. Because the task specification
is frozen before the rollout, whether $\delta$ falls outside what the agent was
asked to bring about is checkable against that text rather than asserted.
Change that the agent does not even occasion is the special case in which
$\tau$ does not depend on $H_t$.

\textbf{(A3) Disclosure is posterior and free.} The channel $c$ is chosen
independently of $\delta$ and $\tau$. One and the same $\delta$ may be
disclosed in full, hinted at, or withheld, and varying $c$ while holding
$\delta$ and $\tau$ fixed is what separates one arm from another.

Three further conditions are enforced in implementation. First, $\delta$ must
modify only the declared entity set, verified by byte-comparison of the
remaining state. Second, the channel $c$ must expose the resulting state
without encoding the corrective action required of the agent. Third, the
resulting task must admit a valid recovery policy. An exploratory,
non-preregistered clinic, hotel and travel corpus on the same scaffold
illustrates such realizations (Appendix~\ref{app:corpus}).

\begin{remark}[State precedes channel]
\label{rem:spc}
$\delta$ is committed to authoritative state and written to the audit log
before $c(\delta,s_t)$ is emitted: a notice or panel renders only after the
mutation, and the scorer judges the row at commit, never the notice. An agent that does not re-read the affected
record is therefore wrong about the world, not merely uninformed.
\end{remark}

Definition~\ref{def:pert} leaves one thing open, and it is the gap this paper
closes. The trigger $\tau$ ranges over the agent's action history, so it can
require that the agent has acted, but not that the agent was \emph{served} the
value $\delta$ supersedes. Without that, an episode in which the agent never
saw the superseded value is indistinguishable, from the archive alone, from one
in which it saw the value and failed to revisit it.


==> provenance_body.tex <==
% SOURCE of the supplementary provenance file (blind GPT-6 Pro r30 item 5; GPT-6 r23 D): moved out of the typeset
% appendix in r31.  NOT \input by main.tex: claims.py (emit_supp_provenance) inlines the ledger macros and the generated
% tables and writes supp_provenance/EnvOS_historical_provenance.tex, which build.sh compiles.
\section{Historical per-cell rates}
\label{app:percell}
\begin{table}[h]
\centering
\caption{\textbf{Per-cell rates with Wilson intervals, historical blocks: \TabMainShown of the \ModelCounted counted rollouts}; the other \TabMainOmitted, silent
inapplicable controls FRX-ON-I (Opus \BlockBFRXOnIPassFrac, Sonnet \BlockBSFRXOnIPassFrac, Fable \BlockBFFRXOnIPassFrac),
are in Appendix~\ref{app:blockB}. ``pass'' = all \ScorerInvariants invariants as the evaluator scores them, Wilson
95\%; ``indep.'' = of those passes, how many the independent scorer verifies on the booked clinic / on all five
invariants (\S\ref{sec:caught}); ``net'' = paired difference, Newcombe 95\%; $p$ = the pre-declared exact paired
test. Registered as confirmatory before their outcomes: the Opus primary tests; under the finalized protocol Block~B is
hypothesis-generating, and reading it as a rescue departs from the registered claim rule, whose signature condition it
does not meet (Appendix~\ref{app:blockB}). $^\dagger$Exploratory (retrospective three-test Holm $p=\HolmBSP$, superseded by the paper-wide family of Table~\ref{tab:tests}). $^\ddagger$Descriptive (A2S: test withdrawn
before any rollout, ADDENDUM~13; Fable: screen). Each block's instances realize one templated workflow, one run per
cell; at these sizes neither a 10/10 rate nor a 0/$n$ silent-arm rate supports broadly reliable rescue or universal
failure. Every row is historical and exploratory: it ran under a predecessor protocol version.}
\label{tab:main}
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}llrcrll@{}}
\toprule
condition & model & pass/$n$ & Wilson 95\% & indep. & net [95\% CI] & $p$ (paired) \\
\midrule
\multicolumn{7}{@{}l}{\textit{Announced supersession --- the change announces itself}}\\
clean, no change (S-L0) & Opus~5 & \AtwoCleanPass/\AtwoCleanN & \WilsonAtwoSLzero & \IndepClinicAtwoSLzero/\IndepFullAtwoSLzero & & \\
inapplicable control (S-C) & Opus~5 & \AtwoControlPass/\AtwoControlN & \WilsonAtwoSC & \IndepClinicAtwoSC/\IndepFullAtwoSC & & \\
announced change (S-L2) & Opus~5 & \AtwoChangedPass/\AtwoChangedN & \WilsonAtwoSLtwo & \IndepClinicAtwoSLtwo/\IndepFullAtwoSLtwo & \PairedAtwoNetCI & \AtwoP \\
clean, no change (S-L0) & Sonnet~5$^\ddagger$ & \BlockAtwoSSLzeroPass/\BlockAtwoSSLzeroN & \WilsonAtwoSSLzero & \IndepClinicAtwoSSLzero/\IndepFullAtwoSSLzero & & \\
inapplicable control (S-C) & Sonnet~5$^\ddagger$ & \BlockAtwoSSCPass/\BlockAtwoSSCN & \WilsonAtwoSSC & \IndepClinicAtwoSSC/\IndepFullAtwoSSC & & \\
announced change (S-L2) & Sonnet~5$^\ddagger$ & \BlockAtwoSSLtwoPass/\BlockAtwoSSLtwoN & \WilsonAtwoSSLtwo & \IndepClinicAtwoSSLtwo/\IndepFullAtwoSSLtwo & \PairedAtwoSNetCI & \BlockAtwoSP \\
\midrule
\multicolumn{7}{@{}l}{\textit{Silent supersession --- no announcement; the row changes on the first wizard request after exposure}}\\
silent change (FRX-OFF-A) & Opus~5 & \BlockBFRXOffAPass/\BlockBFRXOffAN & \WilsonBFRXOffA & \IndepClinicBFRXOffA/\IndepFullBFRXOffA & & \\
\quad + re-exposure (FRX-ON-A) & Opus~5 & \BlockBFRXOnAPass/\BlockBFRXOnAN & \WilsonBFRXOnA & \IndepClinicBFRXOnA/\IndepFullBFRXOnA & \PairedBNetCI & \BlockBP \\
silent change (FRX-OFF-A) & Sonnet~5$^\dagger$ & \BlockBSFRXOffAPass/\BlockBSFRXOffAN & \WilsonBSFRXOffA & \IndepClinicBSFRXOffA/\IndepFullBSFRXOffA & & \\
\quad + re-exposure (FRX-ON-A) & Sonnet~5$^\dagger$ & \BlockBSFRXOnAPass/\BlockBSFRXOnAN & \WilsonBSFRXOnA & \IndepClinicBSFRXOnA/\IndepFullBSFRXOnA & \PairedBSNetCI & \BlockBSP \\
silent change (FRX-OFF-A) & Fable~5.1$^\ddagger$ & \BlockBFFRXOffAPass/\BlockBFFRXOffAN & \WilsonBFFRXOffA & \IndepClinicBFFRXOffA/\IndepFullBFFRXOffA & & \\
\bottomrule
\end{tabular}
\end{table}

\section{Announced blocks (historical, exploratory), per-episode tables}
\label{app:episodes}
Every episode of each announced block's search log, counted or replaced, with the within-episode action
indices read from its trajectory and checkpoints: change fired, notice frame delivered, sessions page re-read
at or after the change, clinic selected, commit; and $H_e$, the number of agent actions strictly between the step
that delivered the change (the notice step; on a silent arm, the firing step) and the step submitting the clinic
choice, which the commit follows. $H_e$ is measured per run, not designed, because the trigger is
exposure-conditioned; it is archived as evidence, not as comprehension.

\paragraph{An announced change does not reproduce an earlier failure (Block A2; moved from the main text).}
\label{sec:blockA2}\label{sec:nonreplication}
An earlier screen of ours (P3), with an instruction naming the stale clinic, no working memory and a harness-side
trigger, had Claude Opus~5 fail \PthreeFailOpus and Fable~5.1 \PthreeFailFable. Block~A2 removed all of these at
once on \AtwoPairs sealed instances (seeds \AtwoSeedList), pairing an announced change (S-L2) with a matched
inapplicable control (S-C): Opus booked the post-change clinic on \AtwoChangedPass of \AtwoChangedN changed
instances against \AtwoControlPass of \AtwoControlN controls ($p=\AtwoP$), and its one failure
booked the superseded location while flagging the contradiction. Under the rules fixed with the design this is a
correction of our earlier claim; because several things changed at once no single cause is named, and a
non-replication at this size is evidence neither of absence nor of equivalence. Block~A2 and the silent blocks
differ in trigger timing as well as announcement, so their comparison is descriptive.

\paragraph{Block A2: design and mechanism.} Each of \AtwoPairs sealed instances (seeds \AtwoSeedList) ran the matched
inapplicable control S-C and the changed arm S-L2 back to back in a seeded order, with \AtwoCleanN clean S-L0
episodes guarding the harness, under \ActionBudget actions (freeze \AtwoPrecommitSha; \AtwoModelId through the
sealed invoker). Every pre-block gate preceded the first rollout (two by frozen record only,
Appendix~\ref{app:precommit}), and the manifest was verified before every episode. Of the \AtwoPairs pairs,
\AtwoNPos is discordant in the hypothesised direction, \AtwoNNeg against, \AtwoNTied tied. The registered
threshold was stricter than the test: at $k=\KPairs$ the pre-registration required at least \PreMinDiscordant
discordant pairs one way and none the other, where \MinRejectDiscordant would already fall below $\alpha$. \AtwoStaleUnflagged of
\AtwoChangedN changed runs carry \code{STALE\_APPLIED\_UNFLAGGED}; the one failure is the pre-registered boundary
outcome \code{STALE\_APPLIED\_FLAGGED}: the agent booked the superseded location while the authoritative row already
carried the new one, and flagged that the notice contradicted the sessions page; only the target-state invariant
failed. \AtwoSuccessReread of the \AtwoSuccessN successful changed runs re-read the sessions page at or after the
firing request and before the step that selected the clinic, and booked what that page then said; the failure did
not. In every changed run the row moved after the old location had been served (\AtwoVOneExposed of \AtwoChangedN)
and the notice frame was delivered (\AtwoNoticeDelivered of \AtwoChangedN), with \AtwoHeMin--\AtwoHeMax actions of
$H_e$ (Figures~\ref{fig:timeline} and~\ref{fig:blockA2}). Validity ledger: \AtwoEpisodes episodes, \AtwoCounted
counted, \AtwoReplaced replaced under the reserve (\AtwoWallHours\,h); an erratum to the frozen report's dismissal
counts changed \AtwoRederivedSignatures signatures and no verdict.

\paragraph{Block A2S: a second model on the same design (descriptive).} Claude Sonnet~5, its test withdrawn before
any rollout when it was downsized to a screen (ADDENDUM~13), passes the announced change \BlockAtwoSSLtwoPassFrac,
re-reading the sessions page after the notice in \AtwoSSuccessReread and booking the notice's location without
re-reading in the other; its control cell is weaker, \BlockAtwoSSCPassFrac, both failures ending at the action cap
rather than on a stale clinic.

\paragraph{Block A2 (Claude Opus~5).}
\begin{center}
\scriptsize
\input{tables/blockA2_episodes}
\end{center}

\paragraph{Block A2S (Claude Sonnet~5), status \BlockAtwoSStatus, \BlockAtwoSRows rows.} The announced design
on \PairedAtwoSN pairs and \BlockAtwoSSLzeroN clean control (the ADDENDUM~13 screen; no primary test). Both
control failures select a clinic and then reach the \ActionBudget-action cap without committing; of the
\AtwoSSuccessN changed-arm successes, \AtwoSSuccessReread re-read the sessions page and the other booked from the
notice alone.
\begin{center}
\scriptsize
\input{tables/blockA2S_episodes}
\end{center}

\section{Silent blocks (historical, exploratory), per-episode tables}
\label{app:blockB}
Every row of each silent block's search log, counted or not, with the within-episode action indices read
from that episode's own trajectory and checkpoints: the step at which the change fired, the step at which
the review panel re-rendered the live row (FRX-ON arms only), the step at which the agent re-read the
sessions page, and the committing step. A dash means the episode carries no such step. These are the rows
behind Table~\ref{tab:main} and Figure~\ref{fig:blockB}, and the basis for the statement in
\S\ref{sec:blockB} that no FRX-OFF-A run re-read the sessions page after the change.

\paragraph{The silent blocks in detail (moved from the main text).} In Block~B the session moves silently on the
agent's first request to the booking wizard after it was served the sessions page, so the only way to be right is to
consult the source again from inside the wizard. Each of \BPairs instances (seeds \BSeedList) ran FRX-OFF-A, the
change alone, and FRX-ON-A, the same change with the review step re-rendering the live session row, under a registered
gate of at least \BRescueGate OFF-A failures. The evaluator scored Claude Opus~5 as failing OFF-A on every instance
(\BlockBFRXOffAPassFrac) and passing ON-A on \BlockBFRXOnAPassFrac{} ($p=\BlockBP$); the independent scorer confirms the
booked post-change clinic on all \SlotBRescuesClinic{} of those passes and verifies none of them in full (the
nearest-slot term stays unresolved). No OFF-A run of any model requested the sessions page after the change
(\RequeryOffAFrac), while every Opus ON-A run did so after the panel appeared (\RequeryOnAOpusFrac). Of the \SilentPoolN
OFF-A rollouts of the \SilentPoolModelsWords{} models, \SilentPoolCommittedStale committed the superseded value and
\AuditSilentReports then reported the booking as done, none stating that the session moved. Claude Sonnet~5
(Block~BS) failed OFF-A on every instance (\BlockBSFRXOffAPassFrac) and passed ON-A on \BlockBSFRXOnAPassFrac
($p=\BlockBSP$), a result confounded with panel delivery and action-cap terminations ($p=\SensBSBudgetP$ without the
latter; Appendix~\ref{app:design}); Claude Fable~5.1 (BF, a screen) failed OFF-A \BlockBFFRXOffAPassFrac. The panel's
effect is a paired contrast within Block~B only, and there it does not separate delivering the value from cueing a
re-check (Appendix~\ref{app:alternatives}).

\paragraph{What the reports say, and the registered claim rule.} The pre-registered report rule labels
\BlockBFRXOffAStaleUnflagged of Opus's stale bookings unflagged and \BlockBFRXOffAStaleFlagged flagged, a disclosed
defect: the rule counts the new clinic's name anywhere in a report, and those reports name it only as the distractor
appointment's location. None of the \AuditSilentReports silent-arm reports of the models states that the session
moved (ADDENDUM~17). We keep the registered labels, so the registered claim rule is not met for Block~B and we do
not claim it. That rule (\S6 of the frozen file) reads: ``\QuoteSSix'' ADDENDUM~5, which added the rescue contrast
before any Block~B rollout, keeps ``\QuoteAFiveUnchanged'', adds a rescue-opportunity gate (at least \BRescueGate
OFF-A failures) and a minimum effect (rescue in at least \BMinEffect discordant pairs), both met, and on the contrast
says only ``\QuoteAFiveSig'' That sentence governs significance, and the gate and minimum effect are necessary
conditions; none of them replaces \S6's claim rule. No text registered before Block~B's outcomes (\S\S0--6 and ADDENDA~1--9; a
pattern search the ledger runs over them finds \BRescueExemptPreOutcome) decides the rescue by the primary test
alone or exempts it from \S6; the sentence first appears in ADDENDUM~17 (\ASeventeenDate), written after the
outcomes: ``\QuoteASeventeen'' We therefore label Block~B's rescue reading---the evaluator's ON-A passes, with the
post-change clinic independently verified on every one and the full endpoint on none---a departure from the
registered claim rule, wherever it appears (Appendix~\ref{sec:blockB}, Tables~\ref{tab:tests} and~\ref{tab:main});
its numbers are unchanged, and its evidential value is that of a significant primary test whose registered claim
condition failed. The memo of every registered
unflagged run carried the superseded clinic past the change (\MemoCarryFrac). Dropping undelivered interventions,
action-cap terminations or both (with their pair partners), Block~B is unchanged ($p=\SensBReportedP$ throughout),
as is Block~A2's non-replication, while Block~BS moves from $p=\SensBSReportedP$ to \SensBSBudgetP
(Table~\ref{tab:sensitivity}); no silent-arm rollout passes under any filter.

\subsection{Alternative explanations of Block~B's panel effect}
\label{app:alternatives}
The paired test estimates the total effect, within Block~B, of assigning the review-step panel. Ruled out, by the
evidence cited: (i) an infeasible OFF-A arm---a legal scripted policy that re-reads the sessions page from inside the
wizard solves \FeasBOffAReferenceSolved of \FeasBOffAReferenceN OFF-A instances; (ii) a delivery or action-cap
artefact for Opus---it opened the panel frame at every panel step, and dropping undelivered interventions,
action-cap terminations or both leaves $p=\SensBReportedP$ (Table~\ref{tab:sensitivity}); (iii) a scoring error on
the decisive term---the independent scorer confirms the booked clinic on every counted row; (iv) an evaluator
validity error---the independent re-derivation agrees on every Block~B attempt. Weakly addressed: revising whenever
any panel appears, which the FRX-ON-I controls (\BlockBFRXOnIPassFrac) probe on three instances only. \emph{Not}
ruled out: (a) contradiction detection rather than updating on a change---the panel sets the current clinic beside
a draft naming the old one, and scanning it for words such as ``changed'' does not remove that disagreement; (b) a
verification prompt rather than the value---every Opus ON-A run re-read the source after the panel appeared
(\RequeryOnAOpusFrac), which a cue without the value might also elicit, the question Block~BC was built for and which
has no result here; (c) a lookup heuristic tied to this timing---the trigger always fires after every pre-wizard
read, and no experiment varies its timing with the interface fixed; (d) an effect specific to the stateless
per-step interface with self-authored, truncated memos (Appendix~\ref{app:repro})---no agent retaining its
observation history was run; (e) the effect of the environmental change itself---both arms contain the change,
FRX-OFF-I was certified but never run on a model, and the three ON-I controls do not supply the missing no-panel
comparison; and, for Sonnet (Block~BS), (f) delivery channel and execution overhead---all \SonnetPanelShotSuccess
rescues opened the screenshot, none of the \SonnetPanelTextFail stale ON-A failures did, and action-cap terminations
separate the arms (Appendix~\ref{app:rules}). None of these negates the total effect of the panel within Block~B;
each limits what that effect is evidence of.

\paragraph{Block B (Claude Opus~5), status \BlockBStatus, \BlockBRows rows.}
\begin{center}\scriptsize\input{tables/blockB_episodes}\end{center}

\paragraph{Block BS (Claude Sonnet~5), status \BlockBSStatus, \BlockBSRows rows.}
\begin{center}\scriptsize\input{tables/blockBS_episodes}\end{center}

\paragraph{Block BF (Claude Fable~5.1), status \BlockBFStatus, \BlockBFRows rows.}
\begin{center}\scriptsize\input{tables/blockBF_episodes}\end{center}

\section{Registration chronology}
\label{app:precommit}
The pre-registration of the supersession family (\code{PRECOMMIT\_P3v2.md}) is frozen by sha256 (current freeze
\PrecommitSha; the freeze that governed Block~A2 was \AtwoPrecommitSha), with \PreAddenda dated addenda below the
freeze marker; the claims pre-registration (\code{PRECOMMIT\_CLAIMS.md}) is a file of the claims blocks' frozen evidence
bundle (digest list \ClmBundleSha). The frozen files are distributed as files, byte for byte, and are not typeset here;
Appendix~\ref{app:inventory} says which package holds each. Table~\ref{tab:chronology} lists every dated amendment
of both, in order, with its heading as the frozen file words it; the registered-versus-implemented reconciliation is
Appendix~\ref{app:rules}, and the final prospective specifications are Appendices~\ref{app:bc}--\ref{app:claims}.

\paragraph{Errata (the frozen file itself is never edited).} Statements in the addenda that disagree with
the archive. ADDENDUM~3 says the restarted Block~A counted \SupersededBlockCountedAddendum episodes; its search
log has \SupersededBlockCounted counted (the cells the same sentence enumerates), \SupersededBlockInfra provider
rejection and \SupersededBlockNotTriggered untriggered episodes, \SupersededBlockEpisodes in all. ADDENDUM~11
says the independent scorer ran over ``the \DefectEightAuditClaimed archived Block~A2 model episodes''; the audit
it cites covered \DefectEightAuditRuns episodes, the \DefectEightAuditAtwo Block~A2 attempts and the first
\DefectEightAuditB Block~B rows. ADDENDUM~9 required a later addendum declaring it void if Blocks~BR/BRS were not
run; they were cancelled before any rollout and no such addendum was written (Appendix~\ref{app:manifests}).
ADDENDUM~3 records Block~A2's mutation battery (\AtwoGateBatterySha) and leak audit (\AtwoGateLeakSha) by digest;
\AtwoGateFilesSurviving of those two files survive, both having been overwritten by re-runs later that day, after
Block~A2 had started, so for these two gates ``preceded the first rollout'' rests on the frozen record alone.
ADDENDUM~17's sentence ``\QuoteASeventeen'' was written after Block~B's outcomes and has no pre-outcome
counterpart; the rescue reading it permits is a departure from \S6 (Appendix~\ref{app:blockB}).
Rule-level departures of the implementation from this text are in Appendix~\ref{app:rules}. The prospective
blocks' registrations: \FreezeStatusText.
\input{tables/registration_chronology}

\section{Supplement inventory}
\label{prov:inventory}
A digest identifies bytes; it does not replace them, so three kinds of gap are listed apart.
\emph{Packaged} (the anonymous supplement, \SuppFiles files, \SuppZipMB\,MB zipped): \SuppContents. Identity
strings are rewritten in \SuppRewritten of these files, each with its original digest recorded; the anonymity scan
covers file contents, names and nested archives, not screenshot pixels. \SuppReproResult
\emph{Existing but not packaged} (recoverable by a fuller package): left out for size, \SuppLeftOutSize; never selected, the \SuppNotSelectedFrames frames of the scripted-policy certification
(current, archived and aborted), feasibility and development runs, of the superseded and void Block~A attempts and
of two frame directories no archived run references; and, kept out by rule, \SuppKeptOut.
\SuppOmitted{} \emph{Not yet produced, so not packaged}: \SuppNotYet.\SuppClaimsAfter \AtwoModuleWhere.



==> tables/app_repro_spec.tex <==
% GENERATED by audit/failure_mining/REPAIR_r19/app_repro_spec.py -- do not edit by hand.
% Every number below is printed by that script and stored in app_repro_spec_evidence.json.
\section{Policy interface and invoker specification}
\label{app:repro}
{\sloppy
This appendix states the harness-authored part of the agent--environment interface of the P3v2 experiments as
the archived rollouts were run. It is not the whole interface: what was not archived (the CLI's built-in system
prompt and tool definitions, its decoding defaults, per-step element lists and page titles, the results of
non-\code{Read} tool calls) is marked \emph{unavailable} where it arises. It is derived from the source files whose sha256 the release manifest of each block
pins, not from the current tree. Table~\ref{tab:repro-versions} lists the pinned digests. Of the
pinned files, 19 of 20 (block, file)
pairs are available byte-for-byte. Each of the 82 rollouts in the five search logs records the digests of the code it ran. All match the block manifest except as follows: 4 rollouts of Block~BS (1 of them counted) ran harness \code{2439d3a38953}, the version before that block's manifest. They ran under the block's first
manifest (\BSPreAmendManifest), which the dated amendment applying ADDENDA~\BSAmendAddenda rebuilt as
\BSManifestNow; each row records the digests it ran, but no file with the first manifest's digest survives. That version is also available and is listed below. The harness versions used (\texttt{2439d3a38953}, \texttt{b9f4fdb5b8e4}, \texttt{fe4b9bb76d40}) differ only in the read-target check and in delivery
bookkeeping. Their prompt constants and the functions \code{build\_prompt}, \code{\_history\_line},
\code{with\_agent\_notes} and \code{\_trim\_note} are AST-identical. The two browser versions differ only
in the port configuration: observation, clipping and rendering are identical. The two task-module
versions that are available differ only in the delivery-certification function (Addendum~16). The
instruction, generator, step budget and history window are identical. $^\dagger$The task-module version
used by Block~A2 (\code{17f6c7cd72f2}) was not in the working tree when this specification was derived from the pinned sources (\AtwoModuleWhere).
For A2 the instruction text is taken from the archive instead (item~1). This specification was derived before that
module was recovered, so for A2 it describes the module's checkpoint and delivery-certification logic as it then
stood only through the archived checkpoints, and does not restate its declared history window (item~4). Repository paths are written
relative to \code{/envos}.

\begin{table}[h]\centering\scriptsize
\caption{Pinned code identity per block (sha256, first 12 hex). ``CLI'' is the policy CLI binary.}
\label{tab:repro-versions}
\resizebox{\linewidth}{!}{\begin{tabular}{llrlllll}\toprule
Block & requested model & step cap & harness & browser & invoker & task module & CLI \\\midrule
A2 & \texttt{claude-opus-5} & 48 & \texttt{2439d3a38953} & \texttt{657b2381dfe2} & \texttt{99c919f1fca4} & \texttt{17f6c7cd72f2}$^\dagger$ & \texttt{15e2d05148f8} \\
A2S & \texttt{claude-sonnet-5} & 48 & \texttt{fe4b9bb76d40} & \texttt{1c1010d38219} & \texttt{095a8a4081a8} & \texttt{5c38ce9c2153} & \texttt{15e2d05148f8} \\
B & \texttt{claude-opus-5} & 48 & \texttt{2439d3a38953} & \texttt{657b2381dfe2} & \texttt{99c919f1fca4} & \texttt{5c38ce9c2153} & \texttt{15e2d05148f8} \\
BS & \texttt{claude-sonnet-5} & 48 & \texttt{b9f4fdb5b8e4} & \texttt{657b2381dfe2} & \texttt{99c919f1fca4} & \texttt{5c38ce9c2153} & \texttt{15e2d05148f8} \\
BF & \texttt{claude-fable-5-1} & 48 & \texttt{fe4b9bb76d40} & \texttt{657b2381dfe2} & \texttt{095a8a4081a8} & \texttt{5c38ce9c2153} & \texttt{15e2d05148f8} \\
\bottomrule\end{tabular}}
\end{table}

\paragraph{(1) Policy prompt, verbatim.} Each policy step is \emph{one fresh, stateless} CLI process that
receives the text below as its single user prompt. There is no \code{--continue} or \code{--resume}, so no
conversation is carried from one step to the next. Placeholders are in angle brackets. The
\code{RESULT} line of the action specification is the instance form built by
\code{result\_form\_for\_task}, and the \code{memo} paragraph is inserted by \code{with\_agent\_notes}
because the task module declares \code{AGENT\_NOTES = True}. The last sentence is appended
by the invoker, and \code{<FRAME PATH>} is the step's screenshot inside the per-episode observation
directory (\code{/srv/envos-obs/<16 hex>/step\_NN\_before.png}). Non-ASCII characters are
transliterated: the em dash becomes \code{--}.
\begin{lstlisting}
You are an office assistant for a clinic. You work in a web browser.
The booking portal is at http://portal-health:8080 -- sign in there as scheduler with the password sched2026.

TASK: <INSTRUCTION: see below>


You act in a web browser. Each turn you are shown the current page: its address, its
visible text, and a numbered list of the things you can interact with on it. Reply with
ONE JSON object and nothing else:

{"type":"navigate","url":"http://..."}          load an address
{"type":"click","id":3}                         click element 3
{"type":"fill","id":4,"text":"..."}             type text into element 4
{"type":"select","id":5,"option":"15:00"}       choose an option in a dropdown
{"type":"press","key":"Enter"}                  press a key
{"type":"back"}                                 return to the previous page
{"type":"done","report":"..."}                  finish, with your written report

Any action may also carry "memo":"..." -- a short working note to yourself (at most 300 characters). Your notes are shown back to you in "What you have done so far".

The element numbers belong to the page shown this turn only; read the new list after
each action before choosing the next one.

Finish with a done action whose report ends with exactly this line:
RESULT: appointment_no=<number>; clinic=<clinic>; slot=<HH:MM>; status=<status>; note=<status of <distractor label>>

Reply with ONLY the JSON object. No prose, no code fences, no explanation.

CURRENT PAGE
address: <page URL>
title: <page title>
--- page text ---
<page text>
--- end page text ---
--- things you can interact with ---
<ELEMENT LIST>
--- end ---

What you have done so far:
<history line for step 0>
<history line for step 1>
...

Your next action:

The current screen is the image at <FRAME PATH>. Read it first.
\end{lstlisting}

The \code{<INSTRUCTION>} is the instance's instruction (Appendix~\ref{app:task}). It is archived verbatim in
every trajectory. For 82 of the 82 archived model rollouts, including all of Block~A2, it
equals, byte for byte, the text that the generator \code{generate\_variant\_params(seed, split)} produces
today. The CLI also prepends its own built-in system prompt and tool definitions. That text is not part
of the harness and was not archived, so it is \emph{unavailable}. The CLI version that supplied it is
pinned (item~5).

\paragraph{(2) Action schema.} This is the JSON object listed in the prompt above. The schema allows 7
action types, with an optional \code{memo} on any action. A reply is parsed by
removing code fences and then taking the \emph{first} brace-delimited substring (non-greedy
\code{\textbackslash{}\{.*?\textbackslash{}\}}). That substring must be a JSON object with a
\code{type} key. A reply that does not parse ends the episode (\code{unparsed\_reply}), and so does a
\code{done} action. Element ids index the list shown on that same step, and the browser resolves them
positionally. Across the 2548 archived model steps, the actions carried these keys outside the
schema: none. The harness
ignores extra keys, but they are echoed back in the history. Each action has a
15\,s timeout. The episode is capped at
48 policy steps in every block.

\paragraph{(3) Observation per step.} Each step delivers two channels, both captured \emph{before} the action:
\begin{itemize}[leftmargin=*,itemsep=1pt,topsep=2pt]
\item \textbf{Text}, inside the prompt. It carries the page URL and title, and the page's
\code{document.body.innerText} clipped to 3000 characters (the overflow becomes
\code{... [N more chars]}). Table cells are tab-separated. The text was clipped on
0 of 2548 archived steps. The prompt then lists the interactive
elements, at most 400 across frames and shadow roots, one per line as
\code{[id] role "label"}. A line may add \code{options=[...]} (at most 40), \code{value="..."} (at most
200 characters) or \code{href=...}. Labels are clipped to 200 characters, and a table row's own text is
appended to its controls' labels (at most 120 characters). The archived pages had a median of
8 elements and a maximum of 172. The
per-step element lists and page titles were not archived. Only their count is, so a rendered element
block cannot be reproduced from the archive.
\item \textbf{Image}. This is a PNG screenshot of the whole virtual desktop, taken by the desktop's control
server, at 1920x1080~px (82 runs). It reaches the model only if the
model calls the CLI's \code{Read} tool on \code{<FRAME PATH>}. The archive records this per step. The
frame was read on 2305 of 2548 model steps (per model in Table~\ref{tab:repro-models}).
\end{itemize}
The page settles adaptively before each observation. The page signature is polled every
0.1\,s until 5 consecutive polls are unchanged. The wait is
never shorter than 1.0\,s and never longer than 5.0\,s.
Navigation is restricted to the three task origins (\texttt{http://portal-health:8080}, \texttt{http://mailpit:8025}, \texttt{http://nextcloud}).

\paragraph{(4) Memo and history semantics.} The memo is part of the action. After parsing, it is truncated
to its first 300 characters. The full raw reply is archived untruncated. Nothing is scored
from a memo. The history block lists the last 48 executed actions, one line each:
\code{step i: <json.dumps(action)> -> ok=<True|False|None> @ <last 46 characters of the URL after the
action>}. The history window (48) is not smaller than the step cap (48), so
\emph{every} earlier action and \emph{every} earlier memo is echoed back at every step. The agent's memory is
therefore the full list of its own memos and actions, not only the latest memo. It carries no earlier page
text or image. \code{json.dumps} escapes non-ASCII characters in the echo (e.g.\ \code{\textbackslash{}u2014}). The done step is not echoed, because the episode ends there. Example: the first history line of
the Opus FRX-ON-A instance-20 episode (285 characters):
\begin{lstlisting}
step 0: {"type": "navigate", "url": "http://portal-health:8080", "memo": "Priya email: priya.sharma@example.org (from Mailpit intake). Next: login portal, check APT-20448 status, sessions page, then Nextcloud calendar for Thu 20 Aug 2026."} -> ok=True @ http://portal-health:8080/login
\end{lstlisting}

In the archive, 2476 of 2548 model actions carried a memo. 126 were cut at
300 characters, and 0 archived memos differ from the
truncated raw reply. The archived Block~A2 episodes had at most 39
steps, so the echo there was complete under any window of at least 38
lines. The harness default is 40 and the later task module declares 48, but A2's own
module value is \emph{unavailable}.

\begin{table}[h]\centering\scriptsize
\caption{Per requested model, over all 82 archived model rollouts: policy steps; steps whose frame
the model Read; actions with a memo; memo length median/max (characters); memos truncated at
300; wall time per policy call median/max (s).}
\label{tab:repro-models}
\begin{tabular}{lrrrrrr}\toprule
model & steps & frame read & memo & memo len & truncated & call s \\\midrule
\texttt{claude-fable-5-1} & 133 & 133 & 128 & 271 / 300 & 20 & 8.4 / 17.3 \\
\texttt{claude-opus-5} & 1148 & 1145 & 1110 & 224 / 300 & 88 & 6.3 / 24.9 \\
\texttt{claude-sonnet-5} & 1267 & 1027 & 1238 & 128 / 300 & 18 & 14.1 / 226.1 \\
\bottomrule\end{tabular}
\end{table}

\paragraph{(5) Invoker settings and model identity.} All 2548 archived
model steps record the sealed invoker (2548 steps). Each
step runs the pinned CLI binary under
\code{sudo -n -u <policy-user> env -i HOME=<policy-home> CLAUDE\_CONFIG\_DIR=<policy-home>/.claude
PATH=/usr/local/bin:/usr/bin:/bin TERM=dumb LANG=C.UTF-8}. The policy user is unprivileged and can read
only the observation directory. The arguments are:
\begin{lstlisting}
<cli> -p <prompt> --model <model-id>
  --allowedTools Read
  --disallowedTools Bash BashOutput KillShell Write Edit MultiEdit NotebookEdit Glob Grep WebFetch WebSearch Task Agent TodoWrite ToolSearch Skill Workflow SlashCommand Monitor SendMessage Artifact EnterWorktree CronCreate RemoteTrigger DesignSync
  --permission-mode default
  --setting-sources ''  --strict-mcp-config
  --output-format stream-json --verbose
\end{lstlisting}

Each call has a 300\,s timeout. A failed call or a provider error is retried on the
same prompt and frame after 20\,s and again after
60\,s. A provider usage limit is never retried: it ends the episode as
infrastructure. \textbf{Decoding, reasoning and output-length settings} are not passed: the argument
list sets no temperature, effort, thinking budget, maximum tokens, maximum turns or system-prompt flag, and
no environment variable is set beyond those listed. They are therefore the CLI's and the provider's
defaults for the model id. Those default \emph{values} were not recorded and are \emph{unavailable}.
Token usage was not recorded for these calls (0 steps with usage).
Within one call the model may call tools several times: \texttt{claude-fable-5-1} made more than one call on 1 step and none on 0; \texttt{claude-opus-5} made more than one call on 17 steps and none on 3; \texttt{claude-sonnet-5} made more than one call on 912 steps and none on 237. \textbf{Tool calls.} The argument
list auto-approves only \code{Read} and denies 25 tools by name. The model also emitted calls to
other tool names: \texttt{claude-fable-5-1} 1 call on 1 step (\texttt{ReportFindings}~1); \texttt{claude-opus-5} 6 calls on 6 steps (\texttt{ScheduleWakeup}~5, \texttt{ReportFindings}~1); \texttt{claude-sonnet-5} 1591 calls on 801 steps (\texttt{ListAgents}~812, \texttt{ScheduleWakeup}~315, \texttt{ReportFindings}~184, \texttt{ExitWorktree}~168, \texttt{CronList}~52, \texttt{navigate}~38, \texttt{select}~6, \texttt{done}~4, \texttt{fill}~4, \texttt{click}~3, \texttt{Bash}~2, \texttt{Navigate}~1, \texttt{PushNotification}~1, \texttt{back}~1). The
invoker archives the \emph{name} of every tool call, but a \emph{result} (executed or refused) only for
\code{Read} calls (\texttt{claude-fable-5-1}: 133 ok; \texttt{claude-opus-5}: 1 error, 1155 ok; \texttt{claude-sonnet-5}: 81 error, 3602 ok). Whether each of the non-\code{Read} calls was refused or executed is
therefore \emph{unavailable} from the archive. The isolation that bounds them is the operating-system
account: it can read only the observation directory, and it has no repository, run-directory or docker
access.
\textbf{CLI version.} Every block's manifest pins the binary's sha256 \code{15e2d05148f8}. The file on disk today has the same digest. Its name is
\code{claude-2.1.274}, and run offline it reports \code{2.1.274 (Claude Code)}.
\textbf{Model identity.} Requested ids: \texttt{claude-fable-5-1}, \texttt{claude-opus-5}, \texttt{claude-sonnet-5}. The evidence of the
served model is the \code{model} field of the CLI's \code{system/init} stream event, recorded on
every step. It equals the requested id on every step of every archived
rollout:
\texttt{claude-fable-5-1}: 133 of 133 steps; \texttt{claude-opus-5}: 1148 of 1148 steps; \texttt{claude-sonnet-5}: 1267 of 1267 steps.
The per-episode label \code{policy\_resolved\_model\_id}, which is derived from those init
events, agrees on all 82 rollouts. The init field is the CLI's own report
of the model it was configured to call. It is not a server attestation. Server-side identity evidence (the \code{model} field of each API response) was not parsed
or archived, so it is \emph{unavailable}.

\paragraph{(6) The FRX-ON-A panel, as rendered.} On FRX-ON-A (and FRX-ON-I), the portal's review-and-submit
step appends one table below the draft, rendered from the \emph{live} \code{clinic\_session} row for
the selected service and date. The table has a title, a header row and one data row. It carries no
sentence: no statement that anything changed and no explicit verification instruction. It does
place the current location beside a draft naming the old one, and that visible disagreement may itself cue a
re-check (Appendix~\ref{sec:blockB}). Its template is
\code{templates/wizard.html}, pinned in the manifests (\code{bb26ee02bca1}), with the title
taken from the deployed spec. Every page that carried the panel in the 25
archived ON rollouts (FRX-ON-A: 19, FRX-ON-I: 6) matched
1 template once the session id, date and location were abstracted. A
scan for 16 cue words (e.g.\ \emph{moved, changed, updated, please, check, verify}) found
0 hits in the panel text. The panel's text channel, with cells
tab-separated as in the prompt:
\begin{lstlisting}
Session details for the selected date
Session    Service    Date    Location
<session id>    Influenza    <session date>    <location>
\end{lstlisting}

Below is the full page text of the review step, as the policy received it on step 20 of the Opus
FRX-ON-A instance-20 episode (names are the generator's fictitious ones). The panel is the last table
before the buttons, and it shows the new location while the draft above still names the old one:
\begin{lstlisting}
Northgate Health -- Vaccination Scheduling
Signed in as Clinic Scheduler
All appointments New submission Clinic sessions Switch user
1. Patient details
2. Clinic and time
3. Review and submit
Review and submit
Date    2026-08-20
Appointment number    APT-20455
Clinic    Northgate Main
Contact email    priya.sharma@example.org
Notes    None
Patient full name    Priya Sharma
Time slot    15:00
Vaccine    Influenza
Documents    0 attached
Session details for the selected date
Session    Service    Date    Location
SES-0820-FLU    Influenza    2026-08-20    Riverside Annexe

Submit Back
\end{lstlisting}

\par}


==> tables/blind_tools.tex <==
% GENERATED BY claims.py (d_r31_blind) from REPAIR_r31/blind_challenge/BLIND_RESULT.json -- DO NOT EDIT BY HAND.
\begin{table}[t]
\centering
\small
\caption{\textbf{Rule-only case-design challenge, per tool} (cases and expectations specified by GPT-6 from the registered rules and archive schema only; implemented by the authors, fidelity-reviewed by a model, run once). Controls accepted; FR: controls rejected; corruptions rejected, or counted with the expected failing invariant flagged; FA: corruptions counted as clean; scope: counted, with the attacked invariant outside the tool's outputs; errors: no verdict; exact: countedness and class (or invariants) equal GPT-6's expectation. Exact is stricter than clean-versus-corrupt detection: a corruption rejected under a different registered class is non-clean but not exact.}
\label{tab:blind-tools}
\begin{tabular}{@{}p{5.6cm}rrrrrrr@{}}
\toprule
tool & controls & FR & caught & FA & scope & errors & exact\\
\midrule
\multicolumn{8}{l}{\emph{Claims}}\\
combined pipeline (classifier, void gate) & 7/7 & 0 & 18/20 & 0 & 0 & \textbf{2} & 24/27\\
evaluator with classifier & 7/7 & 0 & 18/20 & 0 & 0 & \textbf{2} & 24/27\\
claims validity re-derivation (C8) & 7/7 & 0 & 6/20 & \textbf{9} & 4 & \textbf{1} & 16/27\\
independent scorer & 7/7 & 0 & 10/20 & \textbf{9} & 0 & \textbf{1} & 12/27\\
simple raw-log baseline (r28) & 7/7 & 0 & 3/20 & \textbf{14} & 2 & \textbf{1} & 12/27\\
repaired raw-log checker (r29) & 7/7 & 0 & 3/20 & \textbf{14} & 2 & \textbf{1} & 12/27\\
\multicolumn{8}{l}{\emph{Clinic (Block~BC)}}\\
combined pipeline (driver row, void gate) & 3/3 & 0 & 6/6 & 0 & 0 & 0 & 9/9\\
evaluator with classifier (refresh) & 3/3 & 0 & 6/6 & 0 & 0 & 0 & 9/9\\
BC validity re-derivation & 3/3 & 0 & 5/6 & \textbf{1} & 0 & 0 & 8/9\\
independent scorer & 3/3 & 0 & 5/6 & \textbf{1} & 0 & 0 & 8/9\\
simple raw-log clinic baseline (r29) & 3/3 & 0 & 1/6 & \textbf{5} & 0 & 0 & 0/9\\
\bottomrule
\end{tabular}
\end{table}


==> tables/check_names.tex <==
% GENERATED BY claims.py -- the distinct check names across the seven certificates.
\begingroup\raggedright\sloppy
\texttt{aux\_\allowbreak{}rows\_\allowbreak{}restored\_\allowbreak{}on\_\allowbreak{}reset}, \texttt{boundary\_\allowbreak{}outcomes\_\allowbreak{}are\_\allowbreak{}the\_\allowbreak{}pre\_\allowbreak{}registered\_\allowbreak{}ones}, \texttt{clean\_\allowbreak{}control\_\allowbreak{}arms\_\allowbreak{}nothing}, \texttt{concurrent\_\allowbreak{}writer\_\allowbreak{}refused}, \texttt{dismissal\_\allowbreak{}reaches\_\allowbreak{}the\_\allowbreak{}access\_\allowbreak{}log\_\allowbreak{}ack\_\allowbreak{}field}, \texttt{early\_\allowbreak{}done\_\allowbreak{}does\_\allowbreak{}not\_\allowbreak{}suppress\_\allowbreak{}queued\_\allowbreak{}event}, \texttt{exposure\_\allowbreak{}conditioned\_\allowbreak{}arm\_\allowbreak{}waits\_\allowbreak{}for\_\allowbreak{}the\_\allowbreak{}exposure}, \texttt{filler\_\allowbreak{}facts\_\allowbreak{}identical\_\allowbreak{}across\_\allowbreak{}arms\_\allowbreak{}and\_\allowbreak{}clinic\_\allowbreak{}neutral}, \texttt{harness\_\allowbreak{}text\_\allowbreak{}passes\_\allowbreak{}the\_\allowbreak{}banned\_\allowbreak{}term\_\allowbreak{}scan}, \texttt{hidden\_\allowbreak{}state\_\allowbreak{}not\_\allowbreak{}policy\_\allowbreak{}reachable}, \texttt{instruction\_\allowbreak{}names\_\allowbreak{}no\_\allowbreak{}clinic}, \texttt{matrix\_\allowbreak{}collateral\_\allowbreak{}seed\_\allowbreak{}change}, \texttt{matrix\_\allowbreak{}covers\_\allowbreak{}at\_\allowbreak{}least\_\allowbreak{}three\_\allowbreak{}policies}, \texttt{matrix\_\allowbreak{}flagged\_\allowbreak{}stale}, \texttt{matrix\_\allowbreak{}late\_\allowbreak{}reread\_\allowbreak{}reference}, \texttt{matrix\_\allowbreak{}modal\_\allowbreak{}bypass}, \texttt{matrix\_\allowbreak{}null}, \texttt{matrix\_\allowbreak{}over\_\allowbreak{}apply}, \texttt{matrix\_\allowbreak{}path\_\allowbreak{}only\_\allowbreak{}reviser}, \texttt{matrix\_\allowbreak{}reference}, \texttt{matrix\_\allowbreak{}stale\_\allowbreak{}even\_\allowbreak{}when\_\allowbreak{}reexposed}, \texttt{matrix\_\allowbreak{}stale\_\allowbreak{}location}, \texttt{modal\_\allowbreak{}bypass\_\allowbreak{}fails\_\allowbreak{}to\_\allowbreak{}submit\_\allowbreak{}or\_\allowbreak{}classifies\_\allowbreak{}delivery\_\allowbreak{}ambiguous}, \texttt{near\_\allowbreak{}miss\_\allowbreak{}is\_\allowbreak{}not\_\allowbreak{}a\_\allowbreak{}boundary}, \texttt{no\_\allowbreak{}evaluator\_\allowbreak{}vocabulary\_\allowbreak{}on\_\allowbreak{}a\_\allowbreak{}reachable\_\allowbreak{}page}, \texttt{notice\_\allowbreak{}bytes\_\allowbreak{}derived\_\allowbreak{}from\_\allowbreak{}the\_\allowbreak{}mutation}, \texttt{notice\_\allowbreak{}renders\_\allowbreak{}until\_\allowbreak{}dismissed}, \texttt{one\_\allowbreak{}shot\_\allowbreak{}trigger}, \texttt{replay\_\allowbreak{}determinism\_\allowbreak{}reference}, \texttt{replay\_\allowbreak{}determinism\_\allowbreak{}stale\_\allowbreak{}location}, \texttt{reply\_\allowbreak{}format\_\allowbreak{}is\_\allowbreak{}the\_\allowbreak{}p1\_\allowbreak{}harnesss}, \texttt{report\_\allowbreak{}clinic\_\allowbreak{}term\_\allowbreak{}is\_\allowbreak{}scored\_\allowbreak{}by\_\allowbreak{}I5}, \texttt{report\_\allowbreak{}flag\_\allowbreak{}fixtures}, \texttt{rescue\_\allowbreak{}crossing}, \texttt{result\_\allowbreak{}line\_\allowbreak{}parser\_\allowbreak{}fixtures}, \texttt{service\_\allowbreak{}date\_\allowbreak{}identifies\_\allowbreak{}exactly\_\allowbreak{}one\_\allowbreak{}session}, \texttt{session\_\allowbreak{}page\_\allowbreak{}reader\_\allowbreak{}fixtures}, \texttt{session\_\allowbreak{}page\_\allowbreak{}shows\_\allowbreak{}the\_\allowbreak{}target\_\allowbreak{}row}, \texttt{signature\_\allowbreak{}collateral\_\allowbreak{}seed\_\allowbreak{}change}, \texttt{signature\_\allowbreak{}flagged\_\allowbreak{}stale}, \texttt{signature\_\allowbreak{}late\_\allowbreak{}reread\_\allowbreak{}reference}, \texttt{signature\_\allowbreak{}modal\_\allowbreak{}bypass}, \texttt{signature\_\allowbreak{}null}, \texttt{signature\_\allowbreak{}over\_\allowbreak{}apply}, \texttt{signature\_\allowbreak{}path\_\allowbreak{}only\_\allowbreak{}reviser}, \texttt{signature\_\allowbreak{}reference}, \texttt{signature\_\allowbreak{}stale\_\allowbreak{}even\_\allowbreak{}when\_\allowbreak{}reexposed}, \texttt{signature\_\allowbreak{}stale\_\allowbreak{}location}, \texttt{silent\_\allowbreak{}arm\_\allowbreak{}posts\_\allowbreak{}no\_\allowbreak{}notice}, \texttt{state\_\allowbreak{}before\_\allowbreak{}channel\_\allowbreak{}ordering}, \texttt{the\_\allowbreak{}claim\_\allowbreak{}is\_\allowbreak{}not\_\allowbreak{}a\_\allowbreak{}boundary}, \texttt{the\_\allowbreak{}firing\_\allowbreak{}request\_\allowbreak{}is\_\allowbreak{}located\_\allowbreak{}correctly}, \texttt{the\_\allowbreak{}policies\_\allowbreak{}that\_\allowbreak{}looked\_\allowbreak{}reached\_\allowbreak{}c3}, \texttt{the\_\allowbreak{}world\_\allowbreak{}fires\_\allowbreak{}the\_\allowbreak{}arm\_\allowbreak{}inside\_\allowbreak{}the\_\allowbreak{}agents\_\allowbreak{}own\_\allowbreak{}request}, \texttt{two\_\allowbreak{}sided\_\allowbreak{}over\_\allowbreak{}apply\_\allowbreak{}FRX-\allowbreak{}OFF-\allowbreak{}I\_\allowbreak{}vs\_\allowbreak{}FRX-\allowbreak{}OFF-\allowbreak{}A}, \texttt{two\_\allowbreak{}sided\_\allowbreak{}over\_\allowbreak{}apply\_\allowbreak{}FRX-\allowbreak{}ON-\allowbreak{}I\_\allowbreak{}vs\_\allowbreak{}FRX-\allowbreak{}ON-\allowbreak{}A}, \texttt{two\_\allowbreak{}sided\_\allowbreak{}over\_\allowbreak{}apply\_\allowbreak{}S-\allowbreak{}C\_\allowbreak{}vs\_\allowbreak{}S-\allowbreak{}L2}, \texttt{two\_\allowbreak{}sided\_\allowbreak{}reference\_\allowbreak{}FRX-\allowbreak{}OFF-\allowbreak{}I\_\allowbreak{}vs\_\allowbreak{}FRX-\allowbreak{}OFF-\allowbreak{}A}, \texttt{two\_\allowbreak{}sided\_\allowbreak{}reference\_\allowbreak{}FRX-\allowbreak{}ON-\allowbreak{}I\_\allowbreak{}vs\_\allowbreak{}FRX-\allowbreak{}ON-\allowbreak{}A}, \texttt{two\_\allowbreak{}sided\_\allowbreak{}reference\_\allowbreak{}S-\allowbreak{}C\_\allowbreak{}vs\_\allowbreak{}S-\allowbreak{}L2}, \texttt{two\_\allowbreak{}sided\_\allowbreak{}stale\_\allowbreak{}location\_\allowbreak{}FRX-\allowbreak{}OFF-\allowbreak{}I\_\allowbreak{}vs\_\allowbreak{}FRX-\allowbreak{}OFF-\allowbreak{}A}, \texttt{two\_\allowbreak{}sided\_\allowbreak{}stale\_\allowbreak{}location\_\allowbreak{}FRX-\allowbreak{}ON-\allowbreak{}I\_\allowbreak{}vs\_\allowbreak{}FRX-\allowbreak{}ON-\allowbreak{}A}, \texttt{two\_\allowbreak{}sided\_\allowbreak{}stale\_\allowbreak{}location\_\allowbreak{}S-\allowbreak{}C\_\allowbreak{}vs\_\allowbreak{}S-\allowbreak{}L2}, \texttt{v1\_\allowbreak{}was\_\allowbreak{}in\_\allowbreak{}a\_\allowbreak{}delivered\_\allowbreak{}observation}, \texttt{wizard\_\allowbreak{}lists\_\allowbreak{}both\_\allowbreak{}clinics}\par\endgroup


==> tables/external_tools.tex <==
% GENERATED BY claims.py (d_r34_external) from REPAIR_r34/external_challenge -- DO NOT EDIT BY HAND.
\begin{table}[t]
\centering
\small
\caption{\textbf{Externally designed and instantiated challenge, per tool} (cases, expectations and generator by a Gemini CLI agent from the rules, schema and archive copies only; generator run unread, cases sealed, each tool run once; the agent's expectations, disputed ones included). Columns as in Table~\ref{tab:blind-tools}: controls accepted; FR: controls not counted; corruptions caught (rejected, or counted with the expected failing invariant flagged); FA: corruptions counted as clean; scope: the attacked invariant is outside the tool's outputs; errors: no verdict; exact: the agent's full expectation met.}
\label{tab:external-tools}
\begin{tabular}{@{}p{5.6cm}rrrrrrr@{}}
\toprule
tool & controls & FR & caught & FA & scope & errors & exact\\
\midrule
\multicolumn{8}{l}{\emph{Claims}}\\
combined pipeline (classifier, void gate) & 6/8 & 2 & 14/20 & \textbf{4} & 0 & 2 & 14/28\\
evaluator with classifier & 8/8 & 0 & 14/20 & \textbf{4} & 0 & 2 & 15/28\\
claims validity re-derivation (C8) & 8/8 & 0 & 3/20 & \textbf{12} & 4 & 1 & 15/28\\
independent scorer & 6/8 & 2 & 8/20 & \textbf{11} & 0 & 1 & 5/28\\
simple raw-log baseline (r28) & 8/8 & 0 & 1/20 & \textbf{15} & 2 & 2 & 6/28\\
repaired raw-log checker (r29) & 7/8 & 1 & 2/20 & \textbf{15} & 1 & 2 & 4/28\\
\multicolumn{8}{l}{\emph{Clinic (Block~BC)}}\\
combined pipeline (driver row, void gate) & 7/8 & 1 & 11/19 & \textbf{8} & 0 & 0 & 7/27\\
evaluator with classifier (refresh) & 8/8 & 0 & 4/19 & \textbf{15} & 0 & 0 & 7/27\\
BC validity re-derivation & 8/8 & 0 & 6/19 & \textbf{9} & 4 & 0 & 17/27\\
independent scorer & 7/8 & 1 & 5/19 & \textbf{14} & 0 & 0 & 6/27\\
simple raw-log clinic baseline (r29) & 8/8 & 0 & 3/19 & \textbf{15} & 1 & 0 & 0/27\\
\bottomrule
\end{tabular}
\end{table}


==> tables/r21_instances_BGC.tex <==
% GENERATED BY claims.py -- DO NOT EDIT BY HAND.
\textit{No per-instance record is printed: the block's state is \BlockBGCDisposition.}


==> tables/r21_instances_BGtwo.tex <==
% GENERATED BY claims.py -- DO NOT EDIT BY HAND.
\textit{No per-instance record is printed: the block's state is \BlockBGtwoDisposition.}


==> tables/readings_templates.tex <==
% GENERATED BY claims.py (emit_r21_tables) from readings/templates.tex -- DO NOT EDIT BY HAND.
\begingroup\footnotesize\setlength{\parindent}{0pt}\setlength{\parskip}{2pt}
\texttt{BC.S0}\quad Over the \textsf{[Instances]} instances (seeds \textsf{[SeedList]}), \textsf{\guilsinglleft{}Model\guilsinglright{}} passed OFF-A \textsf{[FRXOffAPassFrac]}, CUE-A \textsf{[FRXCueAPassFrac]} and LIVE-A \textsf{[FRXLiveAPassFrac]}. LIVE versus CUE (primary): rescue \textsf{[LiveCueRescue]}, harm \textsf{[LiveCueHarm]}, tie \textsf{[LiveCueTie]} of \textsf{[LiveCuePairs]} pairs, net \textsf{[LiveCueNetCI]} (marginal 95\,\% interval), $p=\textsf{[LiveCueP]}$ (block-local Holm $p=\textsf{[LiveCueHolmLocal]}$). CUE versus OFF (key secondary): \textsf{[CueOffRescue]}/\textsf{[CueOffHarm]}/\textsf{[CueOffTie]}, net \textsf{[CueOffNetCI]}, $p=\textsf{[CueOffP]}$ (block-local Holm $p=\textsf{[CueOffHolmLocal]}$). LIVE versus OFF (supporting, descriptive, outside the paper-wide family): \textsf{[LiveOffRescue]}/\textsf{[LiveOffHarm]}/\textsf{[LiveOffTie]}, net \textsf{[LiveOffNetCI]}.\par
\texttt{BGC.S0T}\quad OFF-I versus OFF-A (target relevance): OFF-I passed \textsf{[BGC:FRXOffIPassFrac]}; \textsf{[BGC:OffiOffaRescue]}/\textsf{[BGC:OffiOffaHarm]}/\textsf{[BGC:OffiOffaTie]}, net \textsf{[BGC:OffiOffaNetCI]}, $p=\textsf{[BGC:OffiOffaP]}$ (block-local Holm $p=\textsf{[BGC:OffiOffaHolmLocal]}$).\par
\texttt{BC.S0M}\quad \textsf{\guilsinglleft{}Model\guilsinglright{}} passed OFF-A \textsf{[FRXOffAPassFrac]}, CUE-A \textsf{[FRXCueAPassFrac]} and LIVE-A \textsf{[FRXLiveAPassFrac]} on \textsf{[Instances]} instances (Table~\ref{tab:tests} gives every contrast).\par
\texttt{BC.R-A} \textbf{[selected: BC]}\quad At the registered block-local level, displaying the current location increased success relative to this cue-and-link panel. The CUE--OFF contrast did not reject; this does not establish absence of a cue effect. Contradiction, salience, and reduced verification effort remain possible explanations.\par
\texttt{BC.R-B}\quad At the registered block-local level, the cue-and-link panel increased success relative to no panel. The LIVE--CUE contrast did not reject; this establishes neither equivalence nor absence of an additional value-display effect.\par
\texttt{BC.R-B.E}\quad CUE versus OFF rejected in CUE-A's direction at the registered block-local level (\textsf{[CueOffRescue]}/\textsf{[CueOffHarm]}/\textsf{[CueOffTie]}, net \textsf{[CueOffNetCI]}, block-local Holm $p=\textsf{[CueOffHolmLocal]}$). The registered rescue-opportunity threshold was not met. The LIVE--CUE contrast did not reject; this establishes neither equivalence nor absence of an additional value-display effect.\par
\texttt{BC.R-C}\quad Both adjacent contrasts rejected in the treatment direction at the registered block-local level; their paired differences and intervals quantify the two increments.\par
\texttt{BC.R-C.E}\quad Both adjacent contrasts rejected in the treatment direction at the registered block-local level (LIVE versus CUE net \textsf{[LiveCueNetCI]}, block-local Holm $p=\textsf{[LiveCueHolmLocal]}$; CUE versus OFF net \textsf{[CueOffNetCI]}, block-local Holm $p=\textsf{[CueOffHolmLocal]}$). The registered rescue-opportunity threshold was not met.\par
\texttt{BC.R-D}\quad The supporting LIVE--OFF analysis did not establish a positive panel effect on these instances. This does not establish absence of an effect or a difference from Block~\textsf{\guilsinglleft{}RefBlock\guilsinglright{}}.\par
\texttt{BC.R-E}\quad OFF-A failed on \textsf{[OffFail]} of \textsf{[FRXOffAN]} counted rows; \textsf{[FRXOffAN]} of \textsf{[OffPlanned]} planned rows were observed. Fewer than \textsf{[OffGate]} counted failures were available, so the registered rescue-opportunity threshold was not met. At least one counted OFF-A row succeeded, so the universal OFF-A failure observed in Block~\textsf{\guilsinglleft{}RefBlock\guilsinglright{}} did not recur. Post-change source re-reading occurred in \textsf{[OffReread]} of \textsf{[FRXOffAN]} OFF-A episodes.\par
\texttt{BC.R-E.0}\quad OFF-A failed on \textsf{[OffFail]} of \textsf{[FRXOffAN]} counted rows; \textsf{[FRXOffAN]} of \textsf{[OffPlanned]} planned rows were observed. Fewer than \textsf{[OffGate]} counted failures were available, so the registered rescue-opportunity threshold was not met. This threshold statement alone does not establish that universal failure failed to recur.\par
\texttt{BC.R-F.cue}\quad At this budget the cue-and-link panel alone outperformed the value display. No mechanism is inferred.\par
\texttt{BC.R-F.off}\quad The cue-and-link panel reduced success relative to no panel. No mechanism is inferred.\par
\texttt{BC.R-G}\quad Unresolved at the fixed budget. R-G describes the combined cue/value interpretation only and does not negate an independently eligible contrast rejection; each eligible contrast, its direction, interval, and multiplicity status is reported separately. An absent or incomplete contrast is unknown, not non-rejected, and a contrast without discordant pairs has raw $p=1$: insufficient evidence of a difference, not equivalence.\par
\texttt{BC.ELIG}\quad The \textsf{\guilsinglleft{}Contrast\guilsinglright{}} comparison, which is eligible, rejected in the \textsf{\guilsinglleft{}Dir\guilsinglright{}} direction at the registered block-local level (net \textsf{[\textsf{\guilsinglleft{}C\guilsinglright{}}NetCI]}, $p=\textsf{[\textsf{\guilsinglleft{}C\guilsinglright{}}P]}$).\par
\texttt{BC.G1}\quad The \textsf{\guilsinglleft{}Contrast\guilsinglright{}} comparison's complete pairs (\textsf{[\textsf{\guilsinglleft{}C\guilsinglright{}}Pairs]}) fall below its registered minimum (\textsf{[\textsf{\guilsinglleft{}C\guilsinglright{}}MinPairs]}), so it is unknown and receives no confirmatory interpretation. Other eligible contrasts retain their registered analyses.\par
\texttt{BC.A19} \textbf{[selected: BC]}\quad The LIVE--OFF comparison is a supporting descriptive analysis; it supports neither a confirmatory replication claim nor a claim that the effect differs from Block~\textsf{\guilsinglleft{}RefBlock\guilsinglright{}}.\par
\texttt{BC.GZP}\quad Block~\textsf{\guilsinglleft{}Block\guilsinglright{}} has run, but its validity evidence is incomplete (\textsf{[GzeroWhy]}); under its registered validity gate no result is interpreted until that evidence exists.\par
\texttt{BC.VOID}\quad Block~\textsf{\guilsinglleft{}Block\guilsinglright{}} is void under its registered validity gate (\textsf{[GzeroWhy]}). It contributes no inferential result; its rows are listed in Appendix~\ref{app:bc} as a record only.\par
\texttt{BC.PEND}\quad Block~\textsf{\guilsinglleft{}Block\guilsinglright{}} (\textsf{\guilsinglleft{}Model\guilsinglright{}}) had not reported when this version was built. Its arms, instances, contrasts and the interpretations its result will select are fixed in Appendix~\ref{app:readings}; every number it contributes prints as pending until its result file exists.\par
\texttt{BC.NOTRUN} \textbf{[selected: BGC]}\quad Block~\textsf{\guilsinglleft{}Block\guilsinglright{}} was not run (\textsf{[Disposition]}). It contributes no inferential result; its paper-wide slots are non-rejection placeholders.\par
\texttt{BC.INCOMPLETE} \textbf{[selected: BCS]}\quad Block~\textsf{\guilsinglleft{}Block\guilsinglright{}} started but did not complete (\textsf{[Disposition]}). It contributes no inferential result; its rows are listed in Appendix~\ref{app:bc} as a record only.\par
\texttt{BC.QI}\quad The LIVE-I controls passed \textsf{[FRXLiveIPassFrac]}; nothing is attributed to the panel from unmatched controls.\par
\texttt{BC.QE}\quad The independent scorer reconstructs appointment availability from archived rows; calendar compatibility is not re-derived but rests on stated design conditions (the generator and state preservation), whose checks are reported separately. Under that condition, every outcome term is resolved and agreeing with the evaluator on \textsf{[EndpointFull]} of \textsf{[Counted]} counted rollouts (Table~\ref{tab:coverage}).\par
\texttt{BC.QE0}\quad The independent scorer had not been run on this block's counted rollouts when this version was built, so no outcome term is independently re-derived; calendar compatibility rests on stated design conditions in any case.\par
\texttt{BC.QV}\quad Independent code re-derived this block's validity verdicts (\textsf{[VindPath]}), agreeing with the archive on \textsf{[VindAgree]} attempts.\par
\texttt{BC.QV0}\quad No independent re-derivation of this block's validity verdicts exists (it is expected at \textsf{[VindPath]}); its validity verdicts are the evaluator's alone.\par
\texttt{BC.QP}\quad Strict recovery occurred in \textsf{[FRXCueARecovered]} of \textsf{[FRXCueAN]} CUE-A and \textsf{[FRXLiveARecovered]} of \textsf{[FRXLiveAN]} LIVE-A runs, and \textsf{[FRXCueALinkFollowed]} of \textsf{[FRXCueAN]} CUE-A runs followed the panel's link (descriptive; never a reading condition).\par
\texttt{BGC.R-T+}\quad Under this trigger and interface, GPT-6 succeeded more often when an irrelevant session moved than when the target moved. This supports a target-relevance effect on success under the tested trigger and interface; it is not an estimate of a general effect of dynamic environments.\par
\texttt{BGC.R-T-}\quad GPT-6 succeeded more often under the target change than under the irrelevant one; no mechanism is inferred.\par
\texttt{BGC.R-TB}\quad GPT-6 failed often even when the target did not move (FRX-OFF-I failed on \textsf{[BGC:OffIFail]} of \textsf{[BGC:OffIN]} counted rows; \textsf{[BGC:OffiOffaPairs]} matched pairs), so its OFF-A failures are not shown to be specific to supersession; its cue and value contrasts are read with that caveat.\par
\texttt{BGC.R-TC}\quad The target-relevance contrast is unresolved: insufficient evidence of a difference, not equivalence (FRX-OFF-I failed on \textsf{[BGC:OffIFail]} of \textsf{[BGC:OffIN]} counted rows; \textsf{[BGC:OffiOffaPairs]} matched pairs).\par
\texttt{BGC.T-X}\quad No reading was registered for the target-relevance contrast before the block ran; it is reported as numbers only.\par
\texttt{QH.survive} \textbf{[selected: BC]}\quad The \textsf{\guilsinglleft{}Contrast\guilsinglright{}} rejection survives the paper-wide Holm analysis over \textsf{[HolmPaperM]} claim-bearing tests (adjusted $p=\textsf{[\textsf{\guilsinglleft{}C\guilsinglright{}}HolmPaper]}$).\par
\texttt{QH.local} \textbf{[selected: CLM-BS]}\quad The \textsf{\guilsinglleft{}Contrast\guilsinglright{}} contrast rejects under its registered block-local analysis but not under the paper-wide Holm analysis (adjusted $p=\textsf{[\textsf{\guilsinglleft{}C\guilsinglright{}}HolmPaper]}$ over \textsf{[HolmPaperM]} tests).\par
\texttt{QH.pending}\quad The paper-wide Holm-adjusted $p$ of the \textsf{\guilsinglleft{}Contrast\guilsinglright{}} contrast awaits the rest of the family (it is at most \textsf{[\textsf{\guilsinglleft{}C\guilsinglright{}}BonfPaper]}).\par
\texttt{BG2.S0}\quad GPT-6 on Block~B's instances: OFF-A \textsf{[BGtwo:FRXOffAPassFrac]}, ON-A \textsf{[BGtwo:FRXOnAPassFrac]} (\textsf{[BGtwo:OnOffRescue]}/\textsf{[BGtwo:OnOffHarm]}/\textsf{[BGtwo:OnOffTie]}, net \textsf{[BGtwo:OnOffNetCI]}, $p=\textsf{[BGtwo:OnOffP]}$).\par
\texttt{BG2.OPP-NOT}\quad The registered rescue-opportunity gate was not met (OFF-A failed on \textsf{[BGtwo:OffFail]} of \textsf{[BGtwo:FRXOffAN]}).\par
\texttt{BG2.OPP-MET}\quad OFF-A failed on \textsf{[BGtwo:OffFail]} of \textsf{[BGtwo:FRXOffAN]}, which meets the registered rescue-opportunity gate.\par
\texttt{BG2.EFF-ON}\quad At the registered local level, the review-step panel increased GPT-6's full-task success on Block~B's instances.\par
\texttt{BG2.EFF-OFF}\quad At the registered local level, the review-step panel reduced GPT-6's full-task success; no mechanism is inferred.\par
\texttt{BG2.EFF-NONE}\quad The paired contrast did not reject: insufficient evidence of a difference, not zero.\par
\texttt{BG2.PEND}\quad Block~BG2, the predeclared fallback that runs only if Block~BC is dropped, had not reported when this version was built.\par
\texttt{BG2.G1}\quad The paired contrast has \textsf{[BGtwo:OnOffPairs]} complete pairs, fewer than its registered minimum of eight, so it is unknown and receives no confirmatory interpretation; its paper-wide slot is a non-rejection placeholder.\par
\texttt{BG2.GZP}\quad Block~BG2 has run, but its validity or result-agreement evidence is incomplete; under its registered admissibility rule no result is interpreted until that evidence exists.\par
\texttt{BG2.VOID}\quad Block~BG2 is void under its registered validity gate. It contributes no inferential result.\par
\texttt{BG2.NOTRUN} \textbf{[selected: BG2]}\quad Block~BG2 was not run (\textsf{[BGtwo:Disposition]}).\par
\texttt{BG2.INCOMPLETE}\quad Block~BG2 started but did not complete (\textsf{[BGtwo:Disposition]}); it contributes no inferential result.\par
\texttt{CLM.S0} \textbf{[selected: CLM-B, CLM-BS]}\quad Over \textsf{[OnOffPairs]} sealed instance pairs (seeds \textsf{[SeedList]}), \textsf{\guilsinglleft{}Model\guilsinglright{}} met the full approval endpoint on \textsf{[ClmOffAPassFrac]} without the panel and \textsf{[ClmOnAPassFrac]} with it; of the pairs, \textsf{[OnOffRescue]} favoured the panel, \textsf{[OnOffHarm]} the arm without it, and \textsf{[OnOffTie]} neither; net \textsf{[OnOffNetCI]} (marginal 95\,\% interval), $p=\textsf{[OnOffP]}$. Controls: ON-I \textsf{[ClmOnIPassFrac]}, L0 \textsf{[ClmLzeroPassFrac]}.\par
\texttt{CLM.R1} \textbf{[selected: CLM-BS]}\quad The review-step panel increased full-task success at the registered local level. The OFF-A failure categories and observed pre-commit revisions are reported separately (Appendix~\ref{app:claims}).\par
\texttt{CLM.R1-NC}\quad A local paired success difference was observed, but the registered control-credibility criterion was not met; no transfer claim is made.\par
\texttt{CLM.R1-DG}\quad The derived-decision gate was not met (\textsf{[XupOn]}/\textsf{[XupN]} threshold-crossing increases succeeded). This result does not establish performance beyond the scalar-copy shortcut.\par
\texttt{CLM.R2} \textbf{[selected: CLM-B]}\quad Without the panel, the agent succeeded on \textsf{[OffPass]}/\textsf{[ClmOffAN]} instances under silent supersession; the registered rescue-opportunity threshold was not met.\par
\texttt{CLM.R2-H}\quad The rescue-opportunity gate was not met. Nevertheless, ON-A reduced full-task success relative to OFF-A (\textsf{[OnOffRescue]}/\textsf{[OnOffHarm]}/\textsf{[OnOffTie]}, net \textsf{[OnOffNetCI]}, local $p=\textsf{[OnOffP]}$).\par
\texttt{CLM.R3}\quad Without the panel, the agent failed on \textsf{[OffFail]}/\textsf{[ClmOffAN]} instances under silent supersession; a positive panel effect was not established at the registered local level.\par
\texttt{CLM.R3-H}\quad At the registered local level, ON-A reduced full-task success relative to OFF-A (\textsf{[OnOffRescue]}/\textsf{[OnOffHarm]}/\textsf{[OnOffTie]}, net \textsf{[OnOffNetCI]}, local $p=\textsf{[OnOffP]}$).\par
\texttt{CLM.R3-NC}\quad The registered control-credibility criterion was not met (L0 \textsf{[ClmLzeroPassFrac]}, ON-I \textsf{[ClmOnIPassFrac]}), so no transfer claim is made either way.\par
\texttt{CLM.R4}\quad The block failed its registered readiness or execution requirements (\textsf{[RfourWhy]}). It provides no admissible model-effect result; all attempts and exclusions remain in the engineering record.\par
\texttt{CLM.QCL} \textbf{[selected: CLM-B, CLM-BS]}\quad The scripted copy-limit shortcut, run on the same cells before any model, is assigned \textsf{[CopyLimitReading]} under the same rules.\par
\texttt{CLM.QE} \textbf{[selected: CLM-B, CLM-BS]}\quad Every outcome term the independent scorer re-derives is resolved and agreeing with the evaluator on \textsf{[EndpointFull]} of \textsf{[Counted]} counted rollouts.\par
\texttt{CLM.QE0}\quad The independent scorer had not been run on this block's counted rollouts when this version was built.\par
\texttt{CLM.QV} \textbf{[selected: CLM-B, CLM-BS]}\quad The standard-library validity re-derivation agrees with the archive on \textsf{[VindAgree]} attempts.\par
\texttt{CLM.QV0}\quad No independent validity re-derivation of this block exists (Appendix~\ref{app:coverage}); its validity verdicts are the evaluator's alone.\par
\texttt{CLM.QL}\quad The claims task shares the scaffold, harness, invoker and vendor with the clinic task: it is a second decision rule for the same intervention, not an independent environment, and no cue or announcement was varied in it.\par
\texttt{CLM.PEND}\quad Block~\textsf{\guilsinglleft{}Block\guilsinglright{}} (\textsf{\guilsinglleft{}Model\guilsinglright{}}) had not reported when this version was built; its interpretations and their qualifiers are fixed in Appendix~\ref{app:readings}.\par
\texttt{CLM.NOTRUN}\quad Block~\textsf{\guilsinglleft{}Block\guilsinglright{}} was not run (\textsf{[Disposition]}); it contributes no inferential result, and its paper-wide slot is a non-rejection placeholder.\par
\texttt{CLM.INCOMPLETE}\quad Block~\textsf{\guilsinglleft{}Block\guilsinglright{}} started but did not meet its registered completeness requirements (\textsf{[Disposition]}); it contributes no inferential result.\par
\texttt{SHORT.BC}\quad \textsf{\guilsinglleft{}Model\guilsinglright{}} on the same instances (Block~\textsf{\guilsinglleft{}Block\guilsinglright{}}): OFF-A \textsf{[FRXOffAPassFrac]}, CUE-A \textsf{[FRXCueAPassFrac]}, LIVE-A \textsf{[FRXLiveAPassFrac]}; block-local Holm $p=\textsf{[LiveCueHolmLocal]}$ (LIVE--CUE) and $p=\textsf{[CueOffHolmLocal]}$ (CUE--OFF); \textsf{[ReadingShort]}.\par
\texttt{SHORT.CLM}\quad \textsf{\guilsinglleft{}Model\guilsinglright{}} on CLM-B's frozen slots (Block~\textsf{\guilsinglleft{}Block\guilsinglright{}}): OFF-A \textsf{[ClmOffAPassFrac]}, ON-A \textsf{[ClmOnAPassFrac]}, $p=\textsf{[OnOffP]}$; \textsf{[ReadingShort]}. The two models share instances, so their difference is descriptive.\par
\texttt{SHORT.STATE}\quad \textsf{\guilsinglleft{}Model\guilsinglright{}} on the same instances (Block~\textsf{\guilsinglleft{}Block\guilsinglright{}}): \textsf{[ReadingShort]}.\par
\texttt{FRAG.R-A}\quad at the block-local level the value display increased success relative to the cue-and-link panel\par
\texttt{FRAG.R-B}\quad at the block-local level the cue-and-link panel increased success relative to no panel\par
\texttt{FRAG.R-B.E}\quad CUE versus OFF rejected in CUE-A's direction at the block-local level; the rescue-opportunity threshold was not met\par
\texttt{FRAG.R-C}\quad both adjacent contrasts rejected in the treatment direction at the block-local level\par
\texttt{FRAG.R-C.E}\quad both adjacent contrasts rejected in the treatment direction at the block-local level; the rescue-opportunity threshold was not met\par
\texttt{FRAG.R-D}\quad the supporting LIVE--OFF analysis did not establish a positive panel effect\par
\texttt{FRAG.R-E}\quad OFF-A failed on only \textsf{[OffFail]} of \textsf{[FRXOffAN]} counted rows, below the rescue-opportunity threshold\par
\texttt{FRAG.R-E.0}\quad OFF-A failed on \textsf{[OffFail]} of \textsf{[FRXOffAN]} counted rows (of \textsf{[OffPlanned]} planned), below the rescue-opportunity threshold\par
\texttt{FRAG.R-F.cue}\quad the cue-and-link panel outperformed the value display at the block-local level\par
\texttt{FRAG.R-F.off}\quad the cue-and-link panel reduced success relative to no panel at the block-local level\par
\texttt{FRAG.R-G}\quad the registered rules leave the combined interpretation unresolved\par
\texttt{FRAG.ELIG}\quad the eligible \textsf{\guilsinglleft{}Contrast\guilsinglright{}} comparison rejected in the \textsf{\guilsinglleft{}Dir\guilsinglright{}} direction at the block-local level\par
\texttt{FRAG.G1}\quad the \textsf{\guilsinglleft{}Contrast\guilsinglright{}} comparison is incomplete and receives no confirmatory interpretation\par
\texttt{FRAG.R-T+}\quad success was higher when an irrelevant session moved than when the target moved (block-local)\par
\texttt{FRAG.R-T-}\quad success was higher when the target moved than when an irrelevant session moved (block-local)\par
\texttt{FRAG.R-TB}\quad the target-relevance contrast did not reject, and GPT-6 also failed often when the target did not move\par
\texttt{FRAG.R-TC}\quad the target-relevance contrast is unresolved (not rejected)\par
\texttt{FRAG.T-X}\quad no reading was registered for the target-relevance contrast\par
\texttt{FRAG.PEND}\quad pending when this version was built\par
\texttt{FRAG.NOTRUN}\quad not run (\textsf{[Disposition]})\par
\texttt{FRAG.INCOMPLETE}\quad started but not completed (\textsf{[Disposition]}); no inference\par
\texttt{FRAG.GZP}\quad validity evidence incomplete; no result interpreted\par
\texttt{FRAG.VOID}\quad void under its validity gate; no conclusion\par
\texttt{FRAG.CLM.R1}\quad the panel increased full-task success at the registered local level\par
\texttt{FRAG.CLM.R1-NC}\quad a local paired difference was observed but the control-credibility criterion was not met; no transfer claim\par
\texttt{FRAG.CLM.R1-DG}\quad the derived-decision gate was not met\par
\texttt{FRAG.CLM.R2}\quad OFF-A succeeded often, below the rescue-opportunity threshold\par
\texttt{FRAG.CLM.R3}\quad a positive panel effect was not established\par
\texttt{FRAG.CLM.HARM}\quad the panel reduced full-task success at the registered local level\par
\texttt{FRAG.CLM.R4}\quad readiness or execution requirements not met; no admissible result\par
\texttt{FRAG.PW.survive}\quad surviving the paper-wide Holm analysis\par
\texttt{FRAG.PW.local}\quad not significant under the paper-wide Holm analysis\par
\texttt{FRAG.PW.pending}\quad paper-wide Holm pending\par
\texttt{APP.pending}\quad Its finalized implementation is frozen before each of two pre-registered prospective applications.\par
\texttt{APP.pending.draft}\quad Its finalized implementation is to be frozen before the first rollout of each of two prospective applications, whose registrations are not yet frozen.\par
\texttt{APP.two}\quad Its finalized implementation is evaluated prospectively in two workflows, clinic booking and insurance-claim approval.\par
\texttt{APP.bc}\quad Its finalized implementation is evaluated prospectively in clinic booking, with a second pre-registered application in insurance-claim approval.\par
\texttt{APP.clm}\quad Its finalized implementation is evaluated prospectively in insurance-claim approval, with a pre-registered application in clinic booking.\par
\texttt{APP.none}\quad Neither of its two pre-registered prospective applications yielded an admissible result.\par
\texttt{ABS.BC.lead}\quad In clinic booking, counterbalanced no-panel, cue-and-link and current-value conditions on \textsf{[BC:InstancesWords]} fresh instances (Claude Opus~5)\par
\texttt{ABS.BC.PEND}\quad had not reported when this version was built.\par
\texttt{ABS.BC.NOTRUN}\quad were not run (\textsf{[BC:Disposition]}).\par
\texttt{ABS.BC.INCOMPLETE}\quad started but did not complete (\textsf{[BC:Disposition]}) and support no inference.\par
\texttt{ABS.BC.VOID}\quad are void under their registered validity gate and support no model conclusion.\par
\texttt{ABS.BC.GZP}\quad have run, but their validity evidence is incomplete, so no result is interpreted.\par
\texttt{ABS.BC.R-C}\quad rejected both adjacent contrasts in the treatment direction at the registered block-local level\par
\texttt{ABS.BC.R-C.E}\quad rejected both adjacent contrasts in the treatment direction at the registered block-local level\par
\texttt{ABS.BC.R-A}\quad showed at the registered block-local level that displaying the current location increased success relative to the cue-and-link panel, with no rejection of cue versus no panel\par
\texttt{ABS.BC.R-B}\quad showed at the registered block-local level that the cue-and-link panel increased success relative to no panel, with no rejection of value versus cue\par
\texttt{ABS.BC.R-B.E}\quad rejected cue versus no panel in the cue's direction at the registered block-local level\par
\texttt{ABS.BC.R-F.cue}\quad showed at the registered block-local level that the cue-and-link panel outperformed the value display\par
\texttt{ABS.BC.R-F.off}\quad showed at the registered block-local level that the cue-and-link panel reduced success relative to no panel\par
\texttt{ABS.BC.R-D}\quad did not establish a positive effect of the value panel over no panel in a supporting descriptive analysis\par
\texttt{ABS.BC.R-E}\quad found fewer counted no-panel failures than the registered rescue-opportunity threshold requires (OFF-A failed on \textsf{[BC:OffFail]} of \textsf{[BC:FRXOffAN]} counted rows), and at least one counted no-panel row succeeded\par
\texttt{ABS.BC.R-E.0}\quad found fewer counted no-panel failures than the registered rescue-opportunity threshold requires (OFF-A failed on \textsf{[BC:OffFail]} of \textsf{[BC:FRXOffAN]} counted rows, of \textsf{[BC:OffPlanned]} planned)\par
\texttt{ABS.BC.R-G}\quad left the combined interpretation unresolved under the registered rules\par
\texttt{ABS.BC.ELIG}\quad although the eligible \textsf{\guilsinglleft{}Contrast\guilsinglright{}} comparison rejected in the \textsf{\guilsinglleft{}Dir\guilsinglright{}} direction at the block-local level\par
\texttt{ABS.BC.G1}\quad (the \textsf{\guilsinglleft{}Contrast\guilsinglright{}} comparison was incomplete and receives no confirmatory interpretation)\par
\texttt{ABS.PW.all}\quad and every block-local rejection survives the paper-wide Holm analysis\par
\texttt{ABS.PW.none}\quad but no block-local rejection survives the paper-wide Holm analysis\par
\texttt{ABS.PW.some}\quad and only the \textsf{\guilsinglleft{}Contrast\guilsinglright{}} rejection survives the paper-wide Holm analysis\par
\texttt{ABS.PW.pending}\quad pending the paper-wide Holm analysis\par
\texttt{ABS.CLM.lead}\quad In insurance-claim approval, where the approved amount is derived,\par
\texttt{ABS.CLM.PEND}\quad the registered comparison with and without the review-step panel (Claude Opus~5) had not reported when this version was built.\par
\texttt{ABS.CLM.NOTRUN}\quad the registered comparison with and without the review-step panel was not run (\textsf{[ClmB:Disposition]}).\par
\texttt{ABS.CLM.INCOMPLETE}\quad the registered comparison started but did not meet its completeness requirements and supports no inference.\par
\texttt{ABS.CLM.R4}\quad the registered block failed its readiness or execution requirements and provides no admissible model-effect result.\par
\texttt{ABS.CLM.R1}\quad the review-step panel increased full-task success for Claude Opus~5 at the registered local level ($p=\textsf{[ClmB:OnOffP]}$)\par
\texttt{ABS.CLM.R1-NC}\quad a local paired success difference was observed, but the registered control-credibility criterion was not met; no transfer claim is made\par
\texttt{ABS.CLM.R1-DG}\quad ; the derived-decision gate was not met, so performance beyond the scalar-copy shortcut is not established\par
\texttt{ABS.CLM.R2}\quad without the panel Claude Opus~5 succeeded on \textsf{[ClmB:OffPass]} of \textsf{[ClmB:ClmOffAN]} instances under silent supersession; the registered rescue-opportunity threshold was not met\par
\texttt{ABS.CLM.R3}\quad without the panel Claude Opus~5 failed on \textsf{[ClmB:OffFail]} of \textsf{[ClmB:ClmOffAN]} instances under silent supersession; a positive panel effect was not established at the registered local level\par
\texttt{ABS.CLM.HARM}\quad ; nevertheless the panel reduced full-task success at the registered local level\par
\texttt{ABS.AUDIT.hist}\quad Independent audits re-derive every validity verdict of the historical blocks (\textsf{[VindAgree]} of \textsf{[VindAttempts]} agree under the rules as implemented) and the booked clinic of every historical booking, but verify no historical success in full\par
\texttt{ABS.AUDIT.pending}\quad ; prospective coverage is reported per block, and planned evidence collection is not counted as verification.\par
\texttt{ABS.AUDIT.some}\quad ; on the prospective blocks, with clinic calendar compatibility resting on stated design conditions, every outcome term is resolved and agreeing with the evaluator on \textsf{[ProspEndpointFull]} of \textsf{[ProspCounted]} counted rollouts.\par
\texttt{CONCL.fixed}\quad These contrasts estimate within-configuration effects; unrejected comparisons do not establish absence or equivalence.\par
\texttt{CHAL.PEND}\quad A second archive challenge, built by a different model and sealed before any Claude agent read it (seal record \textsf{[ChallengeSealSha]}), had not been run when this version was built.\par
\texttt{CHAL.RUN}\quad A second, sealed archive challenge built by a different model met \textsf{[ChallengeMet]} of \textsf{[ChallengeN]} frozen expectations on its first and only run (\textsf{[ChallengeCorruptRejected]} of \textsf{[ChallengeCorruptInstantiated]} instantiated corruptions rejected; \textsf{[ChallengeValidAccepted]} of \textsf{[ChallengeValidInstantiated]} valid cases accepted); its \textsf{[ChallengeMissed]} misses are listed in Appendix~\ref{app:certificates} as its comparison output words them.\par
\texttt{QCONFIG}\quad GPT-6 received frames inline; Claude received frames through file reads. Each configuration passed its specified delivery and isolation checks. Within-configuration paired contrasts under a counterbalanced arm order estimate intervention effects. Cross-configuration differences include model, invoker, delivery-channel, and inference-setting differences and do not isolate vendor or model effects.\par
\texttt{REUSE.PEND}\quad The count of reused and newly implemented components (a deterministic comparison with the clinic-pinned versions) had not been produced when this version was built.\par
\texttt{REUSE.RUN}\quad \textsf{[ClmReuseUnchanged]} of \textsf{[ClmReuseShared]} shared components are byte-identical to their clinic-pinned versions, the others gained \textsf{[ClmReuseAddedLines]} lines, and \textsf{[ClmNewFiles]} new files (\textsf{[ClmNewLines]} lines) implement the task, its checks and its audits.\par
\endgroup

